Asymptotic dimensioning of stochastic service systems

Stochastic service systems describe situations in which customers compete for service from scarce resources. Think of check-in lines at airports, waiting rooms in hospitals or queues in supermarkets, where the scarce resource is human manpower. Next to these traditional settings, resource sharing is also important in large-scale service systems such as the internet, wireless networks and cloud computing facilities. In these virtual environments, geographical conditions do not restrict the system size, paving the way for the emergence of large-scale resource sharing networks. This thesis investigates how to design large-scale systems in order to achieve the dual goal of operational efficiency and quality-of-service, by which we mean that the system is highly occupied and hence efficiently utilizes the expensive resources, while at the same time, the level of service, experienced by customers, remains high.

==> Chapter_2/Chapter2i.tex <==
 

\chapter{Novel heavy-traffic regimes}


\begin{chapterstart}
In this chapter, we introduce a family of heavy-traffic scalings for a large-scale service system meant to serve jobs coming from a large pool of customers. 
The scaling rules are inspired by the classical QED regime discussed in Chapter 1, but lead to a range of different system behaviors that includes the ED, QED and QD regime as special cases.
To determine the scaling limits, we describe the performance measures in terms of Pollaczek integrals and use asymptotic techniques to evaluate these integrals in the large-system limit. 
\end{chapterstart}

\begin{flushright}
Based on \\
\textbf{Novel heavy-traffic regimes for large-scale service systems}\\
\textit{Guido Janssen, Johan van Leeuwaarden \& Britt Mathijsen}\\
In \textit{SIAM Journal of Applied Mathematics, 75(2), 787-812 (2015)}
\end{flushright}

\newpage

\section{Introduction \& motivation}
We study the workload process of a system, experiencing stochastic demand and deterministic capacity $s_n$ per period, at equidistant time epochs. 
Demand is assumed to be generated by $n$ stochastically identical and independent sources. 
Let $A_{i,j}$ denote the workload brought into the system by source $i$ in period $j$, for which $\E[A_{i,j}] =\mu$ and $\Var A_{i,j} = \sigma^2$.
Then the total amount of demand arriving to the system in period $j$ is $A^{(n)}_j=\sum_{i=1}^n A_{i,j}$ with $\E[A^{(n)}_j] = n\mu$ and $\Var A^{(n)}_j = n\sigma^2$.
As explained in Chapter 1, a good capacity sizing rule for achieving economies-of-scale is $s_n = n\mu+\beta\sqrt{n}\sigma$ for some $\beta>0$.
If we denote the system utilization by $\rho_n := n\mu/s_n$, then this dimensioning rule in the bulk service queue with many sources is tantamount to the heavy-traffic scaling
\begin{equation}\label{bb1}
\sqrt{n}(1-\rho_n) \to \gamma = \frac{\beta\sigma}{\mu}, \qquad {\rm as }\ n\to\infty.
\end{equation}
Starting from this setting, we introduce a novel family described in terms of a parameter $\eta$ for which we assume that
\begin{equation}\label{bb}
n^{\eta}(1-\rho_n)\rightarrow \gamma, \quad {\rm as} \ n\to  \infty,  \ \gamma> 0.
\end{equation}
The parameter $\eta\geq 0$ defines a whole range of possible scaling regimes, including the classical case $\eta=1/2$. 
In terms of a capacity sizing rule for systems with many customers, the condition \eqref{bb} is tantamount to $s_n=n\mu+\beta \sigma n^{1-\eta}$. 
Similar capacity sizing rules have been considered in \cite{Bassamboo2010,maman} for many-server systems with uncertain arrival rates. Hence, for $\eta\in(0,1/2)$ the variability hedge is relatively large, so that the regime parameterized by $\eta\in(0,1/2)$ can  be seen as {\it moderate} heavy traffic: heavy-traffic conditions in which the full occupancy is reached more slowly, as a function of $n$, than for classical heavy traffic. For opposite reasons the range $\eta\in(1/2,\infty)$ corresponds to {\it extreme} heavy traffic due to a relatively small variability hedge. Note that the case $\eta=0$ does not lead to 100\% system utilization when $n\to\infty$.

In this chapter we show that economies-of-scale can be achieved for a large range of $\eta$, although the nature of the benefits obtained by operating on large scale depends on the precise capacity sizing rule (hence the parameter $\eta$). We quantify performance in terms of stationary  measures: The mean and variance of the congestion in the system, and the probability of an empty system. For these performance measures we derive heavy-traffic limits under the scalings \eqref{bb} that
 are relatively simple functions of only the first two moments of the demand per period. Such parsimonious expressions are useful for quantifying and improving system behavior. The heavy-traffic limits, however, provide also qualitative insight into the system behavior. Our asymptotic analysis shows that mean congestion is $O(n^\eta)$, which implies
that delays experienced by the customers are negligible for all values of $\eta\in [0,1)$, are roughly constant for $\eta=1$, and grow without bound for $\eta>1$.  We expect this qualitative behavior to be universal for a wide range of stochastic models to which the regime \eqref{bb} is applied.
We further show the existence of the following trichotomy as $n\to \infty$ under \eqref{bb}: For $\eta \in (0,1/2)$ the empty-system probability converges to $1$, for $\eta\in (1/2,1)$ it converges to $0$, while only for $\eta=1/2$ there is a limiting value in $(0,1)$. Hence, as expected, the system performance deteriorates with $\eta$, in a rather crude way for the empty-system probability, and in only a mild way for mean congestion levels. The regime \eqref{bb} thus presents a range of possible capacity sizing rules that all lead to economies-of-scale, and depending on what is the desired nature of performance for a particular service system, an appropriate $\eta$ can be selected. From the quantitative perspective, our detailed asymptotic analysis leads to more precise asymptotic estimates for the performance measures in heavy traffic, which reveal the exact manner in which congestion is influenced by $\eta$ and $\gamma$.\\
\\
\noindent\textbf{Motivating examples.}
The bulk service queueing model is one of the canonical models in queueing theory, having a wide range of applications in fields like digital communication, wireless networks, road traffic, reservation systems, health care and many more (see \cite{Bruneel1993} and \cite[Chap.~5]{johanthesis} for an overview). 
In road traffic, the basic model for congestion at an intersection, known as the fixed-cycle traffic-light queue \cite{Newell1960,Leeuwaarden2006}, is related to our discrete bulk service queue. 
Then $s_n$ represents the maximum number of delayed cars in front of a traffic light that can depart during one green period, while $A^{(n)}_j$ is the number of newly arriving cars during a consecutive green and red period. 

An example from health care is panel sizing  \cite{Zacharias2014}. 
Say a general practitioner has a pool of $n$ clients (typically in the order of \cite{Green2008}), all of which are potential patients, and together require $A^{(n)}_j$ consults per day. 
Further assume that the practitioner can see a maximum number of $s_n$ patients per day. 
What is then an appropriate patient panel size $n$, which strikes a reasonable balance between accessing medical care in a timely manner and restricting the time that the practitioner sits idle? 
The panel size application is one of many examples of an appointment book, referring to some schedule of appointments for a fixed period, with capacity $s_n$ appointments per period and newly arriving appointment $A^{(n)}_j$ per period. 
See \cite{Dai2014} for another recent example of an appointment book in a health care setting, again in terms of our bulk service queue, with $A^{(n)}_j$ the new patients per day and $s_n$ the number of available beds. 

For all examples above, and many more, our new class of heavy-traffic scalings \eqref{bb} presents capacity sizing rules for which the expected performance can be quantified using the results in this chapter. This will be helpful in dimensioning the systems (How much capacity is needed to achieve a certain target performance?) while exploiting economies-of-scale. For appointment books our model together with the capacity sizing rules \eqref{bb} are particularly relevant for {\it advanced access} \cite{Green2008}, a scheduling approach in health care designed to reduce delays by offering every patient a same-day appointment, regardless of the urgency of the problem. In that way, patients do not have to wait long for appointments, and practices do not waste capacity by holding appointments in anticipation of urgent cases.\\
\\*
\noindent\textbf{Pollaczek's formula.}
Next to the freedom to model different situations, another advantage of our model is that it is mathematically tractable, in the sense that it can be subjected to powerful mathematical methods from complex and asymptotic analysis. In order to establish the heavy-traffic limits we start from Pollaczek's formula for the transform of the stationary queue length distribution in terms of a contour integral. From this famous transform representation, contour integrals for the empty-system probability and the mean and variance of the congestion immediately follow. Contour integrals are often amenable to asymptotic evaluation (see e.g.~\cite{Cohen1982}), particularly for obtaining classical heavy-traffic asymptotics. 
We also subject the contour integral representations to asymptotic evaluation, but not under classical heavy-traffic scaling. 
This asymptotic analysis requires a {\it non-standard} saddle point method, tailored to the specific form of the integral expressions that arise under the capacity sizing rule \eqref{bb}. \\
\\*
\noindent
\textbf{Saddle point method.}
In complex analysis, the saddle point method in its standard form is a useful technique to estimate the asymptotic behavior of integrals of the form
\begin{equation}
\label{eq:sp_integral}
I(n) = \int_C h(z)\, \ee^{n f(z)}\, \dd z, 
\end{equation}
as $n\to\infty$, where $C$ is a contour in the complex plane, and $f(z)$ and $h(z)$ are functions that are analytic in some neighborhood of $C$. 
The main idea behind the saddle point method is that if the integrand in \eqref{eq:sp_integral} exhibits a sharp peak along the contour, then one may naturally expect that a small neighborhood around this peak provides the dominant contribution to the integral. 
More specifically, for large values of $n$, the function $f$ and its associated maximum $f(z^*)$ for $z^*\in C$ to a large extent determine the magnitude of the integrand (where $z^*$ is well-defined due to analytically of $f$. 
In the setting of this chapter, $C$ is a closed curve, which implies that the value $z^*$ must be a \textit{saddle-point} of $f$, i.e.~$f'(z^*) = 0$. 
Subsequently, one can replace $f(z)$ in \eqref{eq:sp_integral} by its Taylor expansion around $z^*$ and deduce through the Laplace method, see e.g.~\cite{debruijn}, that
\begin{equation}
I(n) = \sqrt{2\pi}\,i\frac{h(z^*)\,\ee^{n f(z^*)}}{\sqrt{n\, |f''(z^*)|}}\Bigl( 1+ O(1/n)\Bigr),
\end{equation}
as $n\to\infty$.
In Section \ref{spSec}, we show how the contour integrals describing stationary measures for the queue length, derived through Pollaczek's formula, can be reformulated into the shape of \eqref{eq:sp_integral}.
However, we will show that the saddle-point method in its standard from cannot be applied to asymptotically characterize other stationary measures like the mean or mass at zero. 
Indeed, for our model the saddle point (the solution of \eqref{e21}) converges to one (as $n\to\infty$), which is a singular point of the integrand, and renders the standard saddle point method useless.
Non-standard saddle point method discussed in this chapter, originally proposed by \cite{debruijn}, is made specifically to overcome this complication. This leads to asymptotic expansions for the  performance measures, of which the limiting forms correspond to the heavy-traffic limits, and pre-limit forms present refined approximations for pre-limit systems ($n<\infty$) in heavy traffic. Such refinements to heavy-traffic limits are commonly referred to as {\em corrected diffusion approximations} \cite{Siegmund1978,Blanchet2006,Asmussen2003}.



\noindent{\bf Further connections to the literature.}
We now discuss two classes of stochastic systems for which the heavy-traffic regime \eqref{bb1} has been studied extensively, and for which our new family of regimes \eqref{bb} is largely unexplored. We discuss these classes because, despite the Pollaczek formula not to hold, we believe the qualitative results that we reveal for our particular model should to a large extent carry over to these settings as well, presenting some interesting avenues for further research (see Section \ref{subsec62}).

The first class concerns so-called  {\it nearly-deterministic} systems \cite{Sigman2011a,Sigman2011b}, denoted by $G_n/G_n/1$ system, where $G_n$ stands for {\it cyclic thinning} of order $n$, indicating that some  point process is thinned to contain only every $n$th point. As $n\to  \infty$, the $G_n/G_n/1$ systems approach the deterministic $D/D/1$ system. For $G_n/G_n/1$ systems, \cite{Sigman2011a} establishes stochastic-process limits, and \cite{Sigman2011b} derives heavy-traffic limits for stationary waiting times. In the framework of \cite{Sigman2011a,Sigman2011b}, our stochastic model corresponds to a $D/G_n/1$ queue, where the sequence of service times $\{A^{(n)}_j\}_{j\geq 1}$ follows from a cyclically thinned sequence of i.i.d.~random variables $A_{i,j}$. It follows from \cite[Theorem 3]{Sigman2011b} that the rescaled stationary waiting time process converges under \eqref{bb1} to a reflected Gaussian random walk. Hence, the performance measures of the nearly deterministic system, under \eqref{lind} and  \eqref{bb1}, should be well approximated by the performance measures of the reflected Gaussian random walk, giving rise to heavy-traffic approximations. This connection is discussed in detail in Section \ref{subsec3.2}. It seems likely that results similar as in this chapter can be obtained for applying the scaling \eqref{bb} to the nearly-deterministic systems in \cite{Sigman2011a,Sigman2011b}, and because Pollaczek's formula also applies to this setting, the non-standard saddle point method developed in this chapter can provide the appropriate methodology.

The second class concerns multi-server systems, and in particular the many-server regime. When we interpret $s_n$ as the number of servers, instead of capacity per time slot or order of thinning, the scaling \eqref{bb1} is similar to the QED or Halfin-Whitt regime for the $M/M/s_n$ system.
As we have reviewed in Chapter 1, the QED regime is characterized by a delay probability that converges to a non-degenerate limit away from both zero and one, and the mean delay is asymptotically negligible as the number if servers grows large. The QED regime \eqref{bb1} is naturally positioned in between the Quality-Driven (QD) regime and the Efficiency-Driven (ED) regime. In the QD regime, the load remains bounded away from 1, which corresponds to setting $\eta=0$ in \eqref{bb}. Hence, the range $\eta\in(0,1/2)$ bridges the gap between the QED regime and the QD regime. Likewise, the ED regime corresponds to setting $\eta=1$ in \eqref{bb}, so that the range $\eta\in(1/2,1]$ connects the QED regime and ED regime. For the birth-death process describing the $M/M/s_n$ system, Maman \cite{maman} introduced a scaling similar to \eqref{bb}, and called it the QED-$c$ regime, also bridging the ED and QD regimes. 
Theorem 4.1 of \cite{maman} says that the expected waiting time under the scaling $s_n = n\mu+\beta\sigma n^{1-\eta}$ is of order $s_n^{1-\eta}$, which is equivalent to the expected queue length being of order $n^\eta$ by Little's law. We should stress though that we expect the mathematical techniques that are needed to establish heavy-traffic results could be entirely different than in this chapter, because Pollaczek's formula does not apply to many-server settings. 

The specific model assumptions will determine to a large extent the appropriate methodology. Under Markovian assumptions leading to the $M/M/s_n$ system, product-form solutions are available for the stationary distribution. This makes it possible to describe performance measures like the mean congestion directly in terms of real integrals. Where the saddle point method is used for integrals in the complex plane, the Laplace method (see e.g.~\cite{flajolet}) is used for real integrals. Hence, for the asymptotic evaluation of the $M/M/s_n$ system under the scaling \eqref{bb}, the Laplace method seems an appropriate methodology, although again one needs to deal with possible singularities in the integrand. For $G/D/s_n$ systems, which assume deterministic service times, it has been shown in \cite{Jelenkovic2004} that using a decomposition property the dynamics of this multi-server systems can be captured in terms of a single-server system. Hence, for these systems, Pollaczek's formula applies, and our saddle point method can most likely be applied to obtain heavy-traffic results in the regimes \eqref{bb}. Under more general conditions, for instance leading to a $G/G/s_n$ system, it is simply unclear at this stage how to obtain precise heavy-traffic approximations for \eqref{bb}, because a tractable description of the performance measures is not available; see Section 1.2.4 for details.\\
\\
\\*
\noindent{\bf Structure of the chapter.}
In Section \ref{sec1} we present in detail the model and the family of heavy-traffic scalings. In Section \ref{spSec} we introduce the saddle point method. In Section \ref{sec3} we apply the saddle point method for the mean congestion level. Theorem \ref{mainthm} gives for all heavy-traffic scalings the limiting behavior in terms of an integral expression. As a consequence, we show in
 Proposition \ref{prop1} that there are two types of heavy-traffic behavior, depending on whether $\eta\in(0,1/2)$ or $\eta\geq 1/2$.
In Section \ref{subsec3.2} we discuss for the case $\eta=1/2$ the connection with the Gaussian random walk and the Riemann zeta function.
In fact, we show that for all $\eta\geq 1/2$ there exists a connection between the integral expression in Theorem \ref{mainthm} and the Riemann zeta function.
In Section \ref{more} we apply the saddle point method to obtain several more heavy-traffic results, including refined heavy-traffic approximations for the mean congestion level, and the leading heavy-traffic behavior for the variance of the stationary congestion level and for the empty-system probability.
Finally, in Section \ref{numm} we confirm through numerical experiments the accuracy of our heavy-traffic approximations, and moreover show that under \eqref{bb}, various multi-server systems behave similar to our discrete bulk service queue.

\section{Model description \& heavy-traffic regimes}\label{sec1}
We thus consider a discrete stochastic model in which time is divided into periods of equal length. At the beginning of each period $j=1,2,3,...$ new demand $A^{(n)}_j$ arrives to the system. The demands per period $A^{(n)}_1,A^{(n)}_2,\ldots$ are assumed independent and equal in distribution to some non-negative integer-valued random variable $A^{(n)}$.
We will omit the superscript $(n)$ if no ambiguity is possible.
The system has a service capacity $s_n\in\mathbb{N}$ per period, so that the recursion
\begin{equation}
\label{lind}
Q(j+1) = \max\{Q(j) + A^{(n)}_j - s_n,0\},\qquad j=1,2,...,
\end{equation}
assuming $Q(0)=0$, gives rise to a Markov chain $\{Q(j)\}_{j\geq 1}$ that describes the congestion in the system over time. The probability generation function (pgf)
\begin{equation} \label{e2}
\tilde A(z)=\sum_{k=0}^{\infty} \mathbb{P}\big(A^{(n)}=k\big) z^k
\end{equation}
of $A^{(n)}$ is assumed analytic in a disk $|z|<r$ with $r>1$, which implies that all moments of $A^{(n)}$ exist. We also assume that
\begin{equation} \label{e3}
\tilde A'(1)=\E[A^{(n)}_j]=\mu_A<s_n.
\end{equation}

Under the assumption (\ref{e3}) the function $z^{s_n}-\tilde A(z)$ has exactly $s_n$ zeros in the closed unit disk, one of these being $z=1$ (see \cite{rouche}).
We further assume that $\mathbb{P}(A^{(n)}=j)>0$ for some $j>s_n$.
Under this assumption the function
$z^{s_n}-\tilde A(z)$ also has zeros outside $|z|\leq 1$, and we let $r_0$ be the minimum modulus of these zeros.
The number $r_0$ is the unique zero of $z^{s_n}-\tilde A(z)$ with real $z>1$; see e.g.~\cite{Janssen2005}.


Under the assumption (\ref{e3}) the stationary distribution $\lim_{k\to  \infty}\mathbb{P}\left(Q(j)=k\right)=\P(Q=k)$, $k=0,1,\ldots$ exists, with the random variable $Q$ defined as having this stationary distribution.

We let
\begin{equation} \label{e4}
\tilde Q(w)=\sum_{j=0}^{\infty}\mathbb{P}(Q=j)w^j
\end{equation}
be the pgf of the stationary distribution. $\tilde Q(w)$ is analytic in $|w|<r_0$, and given by Pollaczek's formula (see e.g.~\cite{Abate1993, Cohen1982}).
In our discrete setting, we shall first derive a useful expression for $\tilde{Q}(w)$.

\begin{lemma}
For any $\eps>0$ with $1+\eps<r_0$,
\begin{equation} \label{e111}
\tilde Q(w)=\exp\Big(\frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,{\rm ln}\Big(\frac{w-z}{1-z}\Big)\,\frac{(z^{s_n}-\tilde A(z))'}{z^{s_n}-\tilde A(z)}\,\dd z\Big)
\end{equation}
holds when $|w|<1+\eps$. 
\end{lemma}
\begin{proof}
We shall establish (\ref{e111}) for any $w\in(1,1+\eps)$, and then the full result follows from analyticity of $\tilde{Q}(w)$ and of
\begin{equation} \label{e112}
{\rm ln}\Big(\frac{w-z}{1-z}\Big)={\rm ln}\Big(\frac{1-w/z}{1-1/z}\Big)={-}\,\sum_{k=1}^{\infty}\,\frac1k\,\Big(\Big(\frac{w}{z}\Big)^k-\Big(\frac1z\Big)^k\Big)
\end{equation}
in $w$, $|w|<1+\eps$ for any $z$ with $|z|=1+\eps$.

Our starting point is the formula, see \cite{Boudreau1962},
\begin{equation} \label{e113}
\tilde Q(w)=\frac{(s_n-\mu_A)(w-1)}{w^{s_n}-\tilde A(w)}\,\to \sum_{k=1}^{s_n-1}\,\frac{w-z_k}{1-z_k}
\end{equation}
that holds for all $w$, $|w|<r_0$, in which $z_1,\ldots,z_{s_n-1}$ are the $s_n-1$ zeros of $z^{s_n}-\tilde  A(z)$ in $|z|<1$. Fix $w\in(1,1+\eps)$. Then ${\rm ln}\,[(w-z)/(1-z)]$ is analytic in $z\in\mathbb{C}\backslash [1,w]$. It follows that
\begin{align}
 I_C &= \frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,{\rm ln}\Big(\frac{w-z}{1-z}\Big)\,\frac{(z^{s_n}-\tilde A(z))'}{z^{s_n}-\tilde A(z)}\,\dd z \nonumber \\
&=~\sum_{k=1}^{s_n-1}\,{\rm ln}\Big(\frac{w-z_k}{1-z_k}\Big)+\frac{1}{2\pi i}\,\int_C\,{\rm ln}\Big(\frac{w-z}{1-z}\Big)\,\frac{(z^{s_n}-\tilde A(z))'}{z^{s_n}-\tilde A(z)}\,\dd z ,
\label{e114}
\end{align}
where $C$ is a contour encircling $[1,w]$ in the positive sense with none of the $z_k$'s in its interior. We let $\delta\in(0,\frac{w-1}{2})$ and we take $C$ the union of two line segments, from $1+\delta-i0$ to $w-\delta-i0$ and from $w-\delta+i0$ to $1+\delta-i0$, and two circles, of radius $\delta$ and encircling 1 and $w$ in positive sense.
A careful administration of the various contributions to the integral $I_C$ in \eqref{e114}, taking account of the branch cut $[1,w]$, yields
\begin{equation}\label{e115}
I_C = {\rm ln }\left(\frac{(s_n-\mu_A)(w-1)}{w^s-\tilde A(w)}\right) + O(\delta\,{\rm ln}\, \delta ).
\end{equation}
Using this in \eqref{e113} and letting $\delta \downarrow 0$, we get \eqref{e111} for $w\in(1,1+\varepsilon)$ and the proof is complete.
\end{proof} 

Using $\mathbb{P}(Q=0)=\tilde Q(0)$, $\mu_Q=\tilde Q'(1)$ and $\sigma_Q^2  =  \tilde Q''(1)+\tilde Q'(1)-(\tilde Q'(1))^2$,   it follows by straightforward manipulations that
\begin{align} \label{e6}
\mathbb{P}(Q=0)&=\exp\,\Big[\frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,\ln\Big(\frac{z}{z-1}\Big)\frac{(z^{s_n}-\tilde A(z))'}{z^{s_n}-\tilde A(z)}\,\dd z\Big] , \\
\label{e7}
\mu_Q&=\frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,\frac{1}{1-z}~\frac{(z^{s_n}-\tilde A(z))'}{z^{s_n}-\tilde A(z)}\,\dd z ,\\
\label{e8}
\sigma_Q^2 &= \frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,\frac{-z}{(1-z)^2}~\frac{(z^{s_n}-\tilde A(z))'}{z^{s_n}-\tilde A(z)}\,\dd z .
\end{align}
Because $s_n$ appears directly in expressions \eqref{e6}-\eqref{e8}, we will be conducting our analysis with respect to $s_n$ rather than $n$. Note that this has no consequences for our results on the convergence speed of the performance metrics, since $s_n = O(n)$. Furthermore, we will omit the index $n$ when describing the capacity $s_n$ in the remainder of the chapter for brevity.

We next discuss in more detail the family of heavy-traffic scalings considered in this chapter, which combines two features. First, we have assumed that
 $A^{(n)}_j$ is in distribution equal to the sum of work generated by all sources, $A_{1,k}+...+A_{n,j}$, where the $A_{i,j}$ are for all $i$ and $k$ i.i.d.~copies of a random variable $X$, of which the pgf $\tilde X(z)=\sum_{k=0}^{\infty}\mathbb{P}(X=k)z^k$ has radius of convergence $r>1$, and
\begin{equation} \label{e9}
0< \E[A^{(n)}] =n\mu = n \tilde X'(1)<s_n .
\end{equation}
Hence
\begin{equation} \label{e10}
\vartheta:=\frac{n}{s_n}\in(0,1/\mu) .
\end{equation}
Second, we scale the system according to \eqref{bb}, for which we assume that
\begin{equation} \label{e11}
\rho_{s_n} =\vartheta\,\mu =1-\frac{\gamma}{s_n^\eta}
\end{equation}
in which $\gamma>0$ is bounded away from 0 and $\infty$ as $s_n\to  \infty$.
In the remainder of this chapter, we will omit the subscript in $s_n$. 
The condition that $\mathbb{P}(A^{(n)}=k)>0$ for some $k>s$ holds when the degree $d$ of $\tilde X(z)$ (with $d=\infty$ if $\tilde X(z)$ is not a polynomial) is such that $nd>s$.

To avoid certain complications when applying the saddle point method, we further assume that
\begin{equation} \label{e12}
|\tilde X(z)|<\tilde X(r_1) ,~~~~~~|z|=r_1\,,~~z\neq r_1 ,
\end{equation}
for any $r_1\in(0,r)$. This implies that $r_0$ is the unique zero of $z^s-\tilde A(z)$ on $|z|=r_0$.
This condition is related to Cram\'er's condition, see \cite[pp.~189 and 355]{Asmussen2003}, and it has also been used in \cite{relaxation}.
Condition \eqref{e12} holds when the set of all $j=0,1,\ldots$ such that $\mathbb{P}(X=k)>0$ is not contained in an  arithmetic progression with a ratio larger than one (see also \cite{rouche}).


\section{Non-standard saddle point method}\label{spSec}
\noindent
We illustrate our saddle point method for $\mu_Q$.
As a first step, we bring  (\ref{e7}) in a form which is amenable to saddle point analysis.
\begin{lemma}
\begin{equation} \label{e18}
\mu_Q  =  \frac{s}{2\pi i}\,\int_{|z|=1+\eps}\,\frac{g'(z)}{z-1}~\frac{\exp(s\,g(z))}{1-\exp(s\,g(z))}\,\dd z
\end{equation}
with
\begin{equation} \label{e15}
g(z)={-}{\rm ln}\,z+\vartheta\,{\rm ln}(\tilde X(z)) .
\end{equation}
\end{lemma}
\begin{proof}
With $\tilde A(z)=\tilde X^n(z)$,
\begin{align} \label{e13}
\frac{(z^s-\tilde A(z))'}{z^s-\tilde A(z)} & =  \frac{s\,z^{s-1}-n\,\tilde X'(z)\,\tilde X^{n-1}(z)}{z^s-\tilde X^n(z)} \nonumber \\
& =  \frac{s}{z}-\frac{s}{z}\,\Big(\frac{n}{s}~\frac{z\,\tilde X'(z)}{\tilde X(z)}-1\Big)\,\frac{z^{-s}\,\tilde X^n(z)}{1-z^{-s}\,\tilde X^n(z)} .
\end{align}
Write
$
z^{-s}\,\tilde X^n(z)=\exp(s\,g(z))$.
Noting that
\begin{equation} \label{e16}
\frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,\frac{s}{z}~\frac{1}{1-z}\,\dd z=0 ,
\end{equation}
and that
\begin{equation} \label{e17}
g'(z)=\frac1z\,\Big(\vartheta\,\frac{z\,\tilde X'(z)}{\tilde X(z)}-1\Big) ,
\end{equation}
gives \eqref{e18}. \end{proof}

Let us now explain how the standard saddle point method can be applied to \eqref{e18}.
Since
\begin{equation} \label{e19}
g(1)=g(r_0)=0~;~~~~~~g(z)<0\,,~~1<z<r_0 ,
\end{equation}
and by strict convexity of
\begin{equation} \label{e20}
z^{-s}\,\tilde X^n(z)=z^{-s}\tilde A(z)=\sum_{k=0}^{\infty}\,a_k\,z^{k-s} ,~~~~~~z\in(0,r) ,
\end{equation}
 $g(z)$ has a unique minimum on $[1,r_0]$. This minimum is found by solving $z\in[1,r_0]$ from $g'(z)=0$, and this yields the equation
\begin{equation} \label{e21}
\tilde X(z)=\vartheta\,z\,\tilde X'(z) .
\end{equation}
Denote the solution $z\in(1,r_0)$ of (\ref{e21}) by $z_{\rm sp}$, and observe that $z_{\rm sp}$ is a saddle point of $g(z)$, explaining the notation. Thus, the saddle point method can be used for the integral in (\ref{e18}) by taking $1+\eps=z_{\rm sp}$.

In the case that $\vartheta=n/s$ is bounded away from $1/\mu$ as $s\to  \infty$, we have that the minimum value of $g(z)$, $1\leq z\leq r_0$, is negative and bounded away from 0. Furthermore, $z_{\rm sp}$ is bounded away from 1, and the saddle point method can be applied in the classical way by replacing
\begin{equation} \label{e22}
\frac{\exp(s\,g(z))}{1-\exp(s\,g(z))}~~~~{\rm by}~~~~\exp(s\,g(z)) ,
\end{equation}
at the expense of an exponentially small relative error, and performing an expansion of $g'(z)/(z_{\rm sp}-1)=d_1(z-z_{\rm sp})+O((z-z_{\rm sp})^2)$ with $d_1=g''(z_{\rm sp})/(z_{\rm sp}-1)\neq 0$.
 Using that $g(z^{\ast})=(g(z))^{\ast}$, where the $^*$ denotes complex conjugation, it can be shown that
\begin{equation} \label{e23}
\mu_Q=\frac{\exp(s\,g(z_{\rm sp}))}{(z_{\rm sp}-1)^2\,\sqrt{2\pi s\,g''(z_{\rm sp})}}\,(1+O(s^{-1})) .
\end{equation}

We next explain why the standard saddle point method does not work for the heavy-traffic scaling considered in this chapter. Since we operate in (\ref{e11}),
 $\vartheta\mu\to  1$ as $s\to  \infty$, and
\begin{align} \label{e24}
z_{\rm sp}-1&=\frac{\gamma}{a_2\,s^\eta}+O(s^{-2\eta}) ,\\
 \label{e25}
g(z_{\rm sp})&=\frac{-\gamma^2}{2a_2s^{2\eta}}+O(s^{-3\eta}) ,\\
 \label{e26}
g''(z_{\rm sp})&=a_2+O(s^{-\eta}) ,
\end{align}
where
\begin{equation} \label{e27}
a_2=\frac{\sigma^2}{\mu}-\frac{\gamma}{s^\eta}\,\Big(\frac{\sigma^2}{\mu}-1\Big) .
\end{equation}
Hence, $\exp(sg(z))$ near $z=z_{\rm sp}$ is (as $s\to  \infty$):
 vanishingly small when $\eta\in(0,1/2)$,
 bounded away from 1, but non-negligible when $\eta=1/2$,
and tending to 1 when $\eta\in(1/2,\infty)$.
Furthermore, $(z-1)^{-1}$ in \eqref{e18} is unbounded near $z=z_{\rm sp}$ as $s\to  \infty$. Therefore, an adaptation of the standard saddle point method is required, and the resulting asymptotic form of $\mu_Q$ will deviate significantly from the standard case (\ref{e23}). In particular, since $z_{\rm sp}\to  1$, this asymptotic form will contain information from $X(z)$ at $z=1$, rather than at a point away from 1 as is the case in (\ref{e23}).


The required adaption of the saddle point method is modeled after a device developed in \cite[Sec.~5.12]{debruijn}. We use a substitution $z=z(v)$ in (\ref{e18}) with real $v$ and $z(0)=z_{\rm sp}$ such that for sufficiently small $v$,
\begin{equation} \label{e29}
g(z(v))=g(z_{\rm sp})-\tfrac12\,v^2\,g''(z_{\rm sp}) .
\end{equation}
This is feasible, since
\begin{equation} \label{e30}
g(z)=g(z_{\rm sp})+\tfrac12\,g''(z_{\rm sp})(z-z_{\rm sp})^2\Big(1+\frac{g'''(z_{\rm sp})}{3g''(z_{\rm sp})}\,(z-z_{\rm sp})+...\Big)
\end{equation}
with $g''(z_{\rm sp})$ positive and bounded away from 0 as $s\to  \infty$. Hence, $z(v)$ can be found for small $v$ by inverting the equation
\begin{equation} \label{e31}
(z-z_{\rm sp})\Big(1+\frac{g'''(z_{\rm sp})}{3g''(z_{\rm sp})}\,(z-z_{\rm sp})+...\Big)^{1/2}=iv .
\end{equation}
By Lagrange's inversion theorem \cite{debruijn}, there is a $\delta>0$ (independent of $s$) such that
\begin{equation} \label{e32}
z(v)=z_{\rm sp}+iv+\sum_{k=2}^{\infty}\,c_k(iv)^k ,~~~~~~|v|<\delta ,
\end{equation}
with real coefficients $c_k$ (since $g(z)$ is real for real $z$) and
\begin{equation} \label{e33}
c_2={-}\,\frac{g'''(z_{\rm sp})}{6g''(z_{\rm sp})} .
\end{equation}
Thus
\begin{equation} \label{e34}
z(v)=z_{\rm sp}+iv-c_2\,v^2+O(v^3) ,~~~~~~|v|\leq\tfrac12\,\delta ,
\end{equation}
where the order term holds uniformly in $s$. The uniformity statement follows from an inspection of the usual argument
by which Lagrange's theorem is proved, noting that the inversion in \eqref{e29} with $g$ as in \eqref{e15} is considered for $\vartheta\to   1/\mu$, $z_{\rm sp}\to   1$ with radius
of convergence $r$ away from $1$.

By (\ref{e12}) we can restrict the integration in (\ref{e18}) to a fixed but arbitrarily small subset of $|z|=z_{\rm sp}$ near $z=z_{\rm sp}$, at the expense of an exponentially small error. Furthermore, by Cauchy's theorem and again at the expense of an exponentially small error, the integration path can be deformed in accordance with the transformation in (\ref{e29})--(\ref{e34}). Set
\begin{equation} \label{e35}
q(v)=g(z_{\rm sp})-\tfrac12\,v^2\,g''(z_{\rm sp})
\end{equation}
and note that from \eqref{e29}
\begin{equation} \label{e36}
g'(z(v))\,z'(v)={-}v\,g''(z_{\rm sp}) .
\end{equation}
Then substituting $z=z(v)$ in (\ref{e18}),  $\mu_Q$ is given with exponentially small error by
\begin{equation} \label{e37a}
\frac{s}{2\pi i}\,\int_{-\frac12\delta}^{\frac12\delta}\,\frac{g'(z(v))}{z(v)-1}~\frac{\exp(s\,g(z(v)))}{1-\exp(s\,g(z(v)))}z'(v)\,\dd v,
\end{equation}
which gives the following result.
\begin{lemma} \label{lemma2} The mean stationary congestion level is given with exponentially small error by
\begin{equation} \label{e37}
\mu_Q =~\frac{-s}{2\pi i}\,g''(z_{\rm sp})\,\int_{-\frac12\delta}^{\frac12\delta}\,\frac{v}{z(v)-1}~\frac{\exp(s\,q(v))}{1-\exp(s\,q(v))}\,\dd v .
\end{equation}
\end{lemma}


In a similar fashion we get that $\mathbb{P}(Q=0)$ and $\sigma_Q^2$, see (\ref{e6}) and (\ref{e8}), are given, both with exponentially small error, by
\begin{equation} \label{e39}
\frac{-s}{2\pi i}\,g''(z_{\rm sp})\,\int_{-\frac12\delta}^{\frac12\delta}\,v\,{\rm ln}\Big(\frac{z(v)}{z(v)-1}\Big)\frac{\exp(s\,q(v))}{1-\exp(s\,q(v))}\,\dd v
\end{equation}
and
\begin{equation} \label{e38}
\frac{-s}{2\pi i}\,g''(z_{\rm sp})\,\int_{-\frac12\delta}^{\frac12\delta}\,\frac{v\,z(v)}{(z(v)-1)^2}~\frac{\exp(s\,q(v))}{1-\exp(s\,q(v))}\,\dd v,
\end{equation}
respectively.

\section{Heavy-traffic limits for the mean congestion level} \label{sec3}
In this section we apply the non-standard saddle point method explained in Section \ref{spSec} to the Pollaczek integral representation for the mean stationary congestion level $\mu_Q$. In Section \ref{subsec3.1} we first derive an integral representation for the leading order behavior of $\mu_Q$  with a relative error of order $O(s^{-1})$, which serves as a heavy-traffic approximation in the regime $\rho_s=1-\gamma/s^\eta$ with $\eta>0$. We also consider separately the cases of moderate heavy traffic ($\eta\in(0,1/2)$) and extreme heavy traffic ($\eta\in(1/2,\infty)$), for which the integral representation leads to vastly different alternative expressions. We find that $\mu_Q\to   0$ more rapidly than any power of $1/s$ when $\eta\in(0,1/2)$. When $\eta\geq 1/2$ the saddle point method yields an integral representation with relative error $O(s^{-\min(1,\eta)})$.
In Section \ref{subsec3.2} we specialize this general result to the CLT case $\eta=1/2$, and make a connection with existing results.



\subsection{Leading order behavior in integral form} \label{subsec3.1}

 \begin{theorem}\label{mainthm}
The mean stationary congestion level is given by
\begin{equation} \label{e48a}
 \mu_Q=\frac{2}{\pi}\,\sigma\,\sqrt{\dfrac{s}{2\mu}}\,\int_0^{\infty}\,\frac{t^2}{d^2(s)+t^2}~\frac{\exp({-}d^2(s)-t^2)}{1-\exp({-}d^2(s)-t^2)}\,\dd t\,\left(1+O({s^{{-}\min(1,\eta)}})\right)
\end{equation}
with $
d^2(s) = s^{1-2\eta}\gamma^2\mu/(2\sigma^2)$.
\end{theorem}

\begin{proof}
According to Lemma \ref{lemma2}, $\mu_Q$ is given with exponentially small error by (\ref{e37}) with $q(v)$ given in (\ref{e35}). Since $z({-}v)=z^{\ast}(v)$ for real $v$, we have
\begin{eqnarray} \label{e40}
\frac{v}{z(v)-1}+\frac{-v}{z({-}v)-1} &=& {-}2iv\,\frac{{\rm Im}(z(v))}{|z(v)-1|^2}\nonumber\\
&=&~\frac{-2iv^2+O(v^4)}{(z_{\rm sp}-1)^2+v^2-2c_2(z_{\rm sp}-1)\,v^2+O(v^4)} ,
\end{eqnarray}
where (\ref{e34}) and $c_k\in\mathbb{R}$ have been used. Using (\ref{e40}) in (\ref{e37}) and extending the integration range from $[{-}\tfrac12\delta,\tfrac12\,\delta]$ to $({-}\infty,\infty)$ while using symmetry of $q(v)$, we get that $\mu_Q$ is given with exponentially small error by
\begin{eqnarray} \label{e41}
\frac{s\,g''(z_{\rm sp})}{\pi}\,\int_0^{\infty}\,\frac{v^2+O(v^4)}{(z_{\rm sp}-1)^2+v^2-2c_2(z_{\rm sp}-1)\,v^2+O(v^4)}\frac{\exp(s\,q(v))}{1-\exp(s\,q(v))}\dd v .
\end{eqnarray}
With
\begin{equation} \label{e42}
B=\exp(s\,g(z_{\rm sp})) ,~~~~~~\alpha =g''(z_{\rm sp}),
\end{equation}
Equation \eqref{e41} takes the form
\begin{eqnarray} \label{e43}
\frac{s\alpha }{\pi}\,\int_0^{\infty}\,\frac{v^2+O(v^4)}{(z_{\rm sp}-1)^2+v^2-2c_2(z_{\rm sp}-1)\,v^2+O(v^4)} \cdot \frac{B\,\exp({-}\tfrac12\,s\,\alpha \,v^2)}{1-B\,\exp({-}\tfrac12\,s\,\alpha \,v^2)}\dd v .
\end{eqnarray}
In leading order, the integrand in (\ref{e43}) has the form
\begin{equation} \label{e43a}
\frac{B\,v^2\,\exp(-s\,D\,v^2)}{(v^2+C\,s^{-2\eta})(1-\exp({-}s\,D\,v^2))},
\end{equation}
and this is reminiscent of the integrand in \cite[(5.12.3)]{debruijn} for the case  $\kappa=2\eta$. Proceeding as in \cite[Sec.~5.12]{debruijn}, the substitution $v=t\sqrt{{2}/(s\alpha )}$ brings (\ref{e43}) into the form
\begin{eqnarray} \label{e44}
\frac{2}{\pi}\sqrt{\tfrac12 s\,\alpha }\int_0^{\infty}\frac{t^2(1+O(t^2/s))}{\tfrac12 s\,\alpha (z_{\rm sp}-1)^2+t^2-2c_2(z_{\rm sp}-1)t^2+O(t^4/s)} \,\frac{B\,\exp({-}t^2)}{1-B\,\exp({-}t^2)}\dd t .
\end{eqnarray}
From (\ref{e24})--(\ref{e27}) and (\ref{e42}),
\begin{align}
\frac{2}{\pi}\,\sqrt{\frac{s\alpha }{2}} &= \frac{2}{\pi}\,\sigma_X\,\sqrt{\frac{s}{2\,\mu}}\,(1+O(s^{-\eta})),\label{y45}\\
\tfrac12\,s\,\alpha \,(z_{\rm sp}-1)^2 &= d^2(s) + O(s^{1-3\eta}),\label{y46}\\
2\,c_2(z_{\rm sp}-1) &= O(s^{-\eta}),\label{y47}\\
s\,g(z_{\rm sp}) &= -d^2(s) + O(s^{1-3\eta}),\label{y48}
\end{align}
where
\begin{equation} \label{y49}
d^2(s) = \frac{b_0^2}{s^{2\eta-1}},\quad b_0^2 := \frac{\gamma^2\mu}{2\,\sigma^2}.
\end{equation}
In the case that $2\eta-1<0$, we have that $\tfrac12\,s\,\alpha \,(z_{\rm sp}-1)^2 \to   \infty$ and that
\begin{equation} \label{y50}
B = \exp(s\,g(z_{\rm sp})) = O(\exp({-}b^2s^{1-2\eta}))
\end{equation}
for any $b\in(0,b_0)$. From \eqref{e44} it then follows that $\mu_Q = O(\exp({-}b^2\,s^{1-2\eta}))$ for any $b\in(0,b_0)$.
In the case that $2\,\eta-1\geq 0$, we have that $d^2(s)$ is bounded, and using that $1/s^{3\eta-1} = O(d^2(s)/s^\eta)$, we get
\begin{align}
\tfrac12\,s\,\alpha \,(z_{\rm sp}-1)^2 &+ t^2-2\,c_2\,(z_{\rm sp}-1)\,t^2+O(t^4/s) \nonumber\\
&= d^2(s) + t^2 + O\left(s^{-\eta}\,(d^2(s)+t^2)\right) + O(t^4/s)\nonumber\\
&= \left(d^2(s)+t^2\right)\left(1+O(s^{-\eta})+O(t^2/s)\right).\label{y51}
\end{align}
Hence, in this case,
\begin{align} 
& \frac{t^2(1+O(t^2/s))}{\tfrac12 s\,\alpha (z_{\rm sp}-1)^2+t^2-2c_2(z_{\rm sp}-1)t^2+O(t^4/s)}\nonumber\\
 & \qquad \qquad \qquad \qquad = \frac{t^2}{d^2(s)+t^2}\left(1+O(s^{-\eta})+O(t^2/s)\right),\label{y52}
\end{align}
where we restrict to $t$ in a range $[0,s^{1/4}]$. Furthermore,
\begin{align}
1-B\,\exp(-t^2) &= 1-\exp({-}d^2(s)-t^2)\,\left(1+d^2(s)\,O(s^{-\eta})\right)\nonumber\\
&=(1-\exp({-}d^2(s)-t^2))\,\Big(1+\frac{d^2(s)}{\exp(d^2(s)+t^2)-1}O(s^{-\eta})\Big)\nonumber\\
&= (1-\exp({-}d^2(s)-t^2))\,(1+O(s^{-\eta})),\label{y53}
\end{align}
It follows therefore that
\begin{equation} \label{y56}
\frac{B\,\exp({-}t^2)}{1-B\,\exp({-}t^2)} = \frac{\exp({-}d^2(s)-t^2)}{1-\exp({-}d^2(s)-t^2)}\,(1+O(s^{-\eta})).
\end{equation}
Combining the three items \eqref{y45}, \eqref{y52} and \eqref{y56}, we obtain for \eqref{e44} the result
\begin{equation} \label{y58}
\frac{2}{\pi}\,\sigma\,\sqrt{\frac{s}{2\,\mu}}  \int_0^{\infty}\frac{t^2}{d^2(s)+t^2} \cdot \frac{\exp({-}d^2(s)-t^2)}{1-\exp({-}d^2(s)-t^2)}\dd t
\left(1+O(s^{-\eta})+O(s^{-1})\right),
\end{equation}
where the integration range $[0,\infty)$ is, at the expense of relative errors of type\\ $\exp({-}s^{1/4})$, first restricted to the range $[0,s^{1/4}]$, where \eqref{y52} holds, and then restored again to the full range. \end{proof}

Theorem \ref{mainthm} gives the leading-order behavior of $\mu_Q$ as $s\to  \infty$ with a relative error of $O(s^{{-}\min(1,\eta)})$. By considering in more detail the integral expressions, we obtain the following result, describing two different heavy-traffic behaviors.

\begin{proposition}\label{prop1}
If $\eta\in(0,1/2)$ the mean congestion level satisfies
\begin{equation} \label{y59}
\mu_Q=O\left(\exp(-b^2s^{1-2\eta})\right),
\end{equation}
for any $b\in (0,b_0)$. If $\eta\in[1/2,\infty)$ the mean congestion level $\mu_Q$ is given by
\begin{equation} \label{y60}
s^\eta\,\frac{\sigma^2}{2\mu\gamma}\,\left(1+O(s^{\max(1/2-\eta,-1)})\right).
\end{equation}
\end{proposition}
The first assertion in Proposition \ref{prop1} follows from the observation in \eqref{y50}, together with \eqref{e44}. The second assertion is based on a connection between the integral in Theorem \ref{mainthm} and the Riemann zeta function, which is explained in the next subsection.



\subsection{Classical heavy traffic and the Gaussian random walk}
\label{subsec3.2}
We now build on Theorem \ref{mainthm} to obtain further results for the  classical heavy traffic case $\eta=1/2$,
for which we know from \cite[Thm.~3]{Sigman2011b} that the rescaled congestion process converges under \eqref{bb1} to a reflected Gaussian random walk. The latter is defined as
 $(S_\beta(k))_{k\geq 0}$ with $S_\beta(0)=0$ and
\begin{equation}
S_\beta(j)=Y_1+\ldots+Y_j
\end{equation}
with $Y_1,Y_2,\ldots$ i.i.d.~copies of a normal random variable with mean $-\beta$ and variance 1.
Assume $\beta>0$ (negative drift), and denote the all-time maximum of this random walk by ${M}_\beta$.


 Denote by $Q^{(s)}_\infty$ the stationary congestion level for a fixed $s$ (that arises from taking
 $j\to   \infty$ in \eqref{lind}), and remember that we have assumed $\vartheta=n/s$ fixed.
Then, using $\rho_s=1-\gamma/\sqrt{s}$, with
 \begin{equation}\label{gammachoice}
 \gamma=\frac{\beta\sigma}{\mu\sqrt{\vartheta}},
\end{equation}
the spatially-scaled stationary congestion levels reach the limit
$Q^{(s)}_\infty/(\sigma\sqrt{n}) \Rightarrowd {M}_\beta$ as $s,n\to  \infty$ (see \cite{Jelenkovic2004,Sigman2011a,Sigman2011b}). From \cite[Thm.~4]{Sigman2011b} we then know that under the standard heavy-traffic scaling \eqref{bb1}
\begin{equation}
   \frac{\mathbb{E}Q^{(s)}_\infty}{\sigma\sqrt{n}}\to   \mathbb{E}{M}_\beta, \quad {\rm as} \ s,n\to  \infty,
\end{equation}
   from which it follows that
   \begin{equation} \label{e48}
\mu_Q\approx \sigma\sqrt{n}\ \mathbb{E}M_\beta.
\end{equation}
The random variable ${M}_\beta$ was studied in  \cite{Chang1997,Janssen2006}. In particular, \cite[Thm.~2]{Janssen2006} yields, for $\beta<2\sqrt{\pi}$,
\begin{equation}\label{wdfegfw571}
\mathbb{E}{M}_\beta= \frac{1}{2\beta}+\frac{\zeta(1/2)}{\sqrt{2\pi}}+\frac{\beta}{4}+\frac{\beta^2}{\sqrt{2\pi}}\sum_{r=0}^{\infty}\frac{\zeta(-1/2-r)}{r!(2r+1)(2r+2)}\left(\frac{-\beta^2}{2 }\right)^r,
\end{equation}
where $\zeta$ denotes the Riemann zeta function. 
Hence, for small values of $\beta$,
   \begin{equation} \label{estimate}
\mu_Q\approx \sigma\sqrt{n}\ \mathbb{E}M_\beta \approx \frac{\sigma\sqrt{n}}{2\beta} = \sqrt{s}\,\frac{\sigma^2}{2\mu\gamma}.
\end{equation}
We will now show how the approximation \eqref{estimate} follows from Theorem \ref{mainthm}, and also how similar steps give rise to Proposition \ref{prop1}.

Consider the integral
\begin{equation} \label{e49}
G_0(b)=G_1(b)-G_2(b)=\int_0^{\infty}\,\frac{t^2}{b^2+t^2}~\frac{\exp({-}b^2-t^2)}{1-\exp({-}b^2-t^2)}\,\dd t ,
\end{equation}
where $b>0$ and
\begin{equation} \label{e50}
G_1(b)=\int_0^{\infty}\,\frac{\exp({-}b^2-t^2)}{1-\exp({-}b^2-t^2)}\,\dd t\,,~~~~G_2(b)=\int_0^{\infty}\,\frac{b^2}{b^2+t^2}~\frac{\exp({-}b^2-t^2)}{1-\exp({-}b^2-t^2)}\dd t .
\end{equation}
We have, as in \cite[Sec.~2]{Janssen2006},
\begin{align} \label{e51}
G_1(b) & =  \sum_{k=0}^{\infty}\:\int_0^{\infty}\,\exp({-}(k+1)(b^2+t^2))\,\dd t \nonumber \\
& =  \frac{\sqrt{\pi}}{2}\,\sum_{k=0}^{\infty}\,\frac{\ee^{-(k+1)b^2}}{\sqrt{k+1}} = \frac{\sqrt{\pi}}{2}\,\ee^{-b^2}\,\Phi(\ee^{-b^2},1/2,1) \nonumber \\
& =  \frac{\pi}{2b}+\frac{\sqrt{\pi}}{2}\,\sum_{r=0}^{\infty}\,\zeta(\tfrac12-r)\,\frac{({-}1)^r\,b^{2r}}{r!} ,
\end{align}
where $\Phi(z,s,v)$ is Lerch's transcendent and where the last identity holds when $0<b<\sqrt{2\pi}$.

As to $G_2(b)$, we make a connection with the complementary error function
\begin{equation} \label{e52}
{\rm erfc}(z)=\frac{2}{\sqrt{\pi}}\,\int_z^{\infty}\,\ee^{-t^2}\,\dd t=\frac{2}{\pi}\,\ee^{-z^2}\,\int_0^{\infty}\,\frac{\ee^{-z^2t^2}}{1+t^2}\dd t ,
\end{equation}
see \cite[Secs.~7.2 and 7.7.1]{NIST} We thus compute
\begin{align} \label{e53}
G_2(b) & =  \sum_{k=0}^{\infty}\,\ee^{-(k+1)b^2}\,\int_0^{\infty}\,\frac{b^2}{b^2+t^2}\,\ee^{-(k+1)t^2}\dd t \nonumber \\
& =  \frac{\pi}{2}\,b\,\sum_{k=0}^{\infty}\,{\rm erfc}(b\,\sqrt{k+1}) .
\end{align}
From \cite[(4.3) and (4.23)]{Janssen2006},
\begin{equation} \label{e54}
\sum_{n=1}^{\infty}\,\frac{1}{\sqrt{2\pi}}\,\int_{\beta\sqrt{n}}^{\infty}\,\ee^{-x^2/2}\,dx= \frac{1}{2\beta^2}-\frac14-\frac{1}{\sqrt{2\pi}}\,\sum_{r=0}^{\infty} \frac{\zeta({-}1/2-r)({-}1/2)^r} {r!\,(2r+1)}\,\beta^{2r+1}
\end{equation}
in which $0<\beta<2\sqrt{\pi}$. Taking $\beta=b\,\sqrt{2}$ in (\ref{e54}), we get
\begin{equation} \label{e55}
G_2(b)=\frac{\pi}{4b}-\frac{\pi}{4}\,b-\sqrt{\pi}\,\sum_{r=0}^{\infty}\,\frac{\zeta({-}1/2-r)({-}1)^r\,b^{2r+2}}{r!\,(2r+1)}
\end{equation}
when $0<b<\sqrt{2\pi}$. The two results in (\ref{e51}) and (\ref{e55}) can be combined, as in \cite[Sec.~ \ref{sec4}]{Janssen2006}, and this yields
\begin{equation} \label{e56}
G_0(b)=\frac{\pi}{4b}+\frac{\pi}{4}\,b+\frac{\sqrt{\pi}}{2}\,\zeta(1/2)+\sqrt{\pi}\,\sum_{r=0}^{\infty}\frac{\zeta({-}1/2-r)({-}1)^r\,b^{2r+2}}{r!\,(2r+1)(2r+2)}
\end{equation}
when $0<b<\sqrt{2\pi}$. 

Using (\ref{e56}) in (\ref{e48}), we find that the leading order behavior of $\mu_Q$ is given as
\begin{equation} \label{e57}
\sigma_X\,\sqrt{\dfrac{s}{2\mu}}\,\left[\frac{1}{2b_0}+\frac{b_0}{2}+\frac{\zeta(1/2)}{\sqrt{\pi}}+\frac{2}{\sqrt{\pi}}\,\sum_{r=0}^{\infty}\,\frac{\zeta({-}1/2-r)({-}1)^r b_0^{2r+2}} {r!\,(2r+1)(2r+2)}\right]
\end{equation}
with relative error of $O(s^{-1/2})$ in which $b_0$ is given by \eqref{y49}. The expression (\ref{e57}) is exactly equal to the right-hand side of \cite[(4.25)]{Janssen2006} times $\sqrt{s}$ when we take there $\sigma=\mu=1$ and $\beta=b_0\,\sqrt{2}$.
Notice that, with $\gamma$ as in \eqref{gammachoice},
\begin{equation} \label{e57a}
\sigma\,\sqrt{\dfrac{s}{2\mu}}\frac{1}{2b_0}=\frac{\sigma\sqrt{n}}{2\beta},
\end{equation}
which confirms the approximation \eqref{estimate}.

According to Theorem \ref{mainthm}, we have for $\eta\geq 1/2$,
\begin{equation} \label{y61}
\mu_Q = \frac{2}{\pi}\,\sigma\,\sqrt{\frac{s}{2\,\mu}}G_0(d(s))\,\left(1+O(s^{{-}\min(1,\eta)})\right).
\end{equation}
When $\eta=1/2$, so that $d(s) = b_0$ is independent of $s$, the series representation for $G_0$ in \eqref{e56} can be used, as long as $b_0\in(0,\sqrt{2\pi})$. When $\eta>1/2$, we have that $d(s) = b_0/s^{\eta-1/2}\to   0$ as $s\to  \infty$, and so this series representation can be used when $s$ is large enough. We then have from \eqref{e56} and $b_0^2 = \gamma^2\mu/2\,\sigma^2$, while replacing the whole series at the right-hand side by $O(b^2)$, for $\mu_Q$ the leading order behavior
\begin{equation} \label{y62}
s^\eta\left[\frac{\sigma^2}{2\,\gamma\,\mu}+\frac{\sigma\,\zeta(1/2)}{\sqrt{2\,\pi\,\mu}}\,\frac{1}{s^{\eta-1/2}}+\frac{1}{4}\,\gamma\,\frac{1}{s^{2\eta-1}}+O(s^{3/2-3\eta})\right]
\end{equation}
with relative error $O(s^{{-}\min(1,\eta)})$. Retaining the constant term $\sigma^2/(2\gamma\mu)$ and estimating the other terms between the brackets in \eqref{y62} as $O(s^{1/2-\eta})$, we get Proposition \ref{prop1}.
\section{More heavy-traffic results}\label{more}
In this section we apply the non-standard saddle point method to obtain several more heavy-traffic results. In Section \ref{subsec3.3} we derive refined heavy-traffic approximations for the mean congestion level by considering higher-order correction terms. In Section \ref{sec4} we derive the leading heavy-traffic behavior for the variance of the stationary congestion level, and in Section \ref{sec5} for the empty-system probability. To keep the developments tractable, we restrict Section \ref{subsec3.3} to $\eta=1/2$, and Section \ref{sec4} and Section \ref{sec5} to $\eta\in(0,1]$, although the same technique will work for all values $\eta>0$.


\subsection{Correction term for the mean congestion level for $\eta = 1/2$} \label{subsec3.3}
Our saddle point method not only establishes the leading-order heavy-traffic approximations, but also allows to derive refinements to these approximations. In this section we demonstrate how this works for the mean congestion level in the case $\eta=1/2$.

To obtain a refinement or correction term from (\ref{e44}), we must be more precise about the $O(s^{{-}\eta})$ terms that occur in the approximations in Section \ref{subsec3.1} for $\frac12\,s\,\alpha (z_{\rm sp}-1)^2$, $B$ and $\sqrt{s\,\alpha /2}$. When higher-order corrections are required, we should include higher-order terms in the approximations of these quantities, and be more specific about the $O(t^2/s)$ and $O(t^4/s)$  in the integrand in (\ref{e44}).

Denote, see \eqref{e10} and (\ref{e15}) with $\vartheta=(1-\gamma/s^\eta)\,\mu^{-1}$,
\begin{equation} \label{e58}
a_i=g^{(i)}(1);~~~~~~g(z)={-}{\rm ln}\,z+\vartheta\,{\rm ln}\,\tilde X(z) .
\end{equation}
Dropping the $X$ from $\mu$ and $\sigma^2$ for brevity, we have
\begin{equation} \label{e59}
a_1={-}\,\frac{\gamma}{s^\eta} ,~~~~~~a_2=\frac{\sigma^2}{\mu}-\frac{\gamma}{s^\eta}\,\Big(\frac{\sigma^2}{\mu}-1\Big) ,
\end{equation}
\begin{equation} \label{e60}
a_3={-}2+\Big(1-\frac{\gamma}{s^\eta}\Big)\Big(\frac{\tilde X'''(1)}{\tilde X'(1)}-3\tilde X''(1)+2(\tilde X'(1))^2\Big) .
\end{equation}
For the purpose of finding a first-order correction term, we note that
\begin{align} \label{e61}
\alpha &=g''(z_{\rm sp})=a_2+(z_{\rm sp}-1)\,a_3+O(s^{-1}) ,\\
\label{e62}
z_{\rm sp}-1&={-}\,\frac{a_1}{a_2}-\frac{a_3}{2a_2}\,\Big(\frac{a_1}{a_2}\Big)^2+O(s^{-3/2}) ,\\
 \label{e63}
c_2&={-}\,\frac{g'''(z_{\rm sp})}{6g''(z_{\rm sp})}={-}\,\frac{a_3}{6a_2}+O(s^{-1/2}) ,\\
 \label{e64}
g(z_{\rm sp})&={-}\,\frac{a_1^2}{2a_2}-\frac{a_3}{6a_2^3}\,a_1^3+O(s^{-2}) .
\end{align}
This gives rise to
\begin{align} \label{e65}
\sqrt{\tfrac12\,s\,\alpha }&=\sigma\,\sqrt{\dfrac{s}{2\mu}}\,\Big(1+\frac{C_1}{\sqrt{s}}+O(s^{-1})\Big) ,\\
\tfrac12\,s\,\alpha (z_{\rm sp}-1)^2&=\frac{\gamma^2\,\mu}{2\sigma^2}+\frac{C_2}{\sqrt{s}}+O(s^{-1}) ,\\
\label{e67}
2c_2(z_{\rm sp}-1)&=\frac{C_3}{\sqrt{s}}+O(s^{-1}) ,\\
 \label{e68}
B=\exp(s\,g(z_{\rm sp}))&=\exp\Big({-}\,\frac{\gamma^2\,\mu}{2\sigma^2}\Big)\Big(1+\frac{C_4}{\sqrt{s}}+O(s^{-1})\Big) ,
\end{align}
with explicitly computable constants $C_1$, $C_2$, $C_3$, $C_4$. Remembering that $b_0^2=\gamma^2\mu/2\sigma^2$, see \eqref{y49}, we then get with errors of order $1/s$
\begin{eqnarray} \label{e69}
& \mbox{} & \frac{t^2(1+O(t^2/s))}{\frac12\,s\,\alpha (z_{\rm sp}-1)^2+t^2-2c_2(z_{\rm sp}-1)\,t^2+O(t^4/s)} \nonumber \\[3mm]
& & \qquad =~\frac{t^2}{b_0^2+t^2}-\frac{1}{\sqrt{s}}\,\Big((C_2+ b_0^2\,C_3)\,\frac{t^2}{(b_0^2+t^2)^2}-C_3\,\frac{t^2}{b_0^2+t^2}\Big) ,
\end{eqnarray}
and
\begin{equation} \label{e70}
\frac{B\,\exp({-}t^2)}{1-B\,\exp({-}t^2)}=\frac{\exp({-}b_0^2-t^2)}{1-\exp({-}b_0^2-t^2)}+\frac{C_4}{\sqrt{s}}~\frac{\exp({-}b_0^2-t^2)}{(1-\exp({-}b_0^2-t^2))^2} .
\end{equation}
Using (\ref{e65}), (\ref{e69}) and (\ref{e70}) in (\ref{e44}) we get with an absolute error of order $1/\sqrt{s}$
\begin{align} \label{e71}
\mu_Q & =\frac{2}{\pi}\,\sigma\,\sqrt{\dfrac{s}{2\mu}}\,\Big(1+\frac{C_1}{\sqrt{s}}\Big)\nonumber \\
& \qquad\qquad \cdot \int_0^{\infty}\,\Big(\frac{t^2}{b_0^2+t^2}-\frac{1}{\sqrt{s}}\,\Big((C_2+b_0^2\,C_3)\,\frac{t^2}{(b_0^2+t^2)^2}-C_3\,\frac{t^2}{b_0^2+t^2}\Big)\Big) \nonumber \\
& \qquad\qquad\qquad \cdot~\Big(\frac{\exp({-}b_0^2-t^2)}{1-\exp({-}b_0^2-t^2)}+\frac{C_4}{\sqrt{s}}~\frac{\exp({-}b_0^2-t^2)}{(1-\exp({-}b_0^2-t^2))^2}\Big)\dd t \nonumber \\
& =\frac{2\sigma}{\pi}\,\sqrt{\dfrac{s}{2\mu}}\,G_0(b_0)\nonumber\\
& \qquad\qquad + ~\frac{2\sigma}{\pi}\,\sqrt{\dfrac{1}{2\mu}}\,\big((C_1+C_3)\,G_0(b_0)-(C_2+b_0^2\,C_3)\,G_3(b_0)+C_4\,G_4(b_0)\big) ,
\end{align}
where $G_0$ is as in (\ref{e49}), and
\begin{align} \label{e72}
G_3(b_0)&=\int_0^{\infty}\,\frac{t^2}{(b_0^2+t^2)^2}~\frac{\exp({-}b_0^2-t^2)}{1-\exp({-}b_0^2-t^2)}\dd t ,\\
\label{e73}
G_4(b_0)&=\int_0^{\infty}\,\frac{t^2}{b_0^2+t^2}~\frac{\exp({-}b_0^2-t^2)}{(1-\exp({-}b_0^2-t^2))^2}\dd t .
\end{align}
We shall express the integrals in (\ref{e72}) and (\ref{e73}) in terms of $\zeta$-functions. By partial integration
\begin{align} \label{e74}
G_3(b) & =  \frac12\,\int_0^{\infty}\,\frac{1}{b^2+t^2}~\frac{\exp({-}b^2-t^2)}{1-\exp({-}b_0^2-t^2)}\,\dd t \nonumber \\ 
&\qquad\qquad -~\int_0^{\infty}\,\frac{t^2}{b^2+t^2}~\frac{\exp({-}b^2-t^2)}{(1-\exp({-}b^2-t^2))^2}\dd t \nonumber \\
& =  \frac{1}{2b^2}\,G_2(b)-G_4(b) ,
\end{align}
see (\ref{e49}) and (\ref{e73}). Since $G_2(b)$ is expressed in terms of $\zeta$-functions in (\ref{e55}), it is sufficient to consider $G_4(b)$.

As to $G_4(b)$,
\begin{equation} \label{e75}
G_4(b)=G_5(b)-G_6(b) ,
\end{equation}
where
\begin{align} \label{e76}
G_5(b)&=\int_0^{\infty}\,\frac{\exp({-}b^2-t^2)}{(1-\exp({-}b^2-t^2))^2}\,\dd t ,\\
 \label{e77}
G_6(b)&=\int_0^{\infty}\,\frac{b^2}{b^2+t^2}~\frac{\exp({-}b^2-t^2)}{(1-\exp({-}b^2-t^2))^2}\,\dd t .
\end{align}
We have, compare (\ref{e51}),
\begin{align} \label{e78}
G_5(b) & =  \sum_{k=0}^{\infty}\,(k+1)\,\int_0^{\infty}\,\ee^{-(k+1)(b^2+t^2)}\,\dd t \nonumber \\[3.5mm]
& =  \frac{\sqrt{\pi}}{2}\,\ee^{-b^2}\,\Phi(\ee^{-b^2},{-}\tfrac12,1) =  \frac{\pi}{4b^3}+\frac{\sqrt{\pi}}{2}\,\sum_{r=0}^{\infty}\,\zeta({-}\tfrac12-r)\,\frac{({-}1)^r\,b^{2r}}{r!} ,
\end{align}
the last identity being valid when $0<b<\sqrt{2\pi}$. Next we have, compare (\ref{e53}),
\begin{align} \label{e79}
G_6(b) & =  \sum_{k=0}^{\infty}\,(k+1)\,b^2\,\int_0^{\infty}\,\frac{\exp({-}(k+1)(b^2+t^2))}{b^2+t^2}\dd t \nonumber \\
& =  \frac{\pi}{2}\,b\,\sum_{k=0}^{\infty}\,(k+1)\,{\rm erfc}(b\,\sqrt{k+1}) .
\end{align}
From \cite[(5.4) and (5.21)]{Janssen2006} we have
\begin{eqnarray} \label{e80}
\sum_{n=1}^{\infty}\frac{n}{\sqrt{2\pi}}\int_{\beta\sqrt{n}}^{\infty}\ee^{-x^2/2}\,dx = \frac{3}{4\beta^4}-\frac{1}{24}-\frac{1}{\sqrt{2\pi}}\sum_{r=0}^{\infty}\frac{\zeta({-}3/2-r)({-}1/2)^r}{r!\,(2r+1)}\,\beta^{2r+1}
\end{eqnarray}
when $0<\beta<2\sqrt{\pi}$. Taking $\beta=b\,\sqrt{2}$ in (\ref{e80}), we get
\begin{equation} \label{e81}
G_6(b)=\frac{3\pi}{16b^2}-\frac{\pi b}{24}-\sqrt{\pi}\,\sum_{r=0}^{\infty}\frac{\zeta({-}3/2-r)({-}1)^r}{r!\,(2r+1)}\,b^{2r+2}
\end{equation}
when $0<b<\sqrt{2\pi}$. The two results (\ref{e78}) and (\ref{e81}) can be combined, as in \cite[Sec.~5]{Janssen2006} and this yields
\begin{equation} \label{e82}
G_4(b)=\frac{\pi}{16b^3}+\frac{\pi b}{24}+\tfrac12\,\zeta({-}1/2)\,\sqrt{\pi}+\sqrt{\pi}\,\sum_{r=0}^{\infty}\frac{\zeta({-}3/2-r)({-}1)^r\,b^{2r+2}}{r!\,(2r+1)(2r+2)}
\end{equation}
when $0<b<\sqrt{2\pi}$.

Finally, we can use (\ref{e82}) in (\ref{e74}), and we obtain with (\ref{e55}), for $0<b<\sqrt{2\pi} $,
\begin{align} \label{e83}
G_3(b) = &  \frac{\pi}{16b^3}-\frac{\pi}{8b}-\frac{\pi b}{24}-\zeta({-}1/2)\,\sqrt{\pi}  -~2\sqrt{\pi}\,\sum_{r=0}^{\infty}\,\frac{\zeta({-}3/2-r)({-}1)^r\,b^{2r+2}}{r!\,(2r+1)(2r+2)(2r+3)}.
\end{align}
The right-hand side of (\ref{e83}) equals the right-hand side of \cite[(2.3)]{Janssen2006} multiplied by ${\pi}/{(2b)}$ with $\beta=b\,\sqrt{2}$. 
\subsection{Variance of the congestion level}\label{sec4}
We have from (\ref{e38}) in Section \ref{sec1}, using the same approach and notation as in Section \ref{subsec3.1} for $\mu_Q$, that $\sigma_Q^2$ is given with exponentially small error by
\begin{equation} \label{e84}
\frac{-s\,\alpha }{2\pi i}\,\int_{-\frac12\delta}^{\frac12\delta}\,\frac{v\,z(v)}{(z(v)-1)^2}~\frac{B\,\exp({-}\frac12\,s\,\alpha \,v^2)}{1-B\,\exp({-}\frac12\,s\,\alpha \,v^2)}\dd v,
\end{equation}
with $B$ and $\alpha $ given in (\ref{e42}). From $z({-}v)=z^{\ast}(v)$ for real $v$ we now compute
\begin{equation} \label{e85}
\frac{z(v)}{(z(v)-1)^2}-\frac{z({-}v)}{(z({-}v)-1)^2}={-}2i\,\frac{|z(v)|^2-1}{|z(v)-1|^4}\,{\rm Im}(z(v)) ,
\end{equation}
and so (\ref{e84}) becomes
\begin{equation} \label{e86}
\frac{s\alpha }{\pi}\,\int_0^{\frac12\delta}\,\frac{|z(v)|^2-1}{|z(v)-1|^4}\,v\,{\rm Im}(z(v))\,\frac{B\,\exp({-}\frac12\,s\,\alpha \,v^2)}{1-B\,\exp({-}\frac12\,s\,\alpha \,v^2)}\dd v .
\end{equation}
From
\begin{equation} \label{e87}
{\rm Im}(z(v))=v+O(v^3) ,~~~~~~|z(v)|^2-1=z_{\rm sp}^2-1+O(v^2) ,
\end{equation}

we get for the expression in \eqref{e86}
\begin{equation} \label{y70}
\frac{s\alpha }{\pi}\,\int_0^{\frac{1}{2}\delta}\,\frac{v^2\,(z_{\rm sp}^2-1+O(v^2))(1+O(v^2))}{((z_{\rm sp}-1)^2+v^2 + O((z_{\rm sp}-1)\,v^2)+O(v^4))^2}
\frac{B\,\exp({-}\frac12\,s\,\alpha \,v^2)}{1-B\,\exp({-}\frac12\,s\,\alpha \,v^2)}\dd v.
\end{equation}
 When $2\eta-1<0$, we have as for the case of $\mu_Q$ in Section \ref{subsec3.1} that the whole expression in \eqref{y70} is $O(\exp({-}b^2\,s^{1-2\eta}))$ for any $b\in(0,b_0)$, as $s\to  \infty$. When $2\eta-1\geq 0$, we get as in the case of $\mu_Q$ after substitution $v = t\sqrt{{2}/{(s\,\alpha })}$ for the expression in \eqref{y70}
\begin{equation}  \label{y71}
\frac{2}{\pi}\,\Big(\frac{s\,\alpha }{2}\Big)^{3/2}\,\int_0^\infty\frac{t^2\,(z_{\rm sp}^2-1+O(t^2/s))(1+O(t^2/s))}{(d^2(s)+t^2)^2\,(1+O(1/s^{\eta})+O(t^2/s))}~\frac{B\,\ee^{{-}t^2}}{1-B\,\ee^{{-}t^2}}\dd t.
\end{equation}
When $2\eta-1\geq 0$, the leading order behavior of $\sigma_Q^2$ depends crucially on the factor $z_{\rm sp}^2-1+O(t^2/s)$, where
\begin{equation} \label{y72}
z_{\rm sp}^2-1 = \frac{2\,\gamma\,\mu}{\sigma^2\,s^\eta}\,\left(1+O(s^{-\eta})\right)
\end{equation}
is dominant when $\eta<1$, while the $O(t^2/s)$ is dominant when $\eta>1$. In the case that $\eta\in(1/2,1)$, we get for the leading order behavior of $\sigma_Q^2$
\begin{align}
\frac{2}{\pi}\,\Big(\frac{s\,\alpha }{2}\Big)^{3/2}& \,\frac{2\,\gamma\,\mu}{\sigma^2\,s^\eta}\,\int_0^\infty\frac{t^2}{(d^2(s)+t^2)^2}\cdot~\frac{\ee^{{-}d^2(s)-t^2}}{1-\ee^{{-}d^2(s)-t^2}}\dd t\,\left(1+O(s^{\eta-1})\right)\nonumber\\
&= \frac{\gamma\,\sigma}{\pi}\,\Big(\frac{2}{\mu}\Big)^{1/2}\,s^{3/2-\eta}\,G_3(d(s))\,\left(1+O(s^{\eta-1})\right), \label{y73}
\end{align}
where \eqref{e26}, \eqref{e27} and \eqref{e42} have been used for $\alpha  = g''(z_{\rm sp})$ and where $G_3$ is given in \eqref{e72}.

When we insert the expansion \eqref{e83} for $G_3(b)$, with the whole series on the second line being $O(b^2)$, we get the leading order behavior of $\sigma_Q^2$ as
\begin{align}
s^{2\eta}\,\Big( \frac{\sigma^4}{4\,\gamma^2\mu^2}- \frac{\sigma^2}{4\,\mu}&\,\frac{1}{s^{2\eta-1}} - \Big(\frac{2\,\sigma^2}{\pi\,\mu}\Big)^{1/2}\,\frac{\gamma\,\zeta(-1/2)}{s^{3\eta-3/2}}\nonumber\\
& - \frac{\gamma^2}{24\,s^{5\eta-5/2}}+O(s^{1-4\eta})\Big)\,\left(1+O(s^{\eta-1})\right)\nonumber \\
&\ = s^{2\eta}\,\frac{\sigma^4}{4\,\gamma^2\,\mu^2}\,\Big(1+O(s^{\max(1-2\eta,\eta-1)})\Big)\label{y74}
\end{align}
when $\eta\in(1/2,1)$. For the case $\eta=1/2$, we get the leading order behavior, assuming $0<b_0<\sqrt{2\pi}$,
\begin{align}
\frac{\sigma^2 s}{\mu}\left[ \frac{1}{8\,b_0^2} - \frac{1}{4}-\frac{1}{12}\,b_0^2 - \frac{2\,\zeta(-1/2)}{\sqrt{\pi}}\,b_0- \frac{4}{\sqrt{\pi}}\,\sum_{r=0}^\infty \frac{\zeta(-3/2-r)\,(-1)^r\,b_0^{2r+3}}{r!\,(2r+1)\,(2r+2)\,(2r+3)} \right]\label{y75}
\end{align}
with relative error $O(s^{-1/2})$. The expression between brackets in \eqref{y75} coincides with the right-hand side of \cite{Janssen2006}, (2.3) with $\beta = b_0\,\sqrt{2}$.

This leads to the following two results.
\begin{theorem} \label{varthm}
For $\eta\in[1/2,1)$,
\begin{equation} \label{y76}
\sigma_Q^2 = \frac{\gamma\,\sigma_X}{\pi}\,\sqrt{\frac{2}{\mu}}\,s^{3/2-\eta}\,G_3(d(s))\,\left(1+O(s^{\eta-1})\right)
\end{equation}
with $G_3$ given in \eqref{e72}.
\end{theorem}

\begin{proposition}\label{varprop}
For $\eta\in(0,1/2)$, and for all $b<b_0$,
\begin{equation}
\sigma_Q^2 = O(\exp({-}b^2\,s^{1-2\eta})).
 \end{equation}
 For $\eta = 1/2$, $\sigma_Q^2$ equals expression \eqref{y75} with relative error $O(s^{-1/2})$. For $\eta\in(1/2,1)$ and $b_0\in(0,\sqrt{2\pi})$, $\sigma_Q^2$ has the form in \eqref{y74}.
\end{proposition}

As in Section \ref{subsec3.3} for the mean congestion level
with $\eta=1/2$, it is possible to give a correction term which involves now integrals and series with $\zeta$-functions as considered in \cite[Secs.~4-5]{Janssen2007}.


\subsection{The empty-system probability} \label{sec5}

We have from (\ref{e6}) by proceeding as in (\ref{e13})--(\ref{e17}) that
\begin{align} \label{e100}
{\rm ln}\,[Q(0)] & =  \frac{s}{2\pi i}\,\int_{|z|=1+\eps}\,{\rm ln}\Big(\frac{z}{z-1}\Big)\,\frac{g'(z)\,\exp(s\,g(z))}{1-\exp(s\,g(z))}\,dz \nonumber \\[3.5mm]
& =  \frac{1}{2\pi i}\,\int_{|z|=1+\eps}\,\frac{1}{z(z-1)}\,{\rm ln}\left(1-\exp(s\,g(z))\right)\,dz ,
\end{align}
where in the last step we used partial integration (noting that ${\rm Re}\,[g(z)]<0$ on $|z|=1+\eps$). Then, as in Section \ref{sec1} for $\mu_Q$, the last integral in (\ref{e100}) is, with exponentially small error, given by
\begin{equation} \label{e101}
\frac{1}{2\pi i}\,\int_{-\frac12\delta}^{\frac12\delta}\,\frac{z'(v)}{z(v)(z(v)-1)}\,{\rm ln}\left(1-B\,\ee^{-\frac12 s\alpha  v^2}\right)\,\dd v .
\end{equation}
Now for $v\geq0$ from $z({-}v)=z^{\ast}(v)$, $z'({-}v)={-}(z'(v))^{\ast}$
\begin{eqnarray} \label{e102}
& \mbox{} & \hspace*{-6mm}\frac{z'(v)}{z(v)(z(v)-1)}+\frac{z'({-}v)}{z({-}v)(z({-}v)-1)}=2i\,{\rm Im}\,\Big[\frac{z'(v)}{z(v)(z(v)-1)}\Big] \nonumber \\[3.5mm]
& & \hspace*{-6mm}=~2i\,{\rm Im}\,\Big[\frac{z'(v)\,z^{\ast}(v)(z^{\ast}(v)-1)}{|z(v)|^2\,|z(v)-1|^2}\Big] \nonumber \\[3.5mm]
& & \hspace*{-6mm}=~2i\,\frac{z_{\rm sp}-1+O(v^2)}{(z_{\rm sp}+O(v^2))((z_{\rm sp}-1)^2+v^2-2c_2(z_{\rm sp}-1)\,v^2+O(v^4))}\,,
\end{eqnarray}
where we used \eqref{e32} and the fact that $z_{\rm sp}$ and $c_k$ are real with $z_{\rm sp}>1$. Therefore, we get for the expression in \eqref{e101}
\begin{align} 
\frac{1}{\pi} &\int_0^{\frac{1}{2}\delta}\frac{1}{z_{\rm sp}{\rm +}O(v^2)}\frac{z_{\rm sp}-1+O(v^2)}{(z_{\rm sp}-1)^2+v^2+O((z_{\rm sp}-1)v^2)+O(v^4)}\nonumber \\
&{\rm ln}\left(1-B\exp(-\tfrac12 s\alpha  v^2)\right)\dd v.
\label{y77}
\end{align}
In the case that $2\eta-1<0$, we have as earlier that the whole expression in \eqref{y77} is $O(\exp({-}b^2\,s^{1-2\eta}))$ for any $b\in(0,b_0)$, as $s\to  \infty$. In the case that $2\eta-1\geq 0$, we substitute $v=t\sqrt{{s}/{(2\,\alpha )}}$, and we get as earlier for the expression \eqref{y77}, assuming also that $\eta<1$,
\begin{align}
\frac{1}{\pi}&\,\sqrt{s\,\alpha /2}\,\int_0^{\infty}\frac{z_{\rm sp}-1+O(t^2/s)}{(d^2(s)+t^2)\,(1+O(s^{-\eta})+O(t^2/s))}\,{\rm ln}(1-B\,\ee^{-t^2}) \dd t\nonumber\\
&= \frac{1}{\pi}\,\int_0^{\infty}\frac{\sqrt{s\,\alpha /2} \ (z_{\rm sp}-1)}{d^2(s)+t^2}{\rm ln}(1-B\,\ee^{-t^2})\dd t\,\left(1+O(s^{\eta-1})\right)\nonumber\\
&= \frac{1}{\pi}\,\int_0^{\infty}\frac{d(s)}{d^2(s)+t^2}{\rm ln}(1-\ee^{{-}d^2(s)-t^2})\dd t\,\left(1+O(s^{\eta-1})\right).
\label{y78}
\end{align}
Here we also used \eqref{y46} and that $1/s^{3\eta-1} = O(d^2(s)/s^\eta)$, so that
\begin{equation} \label{y79}
(\tfrac12\,s\,\alpha )^{1/2}\,(z_{\rm sp}-1) = d(s)\,\left(1+O(s^{-\eta})\right) = d(s)\left(1+O(s^{\eta-1})\right),
\end{equation}
since $\eta\geq 1/2$.

We have for $b>0$
\begin{align}
\frac{1}{\pi}&\int_0^\infty \frac{b}{b^2+t^2}\,{\rm ln}(1-\exp({-}b^2-t^2))\dd t =-\frac12\sum_{k=0}^{\infty}\,\frac{1}{k+1}\,{\rm erfc}(b\,\sqrt{k+1}) = -F(b\,\sqrt{2}),\label{y80}
\end{align}
where according to \cite[(3.3) and (3.12)]{Janssen2006} for $\beta>0$
\begin{align}
F(\beta) &= \sum_{n=1}^\infty\,\frac{1}{n}\,\frac{1}{\sqrt{2\pi}}\,\int_{\beta\sqrt{n}}^\infty \ee^{-x^2/2}dx\nonumber\\
&= -{\rm ln}\,\beta - \frac12\,{\rm ln}2 - \frac{1}{\sqrt{2\pi}}\,\sum_{r=0}^\infty \frac{\zeta(1/2-r)\,(-1/2)^r\,\beta^{2r+1}}{r!\,(2r+1)},\label{y81}
\end{align}
the last identity being valid for $0<\beta<2\sqrt{\pi}$.

Using \eqref{y81} with $\beta^2 = d^2(s)= b_0^2/s^{2\eta-1}$, with the entire series on the second line being $O(\beta)$, we get the leading order behavior of ${\rm ln}[Q(0)]$ as
\begin{equation} \label{y82}
\Big({-}(\eta-1/2)\,{\rm ln}\,s+{\rm ln}(2\,b_0)+O(s^{1/2-\eta})\Big)\left(1+O(s^{\eta-1})\right)
\end{equation}
when $\eta\in(1/2,1)$. For $\eta = 1/2$, we get the leading order behavior, assuming $0<b_0<\sqrt{2\pi}$,
\begin{equation} \label{y83}
{\rm ln}(2\,b_0) + \frac{1}{\sqrt{\pi}}\,\sum_{r=0}^\infty \,\frac{\zeta(1/2-r)\,(-1)^r}{r!\,(2r+1)}\,b_0^{2r+1}
\end{equation}
with relative error $O(s^{-1/2})$. The expression \eqref{y83} coincides with ${\rm ln}[\mathbb{P}(M=0)]$ as given by \cite[(2.1)]{Janssen2006} with $\beta = b_0\,\sqrt{2}$. The next two results summarize the above.

\begin{theorem} \label{emptythm}
For $\eta\in(1/2,1)$,
\begin{equation} \label{y84}
{\rm ln}[\mathbb{P}(Q=0)] = - F\big(d(s)\,\sqrt{2}\big)\left(1+O(s^{\eta-1})\right)
\end{equation}
with $F$ given by \eqref{y81}.
\end{theorem}
\begin{proposition} \label{emptyprop}
For $\eta\in (0,1/2)$, and for all $b<b_0$,
\begin{equation}
{\rm ln}[\mathbb{P}(Q=0)] = O(\exp({-}b^2\,s^{1-2\eta})).
 \end{equation}
 For $\eta=1/2$, ${\rm ln}[\mathbb{P}(Q=0)]$ equals $-F(b_0\,\sqrt{2})$ with a relative error $O(1/\sqrt{s})$. For $\eta\in (1/2,1)$ and $0<b_0<\sqrt{2\pi}$, ${\rm ln}[\mathbb{P}(Q=0)]$ has leading order behavior as in \eqref{y82}.
\end{proposition}

As in Section \ref{subsec3.3} for the mean congestion level case
with $\eta=1/2$, it is possible to give a correction term which involves now the integrals in \eqref{y80} and \eqref{e51}.

\section{Numerical examples}\label{numm}
\subsection{Accuracy of the approximations}
In this subsection we present a numerical example that serves to illustrate the accuracy of the derived heavy-traffic approximations. Consider the Poisson case
\begin{equation}
\tilde X(z)=\ee^{z-1},\quad \mu = \sigma^2 = 1.
\end{equation}
We fix $\mu$ and vary $n$ with the value of $s$, according to
\begin{equation}
\vartheta = \frac{n}{s} = 1-\frac{\gamma}{s^\eta}
\end{equation}
for some $\gamma>0$ and $\eta\geq 1/2$. To calculate the exact value of the mean congestion level we use the expression, see \cite{Boudreau1962},
\begin{equation}\label{x73}
\mu_Q=\frac{\sigma_A^2}{2(s-\mu_A)}-\frac{s-1+\mu_A}{2}+\sum_{k=1}^{s-1}\frac{1}{1-z_k}.
\end{equation}
Here $z_1,\ldots,z_{s-1}$ are the zeros of $z^s-A(z)$ in $|z|<1$. We apply the method of successive substitution described in \cite{Janssen2005} to obtain accurate numerical approximations for $z_1,...,z_{s-1}$ and consequently $\mu_Q$.

From Theorem \ref{mainthm}, we find that the leading order behavior of $\mu_Q$ is given by
\begin{equation} \label{x18}
\frac{\sqrt{2s}}{\pi}\,G_0\Big(\frac{\gamma}{\sqrt{2}\,s^{\eta-\frac{1}{2}}}\Big).
\end{equation}
In order to find the correction terms, we proceed by setting $\eta = 1/2$. Deriving constants $C_1,C_2,C_3,$ and $C_4$ for our setting and substituting these into \eqref{e71},  we get for $\mu_Q$, with an absolute error of $O(s^{-1/2})$, the approximation
\begin{equation}\label{x19}
\frac{\sqrt{2\,s}}{\pi}\Big(\Big(1-\frac{\gamma}{3\,\sqrt{s}}\Big)\,G_0(b_0)-\frac{\gamma^3}{3\,\sqrt{s}}\,(\,G_3(b_0)+G_4(b_0))\Big),
\end{equation}
which by \eqref{e49} and \eqref{e74} reduces to
\begin{equation}\label{x20}
\frac{\sqrt{2\,s}}{\pi}\,G_0(b_0)-\frac{\sqrt{2}\,\gamma}{3\,\pi}\,G_1(b_0).
\end{equation}


\begin{table}\label{tab:poisson1}
\centering
\begin{tabular}{|r|rrrr|}
\hline
$s$ & $\rho$ & $\mu_Q$ & \eqref{x18} & \eqref{x20} \bigstrut \\
\hline
 10 & 0.683 & 0.244 & 0.399 & 0.247 \bigstrut[t] \\
 20 & 0.776 & 0.410 & 0.565 & 0.412 \\
 50 & 0.858 & 0.739 & 0.893 & 0.741 \\
 100 & 0.900 & 1.110 & 1.263 & 1.111 \\
 200 & 0.929 & 1.633 & 1.787 & 1.634 \\
 500 & 0.955 & 2.672 & 2.825 & 2.673 \\
 1000 & 0.968 & 3.843 & 3.996 & 3.843 \bigstrut[b]\\
 \hline
\end{tabular}
\caption{Numerical results for $\gamma = 1$.}
\end{table}

\begin{table}\label{tab:poisson2}
\centering
\begin{tabular}{|r|rrrr|}
\hline
$s$ & $\rho$ & $\mu_Q$ & \eqref{x18} & \eqref{x20} \bigstrut \\
\hline
 10 & 0.968 & 13.707 & 14.046 &13.732 \bigstrut[t] \\
 20 & 0.977 & 19.533 & 19.865 &19.551\\
 50 & 0.985 & 31.084 & 31.409 &31.095\\
 100 & 0.990 & 44.097 & 44.419 &44.106\\
 200 & 0.992 & 62.499 & 62.819 &62.505\\
 500 & 0.995 & 99.008 & 99.325 &99.011\\
 1000 & 0.996 & 140.152 & 140.468 & 140.154 \bigstrut[b]\\
 \hline
\end{tabular}
\caption{Numerical results for $\gamma = 0.1$.}
\end{table}

\begin{table}\label{tab:poisson3}
\centering
\begin{tabular}{|r|rr|rr|rr|}
\cline{2-7}
 \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{$\eta=0.6$} & \multicolumn{2}{c|}{$\eta=0.75$} & \multicolumn{2}{c|}{$\eta=0.9$} \bigstrut\\
 \hline
$s$ &  $\mu_Q$ & \eqref{x18} &  $\mu_Q$ & \eqref{x18} &  $\mu_Q$ & \eqref{x18} \bigstrut\\
\hline
 10 & 17.781 & 18.125 & 25.970 & 26.318 & 37.553 & 37.905 \bigstrut[t]  \\
 20 & 27.309 & 27.647 & 44.391 & 44.734 & 71.195 & 71.541 \\
 50 & 47.948 & 48.281 & 89.623 & 89.961 & 164.637 & 164.978 \\
 100 & 73.245 & 73.574 & 152.031 & 152.367 & 309.353 & 309.692 \\
 200 & 111.752 & 112.079 & 257.435 & 257.769 & 580.170 & 580.507 \\
 500 & 195.082 & 195.409 & 515.443 & 515.776 & 1329.581 & 1329.917 \\
 1000 & 297.122 & 297.448 & 870.524 & 870.857 & 2487.227 & 2487.562 \bigstrut[b]\\
 \hline
\end{tabular}
\caption{Numerical results for $\gamma=0.1$ and several values of $\eta$.}
\end{table}
\noindent Numerical results for $\eta=1/2$ and various values of $s$ are given in Table 1 and 2, for $ \gamma = 1$ and  $\gamma = 0.1$, respectively.
We note that for small $s$ the leading order approximation is still off by a significant amount, while the refinement only shows an error in the second decimal for $\gamma = 0.1$. This seems to justify the use of the correction term.
In Table 3 we compare the approximation \eqref{x18} against the exact value of $\mu_Q$ for three values of $\eta\geq 1/2$ to assess the influence of $\eta$. Clearly, the leading order approximation is relatively accurate for all three scenarios. As expected, the mean congestion increases along with $\eta$, since utilization approaches 1 more rapidly in this case.
\subsection{Connection to other queueing models}\label{subsec62}
As argued in the introduction, we believe that the heavy-traffic behavior for the discrete model in this chapter will up to leading order be universal for a wide range of other models (when subjected to the same heavy-traffic regime \eqref{bb}). We shall now substantiate this for many-server systems, for which under \eqref{bb}, it turns out that the mean congestion is $O(s^\eta)$.  We compare the mean congestion level in our discrete queue with that in the multi-server systems $M/M/s$, $M/D/s$ and Gamma/Gamma/$s$, all with unit mean service time and occupation rate $1-\gamma/s^\eta$.

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	xmin = 2.5,
	xmax = 6.5,
	ymin = 0,
	ymax = 7.2,
	xlabel = {$\log(s)$},
	ylabel = {$\log(\mu_Q)$},
	x label style={at={(0.6,-0.1)}},
	y label style={at={(-0.06,0.7)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 6.4,0.2)},anchor = south east},
	yscale = 0.8,
	xscale = 1
]

\addplot[thick,mark = o,mark options={scale=1.25}] table[x=log_s,y=mms] {novel_figure1.txt};
\addplot[thick, mark=triangle,dashed,mark options={scale=1.25,solid}] table[x=log_s,y=mds] {novel_figure1.txt};
\addplot[thick,mark=square,dotted,mark options={scale=1.25,solid}] table[x=log_s,y=ggs] {novel_figure1.txt};

\legend{$M/M/s$,$M/D/s$,Gamma/Gamma/$s$}
\end{axis}

\end{tikzpicture}
\caption{$\mu_Q$ plotted against $s$ on log scale for 3 queues for $\eta=0.75$.}
  \label{fig1}
\end{figure}
\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	xmin = 0.2,
	xmax = 6.5,
	ymin = 0,
	ymax = 9,
	xlabel = {$\log(s)$},
	ylabel = {$\log(\mu_Q)$},
	x label style={at={(0.6,-0.1)}},
	y label style={at={(-0.06,0.7)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 6.75,4.2)},anchor = west},
	yscale = 0.8,
	xscale = 1
]

\addplot[thick,only marks,mark = o,mark options={scale=1.25}] table[x=n01,y=m01] {novel_figure2.txt};
\addplot[thick,only marks,mark = square,mark options={scale=1.25}] table[x=n025,y=m025] {novel_figure2.txt};
\addplot[thick,only marks,mark = *,mark options={scale=1.25}] table[x=n05,y=m05] {novel_figure2.txt};
\addplot[thick,only marks,mark = square*,mark options={scale=1.25}] table[x=n075,y=m075] {novel_figure2.txt};
%\addplot[thick,only marks,mark = square*,mark options={scale=1.25}] table[x=n09,y=m09] {./tikz/novel_figure2.txt};
\addplot[thick,only marks,mark = triangle*,mark options={scale=1.25}] table[x=n1,y=m1] {novel_figure2.txt};

\addplot[dashed] coordinates{ (0,2.25) (7,9.25) };
\addplot[dashed] coordinates{ (0,2.25) (7,7.5) };
\addplot[dashed] coordinates{ (0,2.25) (7,5.75) };
\addplot[dashed] coordinates{ (0,2.25) (7,4) };
\addplot[dashed] coordinates{ (0,2.25) (7,2.95) };
\legend{\ $\eta=0.1$,\ $\eta=0.25$,\ $\eta=0.5$,\ $\eta=0.75$,\ $\eta=1$}
\end{axis}

\end{tikzpicture}
  \caption{$\mu_Q$ of $M/M/s$ plotted against $s$ on log scale for different values of $\eta$.}
  \label{fig2}
\end{figure}
Figure \ref{fig1} shows on logarithmic scale the mean congestion levels for $\gamma=0.1$ and  $\eta=0.75$  under the specified scaling for three systems. We also display three lines with slope 0.75 for comparison, which confirms that mean congestion levels are of the order $s^\eta$, also in these multi-server system. Formally establishing this heavy-traffic behavior for these multi-server system is an important open problem and requires other mathematical approaches than the ones taken in this chapter (see the introduction for more details).

Figure \ref{fig2} shows the mean queue length in the $M/M/s$ system for several values of $\eta$, again on logarithmic scale, together with lines with slope $\eta$. For $\eta\geq 1/2$, we see the same $O(s^\eta)$ behavior, similar as for $\mu_Q$ in our discrete model. For $\eta<1/2$ the mean queue length decays, again in agreement with our results for $\mu_Q$. We note that this qualitative behavior of the $M/M/s$ system was also observed by \cite[Thm.~4.1]{maman}, by proving that the mean waiting time in the $M/M/s$ queue under \eqref{bb} is of order $1/s^{1-\eta}$, which by Little's law implies the mean queue length to be of order $s^\eta$.



==> Chapter_3/Chapter3i.tex <==


\chapter{Overdispersion}

\begin{chapterstart}
Arrival processes to service systems often display fluctuations that are wilder than anticipated under the Poisson assumption, a phenomenon that is referred to as \textit{overdispersion}.
Motivated by this, we analyze a class of discrete stochastic models for which we derive heavy-traffic approximations that are scalable in the system size.
Subsequently, we show how this leads to novel capacity sizing rules that acknowledge the presence of overdispersion. This, in turn, leads to robust approximations for performance characteristics of systems that are of moderate size and/or may not operate in heavy traffic. 
\end{chapterstart}

\begin{flushright}
Based on\\
\textbf{Robust heavy-traffic approximations for\\ service systems facing overdispersed demand}\\
\textit{Britt Mathijsen, Guido Janssen, Johan van Leeuwaarden \& Bert Zwart}\\
arxiv.org/abs/1512.05581
\end{flushright}
\newpage 

\section{Introduction}\label{intro}

In the previous chapter, we analyzed the scaling limit of a queueing model in which demand exhibits stochastic fluctuations that are asymptotically proportional to the square-root of the nominal load, while we deliberately chose to deviate from the square-root staffing principle by allocating a variability hedge that does not match the order of these fluctuations.
This chapter in some ways does the opposite. 
We assume the demand faced by the queueing system is more volatile than anticipated by the independent many-sources paradigm that leads to Poisson traffic models. 
As will become clear in this chapter, this in fact \emph{requires} an adaption of the square-root staffing principle in order to maintain the desirable properties of QED regime. 
We start by motivating our research through empirical evidence of the presence of so-called \emph{overdispersion} in arrival processes faced by service systems reported by recent literature. \\

\noindent
\textbf{Motivation.}
The bulk of the queueing literature assumes perfect knowledge about the model primitives, including the mean demand per time period. For large-scale service systems, like health care facilities, communication systems or call centers, the dominant assumption is that demand arrives according to a (non)homogeneous Poisson process, which in practice translates into the assumption that arrival rates are known for each basic time period (second, hour or day).
Although natural and convenient from a mathematical viewpoint, the Poisson assumption often fails to be confirmed in practice. A deterministic arrival rate implies that the demand over any given period is a Poisson random variable, whose variance equals its expectation. A growing number of empirical studies shows that the variance of demand typically deviates from the mean significantly. Recent work of \cite{Kim2015b,Kim2015a} reports variance being strictly less than the mean in health care settings employing a appointment booking system. This reduced variability, known as underdispersion, can be accredited to the goal of the booking system to create a more predictable arrival pattern. On the other hand, in other scenarios with no control over the arrivals, the variance typically dominates the mean, see \cite{Avramidis:2004, Bassamboo2010, Bassamboo2009, Brown2005, Chen2001, Gans2015, Gurvich2010, koolejongbloed, kimwhitt,  maman, Mehrotra2010, Robbins2010, Steckley2009, Zan2012}. The feature that variability is higher than one expects from the Poisson assumption is referred to as overdispersion. The latter concept will be the center of our attention in this chapter. 

Stochastic models with the Poisson assumption have been widely applied to optimize capacity levels in service systems. The goal is to minimize operating costs while providing sufficiently high QoS in terms of performance measures such as mean delay or excess delay. When stochastic models, however, do not take into account overdispersion, resulting performance estimates are likely to be overoptimistic. The system then ends up being underprovisioned, which possibly causes severe performance problems, particularly under critical loading.
%, it is well known that stochastic fluctuations can have a detrimental effect on system performance.
\\
\\*
\noindent
\textbf{Causes of overdispersion.} 
The literature discussed above proves that the presence of overdispersion is widespread across applications.
It however does not specify what causes the increased variability in the arrival process. 
We name two possible explanations. 

First, we revisit the many-sources characterization of demand inflow discussed in Chapter 2. 
Recall that in this setting, demand is generated by a large number $n$ of stochastically identical and independent sources, for that workload arriving to the system in period $j$ is given by $A^{(n)}_j = \sum_{i=1}^n A_{i,j}$, where $A_{i,j}$, $i=1,2,\ldots,n$ are i.i.d.~random variables. 
This resulted in nominal workload $\mu_n = n\mu$ and $\sigma_n^2 = n\sigma^2$, thus both of order $n$. 
If we now relax the assumption on the (pairwise) independence of the sources, but rather consider the scenario in which these are positively correlated, then the nominal load remain to be equal to $n \mu$, while the variance of demand becomes
\begin{equation*}
\sigma_n^2 = \Var A_j^{(n)} = n\, \Var A_{i,1} + n(n-1)\,{\rm Cov}(A_{1,j},A_{2,j}),
\end{equation*}
which is of higher order than $n$ if $n\,{\rm Cov}(A_{1,j},A_{2,j}) \to \infty$ as $n\to\infty$.

A second interpretation of overdispersion in arrival processes relates to \emph{arrival rate uncertainty}. 
The canonical process for modeling the arrival process of a service systems is the Poisson process with a given arrival rate $\lambda$. 
Since model primitives, in particular the arrival rate, are typically estimated through historical data, these are prone to be subject to forecasting errors. 
In the realm of Poisson processes, this inherent uncertainty can be acknowledged by viewing the arrival rate $\Lambda_n$ itself as being stochastic. The resulting doubly stochastic Poisson process, also known as Cox process (first presented in \cite{Cox1955}), implies that demand in a given interval $A_j$ follows a mixed Poisson distribution. 
In this case, the expected demand per period equals $\mu_n = \E[\Lambda_n]$, while the variance is $\sigma_n^2 = \E[\Lambda_n]+\Var\Lambda_n$.
By selecting the distribution of the mixing factor $\Lambda_n$, the magnitude of overdispersion can be made arbitrarily large, and only a deterministic $\Lambda_n$ leads to a true Poisson process.

The mixed Poisson model presents a useful way to fit both the mean and variance to real data, particularly in case of overdispersion. 
The mixing distribution can be estimated parametrically or non-parametrically, see \cite{koolejongbloed,maman}. 
A popular parametric family is the Gamma distribution, which gives rise to an effective data fitting procedure that uses the fact that a Gamma mixed Poisson random variable follows a negative binomial distribution. 
We will in this chapter adopt the assumption of a Gamma-Poisson mixture as the demand process.\\
\\*
\textbf{Adapted QED scaling.} To deal with overdispersion 
new models are needed, scaling rules must be adapted, and existing capacity sizing rules need to be modified in order to incorporate a correct hedge against (increased) variability. 
In this chapter, we consider an extension of the discrete queueing model of Chapter 2 that has a doubly stochastic Poisson process as input, $A_j\sim\,{\rm Pois}(\Lambda_n)$ and we identify the heavy-traffic regime in which it displays QED behavior. 
That is, it fits the three asymptotic characteristics in Section 1.2.3 of this thesis.
As we argued in that particular section, a sensible candidate capacity allocation rule is $s_n = \mu_n + \beta \sigma_n$ for some $\beta>0$, which is equivalent to the scaling 
\begin{equation*}
\frac{\mu_n}{\sigma_n}\,(1-\rho_n) \to \beta. 
\end{equation*}
We will verify mathematically that this is asymptotically the appropriate choice.
Studies that have adressed similar capacity allocation problems with stochastic arrival rates include \cite{Kocaga2015, maman, Whitt1999, Whitt2006}.
Of the aforementioned papers, our work best relates to \cite{maman}, in the sense that we also assess the asymptotic performance of queueing system having a stochastic arrival rate in heavy traffic.
We therefore expand the paradigm of the QED regime, in order to have it accommodate for overdispersed demand that follows from a doubly stochastic Poisson process.
\\
\\*
\textbf{Structure of the chapter}. The remainder of this chapter is structured as follows. Our model is introduced in Section \ref{modelSection} together with some preliminary results. 
In Section 3.3 we derive the classical heavy-traffic scaling limits for the queue length process in the presence of overdispersed arrivals both for the moments and the distribution itself.
Section 3.4 presents our main theoretic result, which provides a robust refinement to the heavy-traffic characterization of the queue length measures in pre-limit systems.
In Section 3.5, we describe the numerical results and demonstrate the heavy-traffic approximation for a real data set coming from a health care setting. Section 3.6 provides some concluding remarks.


\section{Model description}\label{modelSection}
We consider the same mathematical model as in Section 2.2, in which time is divided into periods of equal length. At the beginning of each period $j=1,2,3,...$ new demand $A^{(n)}_j$ arrives to the system. The demands per period $A^{(n)}_1,A^{(n)}_2,...$ are assumed independent and equal in distribution to some non-negative integer-valued random variable $A^{(n)}$.
The system has a service capacity $s_n\in\mathbb{N}$ per period, the steady-state queue length can be characterized as, see (1.27), 
\begin{equation}
   \label{mm3}
   Q^{(n)} \equalD \max_{k\geq 0}\Bigl\{\sum_{i=1}^k (A^{(n)}_i-s_n)\Bigr\}.
   \end{equation}
For brevity, we define $\mu_n:= \E [A^{(n)}_1]$ and $\sigma_n^2 = \Var A^{(n)}_1$.
The behavior of $Q^{(n)}$ predominantly depends on the characteristics of $A^{(n)}$ and $s_n$. As noted before, $\mu_n<s_n$ is a necessary condition for the maximum in \eqref{mm3} to be finite and consequently for the queue to be stable. Before continuing the analysis of $Q^{(n)}$, we impose a set of conditions on the asymptotic properties of $s_n,\mu_n$ and $\sigma_n$.

\begin{assumption}
\label{as1}
\ \\*
\vspace{-6mm}
\begin{enumerate}
\item[{\normalfont (a)}] {\rm (Asymptotic growth)}
\begin{equation*}
\mu_n,\sigma_n \to \infty, \quad \text{\rm for } n\to\infty.
\end{equation*} 
\item[{\normalfont (b)}] {\rm (Persistence of overdispersion)}
\begin{equation*}
\sigma_n^2/\mu_n \to \infty \quad \text{\rm for } n\to\infty.
\end{equation*}
\item[{\normalfont (c)}] {\rm (Heavy-traffic condition)} 
The utilization $\rho_n := \mu_n/s_n \to 1$ as $n\to\infty$, while
\begin{equation}\label{mm5}
s_n = \mu_n + \beta\, \sigma_n,
\end{equation}
for some $\beta > 0$. This is equivalent to requiring
\begin{equation}\label{mm4}
(1-\rho_n)\frac{\mu_n}{\sigma_n} \to \beta.
\end{equation}
\end{enumerate}
\end{assumption}
%
\noindent
Assumption \ref{as1} is assumed to hold throughout the remainder of this chapter.
Since we are mainly interested in the system behavior in heavy traffic, it is appropriate to study the queue length process in a scaled form. Substituting $s_n$ as in Assumption \ref{as1}(c), and dividing both sides of \eqref{mm3} by $\sigma_n$, gives
%
\begin{equation}
\label{mm6}
\frac{Q^{(n)}}{\sigma_n} = \max_{k\geq 0} \Bigl\{{\textstyle\sum_{i=1}^k} \Bigl(\frac{A^{(n)}_i-\mu_n}{\sigma_n} - \beta\Bigr)\Bigr\}.
\end{equation}
%
By defining $\hat{Q}^{(n)} := Q^{(n)}/\sigma_n$ and $\hat{A}^{(n)}_i := (A^{(n)}_i-\mu_n)/\sigma_n$, we see that the scaled queue length process is in distribution equal to the maximum of a random walk with i.i.d. increments distributed as $\hat{A}^{(n)}-\beta$. Besides $\E[\hat{A}^{(n)}] = 0$ and $\Var \hat{A}^{(n)}=1$, the scaled and centered arrival counts $\hat{A}^{(n)}$ has a few other nice properties which we turn to later in this section.

The model in \eqref{mm3} is valid for any distribution of $A^{(n)}$, also for the original case where the number of arrivals follows a Poisson distribution with fixed parameter $\lambda_n$, but in that case Assumption \ref{as1}(b) does not hold. Instead, we assume $A^{(n)}$ to be Poisson distributed with uncertain arrival rate rendered by the  non-negative random variable $\Lambda_n$. This $\Lambda_n$ is commonly referred to as the \emph{prior} distribution, while $A^{(n)}$ is given the name of a Poisson mixture, see \cite{Grandell1997}. Given that the moment generation function of $\Lambda_n$, denoted by $M^\Lambda_n(\cdot)$, exists, we are able to express the probability generating function (pgf) of $A^{(n)}$ through the former. Namely,
\begin{equation}
\label{mm7}
\tilde{A}^{(n)}(z) = \E[\E[ z^{A^{(n)}} | \Lambda_n ] ] = \E[ \exp(\Lambda_n(z-1))] = M^\Lambda_n(z-1).
\end{equation}
From \eqref{mm7}, we get
\begin{equation}
\label{mm8}
\mu_n = \E[A^{(n)}] =  \E[\Lambda_n],\qquad
\sigma_n^2 = \Var A^{(n)} = \Var \Lambda_n + \E[\Lambda_n],
\end{equation}
so that $\mu_n<\sigma_n^2$ if $\Lambda_n$ is non-deterministic. Assumption \ref{as1}(b) hence translates to 
\[\Var \Lambda_n/\E[\Lambda_n]\rightarrow \infty, \qquad n\rightarrow\infty.\]
The next result relates the converging behavior of the centered and scaled $\Lambda_n$ to that of $\hat{A}^{(n)}$.
\begin{lemma}\label{gaussStep}
Let $\mu_n,\sigma_n^2\rightarrow\infty$ and $\sigma_n^2/\mu_n\rightarrow\infty$. If
\begin{equation*}
\hat{\Lambda}_n := \frac{\Lambda_n-\mu_n}{\sigma_n}\Rightarrowd \mathcal{N}(0,1), \qquad \text{\normalfont for } n\rightarrow\infty,
\end{equation*}
then $\hat{A}^{(n)}$ converges weakly to a standard normal variable as $n\rightarrow\infty$.
\end{lemma}
\noindent
The proof can be found in Appendix \ref{formalSec}.
The prevalent choice for  $\Lambda_n$ is the Gamma distribution. The Gamma-Poisson mixture turns out to provide a very good fit to arrival counts experienced by service systems, as was observed by \cite{koolejongbloed}. Assuming $\Lambda_n$ to be of Gamma type with scale and rate parameters $a_n$ and $1/b_n$, respectively, we get for the pgf of $A^{(n)}$:
\begin{equation}
\label{r0}
\tilde{A}^{(n)}(z) = \Bigl(\frac{1}{1+b_n(1-z)}\Bigr)^{a_n},
\end{equation}
in which we recognize the pgf of a negative binomial distribution with parameters $a_n$ and $1/(b_n+1)$, so that
\begin{equation*}
 \label{t21}
 \mu_n = a_nb_n,\qquad \sigma_n^2 = a_nb_n(b_n+1).
 \end{equation*}
Note that in the context of a Gamma prior, the restrictions in Assumption \ref{as1} reduce to only two rules. For completeness, we include the revised list below. 
\begin{assumption}\label{as2}
\ \\*
\vspace{-6mm}
\begin{enumerate}
\item {\rm (Asymptotic regime and persistence of overdispersion)}
\begin{equation*}
a_n, b_n \to \infty, \quad \text{\rm for } n\to\infty.
\end{equation*}
\item {\rm (Heavy-traffic condition)}
Let 
\begin{equation*}
s_n = a_n b_n + \beta \sqrt{a_n b_n(b_n+1)},
\end{equation*}
for some $\beta>0$, or equivalently
\begin{equation*}
(1-\rho_n)\sqrt{a_n} \to \beta, \quad \text{\rm for } n\to\infty.
\end{equation*}
\end{enumerate}
\end{assumption}
The next result follows from the fact that $\Lambda_n$ is a Gamma random variable:
\begin{corollary}\label{scaledLambdaLemma}
Let $\Lambda_n\sim\text{\normalfont Gamma}(a_n,1/b_n)$, $A^{(n)}\sim{\rm Pois }(\Lambda_n)$ and $a_n,b_n\rightarrow \infty$. Then $\hat{A}^{(n)}$ converges weakly to a standard normal random variable as $n\rightarrow \infty$.
\end{corollary}
\begin{proof}
By Lemma \ref{gaussStep}, it is sufficient to prove that $\hat{\Lambda}_n\Rightarrowd\mathcal{N}(0,1)$ for this particular choice of $\Lambda_n$.  
We do this by proving the pointwise convergence of the characteristic function (cf) of $\hat{\Lambda}_n$ to $\exp({-} t^2/2)$, the cf of the standard normal distribution. 
Let $\phi_{G}(\cdot)$ denote the characteristic function of a random variable $G$. By basic properties of the cf,
\begin{align*}
\phi_{\hat{\Lambda}_n}(t) &= \ee^{-i\mu_nt/\sigma_n}\,\phi_{\Lambda_n}(t/\sigma_n)
= \ee^{-i\mu_nt/\sigma_n} \Bigl(1-\frac{i b_nt}{\sigma_n}\Bigr)^{-a_n}\nonumber\\
&= \exp\Bigl[ -\frac{i\mu_nt}{\sigma_n}\, - a_n\,{\rm ln}\Bigl(1-\frac{i b_nt}{\sigma_n}\Bigr)\Bigr]\nonumber\\
\label{g13d}
&= \exp\Bigl[ -\frac{i\mu_nt}{\sigma_n} -a_n\Bigl( {-}\frac{i\,b_nt}{\sigma_n} + \frac{b_n^2t^2}{2\sigma_n^2} + O( b_n^3/\sigma_n^3)\Bigr)\Bigr]  \nonumber\\
&= \exp\Bigl[ -\frac{b_n\,t^2}{2(b_n+1)} + O\left(1/\sqrt{a_n}\right)\Bigr] \rightarrow \exp\big({-} t^2/2\big),
\end{align*}
for $n\rightarrow\infty$. By L\'evy's continuity theorem this implies $\hat{\Lambda}_n$ is indeed asymptotically standard normal. 
\end{proof}
 The characterization of the arrival process as a Gamma-Poisson mixture  be of vital importance in later sections.

\subsection{Expressions for the stationary distribution\label{expressionsSubsec}}
Our main focus is on the stationary queue length distribution, denoted by 
\[\mathbb{P}(Q^{(n)}=i) =\lim_{k\rightarrow\infty} \mathbb{P}(Q^{(n)}(k)=i).\]
Denote the pgf of $Q^{(n)}$ by
\begin{equation*}
\label{t1}
\tilde{Q}^{(n)}(w) := \sum_{i=0}^\infty \P(Q^{(n)}=i) w^i.
\end{equation*}
Furthermore, let $\mu_Q := \E[Q^{(n)}]$ and $\sigma_Q^{2} := \Var Q^{(n)}$ denote the stationary mean and variance of the queue length, respectively. 
To avoid notational complexity, we omit the superscript $(n)$ in these definitions. 
To continue our analysis of $Q^{(n)}$, we need one more condition on $A^{(n)}$. 
\begin{assumption}\label{as3}
The pgf of $A^{(n)}$, denoted by $\tilde{A}^{(n)}(w)$, exists within $|z|<r_0$, for some $r_0>1$, so that all moments of $A^{(n)}$ are finite.
\end{assumption}

We next recall two characterizations of $\tilde{Q}^{(n)}(w)$ that play prominent roles in the remainder of our analysis. 
The first characterization of $\tilde{Q}^{(n)}(w)$ originates from a random walk perspective. As we see from \eqref{mm3}, the (scaled) stationary queue length is equal in distribution to the all-time maximum of a random walk with i.i.d. increments distributed as $A^{(n)}-\beta$ (or $\hat{A}^{(n)}-\beta$ in the scaled setting). Spitzer's identity, see e.g. \cite[Theorem VIII4.2]{Asmussen2003} and Section 1.2.2 of this thesis, then gives
\begin{equation*}
\label{t3}
\tilde{Q}^{(n)}(w) = \exp\left\{\sum_{k=1}^\infty \frac{1}{k}\,Big(\E\Big[w^{\left(\sum_{i=1}^k \{A^{(n)}_i-s_n\}\right)^+}\Big]-1\Big)\right\},
\end{equation*}
where $(x)^+ = \max\{x,0\}$. Hence,
\begin{equation*}
\label{t4}
\mu_Q = \tilde{Q}^{(n)\prime}(1) = \sum_{k=1}^\infty \frac{1}{k}\E\Bigl[ {\sum_{i=1}^k} (A^{(n)}_i - s_n) \Bigr]^+,
\end{equation*}
\begin{equation*}
\label{t4a}
\sigma^{2}_Q = \tilde{Q}^{(n)\prime\prime}(1)+Q^{(n)\prime}(1)-\left(\tilde{Q}^{(n)\prime}(1)\right)^2 = \sum_{k=1}^\infty \frac{1}{k}\E\Bigl[ \Big(\sum_{i=1}^k (A^{(n)}_i - s_n) \Big)^+\Bigr]^2,
\end{equation*}
\begin{align*}
\label{t5}
\P(Q^{(n)}=0) = \tilde{Q}_n(0) &= \exp\Bigl\{{-}{\sum_{k=1}^\infty}\frac{1}{k} \P\Bigl({\textstyle\sum_{i=1}^k} (A^{(n)}_i-s_n) > 0\Bigr) \Bigr\}.
\end{align*}
A second characterization follows from Pollaczek's formula, see \cite{Abate1993} and Section 2.2.2 of this thesis:
\begin{equation}
\label{t6}
\tilde{Q}^{(n)}(w) = \exp\Bigl\{ \frac{1}{2\pi i}\int_{|z|=1+\eps} {\rm ln}\Bigl(\frac{w-z}{1-z}\Bigr) \,\frac{(z^{s_n}-\tilde{A}^{(n)}(z))'}{z^{s_n}-\tilde{A}^{(n)}(z)}\dd z\Bigr\},
\end{equation}
which is analytic for $|w|<r_0$, for some $r_0>1$. Therefore, $\eps>0$ has to be chosen such that $|w|<1+\eps<r_0$. This gives
\begin{align}
\label{t7}
\mu_Q &= \frac{1}{2\pi i} \int_{|z|=1+\eps} \frac{1}{1-z}\,\frac{(z^{s_n}-\tilde{A}^{(n)}(z))'}{z^{s_n}-\tilde{A}^{(n)}(z)} \dd z,\\
\label{t7a}
\sigma_Q^{2} &= \frac{1}{2\pi i} \int_{|z|=1+\eps} \frac{{-}z}{(1-z)^2}\,\frac{(z^{s_n}-\tilde{A}^{(n)}(z))'}{z^{s_n}-\tilde{A}^{(n)}(z)}\dd z,\\
\label{t8}
\P(Q^{(n)}=0) &= \exp\Bigl\{ \frac{1}{2\pi i}\int_{|z|=1+\eps} {\rm ln}\Bigl(\frac{z}{z-1}\Bigr) \,\frac{(z^{s_n}-\tilde{A}^{(n)}(z))'}{z^{s_n}-\tilde{A}^{(n)}(z)}\dd z\Bigr\}.
\end{align}



\section{Heavy-traffic limits}

In this section we present the result on the convergence of the discrete process $\hat{Q}^{(n)}$ to a non-degenerate limiting process and of the associated stationary moments. The latter requires an interchange of limits. Using this asymptotic result, we derive two sets of approximations for $\mu_Q$, $\sigma^2_Q$ and $\P(Q^{(n)}=0)$, that capture the limiting behavior of $Q^{(n)}$. The first set provides a rather crude estimation for the first cumulants of the queue length process for any arrival process $A^{(n)}$ satisfying Assumption \ref{as1}. The second set, which is the subject of the next section, is derived for the specific case of a Gamma prior and is therefore expected to provide more accurate, robust approximations for the performance metrics.


We start by indicating how the asymptotic properties of the scaled arrival process give rise to a proper limiting random variable describing the stationary queue length. The asymptotic normality of $\hat{A}^{(n)}$ provides a link with the Gaussian random walk and nearly deterministic queues \cite{Sigman2011a,Sigman2011b}.
The main results in \cite{Sigman2011a,Sigman2011b} were obtained under the assumption that $\rho_n\sim 1-\beta/\sqrt{n}$, in which case it follows from \cite[Thm.~3]{Sigman2011b} that the rescaled stationary waiting time process converges to a reflected Gaussian random walk.

We shall also identify the Gaussian random walk as the appropriate scaling limit for our stationary system. However, since the normalized natural fluctuations of our system are given by $\mu_n/\sigma_n$ instead of $\sqrt{n}$, we assume that the load grows like $\rho_n \sim 1 - \frac{\beta}{\mu_n/\sigma_n}$. Hence, in contrast to \cite{Sigman2011a,Sigman2011b}, our systems' characteristics display larger natural fluctuations, due to the mixing factor that renders the arrivals. Yet, by matching this overdispersed demand with the appropriate hedge against variability, we again obtain Gaussian limiting behavior. This is not surprising, since we saw in Lemma \ref{gaussStep} that the increments start resembling Gaussian behavior for $n\rightarrow\infty$. The following result summarizes this.

\begin{theorem}
\label{gaussianThm}
Let $\Lambda_n$ be a non-negative random variable such that $(\Lambda_n-\mu_n)/\sigma_n$ is asymptotically standard normal, with $\mu_n$ and $\sigma_n$ as defined in \eqref{mm8}, and $\E[\Lambda_n^3]<\infty$ for all $n\in\mathbb{N}$. Then under Assumption \ref{as1}, for $n\rightarrow \infty$,
\begin{enumerate}
\item[{\rm (i)}] $\hat{Q}^{(n)} \Rightarrowd M_\beta$,
\item[{\rm (ii)}] $\mathbb{P}(Q^{(n)} = 0) \rightarrow \mathbb{P}(M_\beta=0)$,
\item[{\rm (iii)}] $\E[\hat{Q}^{(n)}] \rightarrow \E [M_\beta]$,
\item[{\rm (iv)}] $\sigma^2_Q \rightarrow \Var\, M_\beta$,
\end{enumerate}
where $M_\beta$ is the all-time maximum of a random walk with i.i.d. normal increments with mean $-\beta$ and unit variance.
\end{theorem}
The proof of Theorem \ref{gaussianThm} is given in Appendix \ref{formalSec}. The following result shows that Theorem \ref{gaussianThm} also applies to Gamma mixtures, which is a direct consequence of Corollary \ref{scaledLambdaLemma}.
\begin{corollary}
Let $\Lambda_n\sim$ \normalfont{Gamma}$(a_n,b_n)$. Then under Assumption \ref{as2} the four convergence results of Theorem \ref{gaussianThm} hold true.
\end{corollary}


It follows from Theorem \ref{gaussianThm} that the scaled stationary queueing process converges under \eqref{mm4} to a reflected Gaussian random walk. Hence, the performance measures of the original system should be well approximated by the performance measures of the reflected Gaussian random walk, yielding heavy-traffic approximations.


Like our original system, the Gaussian random walk falls in the classical setting of the reflected one-dimensional random walk, whose behavior is characterized by both Spitzer's identity and Pollaczek's formula. In particular, Pollaczek's formula gives rise to contour integral expressions for performance measures that are easy to evaluate numerically, also in heavy-traffic conditions. The numerical evaluation of such integrals is considered in \cite{Abate1993}. For $\E [M_\beta]$ such an integral is as follows
\begin{equation}
\label{g13e}
\E [M_\beta] = {-}\frac{1}{\pi}\int_0^\infty {\rm Re}\Bigl[\frac{1-\phi(-z)}{z^2}\Bigr]\dd y,
\end{equation}
with $\phi(z) = \exp(-\beta\,z+\tfrac12\,z^2)$, the Laplace transform of a normal random variable with mean $-\beta$ and unit variance, and $z=x+iy$ with an appropriately chosen real part $x$. Note that this integral involves complex-valued numbers. Similar expressions appear for $\mathbb{P}(M_\beta=0)$ and $\Var M_\beta$. The following result simply rewrites these integrals in \eqref{g13e} in terms of a real integral and uses the fact that the scaled queue length process mimics the maximum of the Gaussian random walk for large $n$.

\begin{corollary}\label{abateThm}
Under Assumption \ref{as1}, the leading order behavior of $\mathbb{P}(Q^{(n)}=0)$, $\mu_Q$ and $\sigma^2_Q$ as $n\to\infty$ is characterized by
\begin{align}
\label{h1a}
\mathbb{P}(Q^{(n)} = 0) &\approx \exp\Bigl[\frac{1}{\pi} \int_0^\infty \frac{\beta/\sqrt{2}}{\tfrac12\beta^2+t^2}\,{\rm ln}\Bigl(1-e^{-\tfrac12\beta^2-t^2}\Bigr)\dd t\Bigr],\\
\label{h1}
\mu_Q &\approx \frac{\sqrt{2}\sigma_n}{\pi}\int_0^\infty \frac{t^2}{\tfrac12\beta^2+t^2}\, \frac{\exp(-\tfrac12\beta^2- t^2)}{1-\exp(-\tfrac12 \beta^2 - t^2)} \dd t,\\
\label{h1b}
\sigma^2_Q &\approx \frac{\sqrt{2}\beta\sigma_n^2}{\pi}\,\int_0^\infty \frac{t^2}{(\tfrac12 \beta^2+t^2)^2}\frac{\exp(-\tfrac12\beta^2- t^2)}{1-\exp(-\tfrac12 \beta^2 - t^2)} \dd t.
\end{align}

%Furthermore
%\begin{equation*}
%\label{h3}
%\mathbb{P}(Q^{(n)}=0) \rightarrow \exp\Bigl[-\frac{\sqrt{2}}{\pi}\int_0^\infty \frac{\beta}{\beta^2+v^2}\,{\rm ln}(1-\exp({-}\tfrac12 \beta^2-\tfrac12 v^2))\, dv\Bigr].
%\end{equation*}
\end{corollary}

\begin{proof}
According to \cite[(15)]{Abate1993} we have for the maximum $M_\beta$ of a Gaussian random walk with drift parameter ${-}\beta$ and unit variance
\begin{equation*}
\label{z1}
{-}\,{\rm ln}\,[\mathbb{P}(M_\beta=0)] = c_0,\quad \E[M_\beta]\ = c_1, \quad \Var\, M_\beta = c_2,
\end{equation*}
where
\begin{equation*}
\label{z2}
c_n = \frac{(-1)^nn!}{\pi} \,{\rm Re}\Bigl[\int_0^\infty \frac{{\rm ln}\,(1-\exp(\beta\,z+\tfrac12 z^2))}{z^{n+1}} \dd y\Bigr],
\end{equation*}
in which $z={-}x+i\,y$, $y\geq 0$, and $x$ is any fixed number between 0 and $2\beta$. We take $x=\beta$, so that
\begin{equation*}
 \label{z3}
 \beta z+\tfrac12 z^2 = {-}\tfrac12\beta^2 - \tfrac12 y^2\leq 0,\quad y\geq 0.
 \end{equation*}
For $n=0$, we then have
\begin{align*}
c_0 &= \frac{1}{\pi}\,{\rm Re}\Bigl[\int_0^\infty \frac{{\rm ln}\,(1-\exp({-}\tfrac12 \beta^2-\tfrac12 y^2))}{{-}\beta+i\,y} \dd y\Bigr] \nonumber\\
&= {-}\frac{1}{\pi}\,\int_0^\infty \frac{\beta}{\beta^2+y^2}\,{\rm ln}\,(1-\exp({-}\tfrac12 \beta^2- \tfrac12 y^2)) \dd y\nonumber\\
\label{z4}
&= {-}\frac{1}{\pi}\,\int_0^\infty \frac{\beta/\sqrt{2}}{\tfrac12\beta^2+t^2}\,{\rm ln}\,(1-\exp({-}\tfrac12 \beta^2-t^2)) \dd t,
\end{align*}
where we used that
\begin{equation*}
\label{z5}
{\rm Re }\Bigl[\frac{1}{{-}\beta+i\, y}\Bigr] = \frac{{-}\beta}{\beta^2+y^2},
\end{equation*}
together with the substitution $y=t\sqrt{2}$. For $n=1,2,\ldots,$ we have by partial integration
\begin{align*}
c_n &= \frac{(-1)^n n!}{\pi} \, {\rm Re}\Bigl[\int_0^\infty \frac{{\rm ln}(1-\exp(-\tfrac12\beta^2-\tfrac12 y^2))}{({-}\beta+i\,y)^{n+1}} \dd y\nonumber\\
&= \frac{(-1)^{n-1}(n-1)!}{\pi}\,{\rm Im}\Bigl[\int_0^\infty {\rm ln}(1-\exp(-\tfrac12\beta^2-\tfrac12 y^2))\dd \Bigl(\frac{1}{(-\beta+i\,y)^n}\Bigr)\Bigr]\nonumber\\
\label{z6}
&= {-}\frac{(-1)^{n-1}(n-1)!}{\pi} {\rm Im}\Bigl[ \int_0^\infty \frac{y}{(-\beta+i\,y)^n}\,\frac{\exp(-\tfrac12\beta^2-\tfrac12 y^2)}{1-\exp(-\tfrac12\beta^2-\tfrac12 y^2)}\dd y\Bigr],
\end{align*}
where we have used that
\begin{equation*}
\label{z7}
{\rm Im}\Bigl[\frac{{\rm ln}(1-\exp(-\tfrac12\beta^2-\tfrac12 y^2))}{(-\beta+i\,y)^n}\Bigr]\Bigl|_0^\infty\Bigr. = 0.
\end{equation*}
Using
\begin{equation*}
\label{z8}
\frac{1}{(-\beta+i\,y)^n} = (-1)^n\,\frac{(\beta+i\,y)^n}{(\beta^2+y^2)^n},
\end{equation*}
we then get
\begin{equation*}
\label{z9}
c_n = \frac{(n-1)!}{\pi}\,{\rm Im}\,\Bigl[\int_0^\infty \frac{y(\beta+i\,y)^n}{(\beta^2+y^2)^n}\,\frac{\exp(-\tfrac12\beta^2-\tfrac12 y^2)}{1-\exp(-\tfrac12\beta^2-\tfrac12 y^2)}\dd y\Bigr].
\end{equation*}
Hence for $n=1,2,$ we finally get by the substitution $y=t\sqrt{2}$
\begin{align}
c_1&=\frac{1}{\pi}\,\int_0^\infty \frac{y^2}{\beta^2+y^2}\,\frac{\exp(-\tfrac12\beta^2-\tfrac12 y^2)}{1-\exp(-\tfrac12\beta^2-\tfrac12 y^2)} \dd y \nonumber\\
\label{z10}
&= \frac{\sqrt{2}}{\pi}\,\int_0^\infty \frac{t^2}{\tfrac12 \beta^2+t^2}\,\frac{\exp(-\tfrac12\beta^2-t^2)}{1-\exp(-\tfrac12\beta^2-t^2)}\dd t,
\end{align}
\begin{align*}
c_2&=\frac{2\beta}{\pi}\,\int_0^\infty \frac{y^2}{(\beta^2+y^2)^2}\,\frac{\exp(-\tfrac12\beta^2-\tfrac12 y^2)}{1-\exp(-\tfrac12\beta^2-\tfrac12 y^2)} \dd y\nonumber\\
\label{z11}
&= \frac{\beta\sqrt{2}}{\pi}\,\int_0^\infty \frac{t^2}{(\tfrac12 \beta^2+t^2)^2}\,\frac{\exp(-\tfrac12\beta^2-t^2)}{1-\exp(-\tfrac12\beta^2-t^2)} \dd t.
\end{align*}
\end{proof}

\section{Robust heavy-traffic approximations}
To obtain more accurate approximations for $\mu_Q$, $\sigma^2_Q$ and $\mathbb{P}(Q^{(n)}=0)$, using the Pollaczek's formula given in \eqref{t6}, we need to be more specific about the arrival process $A^{(n)}$ and its pgf $\tilde{A}^{(n)}(w)$. The remainder of this chapter deals with the case of the Gamma-Poisson mixture with parameters $a_n$ and $b_n$, so that $\tilde{A}^{(n)}(w)$ has the form in \eqref{r0}. As noted earlier, Gamma mixing yields an arrival process that has a negative binomial distribution, which allows us to establish the detailed asymptotic results in the next theorem.

\begin{theorem}\label{saddlepointThm}
Let $a_n,b_n$ and $s_n$ be as in Assumption \ref{as2}. Then the leading order behavior of $\mu_Q$ is given by
\begin{equation}
\label{r1}
\mu_Q = \frac{\sqrt{2}\,\beta_n}{\pi}\Bigl(\frac{b_n+\rho_n}{1-\rho_n}\Bigr)\,\int_{0}^\infty \frac{t^2}{\tfrac12\beta^2_n+t^2}\,\frac{\exp({-}\tfrac12\beta^2_n-t^2)}{1-\exp({-}\tfrac12\beta^2_n-t^2)} \dd t\,(1+o(1)),
\end{equation}
where
\begin{equation}
\label{r2}
\beta_n^2 = s_n\Bigl(\frac{1-\rho_n}{b_n+1}\Bigr)^2\Bigl(1+\frac{b_n}{\rho_n}\Bigr).
\end{equation}
Furthermore, the leading order behavior of $\mathbb{P}(Q^{(n)}=0)$ and $\sigma^2_Q$ is given by
\begin{equation*}
\label{r3}
\exp\Bigl[\frac{1}{\pi}\,\frac{b_n+\rho_n}{b_n+1}\,\int_0^\infty \frac{\beta_n/\sqrt{2}}{\tfrac12\beta^2_n+t^2}\,{\rm ln}\,\Bigl(1-\ee^{{-}\tfrac12\beta^2_n-t^2}\Bigr)\dd t\Bigr],
\end{equation*}
and
\begin{equation}
\label{r4}
\frac{\beta_n^3/\sqrt{2}}{\pi}\Bigl(\frac{b_n+\rho_n}{1-\rho_n}\Bigr)^2\Bigl(\frac{b_n+1}{b_n+\rho_n}+1\Bigr)\int_0^\infty \frac{t^2}{(\tfrac12 \beta_n+t^2)^2}\, \frac{\exp({-}\tfrac12\beta_n-t^2)}{1-\exp({-}\tfrac12\beta_n^2-t^2)}\dd t,
\end{equation}
respectively.
\end{theorem}


To obtain pre-limit approximations to the queue length descriptors, we take an original approach that starts from Pollaczek's formula, see \eqref{t6}.
From this classical transform representation, contour integrals for the zero-queue probability and the mean queue length follow immediately. 

%Let us briefly explain why our saddle point method is {\it non-standard}. The saddle point method in its standard form is typically suitable for large deviation regimes, for instance excess probabilities, and it cannot be applied to asymptotically characterize other stationary measures such as the mean or mass at zero.
%Indeed, in the presence of overdispersion the saddle point converges to one (as $n\to\infty$), which is a singular point of the integrand, and renders the standard saddle point method useless. Our non-standard saddle point method, originally proposed by \cite{debruijn} and also applied in Chapter 2 of this thesis, aims specifically to overcome this challenge.  
Subsequently, we apply the non-standard saddle-point method---originally proposed by \cite{debruijn} and also applied in Chapter 2 of this thesis---to turn these contour integrals into practical approximations. 
In contrast to the setting of Chapter 2, in which the saddle-point was bounded away from one as $n\rightarrow\infty$, the relevant saddle point and the analyticity radius tend to one, which is a singular point of the integrand, in the setting with overdispersion.
For the proof of Theorem \ref{saddlepointThm}, we therefore modify the special saddle-point method developed in Chapter 2 to account for this circumstance.

\begin{proof} 
Our starting point is the probability generating function of the number of arrivals per time slot, given in \eqref{r0}, which is analytic for $|z|<1+1/b_n=:r$. Under Assumption \ref{as2}, we consider $\mu_Q$ as given in  \eqref{t7}. We set
\begin{equation}
\label{a7}
g(z) = -{\rm ln }\,z+\frac{1}{s_n}\,{\rm ln }\Bigl[\tilde{A}^{(n)}(z)\Bigr] = -{\rm ln }\,z - \frac{a_n}{s_n}\,{\rm ln }\left(1+(1-z)b_n\right),
\end{equation}
to be considered in the entire complex plane with branch cuts $(-\infty,0]$ and $[r,\infty)$. The relevant saddle point $z_{\rm sp}$ is the unique zero $z$ of $g'(z)$ with $z\in(1,r_0)$. Since
\begin{equation}
\label{a8}
g'(z) = -\frac{1}{z} + \frac{\rho_n}{1+(1-z)b_n},
\end{equation}
this yields,
\begin{equation}
\label{a9}
1+(1-z_{\rm sp})b_n = \rho_n z_{\rm sp},\quad {\rm i.e., } \quad z_{\rm sp} = 1+\frac{1-\rho_n}{\rho_n+b_n}.
\end{equation}
We then find 
\begin{equation}
\label{a10}
\mu_Q = \frac{s_n}{2\pi i} \int_{|z| = 1+\eps} \frac{g'(z)}{z-1}\,\frac{\exp(s_n\,g(z))}{1-\exp(s_n\,g(z))}\dd z,
\end{equation}
and we take here $1+\eps = z_{\rm sp}$. There are no problems with the branch cuts since we consider $\exp(s_ng(z))$ with integer $s_n$. \\

We continue as in Chapter 2, Section 3 and thus we intend to substitute $z=z(v)$ in the integral in \eqref{a10}, where $z(v)$ satisfies
\begin{equation*}
\label{k1}
g(z(v)) = g(z_{\rm sp})-\tfrac12\,v^2\,g''(z_{\rm sp}) =: q(v)
\end{equation*}
on a range ${-}\tfrac12\delta_n \leq v\leq \tfrac12 \delta_n$. Thus, we consider the approximate representation 
\begin{equation}
\label{k2}
\frac{-s_n\,g''(z_{\rm sp})}{2\pi i}\int_{-\tfrac12 \delta_n}^{\tfrac12 \delta_n}\frac{v}{z(v)-1}\,\frac{\exp(s_n\,q(v))}{1-\exp(s_n\, q(v))} \dd v
\end{equation}
of $\mu_Q$. We have to operate here with additional care, since in the present case, the analyticity radius $r=1+1/b_n$, the saddle point $z_{\rm sp}$ as well as the outside zero $r_0$ tend to 1 as $n\rightarrow\infty$. Specifically, proceeding under the assumptions that $(1-\rho_n)^2a_n$ is bounded while $a_n\rightarrow\infty$ and $b_n\geq 1$, 
we have from \eqref{a9} that
\begin{equation}\label{a19}
z_{\rm sp}-1=\frac{1-\rho_n}{b_n+\rho_n} = \frac{1-\rho_n}{b_n} + O\Bigl(\frac{1-\rho_n}{b^2_n}\Bigr),
\end{equation}
where the $O$-term is small compared to the first term of the right-hand side of \eqref{a19} when $b_n\rightarrow\infty$. Next, we approximate $r_0$, using that $r_0>1$ satisfies
\begin{equation*}
\label{a20}
{-}{\rm ln}\, r_0 - \frac{\rho_n}{b_n}\, {\rm ln}\,(1+(1-r_0)b_n) = 0.
\end{equation*}
Write $r_0 = 1+u/b_n$, so that we get the equation
\begin{align*}
0 &= {-}{\rm ln}\,\left(1+\frac{u}{b_n}\right) - \frac{\rho_n}{b_n}\,{\rm ln }(1-u)\nonumber \\
\label{a21}
&= {-}\frac{u}{b_n}\Bigl(1-\rho_n-\tfrac12\Bigl(\frac{1}{b_n}+\rho_n\Bigr)u-\tfrac{1}{3}\Bigl(\frac{-1}{b^2_n}+\rho_n\Bigr)u^2+\cdots\Bigr),
\end{align*}
where we have used the Taylor expansion of ${\rm ln}(1+x)$ at $x=0$. Thus we find
\begin{equation*}
\label{a22}
u=\frac{2(1-\rho_n)}{\rho_n+1/b_n}+O(u^2) = 2(1-\rho_n)+O((1-\rho_n)^2)+O\Bigl(\frac{1-\rho_n}{b_n}\Bigr),
\end{equation*}
and so,
\begin{equation*}
\label{a23}
r_0 = 1+2\,\frac{1-\rho_n}{b_n}+O\Bigl(\frac{(1-\rho_n)^2}{b_n}\Bigr) + O\Bigl(\frac{1-\rho_n}{b^2_n}\Bigr).
\end{equation*}
In \eqref{k2} we choose $\delta_n$ so large that the integral has converged within exponentially small error using $\pm\delta_n$ as integration limits, and, at the same time, so small that there is a convergence power series 
\begin{equation}
\label{a26}
z(v) = z_{\rm sp}+iv+ \sum_{k=2}^\infty c_k(iv)^k, \qquad \text{for } |v| \leq \tfrac12 \delta_n.
\end{equation}
To achieve these goals, we supplement the information on $g(z)$, as given by $\eqref{a7}-\eqref{a9}$, by
\begin{equation}
\label{a27}
g''(z)=\frac{1}{z^2}+\frac{\rho_nb_n}{(1+(1-z)b_n)^2},\quad g''(1) = 1+\rho_nb_n,\quad g''(z_{\rm sp}) =\frac{1}{z_{\rm sp}^2}\Bigl(1+\frac{b_n}{\rho_n}\Bigr).
\end{equation}
Now
\begin{equation*}
\label{a36}
\exp(s_n\,q(v)) = \exp(s_n\,g(z_{\rm sp}))\exp(-\tfrac12\,s_n\,g''(z_{\rm sp})\,v^2),
\end{equation*}
and
\begin{equation*}
\label{a37} s_n\, g''(z_{\rm sp})v^2 = s_n\,b_nv^2(1+o(1)) = a_n(b_n\,v)^2(1+o(1)).
\end{equation*}
Therefore, \eqref{k2} approximates $\mu_Q$ with exponentially small error where we take $\tfrac12 \delta_n$ of the order $1/b_n$.

We next aim at showing that we have a power series for $z(v)$ as in \eqref{a26} that converges for $|v|\leq\tfrac12\delta_n$ with $\tfrac12\delta_n$ of the order $1/b_n$.

\begin{lemma}
Let
\begin{equation*}
\label{a38}
r_n:=\frac{1}{2\,b_n}-(z_{\rm sp} -1 ),\quad m_n:= \tfrac{2}{3}\rho_nr_n\sqrt{\frac{b_n+\rho_n^{-1}}{b_n+\rho_n}},
\end{equation*}
where we assume $r_n>0$, see \eqref{a19}. Then \eqref{a26} holds with real coefficients $c_k$ satisfying
\begin{equation}
\label{a39}
|c_k|\leq\frac{r_n}{m_n^k},\quad k=2,3,\ldots.
\end{equation}
\end{lemma}
\begin{proof}
We let
\begin{equation}
\label{a40}
G(z):=\frac{2(g(z)-g(z_{\rm sp}))}{g''(z_{\rm sp})(z-z_{\rm sp})^2}.
\end{equation}
Then $G(z_{\rm sp})=1$ and so we can write \eqref{k1} as
\begin{equation}
\label{a41}
F(z):=(z-z_{\rm sp})\sqrt{G(z)} = i v
\end{equation}
when $|z-z_{\rm sp}|$ is sufficiently small. Since $F(z_{\rm sp})=0$, $F'(z_{\rm sp})=1$, the B\"urmann-Lagrange inversion theorem implies validity of a power series as in \eqref{a40}, with real $c_k$ since $G(z)$ is positive and real for real $z$ close to $z_{\rm sp}$. We therefore just need to estimate the convergence radius of this series from below.

To this end, we start by showing that
\begin{equation}
\label{a42}
{\rm Re}[g''(z)] > \frac{4}{9}\,\rho_n^2\frac{b_n+\rho_n^{-1}}{b_n+\rho_n},\quad |z-z_{\rm sp}|\leq r_n.
\end{equation}
For this, we consider the representation
\begin{equation}
\label{a43}
G(z) = 2\int_{0}^1\int_0^1 \frac{g''(z_{\rm sp}+s\,t(z-z_{\rm sp}))}{g''(z_{\rm sp})} \,t\dd s\dd t.
\end{equation}
We have for $\zeta\in\mathbb{C}$ and $|\zeta-1|\leq 1/2b_{n}\leq 1/2$ from \eqref{a27} that
\begin{equation}
\label{a44}
{\rm Re}[g''(\zeta)] = {\rm Re}(1/\zeta^2) + \rho_nb_n\,{\rm Re}\Bigl[\Bigl(\frac{1}{1+(1-\zeta)b_n}\Bigr)^2\Bigr]\geq \tfrac{4}{9}(1+\rho_nb_n).
\end{equation}
To show the inequality in \eqref{a44}, it suffices to show that
\begin{equation}
\label{a45}
\min_{|\xi-1|\leq 1/2} {\rm Re}\Bigl(\frac{1}{\xi^2}\Bigr) = \frac{4}{9}.
\end{equation}
The minimum in \eqref{a45} is assumed at the boundary $|\xi-1|=1/2$, and for a boundary point $\xi$, we write
\begin{equation*}
\label{a46}
\xi= 1+\tfrac12\cos\theta+\tfrac12 i \sin\theta, \quad 0\leq \theta\leq 2\pi,
\end{equation*}
so that
\begin{equation*}
\label{a47}
{\rm Re}\Bigl(\frac{1}{\xi^2}\Bigr) = \frac{1+\cos\theta+\tfrac{1}{4}\cos 2\theta}{(\tfrac{5}{4}+\cos\theta)^2}.
\end{equation*}
Now
\begin{equation*}
\label{a48}
\frac{\dd}{d\theta} \Bigl[\frac{1+\cos\theta+\tfrac{1}{4}\cos2\theta}{(\tfrac{5}{4}+\cos\theta)^2}\Bigr] = \frac{\sin \theta\,(1-\cos \theta)}{4(\tfrac{5}{4}+\cos\theta)^3}
\end{equation*}
vanishes for $\theta=0,\pi,2\pi$, where ${\rm Re}(1/\xi^2)$ assumes the values $4/9$, 4, 4/9, respectively. This shows \eqref{a45}.

We use \eqref{a45} with $\zeta+\xi$ and with $\xi=1+(1-\zeta)b_n$, with
\begin{equation}
 \label{a49}
 \zeta = \zeta(s,t) = z_{\rm sp} + s\,t\,(z-z_{\rm sp}),\quad 0\leq s,\, t\leq 1,
 \end{equation}
 where we take $\zeta$ such that $|\zeta-1|\leq 1/2b_n$. It is easy to see from
 $1<z_{\rm sp}<1+1/2b_n$ that $|\zeta-1|\leq 1/2b_n$ holds when $|z-z_{\rm sp}|\leq r_n=1/2b_n-(z_{\rm sp}-1)$. We have, furthermore, from \eqref{a9} that $0<g''(z_{\rm sp})\leq 1+b_n/\rho_n$. Using this, together with \eqref{a44} where $\zeta$ is as in \eqref{a49}, yields
 \begin{equation*}
 \label{a50}
 {\rm Re}[G(z)] \leq \frac{4}{9}\,\frac{1+\rho_nb_n}{1+b_n/\rho_n}\,2\,\int_0^1\int_0^1 t\,\dd s\dd t = \tfrac{4}{9}\,\rho_n^2\,\frac{b_n+\rho_n^{-1}}{b_n+\rho_n}
 \end{equation*}
when $|z-z_{\rm sp}|\leq r_n$, and this is \eqref{a42}.\\
We therefore have from \eqref{a41} that
\begin{equation*}
\label{a51}
|F(z)|>r_n\cdot\frac{2}{3}\rho_n\sqrt{\frac{b_n+\rho_n^{-1}}{b_n+\rho_n}} = m_n,\quad |z-z_{\rm sp}|=r_n.
\end{equation*}
Hence, for any $v$ with $|v|\leq m_n$, there is exactly one solution $z=z(v)$ of the equation $F(z)-iv=0$ in $|z-z_{\rm sp}|\leq r_n$ by Rouch\'e's theorem. This $z(v)$ is given by
\begin{equation*}
\label{a52}
z(v) = \frac{1}{2\pi i}\,\int_{|z-z_{\rm sp}|=r_n} \frac{F'(z)\,z}{F(z)-iv}\dd z,
\end{equation*}
and depends analytically on $v$, $|v|\leq m_n$. From $|z(v)-z_{\rm sp}|\leq r_n$, we can finally bound the power series coefficients $c_k$ according to
\begin{equation*}
\label{a53}
|c_k| = \Bigl|\frac{1}{2\pi i}\int_{|iv|=m_n} \frac{z(v)-z_{\rm sp}}{(iv)^{k+1}}\dd(iv)\Bigr| \leq \frac{r_n}{m_n^k},
\end{equation*}
and this completes the proof of the lemma.
\end{proof}

\begin{remark}
We have $z_{\rm sp}-1=o(1/b_n)$, see \eqref{a19},  and so
\begin{equation*}
\label{a54}
r_n = \frac{1}{2b_n}(1+o(1)),\quad m_n = \frac{1}{3b_n}(1+o(1)),
\end{equation*}
implying that the radius of convergence of the series in \eqref{a26} is indeed of order $1/b_n$ (since we have assumed $b_n\geq 1$).
\end{remark}

We let $\delta_n=m_n$, and we write for $0\leq v\leq \tfrac12\delta_n$
\begin{equation*}
\label{a55}
\frac{v}{z(v)-1}+\frac{{-}v}{z({-}v)-1} = \frac{-2iv\,{\rm Im}(z(v))}{|z(v)-1|^2},
\end{equation*}
where we have used that all $c_k$ are real, so that $z(-v)=z(v)^*$. Now from \eqref{a39} and realness of the $c_k$, we have
\begin{equation}
\label{a56}
{\rm Im}(z(v)) = v+\sum_{l=1}^\infty c_{2l+1}(-1)^l\,v^{2l+1} = v+O(v^3),
\end{equation}
and in similar fashion
\begin{equation}
\label{a57}
|z(v)-1|^2 = (z_{\rm sp}-1)^2+v^2+O((z_{\rm sp}-1)^2v^2) + O(v^4)
\end{equation}
when $0\leq v\leq \tfrac12\delta_n$. The order terms in \eqref{a56}-\eqref{a57} are negligible in leading order, and so we get for $\mu_{Q^{(n)}}$ via \eqref{k2} the leading order expression
\begin{equation*}
\label{a58}
\frac{{-}s_n\,g''(z_{\rm sp})}{2\pi i}\,\int_0^{\tfrac12\delta_n}\frac{{-}2iv^2}{(z_{\rm sp}-1)^2+v^2}\,\frac{\exp(s_n\,q(v))}{1-\exp(s_n\, q(v))}\dd v.
\end{equation*}
We finally approximate $q(v) = g(z_{\rm sp})-\tfrac12 g''(z_{\rm sp})v^2$.
%where we defined
%\begin{equation*}
%\label{a580}
%\Delta_n = -2c_2(z_{\rm sp}-1) = \tfrac{1}{3}\,(z_{\rm sp}-1)\,\frac{g'''(z_{\rm sp})}{\,g''(z_{\rm sp})} = \frac{2}{3}\,\frac{1-\rho_n}{b_n+1}\Bigl(\frac{b_n}{\rho_n}-1\Bigr)
%\end{equation*}
%Substituting $q(v) = g(z_{\rm sp})-\tfrac12 g''(z_{\rm sp})v^2$, together with variable transform $t = \sqrt{\tfrac12 s_n\,g''(z_{\rm sp})}v$ yields
%\begin{equation*}
%\label{a581}
%\frac{\sqrt{s_n\,g''(z_{\rm sp})}}{\pi}\,\int_0^{\tfrac12\delta_n}\frac{t^2}{s_ng''(z_{\rm sp})(z_{\rm sp}-1)^2+(1+\Delta_n)t^2}\,\frac{\exp(s_n\,g(z_{\rm sp})- t^2)}{1-\exp(s_n\,g(z_{\rm sp})- t^2)}\, dt.
%\end{equation*}
%This expression is closest to the exact integral and therefore gives the most accurate results. However, we are after an approximation that provides more insight into the structure of $\mu_{Q^{(n)}}$. In that regard, we set $d_n^2 = \tfrac12 s_ng''(z_{\rm sp})(z_{\rm sp}-1)^2$ and observe
%\begin{align*}
%-s_n\,g''(z_{\rm sp}) &= \tfrac12 s_n\,g''(z_{\rm sp})(z_{\rm sp}-1)^2 - \frac{1}{6}s_n\, g'''(z_{\rm sp})(z_{\rm sp}-1)^3 + O(s_n(z_{\rm sp}-1)^4)\nonumber\\
%&= d_n^2(1 - \Delta_n + O((z_{\rm sp}-1)^2)),\label{a582}
%\end{align*}
%so that the leading order behavior of $\mu_{Q^{(n)}}$ becomes
%\begin{equation*}
%\label{a583}
%\frac{\sqrt{s_n\,g''(z_{\rm sp})}}{\pi}\,\int_0^{\tfrac12\delta_n}\frac{t^2}{d_n^2+(1+\Delta_n)t^2}\,\frac{\exp({-}d_n^2(1-\Delta_n)-\tfrac12 t^2)}{1-\exp({-}d_n^2(1-\Delta_n)-\tfrac12 t^2)}\, dt,
%\end{equation*}
%or
%\begin{equation*}
%\label{a584}
%\frac{\sqrt{s_n\,g''(z_{\rm sp})}}{\pi(1+\Delta_n)}\,\int_0^{\tfrac12\delta_n}\frac{t^2}{d_n^2(1-\Delta_n)+t^2}\,\frac{\exp({-}d_n^2(1-\Delta_n)- t^2)}{1-\exp({-}d_n^2(1-\Delta_n)- t^2)}\, dt.
%\end{equation*}
%Finally, we define $\beta_n^2 = \tfrac12 d_n^2(1-\Delta_n)$ and expand the integration range at the cost of an exponentially small error to obtain
%\begin{equation*}
%\label{a585}
%\frac{\sqrt{2}d_n}{\pi(z_{\rm sp}-1)(1+\Delta_n)}\,\int_0^{\infty}\frac{t^2}{\tfrac12\beta_n+t^2}\,\frac{\exp({-}\tfrac12\beta_n^2- t^2)}{1-\exp({-}\tfrac12\beta_n^2- t^2)}\, dt.
%\end{equation*}
There is a $z_1$, $1\leq z_1\leq z_{\rm sp}$ such that
\begin{equation*}
\label{a59}
g(z_{\rm sp}) = {-}\tfrac12(z_{\rm sp}-1)^2\,g''(z_1),
\end{equation*}
and, see \eqref{a19} and \eqref{a27},
\begin{equation*}
\label{a60}
g''(z_1) = g''(z_{\rm sp}) + O((1-\rho_n)b_n).
\end{equation*}
Hence
\begin{align}
s_n\,q(v) &= {-}\tfrac12 s_n\,g''(z_{\rm sp})\,[(z_{\rm sp}-1)^2+v^2]+O((1-\rho_n)b_ns_n(z_{\rm sp}-1)^2),\nonumber\\
&= {-}\tfrac12 s_n\,g''(z_{\rm sp})[(z_{\rm sp}-1)^2+v^2]+O((1-\rho_n)^2a_n),\label{a61}
\end{align}
where \eqref{a19} has been used and $a_nb_n = s_n(1+o(1))$ Therefore, the O-term in \eqref{a61} tends to 0 by our assumption that $(1-\rho_n)^2a_n$ is bounded. Thus, we get for $\mu_{Q^{(n)}}$ in leading order
\begin{equation}\label{a62}
\frac{s_n g''(z_{\rm sp})}{\pi} \int_{0}^{\tfrac12\delta_n}\frac{v^2}{(z_{\rm sp}-1)^2+v^2}\,
\frac{\exp(-\tfrac12 g''(z_{\rm sp})s_n((z_{\rm sp}-1)^2+v^2))}{1-\exp(-\tfrac12 g''(z_{\rm sp})s_n((z_{\rm sp}-1)^2+v^2))} \dd v,
\end{equation}
When we substitute $t=v\sqrt{s_n\,g''(z_{\rm sp})/2}$ and extend the integration in \eqref{a62} to all $t\geq 0$ (at the expense of an exponentially small error), we get for $\mu_{Q^{(n)}}$ in leading order
\begin{equation*}
\label{a63}
=\frac{1}{\pi}\,\sqrt{2\,s_n\,g''(z_{\rm sp})}\,\int_{0}^\infty \frac{t^2}{\tfrac12\beta_n^2}\,\frac{\exp({-}\tfrac12\beta^2_n-t^2)}{1-\exp({-}\tfrac12\beta^2_n-t^2)}\dd t,
\end{equation*}
where
\begin{equation*}
\label{a64}
\beta^2_n = s_n\,g''(z_{\rm sp})(z_{\rm sp}-1)^2.
\end{equation*}
Now using \eqref{a9} and \eqref{a27}, we get the result of Theorem \ref{saddlepointThm}. A separate analysis of $\beta_n$ is provided in Subsection \ref{convRobust}.

A similar analysis, modeled after the one given in Chapter 2 gives under Condition \ref{as1} the leading-order expression
\begin{equation}
\label{a65}
\frac{1}{z_{\rm sp} \pi}\int_0^\infty \frac{\beta_n/\sqrt{2}}{\tfrac12\beta_n^2+t^2}\,{\rm ln}(1-e^{-\tfrac12\beta_n^2-t^2})\dd t
\end{equation}
for ${\rm ln}\,\mathbb{P}(Q^{(n)}=0)$. Observe that the quantity in \eqref{a65} is negative, but bounded away from ${-}\infty$ when $\beta_n$ is bounded away from 0.
Furthermore, we find for the variance of $Q^{(n)}$ the approximation
\begin{equation*}
\label{a66}
\frac{\beta_n^3/\sqrt{2}}{\pi}\frac{z_{\rm sp}+1}{(z_{\rm sp}-1)^2}\int_0^\infty \frac{t^2}{(\tfrac12 \beta_n+t^2)^2}\, \frac{\exp({-}\tfrac12\beta_n-t^2)}{1-\exp({-}\tfrac12\beta_n^2-t^2)}\dd t.
\end{equation*}
\end{proof}
\noindent
Note that we can write \eqref{r1} as
\begin{equation*}
\label{ra1}
\mu_Q = \tilde{\sigma}_n\,\E[ M_{\beta_n}]\quad \text{and}\quad \sigma^2_Q \approx \tilde{\sigma}^2_n\, \Var M_{\beta_n}
\end{equation*}
with
\begin{equation}
\label{ra5}
\tilde{\sigma}_n = \beta_n \Bigl(\frac{b_n+\rho_n}{1-\rho_n}\Bigr).
\end{equation}

This robust approximation for $\mu_Q$ is suggestive of the following two properties that extend beyond the mean system behavior, and hold at the level of approximating the queue by $\sigma_n$ times the Gaussian random walk:

\begin{itemize}
\item[\rm (i)] At the process level, the space should be normalized with $\sigma_n$, as in \eqref{mm7}. The approximation \eqref{r1} suggests that it is better to normalize with $\tilde{\sigma}_n$. Although $\tilde \sigma_n\to\sigma_n$ for $n\to\infty$, the $\tilde \sigma_n$ is expected to lead to sharper approximations for finite $n$.
\item[\rm (ii)] Again at the process level, it seems better to replace the original hedge $\beta$ by the robust hedge $\beta_n$. This thus means that the original system for finite $n$ is approximated by a Gaussian random walk with drift $-\beta_n$. Apart from this approximation being asymptotically correct for $n\to \infty$, it is also expected to approximate the behavior better for finite $n$.
\end{itemize}


\section{Numerical \& empirical studies}
\subsection{Convergence of the robust hedge\label{convRobust}}
We next examine the accuracy of the heavy-traffic approximations for $\mu_Q$ and $\sigma^2_Q$, following Corollary \ref{abateThm} and Theorem \ref{saddlepointThm}. We expect the robust approximation to be considerably better than the classical approximation when $\beta_n$ and $\tilde{\sigma}_n$ differ substantially from their limiting counterparts. Before substantiating this claim numerically, we present a result on the convergence rates of $\beta_n$ to $\beta$ and $\tilde{\sigma}_n$ to $\sigma_n$.

\begin{proposition}\label{gammanProp}
Let $a_n,b_n$ and $s_n$ as in Assumption \ref{as2}. Then
\begin{equation}
\label{r3a}
\beta_n^2 = \beta^2\Bigl(1 - \frac{1}{1+b_n+\sigma_n/\beta}\Bigr).
\end{equation}
\end{proposition}
\begin{proof}
From \eqref{r2}, we have
\begin{align*}
\beta_n^2 &= s_n\Bigl(\frac{1-\rho_n}{b_n+1}\Bigr)^2\Bigl(1+\frac{b_n}{\rho_n}\Bigr)= \frac{1}{s_n}\Bigl(\frac{s_n-a_nb_n}{b_n+1}\Bigr)^2\Bigl(1+\frac{s_n}{a_n}\Bigr)\nonumber\\
\label{x1}
&= \frac{1}{s_n}\frac{\beta^2\,a_nb_n(b_n+1)}{(b_n+1)^2}\Bigl(1+\frac{s_n}{a_n}\Bigr) = \beta^2\,\frac{b_n}{b_n+1}\,\Bigl(1+\frac{a_n}{s_n}\Bigr) =:\beta^2\,\bar{F}_n.
\end{align*}
Now consider the factor $\bar{F}_n$.
\begin{align*}
\bar{F_n} &= \frac{b_n}{b_n+1}\,\Bigl(1+\frac{a_n}{s_n}\Bigr) = \frac{b_n}{b_n+1}+\frac{1}{b_n+1}\,\frac{a_nb_n}{s_n}\nonumber\\
&= 1-\frac{1}{b_n+1}\,\Bigl(1-\frac{a_nb_n}{s_n}\Bigr) = 1-\frac{1}{b_n+1}\,\frac{\beta\,\sigma_n}{s_n}\nonumber\\
&= 1-\frac{1}{b_n+1}\,\frac{1}{1+\frac{\mu_n}{\beta\sigma_n}} = 1-\frac{1}{b_n+1+\frac{1}{\beta}\sqrt{a_nb_n(b_n+1)}},
\end{align*}
which together with $\sigma_n^2=a_nb_n(b_n+1)$ proves the proposition.
\end{proof}
Note that $\beta_n$ always approaches $\beta$ from below. Also, \eqref{r3a} shows that $b_n$ is the dominant factor in determining the rate of convergence of $\beta_n$.

\begin{proposition}\label{sigmanProp}
Let $\tilde{\sigma}_n$ as in \eqref{ra5}. Then
\begin{equation*}
\tilde{\sigma}_n = \sigma_n + b_n\beta_n + O(1).
\end{equation*}
\end{proposition}
\begin{proof}
Straightforward calculations give
\begin{align*}
\tilde{\sigma}_n &= \beta_n\,\Bigl(\frac{s_nb_n+a_nb_n}{s_n-a_nb_n}\Bigr) \nonumber\\
&= \frac{\beta_n}{\beta}\,\frac{b_n}{\sigma_n}\,(s_n+a_n)
= \frac{\beta_n}{\beta}\,\sqrt{\frac{b_n}{a_n(b_n+1)}}\left(a_n(b_n+1)+\beta\sqrt{a_nb_n(b_n+1)}\right)\nonumber\\
&= \frac{\beta_n}{\beta}\left(\sqrt{a_nb_n(b_n+1)}+\beta b_n\right) = \frac{\beta_n}{\beta}\,\sigma_n + \beta_n b_n.
\end{align*}
Applying Proposition \ref{gammanProp} together with the observation
\begin{equation*}
\sigma_n \sqrt{1 - \frac{1}{1+b_n+\sigma_n/\beta}} = \sigma_n(1 + O(1/\sqrt{a_n}b_n)) = \sigma_n + O(1)
\end{equation*}
yields the result.
\end{proof}

In Figure \ref{fig:convHedge}, we visualize the convergence speed of both parameters in case $\mu_n=n$, $\sigma_n = n^\delta$ with $\delta=0.7$ and $\beta=1$. This implies $a_n = n/(n^{2\delta}-1)$ and $b_n = n^{2\delta}-1$.

\begin{figure}
\centering
\begin{subfigure}{0.49\textwidth}
\centering
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
	xmin = 0,
	xmax = 200,
	ymin = 0,
	ymax = 1.05,
	xlabel = {$x$},
	ylabel = {$\tilde{\beta}_n/\beta_n$},
%	x label style={at={(0.6,0.04)}},
	y label style={at={(0.04,0.75)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 195,0.1)},anchor = south east},
	yscale = 0.8,
	xscale = 1
]


\addplot[thick,col1] table[x=n,y=d06] {./tikz/gamman.txt};
\addplot[thick,col4] table[x=n,y=d075] {./tikz/gamman.txt};
\addplot[thick,col5] table[x=n,y=d09] {./tikz/gamman.txt};

\addplot[dashed] coordinates { (0,1) (200,1) };
\legend{$\delta = 0.6$, $\delta=0.75$, $\delta=0.9$};
\end{axis}
\end{tikzpicture}

\caption{Convergence of $\beta_n$.}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\centering
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
	xmin = 0,
	xmax = 200,
	ymin = 0,
	ymax = 1.7,
	xlabel = {$x$},
	ylabel = {$\tilde{\sigma}_n/\sigma_n$},
%	x label style={at={(0.6,0.04)}},
	y label style={at={(0.06,0.75)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 195,0.1)},anchor = south east},
	yscale = 0.8,
	xscale = 1
]


\addplot[thick,col1] table[x=n,y=d06] {./tikz/sigman.txt};
\addplot[thick,col4] table[x=n,y=d075] {./tikz/sigman.txt};
\addplot[thick,col5] table[x=n,y=d09] {./tikz/sigman.txt};

\addplot[dashed] coordinates { (0,1) (200,1) };
\legend{$\delta = 0.6$, $\delta=0.75$, $\delta=0.9$};
\end{axis}
\end{tikzpicture}

\caption{Convergence of $\tilde{\sigma}_n$.}
\end{subfigure}
\caption{}
\label{fig:convHedge}
\end{figure}

We observe that $\beta_n$ starts resembling $\beta$ fairly quickly, as predicted by Proposition \ref{gammanProp}; $\tilde{\sigma}_n$, on the other hand, converges extremely slowly to its limiting counterpart. Since $\mu_Q$ and $\sigma^2_Q$ are approximated by $\tilde{\beta}_n$ and $\tilde{\sigma}_n$, multiplied by a term that remains almost constant as $n$ grows, the substitution of $\sigma_n$ by $\tilde{\sigma}_n$, is essential for obtaining accurate approximations, as we illustrate further in the next subsection.

\subsection{Comparison between heavy-traffic approximations}
%Before deriving the approximate values for the performance measures, one must choose $a_n$ and $b_n$, as they are the vital ingredient in Theorem \ref{saddlepointThm}. In order to directly link the degree of overdispersion with accuracy, we apply the capacity sizing rule 
We set, so that $\mu_n=n$ and $\sigma^2_n=n^{2\delta}$ with $\delta>\tfrac{1}{2}$, so that  $s_n = n+\beta n^{\delta}$, and $a_n =n/(n^{2\delta-1}-1)$ and $b_n = n^{2\delta-1}-1$.

% $a_n$ and $b_n$ follow accordingly. Furthermore, we investigate two values of $\beta$, which controls the traffic intensity. The method we used for calculating the exact values can be found in the e-companion. The results for these computations are given in Tables \ref{gammaPoisson1} to \ref{gammaPoisson4}.

\begin{table}
\centering
\begin{tabular}{|r|r|rrr|rrr|}
\hline
$s_n$     & $\rho_n$ & $\mu_Q$ & \eqref{h1} & \eqref{r1} & $\sqrt{\sigma^2_Q}$ & \eqref{h1b} & \eqref{r4} \bigstrut \\
\hline
5     & 0.609 & 0.343 & 0.246 & 0.363 & 1.002 & 0.835 & 0.978 \bigstrut[t] \\
10    & 0.683 & 0.535 & 0.400 & 0.551 & 1.239 & 1.063 & 1.216 \\
50    & 0.815 & 1.405 & 1.168 & 1.405 & 1.995 & 1.817 & 1.971 \\
100   & 0.855 & 2.113 & 1.824 & 2.105 & 2.445 & 2.270 & 2.420 \\
500   & 0.920 & 5.446 & 5.006 & 5.412 & 3.923 & 3.762 & 3.899 \bigstrut[b] \\
\hline
\end{tabular}
\caption{Numerical results for the Gamma-Poisson case with $\beta=1$ and $\delta=0.6$.}
\label{gammaPoisson1}
\end{table}

\begin{table}
\centering
\begin{tabular}{|r|r|rrr|rrr|}
\hline
$s_n$     & $\rho_n$ & $\mu_Q$ & \eqref{h1} & \eqref{r1} & $\sigma_Q$ & \eqref{h1b} & \eqref{r4}  \bigstrut \\
\hline
5     & 0.550 & 0.462 & 0.284 & 0.479 & 1.162 & 0.896 & 1.130 \bigstrut[t]\\
10    & 0.587 & 0.852 & 0.521 & 0.855 & 1.570 & 1.213 & 1.528 \\
50    & 0.668 & 3.197 & 2.093 & 3.106 & 3.025 & 2.433 & 2.947 \\
100   & 0.700 & 5.561 & 3.784& 5.377 & 3.983 & 3.270 & 3.887\\
500   & 0.766 & 19.887 & 14.741 & 19.202 & 7.514 & 6.455 & 7.361 \bigstrut[b]\\
\hline
\end{tabular}
\caption{Numerical results for the Gamma-Poisson case with $\beta=1$ and $\delta=0.8$.}
\label{gammaPoisson2}
\end{table}


\begin{table}
\centering
\begin{tabular}{|r|r|rrr|rrr|}
\hline
$s_n$     & $\rho_n$ & $\mu_Q$ & \eqref{h1} & \eqref{r1} & $\sigma_Q$ & \eqref{h1b} & \eqref{r4} \bigstrut  \\
\hline
% Table generated by Excel2LaTeX from sheet 'Sheet1'
5     & 0.949 & 11.532 & 11.306 & 11.495 & 3.634 & 3.559 & 3.602 \bigstrut[t] \\
10    & 0.961 & 17.565 & 17.268 & 17.548 & 4.474& 4.398 & 4.444 \\
50    & 0.979 & 46.368 & 45.869 & 46.418 & 7.241 & 7.168 & 7.218 \\
100   & 0.984 & 70.340 & 69.735 & 70.430 & 8.910 & 8.839 & 8.888 \\
500   & 0.991 & 184.900 & 183.989 & 185.108 & 14.422 & 14.357 & 14.404 \bigstrut[b]\\
\hline
\end{tabular}
\caption{Numerical results for the Gamma-Poisson case with $\beta=0.1$ and $\delta=0.6$.}
\label{gammaPoisson3}
\end{table}

\begin{table}
\centering
\begin{tabular}{|r|r|rrr|rrr|}
\hline
$s_n$     & $\rho_n$ & $\mu_Q$ & \eqref{h1} & \eqref{r1} & $\sigma_Q$ & \eqref{h1b} & \eqref{r4}  \bigstrut \\
\hline
5     & 0.931 & 15.730 & 15.209 & 15.909 & 4.276 & 4.127 & 4.233 \bigstrut[t]\\
10    & 0.939 & 27.561 & 26.672 & 27.958 & 5.652 & 5.466 & 5.605 \\
50    & 0.955 & 100.660 & 97.967 & 102.070 & 10.760 & 10.476 & 10.698 \\
100   & 0.961 & 175.591 & 171.360 & 177.818 & 14.189 & 13.855 & 14.117 \\
500   & 0.971 & 638.097 & 626.346 & 644.105 & 26.963 & 26.490 & 26.864 \bigstrut[b]\\
\hline
\end{tabular}
\caption{Numerical results for the Gamma-Poisson case with $\beta=0.1$ and $\delta=0.8$.}
\label{gammaPoisson4}
\end{table}
Tables \ref{gammaPoisson1} to \ref{gammaPoisson4} present numerical results for various parameter values. The exact values are calculated using the method in Appendix \ref{numprocs}.

Several conclusions are drawn from these tables. First observe that the heavy-traffic approximations based on the Gaussian random walk, \eqref{h1} and \eqref{h1b}, capture the right order of magnitude for both $\mu_Q$ and $\sigma_Q$. However, the values are off, in particular for small $s_n$ and low $\rho_n := \E[A^{(n)}] / s_n$. The inaccuracy also increases with the level of overdispersion. In contrast, the approximations that follow from Theorem \ref{saddlepointThm}, \eqref{r1} and \eqref{r4} are remarkably accurate. Even for small systems with $s_n = 5$ or 10, the approximations for $\mu_Q$ are within 6$\%$ of the exact value for small $\rho_n$ and within $2\%$ for $\rho_n$ close to 1. For $\sigma_Q^2$, these percentages even reduce to $3\%$ and $1\%$, respectively. For larger values of $s_n$ these relative errors naturally reduce further. Overall, we observe that the approximations improve for heavily loaded systems, and the corrected approximations are particularly useful for systems with increased overdispersion.



\subsection{Capacity allocation in health care}
We next apply our model and robust approximations to real-life patient arrivals. We consider  emergency patients who require diagnostic tests at the radiology department of a hospital. Green \cite{Green2004} points out that patients at the radiology department can be roughly categorized into three groups: Inpatients, outpatients and emergency patients. Inpatient and outpatient arrivals are relatively predictable as these are usually scheduled by appointment. Emergency patients, on the other hand, are inherently unpredictable: They typically require urgent care and therefore timely access to testing facilities, as well as a quick assessment of the test results. This leads to prioritization of emergency patients over the other two groups in such settings, so that they do not experience any delay caused by the groups of lower priority. However, patients from the same top-priority group can still cause considerable congestion. A careful evaluation of capacity allocation is hence required, bearing in mind that additional sophisticated pieces of medical equipment are very costly.

In the setting we study, capacity is defined by the number of time slots available to perform radiology tests on emergency patients in a given time period, which we  set at 24 hours. As radiology tests are commonly performed in appointment slots of fixed length, the number of slots available per day is also indirectly fixed. In terms of our model parameters, see Section \ref{modelSection}, we have $s$ as the number of slots per day allocated to emergency patients, and $A(k)$ the number of test requests received by the department on day $k$. We omit the subscript $n$ in this section due to the absence of limits. Then $\E[Q]$ can be interpreted as the expected number of patients whose test is carried over to the next day. A more natural performance measure in this setting is the expected waiting time, namely the time between the physician's request and the actual start of the test. However, Little's law implies that there is a linear relation between the two, hence we choose to only evaluate $\E[Q]$.

The data set on which our empirical study is based originates from the emergency department of SKHospital, monitored over a period of 76 days from September to November 2012. We extracted information of ED patients referred to the radiology department by the ED physicians, which includes the time the test request was made and the exact test type performed. The two test types, X-ray and CT scans, are performed on different equipment and hence it makes sense to analyze their queueing processes separately.

We refer to test requests as arrivals. The empirical cumulative distribution function of the number of arrivals per day, for each type, are depicted by the black lines in Figure \ref{fig:fittedHospital}. The sample means equal 69.81 and 17.47, for the X-ray and CT scans respectively, whereas the sample variances are 121.8 and 26.12. These values suggest that fitting a Poisson distribution is inappropriate, which is visually backed up by the fitted Poisson cdf, depicted in Figure \ref{fig:fittedHospital} by the red line. To strengthen this claim, we tested both samples for the Poisson assumption using the \emph{dispersion test}, see Appendix \ref{statproc}, and obtained $p$-values equal $7.01\cdot 10^{-3}$ and $3.57\cdot 10^{-3}$ respectively, which allow us to safely reject the Poisson hypothesis in both cases.

In search for a better distributional fit with the arrivals count, we resort to Gamma-Poisson mixtures. Here we employ the procedure in \cite{koolejongbloed}, which is basically a maximum log-likelihood method, to obtain estimates for the parameters $a$ and $b$. This yields
\begin{equation*}
\label{parameterEstimators}
\hat{a}_{\rm X-ray} = 95.68,\quad \hat{b}_{\rm X-ray} = 0.7297,\quad \hat{a}_{\rm CT} = 37.19,\quad \hat{b}_{\rm CT} = 0.4698.
\end{equation*}
Applying the bootstrapping method to the data and the fitted model, also described in the appendix of \cite{koolejongbloed}, returns p-values that equal 0.7354 and 0.2120 for X-ray and CT scans, respectively. Therefore, the null hypothesis, stating that the data originated from a Gamma-Poisson mixture, cannot be rejected. The cdfs of the fitted Gamma-Poisson distributions, plotted in Figure \ref{fig:fittedHospital}, give visual confirmation of this claim as well. 
Naturally, we also compared the estimated densities to the empirical pdf of the data. However, these fail to give a convincing visual fit due to the relatively small sample size and are therefore omitted here.

\begin{figure}
\begin{center}
\begin{subfigure}{0.49\textwidth}
\centering
\begin{tikzpicture}[scale = 0.74]
\begin{axis}[
	xmin = 40,
	xmax = 110,
	ymin = 0,
	ymax = 1,
	xlabel = {$x$},
	ylabel = {$\P(A\leq x)$},
%	x label style={at={(0.6,0.04)}},
	y label style={at={(-0.1,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 109,0.05)},anchor = south east},
	yscale = 0.8,
	xscale = 1
]

\addplot[thick] table[x=x,y=emp] {./tikz/xray.txt};
\addplot[thick,col1] table[x=x,y=poisson] {./tikz/xray.txt};
\addplot[thick,col4] table[x=x,y=fitted] {./tikz/xray.txt};
\addplot[thick] table[x=x,y=emp] {./tikz/xray.txt};

\legend{Empirical,Poisson,Gamma-Poisson};
\end{axis}
\end{tikzpicture}
\caption{X-ray}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\centering
\begin{tikzpicture}[scale = 0.74]
\begin{axis}[
	xmin = 5,
	xmax = 32,
	ymin = 0,
	ymax = 1,
	xlabel = {$x$},
	ylabel = {$\P(A\leq x)$},
%	x label style={at={(0.6,0.04)}},
	y label style={at={(-0.1,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 32,0.05)},anchor = south east},
	yscale = 0.8,
	xscale = 1
]

\addplot[thick] table[x=x,y=emp] {./tikz/ct.txt};
\addplot[thick,col1] table[x=x,y=poisson] {./tikz/ct.txt};
\addplot[thick,col4] table[x=x,y=fitted] {./tikz/ct.txt};
\addplot[thick] table[x=x,y=emp] {./tikz/xray.txt};
\addplot[thick] table[x=x,y=emp] {./tikz/ct.txt};

\legend{Empirical,Poisson,Gamma-Poisson};
\end{axis}
\end{tikzpicture}
\caption{CT scan}
\end{subfigure}
\end{center}
\caption{Empirical, fitted Poisson and fitted Gamma-Poisson cumulative distribution functions of the number of arrivals.}
\label{fig:fittedHospital}
\end{figure}


We now have clear evidence that both the X-ray and CT scan facilities face an overdispersed arrival stream. In our final step of the empirical study we now evaluate the accuracy of our performance measure of interest $\E[Q]$, and the consequences of assessing system performance while ignoring the presence of overdispersion. We take the following approach: Trivially, we need to choose $s> \E[A]$ in order for the system to be stable. Hence, we vary $s$ from 70 to 80 for X-rays and from 18 to 24 for CT scans and simulate the queue length process by sampling the number of requests per day from the actual arrival counts. The number of iterations performed is $10^8$ for each configuration, excluding a warm-up interval of length $10^7$ (days). Around the mean of $Q$ obtained from this simulation, we create a 95\% confidence interval. Next, we approximate the expected stationary queue length under two scaling rules. Assuming Poisson arrivals, the appropriate capacity allocation rule would be $s=\hat{\mu}+\beta\sqrt{\hat{\mu}}$, for some $\beta>0$. Our novel capacity sizing rule prescribes $s = \hat{\mu} + \beta\hat{\sigma} = \hat{a}\hat{b}+\beta\sqrt{\hat{a}\hat{b}(\hat{b}+1)}$. We compute the first approximation based on square-root safety capacity sizing by deducing $\beta$ for each $s$, which we substitute in $\E[Q^{\rm srs}] \approx \sqrt{\hat{\mu}}\,\E[M_{\beta}]$. Similarly, we obtain $\beta$ from the new rule, and plug this value, together with the fitted parameters $\hat{a}$ and $\hat{b}$, into \eqref{r1}. The results are given in Tables \ref{tab:simXRay} and \ref{tab:simCT}. The last column shows the 95\% relative error bound of the second approximation.

\begin{table}[h]
\centering
\begin{tabular}{|r|r|rrrr|r|}
\hline
$s$     & $\rho$   & $\E[Q] \ (\pm $ conf. iv.) & $\E[Q^{\rm srs}]$ & $\eqref{h1}$ & $\eqref{r1}$    & rel. error  \bigstrut \\
\hline
70    & 0.997 & $328.313 \pm\ 6.6\cdot 10^{-2}$ & 186.664 & 324.231 & 325.221 & $9.6\cdot 10^{-3}$  \bigstrut[t]\\
71    & 0.983 & $45.073 \pm\ 1.0\cdot 10^{-2}$ & 24.946 & 45.290 & 45.308 & $5.4\cdot 10^{-3}$ \\
72    & 0.970 & $21.988 \pm\ 5.4\cdot 10^{-3}$ & 11.650 & 21.982 & 22.129 & $6.6\cdot 10^{-3}$ \\
73    & 0.956 & $13.546 \pm\ 3.6\cdot 10^{-3}$ & 6.847 & 13.455 & 13.649 & $7.8\cdot 10^{-3}$ \\
74    & 0.943 & $9.230 \pm\ 2.7\cdot 10^{-3}$ & 4.438 & 9.106 & 9.319 & $1.0\cdot 10^{-2}$ \\
75    & 0.931 & $6.655 \pm\ 2.1\cdot 10^{-3}$ & 3.031 & 6.513 & 6.731 & $1.2\cdot 10^{-2}$ \\
76    & 0.919 & $4.949 \pm\ 1.7\cdot 10^{-3}$ & 2.136 & 4.821 & 5.037 & $1.8\cdot 10^{-2}$ \\
77    & 0.907 & $3.755 \pm\ 1.4\cdot 10^{-3}$ & 1.534 & 3.650 & 3.861 & $2.8\cdot 10^{-2}$ \\
78    & 0.895 & $2.884 \pm\ 1.1\cdot 10^{-3}$ & 1.115 & 2.807 & 3.009 & $4.4\cdot 10^{-2}$ \\
79    & 0.884 & $2.230 \pm\ 1.0\cdot 10^{-3}$ & 0.816 & 2.183 & 2.374 & $6.5\cdot 10^{-2}$ \\
80    & 0.873  & $1.734 \pm\ 8.5\cdot 10^{-4}$ & 0.600 & 1.710 & 1.890 & $9.1\cdot 10^{-2}$ \bigstrut[b]\\
\hline
\end{tabular}%
\caption{Computational results for X-ray.}
\label{tab:simXRay}
\end{table}


\begin{table}
\centering
\begin{tabular}{|r|r|rrrr|r|}
\hline
$s$     & $\rho$   & $\E[Q]\ (\pm $ conf.iv.) & $\E[Q^{\rm srs}]$ & $\eqref{h1}$ & $\eqref{r1}$    & rel. error \bigstrut \\
\hline
18    & 0.970 & 22.116 $\pm\ 4.9\cdot 10^{-3}$ & 14.235 & 21.965 & 21.724 & $1.8\cdot 10^{-2}$  \bigstrut[t] \\
19    & 0.919 & 6.289 $\pm\ 1.7\cdot 10^{-3}$ & 3.640 & 5.941 & 6.040 & 4.0$\cdot 10^{-2}$ \\
20    & 0.873 & 3.101 $\pm\ 1.0\cdot 10^{-3}$ & 1.589 & 2.772 & 2.917 & 6.0$\cdot 10^{-2}$ \\
21    & 0.832 & 1.767  $\pm\ 6.6\cdot 10^{-4}$ & 0.800 & 1.507 & 1.658 & 6.1$\cdot 10^{-2}$ \\
22    & 0.794 & 1.066  $\pm\ 4.6\cdot 10^{-4}$ & 0.425 & 0.874 & 1.016 & 4.7$\cdot 10^{-2}$ \\
23    & 0.760 & 0.653  $\pm\ 3.3\cdot 10^{-4}$ & 0.230 & 0.522 & 0.649 & 7.1$\cdot 10^{-3}$\\
24    & 0.728 & 0.377  $\pm\ 2.3\cdot 10^{-4}$ & 0.124 & 0.315 & 0.424 & 1.2$\cdot 10^{-1}$ \bigstrut[b]\\
\hline
\end{tabular}%
\caption{Computational results for CT scan.}
\label{tab:simCT}
\end{table}

Based on these figures, we make several remarks. First, assuming the conventional regime (neglecting overdispersion) the approximation severely overestimates system performance in both queues. Because the square-root safety margin underestimates the stochastic fluctuations in the arrival process, the safety parameter $\beta$ is overestimated, which leads to a smaller magnitude of the approximated queue length process. This clearly illustrates the distorted view estimated performance characteristics can give under the wrong scaling.
Secondly, it is worth noticing the very good proximity of $\eqref{r1}$ to the values obtained through simulation. As we expected, the quality of the approximation deteriorates with increasing values of $s$. This makes sense, because we assumed the system to be in heavy traffic in the derivation of the formulas. What is surprising, on the other hand, is the fact that the approximation performs very well, even though the parameter $b$ is very small for these particular data sets, while the analysis of Theorem \ref{saddlepointThm} assumes that $a$ and $b$ are large. This demonstrates that the approximation scheme is remarkably robust and is able to capture the pre-limit behavior of these types of queues very well.

\section{Conclusion \& future research}
In this chapter, we proposed an adaption to the square-root staffing rule for service systems facing overdispersed demand, using the bulk service queue as a vehicle for our analysis. 
Subsequently, we derive two sets of asymptotic approximations for the scaled steady-state queue length moments for large arrival volumes. 
The first set being based on the resemblance with the maximum of a Gaussian random walk, the second set being derived through a non-standard saddle point method, assuming arrivals follow a Gamma-Poisson mixture. 
Numerical experiments indicated that our approximations capture the pre-limit behavior well under different order of overdispersion, and are robust against any parameter estimation errors. 

Although our method provides a robust way to approximate and dimension queues with overdispersed arrival processes, we see have some interesting directions for future research. 

First, we accentuate that our model is a discrete time queueing model in which a deterministic amount of workload can we handled within each period. 
This approach allowed us to use Pollaczek's formula as a starting point to obtain more refined asymptotic approximations for the performance indicators of the system.
In case we consider queueing models of birth-death-type, such as the $M/M/s$ queue, in the presence of overdispersion demand, different techniques are required to provide derive scaling limits and corresponding capacity allocation rules, see e.g.~\cite{maman}.  
Although we expect that, just as in the novel scaling regimes of Chapter 2, the asymptotic behavior between the bulk service queue and the multi-server queueing models to be similar, this needs proper analysis and understanding. 

Second, empirical work, see e.g. \cite{Avramidis:2004}, shows that in real-life settings, demand in consecutive time periods is often positively correlated, rather than independently distributed as assumed in this chapter. 
This correlation structure obviously alters the queue's dynamics and presumably requires an adaption of the square-root staffing rule as well, making it a worthwhile direction for further analysis.

Last, we have only considered the analysis of the queueing model in steady state. 
Typical service systems however do not face a constant expected arrival rate, nor do they run infinitely long. 
Henceforth, it would be interesting to study the influence of overdispersion on the transient dynamics of the queue and to investigate the capacity allocation problem in scenarios with time-varying demand. 
The theory developed in this chapter may serve as a building block to tackle these more profound questions.


\section*{Appendix}

\addcontentsline{toc}{section}{\hspace{7.1mm} Appendix}

\begin{subappendices}

\settocdepth{chapter}

\section{Proofs of convergence results}
 \label{formalSec}
 
This section presents the details of the proof of Lemma \ref{gaussStep} and Theorem \ref{gaussianThm}, using the random walk perspective of the process $\{Q^{(n)}(k)\}_{k=0}^\infty$. This section is structured as follows. The next two lemmata are necessary for proving the first assertion of Theorem \ref{gaussianThm}, concerning the weak convergence of the scaled process to the maximum of the Gaussian random walk, which is summarized in Proposition \ref{prop6}. The two remaining propositions of this section show convergence of $\hat{Q}^{(n)}$ at the process level as well as in terms of the three characteristics.

Let us first fix some notation:
\begin{equation}
\label{b1}
Y^{(n)}_k := \hat{A}^{(n)}_k-\beta,\quad
S^{(n)}_k = \sum_{i=1}^k Y^{(n)}_i,
\end{equation}
with $S_0^{(n)} = 0$ and $k=1,2,...$. Then \eqref{mm6} can be rewritten as
\begin{equation}
\label{g5a}
 \hat{Q}^{(n)} \equalD \max_{0\leq i \leq k} \Bigl\{{\textstyle \sum}_{i=1}^k Y^{(n)}_i\Bigr\} =: M_\beta^{(n)},
\end{equation}
Last, we introduce the sequence of independent normal random variables $Z_1,Z_2,\ldots$ with mean $\-\beta$ and unit variance 1, and
\begin{equation*}
M_\beta \equalD \max_{k\geq 0} \{{\textstyle \sum}_{i=1}^k Z_i\}
\end{equation*}

\subsection{Proof of Lemma \ref{gaussStep}}
\begin{proof}
We show weak convergence of the random variable $\hat{A}^{(n)}$, as defined in \eqref{b1}, to a standard normal random variable. Since $\hat{\Lambda}_n$ is asymptotically standard normal, its characteristic function converges pointwise to the corresponding limiting characteristic function, i.e.
\begin{equation}
 \label{g8}
 \lim_{n\rightarrow\infty} \phi_{\hat{\Lambda}_n}(t) = \lim_{n\rightarrow \infty} \ee^{-i\mu_nt/\sigma_n}\,\phi_{\Lambda_n}(t/\sigma_n) = \ee^{{-}t^2/2},\qquad \forall t\in \mathbb{R}.
 \end{equation}
Furthermore, by definition of $A^{(n)}$,
\begin{equation*}
\label{g9}
\phi_{A^{(n)}}(t) = \E\left[ \exp(\Lambda_n(\ee^{it}-1))\right] = \phi_{\Lambda_n}\left(-i(\ee^{it}-1)\right),
\end{equation*}
so that
\begin{equation}
\label{g10}
\phi_{\hat{A}_k^{(n)}}(t) = \ee^{-i\mu_nt/\sigma_n}\,\phi_{A_k^{(n)}}(t/\sigma_n) = \ee^{-i\mu_nt/\sigma_n}\phi_{\Lambda_n}\left(-i(\ee^{it/\sigma_n}-1)\right).
\end{equation}
Now fix $t\in\mathbb{R}$. By using
\begin{equation*}
\label{g11}
-i(\e^{it/\sigma_n} - 1) = \frac{t}{\sigma_n} -\frac{it^2}{2\sigma_n^2} + O\left(t^3/\sigma_n^3\right),
\end{equation*}
we expand the last term in \eqref{g10},
\begin{equation*}
\label{g12}
\phi_{\Lambda_n}(t/\sigma_n) + \Bigl(-\frac{i\,t^2}{2\sigma_n^2}+O\left(t^3/\sigma_n^3\right)\Bigr)
\phi_{\Lambda_n}'(t/\sigma_n) + O\Bigl(\Bigl(-\frac{i\,t^2}{2\sigma_n^2}+O\left(\frac{t^3}{\sigma_n^3}\right)\Bigr)^2\phi_{\Lambda_n}''\Big(\frac{t}{\sigma_n}\Big)\Bigr)
\end{equation*}
\begin{equation*}
\label{g13}
= \phi_{\Lambda_n}(t/\sigma_n) - \Bigl(\frac{i\,t^2}{2\sigma_n^2}+O\left(t^3/\sigma_n^3\right)\Bigr)
\phi_{\Lambda_n}'(\zeta)
\end{equation*}
for some $\zeta$ such that $|\zeta - t/\sigma_n| < |i(1-\ee^{it/\sigma_n})-t/\sigma_n|$. Also,
\begin{align}
|\phi_{\Lambda_n}'(u)| &= \left|\frac{\d}{\dd u}\int_{-\infty}^\infty \ee^{iux}\dd F_{\Lambda_n}(x)\right| = \left|\int_{0}^{\infty} ix\,\ee^{iux}\dd F_{\Lambda_n}(x)\right| \nonumber\\
\label{g13a}
&\leq \int_{-\infty}^\infty |ix\,\ee^{iux}|\,\dd F_{\Lambda_n}(x) = \int_0^\infty x\dd F_{\Lambda_n}(x) = \mu_n
\end{align}
for all $u\in\mathbb{R}$. Hence, by substituting \eqref{g10},
\begin{align}
\left| \phi_{\hat{A}_k^{(n)}}(t)-\ee^{-i\mu_nt/\sigma_n}\phi_{\Lambda_n}(t/\sigma_n)\right| &= \left|\ee^{-i\mu_nt/\sigma_n}\,\left(\frac{i\,t^2}{2\sigma_n^2}+O(t^3/\sigma_n^3)\right)\,\phi_{\Lambda_n}'(\zeta)\right|\nonumber\\
& \leq \left(\frac{t^2}{2\sigma_n^2}+O(t^3/\sigma_n^3)\right) |\phi_{\Lambda_n}'(\zeta)|\nonumber\\
& = \frac{\mu_n t^2}{\sigma_n^2} + O\left(\frac{\mu_nt^3}{\sigma_n^3}\right),
\label{g13b}
\end{align}
which tends to zero as $n\rightarrow \infty$ by our assumption that $\mu_n/\sigma_n^2\rightarrow 0$.
Finally,
\begin{equation*}
\label{g13c}
\left| \phi_{\hat{A}_k^{(n)}}(t)-\ee^{-\tfrac12 t^2}\right| \leq \left| \phi_{\hat{A}_k^{(n)}}(t)-\ee^{-i\mu_nt/\sigma_n}\phi_{\Lambda_n}(t/\sigma_n)\right| +
\left| \ee^{-i\mu_nt/\sigma_n}\phi_{\Lambda_n}(t/\sigma_n) - \ee^{-\tfrac12 t^2}\right|,
\end{equation*}
in which both terms go to zero for $n\rightarrow \infty$, by \eqref{g8} and \eqref{g13b}. Hence $\phi_{\hat{A}^{(n)}_k}(t)$ converges to $\ee^{{-}t^2/2}$ for all $t\in\mathbb{R}$, so that we can conclude by L\'evy's continuity theorem that $\hat{A}_k^{(n)} \Rightarrowd \mathcal{N}(0,1)$.
\end{proof}
\subsection{Proof of Theorem \ref{gaussianThm}}
To secure convergence in distribution of $\hat{Q}^{(n)}$ to $M_\beta$, i.e. the maximum of a Gaussian random walk with negative drift, the first assertion of Theorem \ref{gaussianThm}.
 the following property of the sequence $\{Y_k^{(n)}\}_{n\in\mathbb{N}}$ needs to hold.
\begin{lemma}\label{uilemma}
Let $Y^{(n)}_k$ be defined as in \eqref{b1} with $\mu_n,\sigma_n^2 < \infty$ for all $n\in\mathbb{N}$. Then the sequence $\{(Y_k^{(n)})^+\}_{n\in\mathbb{N}}$ is uniform integrable, i.e.
\begin{equation*}
\label{g14}
\lim_{K\rightarrow\infty}\sup_n \E[Y^{(n)\,+}_k|\mathbbm{1}_{\{|Y^{(n)\,+}_k|\geq K\}}] = 0.
\end{equation*}
\end{lemma}
\begin{proof}
Because the sequence $\{Y^{(n)}_k\}_{k\in\mathbb{N}}$ is i.i.d. for all $n$, we  omit the index $k$ in this proof. First, fix $K>0$ and note that
\begin{equation*}
\label{g15}
\E[|Y^{(n)+}|\mathbbm{1}{\{|Y^{(n)\,+}|\geq K\}}] = \E[Y^{(n)+}\mathbbm{1}{\{Y^{(n)+}\geq K\}}] = \E[Y^{(n)}\mathbbm{1}_{\{Y^{(n)}\geq K\}}].
\end{equation*}
This last expression can be bounded from above using the Cauchy-Schwarz inequality, so that
\begin{equation*}
\label{g16}
\E[Y^{(n)}\mathbbm{1}_{\{Y^{(n)}\geq K\}}] \leq \E[ Y^{(n)\,2}]^{1/2}\,\mathbb{P}(Y^{(n)}\geq K)^{1/2}.
\end{equation*}
By the definition of $Y^{(n)}$, we know $\E [Y^{(n)}] = -\beta$ and $\Var Y^{(n)} = \Var A^{(n)} / \sigma_n^2 = 1$. Using this information, we find
\begin{equation*}
   \label{g17}
   \E[Y^{(n)\,2}] = \Var Y^{(n)} + (\E[Y^{(n)}])^2 = 1+\beta^2
   \end{equation*}
   and
   \begin{align*}
   \mathbb{P}(Y^{(n)}\geq K )&=\mathbb{P}(Y^{(n)}+\beta\geq K+\beta) \leq \mathbb{P}(|Y^{(n)}+\beta|\geq K+\beta)\nonumber\\
   &\leq \frac{\Var Y^{(n)}}{(K+\beta)^2} = \frac{1}{(K+\beta)^2},
   \end{align*}
   where we used Chebyshev's inequality for the last upper bound. Therefore,
 \begin{align*}
\lim_{K\rightarrow \infty} \sup_n \E[|Y^{(n)\,+}|\mathbbm{1}_{\{|Y^{(n)\,+}|\geq K\}}] &=
\lim_{K\rightarrow \infty} \sup_n \E[Y^{(n)}\mathbbm{1}_{\{Y^{(n)}\geq K\}}]\nonumber\\
&\leq \lim_{K\rightarrow \infty} \sup_n \E[Y^{(n)\,2}]^{1/2}\,\mathbb{P}(Y^{(n)}\geq K )^{1/2}\nonumber\\
&\leq \lim_{K\rightarrow \infty} \frac{\sqrt{1+\beta^2}}{K+\beta} = 0.
\end{align*}

\end{proof}
By combining the properties proved in Lemma \ref{gaussStep} and \ref{uilemma} with Assumption \ref{as2}, the next result follows directly by \cite[Thm.~X6.1]{Asmussen2003}.
\begin{proposition}\label{maxRWprop}
Let $\hat{Q}^{(n)}$ as in \eqref{g5a}. Then
\begin{equation*}
 \hat{Q}^{(n)}\Rightarrowd M_\beta,\qquad {\rm as}\ n\rightarrow\infty.
\end{equation*}
\end{proposition}


Although Proposition \ref{maxRWprop} tells us that the properly scaled $Q^{(n)}$ converges to a non-degenerate limiting random variable, it does not cover the convergence of its mean, variance and the empty-queue probability. In order to secure convergence of these performance measures as well, we follow the approach similar \cite{Sigman2011b}, using Assumptions \ref{as2} and \ref{as3}.


\begin{proposition}\label{prop6}
Let $\hat{Q}^{(n)}$ as in \eqref{g5a}, $\mu_n,\sigma_n^2 \rightarrow \infty$ such that both $\sigma_n^2/\mu_n\rightarrow \infty$ and $\E[\hat{A}^{(n)3}]$ $<\infty$. Then
\begin{align*}
\label{b16}
\mathbb{P}(\hat{Q}^{(n)}= 0)&\rightarrow \mathbb{P}(M_\beta = 0),\\
\E [\hat{Q}^{(n)}]&\rightarrow \E [M_\beta],\\
\Var \hat{Q}^{(n)}&\rightarrow \Var M_\beta,
\end{align*}
as $n\rightarrow\infty$.
\end{proposition}
\proof
First, we recall that $\hat{Q}^{(n)}\equalD M_\beta^{(n)}$ for all $n\in\mathbb{N}$, so that $\mathbb{P}(\hat{Q}^{(n)} = 0) = \mathbb{P}(M_\beta^{(n)}=0)$, $\E[\hat{Q}^{(n)}]=\E[M_\beta^{(n)}]$ and $\Var\,\hat{Q}^{(n)}=\Var\,M_\beta^{(n)}$ as defined in \eqref{b1}. Our starting point is Spitzer's identity, see \cite[p.~230]{Asmussen2003},
\begin{equation}
\label{b17}
\E[\ee^{it M_\beta^{(n)}}] = \exp\Bigl( \sum_{k=1}^\infty \frac{1}{k} (\E[\ee^{it(S^{(n)}_k)^+}]-1)\Bigr),
\end{equation}
with $S^{(n)}_k$ as in \eqref{b1}, and $M_\beta^{(n)}$ the all-time maximum of the associated random walk. Simple manipulations of \eqref{b17} give
\begin{align}
\label{y1}
{\rm ln}\,\mathbb{P}(M_\beta^{(n)} = 0) &=  -\sum_{k=1}^\infty \frac{1}{k}\,\mathbb{P}(S^{(n)}_k > 0),\\
\label{y2}
\E[M_\beta^{(n)}] &= \sum_{k=1}^\infty \frac{1}{k} \E[S^{(n)\,+}_k] = \sum_{k=1}^\infty \frac{1}{k}\int_0^\infty \mathbb{P}(S^{(n)}_k > x) \dd x,\\
\label{y3}
\Var M_\beta^{(n)} &= \sum_{k=1}^\infty \frac{1}{k} \E[(S^{(n)\,+}_k)^2] =\sum_{k=1}^\infty \frac{1}{k}\int_0^\infty \mathbb{P}(S^{(n)}_k > \sqrt{x}) \dd x.
\end{align}
By Lemma \ref{gaussStep}, we know
\begin{equation*}
\label{y4}
\mathbb{P}(S^{(n)}_k > y) = \mathbb{P}\left( {\sum_{i=1}^k} Y^{(n)}_i > y \right) \rightarrow \mathbb{P}\left({\textstyle\sum_{i=1}^k} Z(i) > y\right),
\end{equation*}
for $n\rightarrow \infty$, where the $Z(i)$'s are independent and identically normally distributed with mean $-\beta$ and variance 1.
Because equivalent expressions to \eqref{y1}-\eqref{y3} apply to the limiting Gaussian random walk, it is sufficient to show that the sums converge uniformly in $n$, so that we can apply dominated convergence to prove the result.

We start with the empty-queue probability. To justify interchangeability of the infinite sum and limit, note
\begin{equation*}
\label{y5}
 \mathbb{P}(S^{(n)}_k > 0) \leq  \mathbb{P}(|S^{(n)}_k+k\beta| > k\beta )\leq \frac{k}{\beta^2k^2} = \frac{1}{\beta^2k},
 \end{equation*}
where we used that $\E[ S^{(n)}_k] = k\E [Y^{(n)}(1)] = -k\beta$ and $\Var S^{(n)}_k = k$ and apply Chebychev's inequality, so that
\begin{equation*}
\label{y6}
\sum_{k=1}^\infty \frac{1}{k}\mathbb{P}(S^{(n)}_k > 0) \leq \sum_{k=1}^\infty \frac{1}{\beta^2 k^2} < \infty, \qquad \forall n\in\mathbb{N}.
\end{equation*}
Hence,
\begin{align*}
\lim_{n\rightarrow\infty} {\rm ln}\,\mathbb{P}(\hat{Q}^{(n)}= 0) &= \lim_{n\rightarrow\infty}  - \sum_{k=1}^\infty \frac{1}{k}\mathbb{P}(S^{(n)}_k > 0) = -\sum_{k=1}^\infty \frac{1}{k} \lim_{n\rightarrow\infty}\mathbb{P}(S^{(n)}_k > 0)\nonumber\\
&= -\sum_{k=1}^\infty \frac{1}{k} \mathbb{P}({\textstyle\sum_{i=1}^k} Z(i) > 0) = {\rm ln}\,\mathbb{P}(M_\beta = 0),
\end{align*}
Finding a suitable upper bound on $\frac{1}{k}\int_0^\infty \mathbb{P}(\hat{Q}^{(n)}>x) dx$ and $\frac{1}{k}\int_0^\infty \mathbb{P}(\hat{Q}^{(n)}>\sqrt{x}) \dd x$ requires a bit more work. We initially focus on the former, the latter follows easily. The following inequality from \cite{Nagaev1979} proves to be very useful:
\begin{equation}
\label{y8}
\mathbb{P}(\bar{S}(k)>y) \leq C_r\,\Bigl(\frac{k\,\sigma^2}{y^2}\Bigr)^2 + k\,\mathbb{P}(X>y/r),
\end{equation}
where $\bar{S}(k)$ is the sum of $k$ i.i.d. random variables distributed as $X$, with $\E[X] = 0$ and $\Var\, X=\sigma^2$, $y > 0$, $r>0$ and $C_r$ a constant only depending on $r$. We take $r=3$ for brevity in the remainder of the proof, although any $r>2$ will suffice. We  analyze the integral in two parts, one for the interval $(0,k)$ and one for $[k,\infty)$. For the first part, we have
\begin{align}
\label{y9}
\int_0^k\mathbb{P}(S^{(n)}_k>x) \dd x &=\int_0^k \mathbb{P}({\textstyle \sum_{i=1}^\infty}\hat{A}^{(n)}_i > x+k\beta)dx\, \leq\, \int_0^k \mathbb{P}({\textstyle \sum_{i=1}^\infty}\hat{A}^{(n)}_i > k\beta)\dd x  \nonumber\\
&= k\,\mathbb{P}({\textstyle \sum_{i=1}^k }\hat{A}^{(n)}_i >  k\beta) \,\leq\, \frac{C_3}{k^2\beta^6} + k^2\mathbb{P}(\hat{A}^{(n)}(1)> \tfrac{1}{3}k),
\end{align}
where we used \eqref{y8} in the last inequality. 
Hence,
\begin{align}
\label{y10}
\sum_{k=1}^\infty\frac{1}{k}\, \int_0^k \mathbb{P}(S^{(n)}_k>x)\dd x &\leq \, \frac{C_3}{\beta^6}\sum_{k=1}^\infty k^{-3} +\sum_{k=1}^\infty k\,\mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}k) \nonumber \\
&\leq C_1^*+\sum_{k=1}^\infty k\,\mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}k).
\end{align}
With the help of the inequality (see \cite{Sigman2011b}),
\begin{equation}
\label{y11}
(b-a)a\,\mathbb{P}(X>b) \leq \int_a^b x\,\mathbb{P}(X>x) \dd x \qquad \forall 0<a<b,
\end{equation}
we get by taking $a=(k-1)/3$ and $b=k/3$,
\begin{align}
\label{y12}
k\,\mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}k) &\leq \frac{9\,k}{k-1}\int_{(k-1)/3}^{k/3} x\,\mathbb{P}(\hat{A}^{(n)}(1)>x) \dd x \nonumber \\
&\leq 18\int_{(k-1)/3}^{k/3} x\,\mathbb{P}(\hat{A}^{(n)}(1)>x) \dd x,
\end{align}
for $k\geq 2$. Since the tail probability for $k=1$ is obviously bounded by 1, this yields
\begin{align}
\label{y13}
\sum_{k=1}^\infty k\,\mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}k) &\leq 1+18\sum_{k=2}^\infty\int_{(k-1)/3}^{k/3} x\,\mathbb{P}(\hat{A}^{(n)}(1)>x) \dd x\nonumber\\
&\leq 1+ \int_{0}^{\infty} x\,\mathbb{P}(\hat{A}^{(n)}(1)>x)\dd x  \leq 1+\E[\hat{A}^{(n)}(1)^2] < \infty,
\end{align}
since $\hat{A}^{(n)}(1)$ has finite variance by assumption. This completes the integral over the first interval. For the second part, we use \eqref{y8} again to find
\begin{align}
\label{y14}
\int_k^\infty \mathbb{P}(S^{(n)}_k>x)dx &=\int_k^\infty \mathbb{P}({\textstyle \sum_{i=1}^\infty}\hat{A}^{(n)}_i > x+k\beta)dx \leq \int_k^\infty \mathbb{P}({\textstyle \sum_{i=1}^\infty}\hat{A}^{(n)}_i > x)\dd x\nonumber \\
&\leq C_3\int_k^\infty \frac{k^2}{x^6} dx + k\int_k^\infty \mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}x)\dd x\nonumber \\
&=  \frac{5 C_3}{k^3}+ k\int_k^\infty \mathbb{P}(\hat{A}^{(n)}_i>\tfrac{1}{3}x) \dd x.
\end{align}
So,
\begin{equation}
\label{y15}
\sum_{k=1}^\infty \frac{1}{k} \int_k^\infty \mathbb{P}(S^{(n)}_k>x)dx \leq C_2^* + \sum_{k=1}^\infty \int_k^\infty \mathbb{P}(\hat{A}^{(n)}_i>\tfrac{1}{3}x) \dd x,
\end{equation}
for some constant $C_2^*$. Last, we are able to upper bound the second term in \eqref{y15} by Tonelli's theorem:
\begin{align}
\sum_{k=1}^\infty \int_k^\infty \mathbb{P}(\hat{A}^{(n)}_i>\tfrac{1}{3}x) dx &\leq \int_1^\infty x\mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}x) \dd x \nonumber\\
\label{y16}
&\leq 9\int_0^\infty y\mathbb{P}(\hat{A}^{(n)}(1)>y) dy = 9\E[\hat{A}^{(n)}(1)^2] < \infty.
\end{align}
Combining the results in \eqref{y10}, \eqref{y13}, \eqref{y15} and \eqref{y16}, we find
\begin{equation*}
\label{y17}
\sum_{k=1}^\infty \frac{1}{k} \int_0^\infty \mathbb{P}(S^{(n)}_k>x)\dd x < \infty,
\end{equation*}
and thus
\begin{align*}
\lim_{n\rightarrow\infty} \E[\hat{Q}^{(n)}] &= \lim_{n\rightarrow\infty}  \sum_{k=1}^\infty \frac{1}{k}\int_0^\infty \mathbb{P}(S^{(n)}_k > x)\dd x \nonumber\\
&= \sum_{k=1}^\infty \frac{1}{k} \int_0^\infty\mathbb{P}({\textstyle\sum_{i=1}^k} Z(i) > x)\dd x = \E [M_\beta].
\end{align*}
Finally, we show how the proof changes for the convergence of $\Var \hat{Q}^{(n)}$. The expressions for $\E [\hat{Q}^{(n)}]$ and $\Var \hat{Q}^{(n)}$ in \eqref{y1} and \eqref{y2} only differ in the term $\sqrt{x}$. Hence only minor modifications are needed to also prove convergence of the variance. Note that boundedness of the integral over the interval $(0,k)$ in \eqref{y9}-\eqref{y13} remains to hold when substituting $\sqrt{x}$ for $x$. \eqref{y14} changes into
\begin{align*}
\label{y18}
\int_k^\infty \mathbb{P}(S^{(n)}_k>\sqrt{x})dx &=\int_k^\infty \mathbb{P}({\textstyle \sum_{i=1}^\infty}\hat{A}^{(n)}_i > \sqrt{x}+k\beta)\dd x \nonumber \\
&\leq C_3\int_k^\infty \frac{k^2}{(\sqrt{x}+k\beta)^6} dx + k\,\int_k^\infty \mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}\sqrt{x}) \dd x \nonumber\\
&\leq \frac{C_4^*}{k}+ k\,\int_k^\infty \mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}\sqrt{x}) \dd x,
\end{align*}
for some constant $C_4^*$, so that
\begin{equation*}
\sum_{k=1}^\infty \frac{1}{k} \int_k^\infty \mathbb{P}(S^{(n)}_k>\sqrt{x})\dd x \leq C_4^* + \sum_{k=1}^\infty \int_k^\infty \mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}\sqrt{x}) \dd x.
\end{equation*}
Lastly, we have
\begin{align*}
\sum_{k=1}^\infty \int_k^\infty \mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}\sqrt{x}) \dd x &\leq \int_1^\infty x\mathbb{P}(\hat{A}^{(n)}(1)>\tfrac{1}{3}\sqrt{x}) \dd x \nonumber\\
\label{y17a}
&\leq 18\int_0^\infty y^2\mathbb{P}(\hat{A}^{(n)}(1)>y) \dd y = 18\E[\hat{A}^{(n)}(1)^3] < \infty.
\end{align*}
Therefore the sum describing the variance is also uniformly convergent in $n$, so that interchanging of infinite sum and limit is permitted and
\begin{align*}
\lim_{n\rightarrow\infty} \Var\,\hat{Q}^{(n)} &= \lim_{n\rightarrow\infty}  \sum_{k=1}^\infty \frac{1}{k}\int_0^\infty \mathbb{P}(S^{(n)}_k > \sqrt{x})\dd x \nonumber \\
&= \sum_{k=1}^\infty \frac{1}{k} \int_0^\infty\mathbb{P}({\textstyle\sum_{i=1}^k} Z(i) > \sqrt{x})\dd x = \Var M_\beta.
\end{align*}


\section{Numerical procedures}\label{numprocs}
An alternative characterization of the stationary distribution is based on the analysis in \cite{Boudreau1962} and considers a factorization in terms of (complex) roots:
\begin{equation*}
\label{t9}
Q^{(n)}(w) = \frac{(s_n-\E [A^{(n)}])(w-1)}{w^{s_n}-\tilde{A}^{(n)}(w)}\,\prod_{k=1}^{s_n-1} \frac{w-z^n_k}{1-z^n_k},
\end{equation*}
where $z_1^n,z_2^n...,z_{s_n-1}^n$ are the $s_n-1$ zeros of $z^{s_n}-\tilde{A}^{(n)}(z)$, in $|z|<1$, yielding
\begin{equation*}
\label{c2}
\mu_Q  = \frac{\sigma_n^2}{2(s_n-\mu_n)}-\frac{s_n-1+\mu_n}{2} + \sum_{k-1}^{s_n-1} \frac{1}{1-z^n_k},
\end{equation*}
\begin{equation*}
\label{c3}
\mathbb{P}(Q^{(n)}=0) = \frac{s_n-\mu_A}{\tilde{A}^{(n)}(0)}\prod_{k=1}^{s-1}\frac{z^n_k}{z^n_k-1},
\end{equation*}
which for our choice of $\tilde{A}^{(n)}(z)$ becomes
\begin{equation*}
\label{c4}
\mu_Q = \frac{a_nb_n(b_n+1)}{2\beta\sqrt{a_n}b_n}-\frac{2a_nb_n+\beta\sqrt{a_nb_n(b_n+1)}-1}{2}+\sum_{k=1}^{s_n-1} \frac{1}{1-z^n_k},
\end{equation*}
\begin{equation*}
\label{c5}
\mathbb{P}(Q^{(n)}=0) = \beta \sqrt{a_nb_n(b_n+1)}(1+b_n)^{a_n}\prod_{k=1}^{s_n-1} \frac{z^n_k}{z^n_k-1}.
\end{equation*}
where $z_1,...,z_{s_n-1}$ denote the zeros of $z^{s_n} - \tilde{A}^{(n)}(z)$ in $|z|<1$. A robust numerical procedure to obtain these zeros is essential for a base of comparison. We  discuss two methods that fit these requirements. The first follows directly from \cite{Janssen2005}. \\
\begin{lemma}\label{fixedIterLemma}
Define the iteration scheme
\begin{equation}
\label{c6}
z_k^{n,l+1} = w^n_k [\tilde{A}^{(n)}(z_k^{n,l})]^{1/s_n},
\end{equation}
with $w^n_k = \ee^{2\pi ik/s_n}$ and $z_k^{n,0}=0$ for $k=0,1,\ldots,s_{n-1}$. Then $z_k^{n,l} \rightarrow z_k^n$ for all $k=0,1,...,s_n-1$ for $l\rightarrow \infty$.
\end{lemma}

\begin{proof}
The successive substitution scheme given in \eqref{c6} is the fixed point iteration scheme described in \cite{Janssen2005}, applied to the pgf of our arrival process. The authors show that, under the assumption of $\tilde{A}^{(n)}(z)$ being zero-free within $|z|\leq 1$, the zeros can be approximated arbitrarily closely, given that the function $[\tilde{A}^{(n)}(z)]^{1/s_n}$ is a contraction for $|z|\leq 1$, i.e.
\begin{equation*}
\label{c7}
\Bigl|\frac{\dd}{\dd z}[\tilde{A}^{(n)}(z)]^{1/s_n}\Bigr| < 1.
\end{equation*}
In our case,
\begin{align}
\label{c8}
\Bigl|\frac{\dd}{\dd z}[\tilde{A}^{(n)}(z)]^{1/s_n}\Bigr| = \Bigl|\frac{\dd}{\dd z}\left(1+(1-z)b_n\right)^{-a_n/s_n}\Bigr| = \frac{a_nb_n}{s_n}\Bigl|1+(1-z)b_n\Bigr|^{-a_n/s_n-1},
\end{align}
where $a_nb_n/s_n = \rho_n$ is close to, but less than 1 and
\begin{align*}
\label{c9}
|1+(1-z)b_n| \geq |1+b_n|-|z|b_n = 1+(1-|z|)b_n \geq 1,
\end{align*}
when $|z|\leq 1$. Hence the expression in \eqref{c8} is less than 1 for all $|z|\leq 1$. Evidently, $\tilde{A}^{(n)}(z)$ is also zero-free in $|z|\leq 1$. Thus \cite[Lemma~3.8]{Janssen2005} shows that $z_k^{n,l}$ as in \eqref{c6} converges to the desired roots $z^n_k$ for all $k$ as $l$ tends to infinity.
\end{proof}

\begin{remark}
The asymptotic convergence rate of the iteration in \eqref{c6} equals \\
\noindent $\frac{\dd}{\dd z}[\tilde{A}^{(n)}(z)]^{1/s_n}$ evaluated at $z=z_k^n$. Hence, convergence is slow for zeros near 1 and fast for zeros away from 1.
\end{remark}

A different approach is based on the B\"urmann-Lagrange inversion formula.
\begin{lemma}\label{BLLemma}
Let $w^n_k = e^{2\pi ik/s_n}$ and $\alpha_n = a_n/s_n$. Then the zeros of $z^{s_n}-\tilde{A}^{(n)}(z)$ are given by
\begin{equation*}
z_k^n = \sum_{l=1}^\infty \frac{1}{l!}\,\frac{\beta[l\alpha_n+l-1)}{\beta(l\alpha_n)}\,\frac{b_n+1}{b_n}\Bigl(\frac{b_n}{(b_n+1)^{\alpha_n+1}}\Bigr)^l (w_k^n)^l,
\end{equation*}
for $k=0,1,...,s_n-1$.
\end{lemma}

\begin{proof}
Note that we are looking for $z$'s that solve
\begin{equation*}
\label{c10}
z\,[\tilde{A}^{(n)}(z)]^{-1/s_n} = z\left(1+(1-z)b_n\right)^{a_n/s_n} = w,
\end{equation*}
where $w = w_k = \ee^{2\pi i k/s_n}$. The B\"urmann-Lagrange formula for $z=z(w)$, as can be found in \cite[Sec.~2.2]{debruijn} for $z=z(w)$ is given by
\begin{align*}
z(w) &= \sum_{l=1}^\infty \frac{1}{l!}\,\left(\frac{\dd}{\dd z}\right)^{l-1}\left[\left(\frac{z}{z(1+(1-z)b_n)^{a_n/s_n}}\right)^l\right]_{z=0}\,w^l\nonumber\\
\label{c11}
&= \sum_{l=1}^\infty \frac{1}{l!}\,\left(\frac{\dd}{\dd z}\right)^{l-1}\left[\left(1+(1-z)b_n)^{-l\,a_n/s_n}\right)\right]_{z=0}\,w^l.
\end{align*}
Set $\alpha_n = a_n/s_n$. We compute
\begin{equation*}
\label{c1}
\left(\frac{\dd}{\dd z}\right)^{l-1}\left[ (1+(1-z)b_n)^{-l\alpha_n}\right]_{z=0} = \frac{\beta(l\alpha_n+l-1)}{\beta(l\alpha_n)}\,\frac{1+b_n}{b_n}\,\left(\frac{b_n}{(1+b_n)^{\alpha_n+1}}\right)^l.
\end{equation*}
With $c_n = b_n/(1+b_n)^{\alpha_n+1}$ and $d_n = (1+b_n)/b_n$, we thus have
\begin{equation*}
\label{c13}
z(w) = d_n\,\sum_{l=1}^\infty \frac{\beta(l\alpha_n+l-1)}{\beta(l+1)\beta(l\alpha_n)} c_n^l\,w^l.
\end{equation*}
By Stirling's formula
\begin{equation*}\label{c14}
\frac{\beta(l\alpha_n+l-1)}{\beta(l+1)\beta(l\alpha_n)}  = \frac{D}{l\sqrt{l}}\left(\frac{(\alpha_n+1)^{\alpha_n+1}}{\alpha_n^{\alpha_n}}\right)^l,
\end{equation*}
where $D=\alpha_n^{1/2}(\alpha_n+1)^{-3/2}(2\pi)^{-1/2}$. Now,
\begin{equation*}
\label{c15}
\frac{(\alpha_n+1)^{\alpha_n+1}}{\alpha_n^{\alpha_n}}\, c_n = \frac{(\alpha_n+1)^{\alpha_n+1}}{\alpha_n^{\alpha_n}}\cdot \frac{b_n}{(1+b_n)^{\alpha_n+1}} = \left(\frac{b_n+\rho_n}{b_n+1}\right)^{\rho_n/b_n + 1}\left(\frac{1}{\rho_n}\right)^{\rho_n/b_n}.
\end{equation*}
This determines the radius of convergence $r_{\rm BL}$ of the above series for $z(w)$:
\begin{equation}
\label{c16}
\frac{1}{r_{\rm BL}} := \left(\frac{b_n+\rho_n}{b_n+1}\right)^{\rho_n/b_n + 1}\left(\frac{1}{\rho_n}\right)^{\rho_n/b_n}.
\end{equation}
The derivative with respect to $\rho_n$ of the quantity
\begin{equation}
\label{c17}
\left(1+\frac{\rho_n}{b_n}\right) {\rm ln }\left(\frac{b_n+\rho_n}{b_n+1}\right)+\frac{\rho_n}{b_n}\,{\rm ln}\left(\frac{1}{\rho_n}\right)
\end{equation}
is given by
\begin{equation*}
\label{c18}
\frac{1}{b_n}{\rm ln }\Bigl(\frac{b_n+\rho_n}{b_n\rho_n+\rho_n}\Bigr) > 0
\end{equation*}
for $0<\rho_n<1$ and $b_n>0$. Furthermore, the quantity in \eqref{c17} vanishes at $\rho_n=1$ and is therefore negative for $0<\rho_n<1$ and $b_n>0$.
\begin{remark}
The formula for the radius of convergence in \eqref{c16} clearly shows the decremental effect of both having a large $b_n$ and or having $\rho_n$ close to 1. The quantities $\beta(l\alpha+l-1)/(\beta(l+1)\beta(l\alpha))$ in the power series for $z(w)$ are not very convenient for recursive computation, although normally $\alpha = a_n/s_n$ is a rational number.\end{remark}
\end{proof}

\section{Statistical procedures}\label{statproc}
To calibrate our model to real data, we now discuss some statistical procedures to show the presence of overdispersion and to estimate the parameters of the mixed Gamma-Poisson distribution. Let $x_1,...,x_n$ denote the observed number of arrivals in consecutive time slots. These observations can be interpreted as realizations of the random variables $A_1,...,A_N$, and
 \begin{equation*}
\bar{a}_N=\frac{1}{N}\sum_{i=1}^N x_i, \qquad \bar{s}_N^2 = \frac{1}{N-1}\sum_{i=1}(x_i-\bar{x}_i)^2,
\end{equation*}
the sample mean and variance with equivalent random variables $\bar{A}_N$ and $S_N^2$, respectively. Several tests with null hypothesis that $x_1,...,x_N$ originate from a (constant rate) Poisson distribution were discussed by \cite{Brown2002}. We  mention two of them. The first is frequently referred to as the \emph{dispersion test}, and is based on the test statistic
\begin{equation*}
\label{dispTest}
D_N = \frac{(N-1)S_N^2}{\bar{A}_N},
\end{equation*}
which is approximately chi-squared distributed with $N-1$ degrees of freedom. When using a significance level $\alpha$, the critical value is equal to the $(1-\alpha)$-th quantile of chi-squared distribution $\chi^2_{N-1,1-\alpha}$. The second test, which is also used in \cite{koolejongbloed}, involves the test statistic
\begin{equation*}
\label{NStest}
T_N = \sqrt{N/2}\,\Bigl(\frac{S_N^2}{\bar{A}_N}-1\Bigr),
\end{equation*}
which is known as the Neyman-Scott test statistic. Under the null hypothesis $T_N$ tends to a standard normal random variable for large $N$. Hence both test statistics rely on the ratio of the sample variance and sample mean, which should be 1 if $A_1,...,A_N$ are indeed i.i.d. Poisson distributed. Excessive values of $D_N$ and $T_N$ therefore raise the suspicion of overdispersed arrivals.

Once either (or both) of the Poisson tests rejects the hypothesis of arrivals originating from a unicomponent Poisson process, we fit the data to the Gamma-Poisson mixture. Note that if we assume $A_i$ to be distributed as a Poisson random variable with random rate $\Lambda_i$, which is in turn Gamma distributed with parameters $a$ and $1/b$, then $A_i$ is in fact a negative binomial random variable with parameters $r = a$ and $p=b/(b+1)$. Finding estimators $\hat{a}$ and $\hat{b}$ therefore is equivalent to fitting a negative binomial distribution to the data to obtain $\hat{r}$ and $\hat{p}$, followed by retrieving $\hat{a} = \hat{r}$ and $\hat{b} = \hat{p}/(1-\hat{p})$. We proceed by applying the maximum likelihood estimation method described in \cite{koolejongbloed} to find $\hat{r}$ and $\hat{p}$. This method prescribes to set $\hat{r}$ to be the value of $r$ for which the \emph{profile loglikelihood function} defined by
\begin{equation*}
L(r) = \frac{1}{N}\,\sum_{i=1}^N\sum_{j=1}^{a_i} {\rm ln}(r+j+1)+r\,{\rm ln}\,r -(r+\bar{a}_N)\,{\rm ln}(r+\bar{a}_N),
\end{equation*}
is attained. Subsequently, $\hat{p} = \hat{r}/(\hat{r}+\bar{a}_N)$, so that $\hat{a} = \hat{r}$ and $\hat{b} = \hat{r}/\bar{a}_N$.

Finally, given the estimators $\hat{a}$ and $\hat{b}$, we need statistical evidence that the obtained Poisson mixture indeed fits the data reasonably well. Here we again cite \cite{koolejongbloed}, who give a method to retrieve the $p$-value for the goodness-of-fit based on bootstrap and Monte-Carlo simulation. In our experiments, we work with $10^6$ replications of the Monte-Carlo simulation to obtain the approximated $p$-value. We refer to the appendix of \cite{koolejongbloed} for further details on this method.

\resettocdepth 

\end{subappendices}


==> Chapter_5/Chapter_5i.tex <==

\chapter{Finite-size effects in critically dimensioned emergency departments}

\begin{chapterstart}
Motivated by health care systems with repeated services that have both personnel (nurse/physician) and space (beds) constraints, we study a restricted version of the Erlang-R model. The space restriction policies we account for are blocking or holding in a pre-entrant queue. We develop many-server approximations for the system performance measures when either policy applies, and explore the connection between them.
We show that capacity allocation of both resources should be determined simultaneously, and derive the methodology to determine it explicitly.
 We show that the system dynamics is captured by the fraction of needy time in the network, and that returning patients should be accounted for both in steady-state and time-varying conditions.
 We demonstrate the application of our policies in two case-studies of resource allocation in hospitals.
\end{chapterstart}

\begin{flushright}
Based on\\
\textbf{Finite-size effects in critically dimensioned emergency departments}\\
\textit{Johan van Leeuwaarden, Britt Mathijsen, Fiona Sloothaak \& Galit Yom-Tov}\\
Submitted to \textit{Operations Research}
\end{flushright}
\newpage

\section{Introduction}

In recent years, operations research techniques have received increased interest from the health care community, as they are able to design and improve workflow processes in health care facilities~\cite{Armony2015,Green2008,Bekker2009b,Hall2006,Hall2012}. 
Because these processes are typically stochastic in nature, it is common practice to use queueing theory for performance analyses and workforce planning. 
As a first step towards understanding the processes going on in health care environments, systems are commonly modeled after a single station queue, such as the $M/M/s$ (Erlang-C), $M/M/s/s$ (Erlang-B) or $M/M/s+M$ (Erlang-A) models, and fluid and diffusion approximations are used to provide insights into the process dynamics. 
However, simple single station models often fail to capture the more intricate dynamics of the settings specific to health care contexts. 
Prime examples include the flows of patients in a hospital from one medical ward to another \citep{Armony2015}, within the Emergency Department (ED) between different stages of treatment \citep{Junfei2015}, or between medical facilities \citep{zychlinski2016bedblocking}.  %through the system is typically more accurately modeled by a more involved queueing \text{network}~
Queueing networks can capture the dependency between several service stages and several types of resources. 
More specifically, we are interested in the ubiquitous feature, particularly present in health care environments, that patients during their stay in the system might require a specific resource multiple times, e.g.~physicians and nurses who treat patients several times during their stay in the medical wards \citep{Jennings2011} or the ED \citep{YomTov2014}, while multiple resources types are limited (e.g.\ medical staff and beds).
In this chapter, we concentrate on the dynamics within EDs. 

An often ignored yet essential feature of medical facilities concerns the restriction of the number of patients that can reside in the facility simultaneously. 
In Chapter 4, we already observed that finite-size restrictions can have a significant effect on the performance of queueing systems. 
In this chapter, we investigate the influence of such multiple restrictions on the network dynamics and the required staffing policies in the context of an ED. \\
\\*
\noindent
\textbf{The restricted Erlang-R model.}
The canonical model for service networks with returns is the Erlang-R model \citep{YomTov2014} in which customers, during their stay in the system receive a random number of services from the same pool of servers. 
Yom-Tov \& Mandelbaum \cite{YomTov2014} showed that such a simple network model can be used to determine staffing in an ED both in stable and time-varying conditions. 
Nevertheless, empirical studies report that some countries, such as the US, use a different operational mode that applies strict restrictions on entering the ED \citep{EDexperiment}. 
In typical US EDs, a patient will not enter the ED until both a bed and a physician are available to treat her. 
Those restrictions can be either physical (beds) restrictions or managerial ones --- for instance by imposing a patient-to-physician ratio.
In this work, we extend the Erlang-R model by enforcing a constraint on the maximum number of available places inside the facility. 
Our model hence incorporates two kinds of resource constraints: servers that provide the actual service and the maximum available places inside the service system. 
Both affect the system in a highly interdependent way. 
The model, presented in Figure \ref{fig:Erlang_R_model}, assumes $s$ servers and a maximum capacity of $n$ concurrent places. 
We assume that patients arrive according to a Poisson process with rate $\lambda$. 
In case a new arrival finds $n$ or more patients already present, we consider two options: either she waits outside the service facility in a holding queue until a vacant space becomes available (Figure \ref{fig:Erlang_R_holding}) or she is blocked (Figure \ref{fig:Erlang_R_blocking}), such as is the case when patients are sent to an alternative facility. 
Once a patient is admitted, she requires assistance from one of the $s$ servers for an exponentially distributed duration with mean $1/\mu$. 
Then, with probability $1-p$, the patient leaves the system or, with probability $p$, returns to service again after an exponentially distributed time with mean $1/\delta$. 
Following Jenning \& de V\'ericourt \cite{Jennings2011} and Yom-Tov  \& Mandelbaum \cite{YomTov2014}, we call patients {\it needy} when they require attention from one of the servers and {\it content} when they are in the delayed return phase. 
In addition, we call patients {\it holding} when they are waiting outside the facility for an available space. We assume that the arrival process, the needy times and content times are mutually independent. 
In the holding queue and the needy queue, we apply the First-Come-First-Served (FCFS) discipline.

\begin{figure} 
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale = 0.55]
\footnotesize
\draw [thick, ->] (-2.75,4.5) -- (-1.25,4.5);
\draw [thick] (-1.5,5) -- (0,5) -- (0,4) -- (-1.5,4);
\draw [thick] (-0.25,4) -- (-0.25,5);
\draw [thick] (-0.5,4) -- (-0.5,5);
\draw [thick] (-0.75,4) -- (-0.75,5);
\draw [thick, ->] (0,4.5) -- (2.5,4.5);
\draw [thick] (2.25,5) -- (3.75,5) -- (3.75,4) -- (2.25,4);
\draw [thick] (3,4) -- (3,5);
\draw [thick] (3.25,4) -- (3.25,5);
\draw [thick] (3.5,4) -- (3.5,5); 
\draw [thick] (4.25,4.5) circle [radius=0.5] node {$s$} node[below= 0.3 cm] {needy} node[above=0.25cm] {$\exp(\mu)$};
\draw [thick,->] (4.75,4.5) -- (7.75,4.5);
\draw [thick,->] (5.75,4.5) -- (5.75,2) -- (4,2);
\draw [thick] (3.5,2) circle [radius=0.5] node {$\infty$} node[below=0.3cm] {content} node[above=0.25cm] {$\exp(\delta)$};
\draw [thick,->] (3,2) -- (1.5,2) -- (1.5,4.5);
\node [above] at (-1.5,2.9) {\footnotesize Pois($\lambda$)};
\node [below] at (5.5,2) {\footnotesize $p$};
\node [above] at (6.25,4.5) {\footnotesize $1-p$};
\draw [thick, dashed] (0.5,0.75) rectangle (7,5.9) node[right] {\footnotesize $n$}; 
\node [above] at (-0.75,5) {\footnotesize holding};
\end{tikzpicture}
\caption{Erlang-R model with holding.}
\label{fig:Erlang_R_holding}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.55]
\footnotesize
\draw [thick, ->] (-1.5,4.5) -- (2.5,4.5);
\draw [thick, ->] (0,4.5) -- (0,2.5) node[below left] {blocked};
\draw [thick] (2.25,5) -- (3.75,5) -- (3.75,4) -- (2.25,4);
\draw [thick] (3,4) -- (3,5);
\draw [thick] (3.25,4) -- (3.25,5);
\draw [thick] (3.5,4) -- (3.5,5); 
\draw [thick] (4.25,4.5) circle [radius=0.5] node {$s$} node[below= 0.3 cm] {needy} node[above=0.25cm] {$\exp(\mu)$};
\draw [thick, ->] (4.75,4.5) -- (7.75,4.5);
\draw [thick,->] (5.75,4.5) -- (5.75,2) -- (4,2);
\draw [thick] (3.5,2) circle [radius=0.5] node {$\infty$} node[below=0.3cm] {content} node[above=0.25cm] {$\exp(\delta)$};
\draw [thick,->] (3,2) -- (1.5,2) -- (1.5,4.5);
\node [above] at (-1.5,3.4) {\footnotesize Pois($\lambda$)};
\node [below] at (5.5,2) {\footnotesize $p$};
\node [above] at (6.25,4.5) {\footnotesize $1-p$};
\draw [thick, dashed] (0.5,0.75) rectangle (7,5.9) node[right] {\footnotesize $n$};
\end{tikzpicture}
\caption{Erlang-R model with blocking.}
\label{fig:Erlang_R_blocking}
\end{subfigure}
\caption{Restricted Erlang-R models with maximally $n$ customers in system.}
\label{fig:Erlang_R_model}
\end{figure}

As mentioned, we consider two versions of the finite-capacity constraint. 
The first version is called \emph{Erlang-R with holding}, in which patients wait for an available space in the system. 
The second version is called \emph{Erlang-R with blocking}, in which patients meeting a full system are blocked.
Naturally, intermediate scenarios can be constructed in which a proportion of the total arrival volume of patients indeed leaves upon finding a full system, while the rest joins the holding queue. 
While this chapter focuses on the two extreme cases, straightforward adaptions can fit these intermediate scenarios. \\
\\*
\noindent
\textbf{Examples of restricted Erlang-R.}
As noted before, an ED operated in the US can be modeled using a restricted Erlang-R model. Another health care example is medical units (MUs) in a hospital.
Such units specialize in specific types of illnesses (cadriatric, oncology, etc.) and have limited resources such as nurses and beds. If the unit is full, new patients are either allocated to an alternative medical unit, i.e.\ blocked, or wait for an available bed. 
Both policies are problematic in terms of quality-of-care, because the personnel in the alternative unit (or the ED) may be less knowledgeable about the patient's medical condition and waiting in the ED was shown to increase mortality.
Moreover, ED waiting may reduce available capacity for treating ED patients \citep{Carmen2016,israelit}, hence endangering both the delayed patient as well as others. Both the number of personnel (nurses and physicians) and the number of beds impact service dynamics and quality-of-care. Research so far looked at the capacity allocation of those resources separately. Green \& Yankovic \cite{GY2011} and Jennings \& de V\'ericourt \cite{Jennings2008} looked at nurse staffing in medical units, while de Bruin et al.~\cite{Bekker2009b} looked into bed allocation. The unified model we suggest enables us to capture the dependency between those two decisions, and its impact on other medical units in the hospital.
At the same time, we capture the two most commonly used modes of operation --- blocking and holding of new patients.  \\
\\*
\noindent
\textbf{Two-fold square-root staffing rule.}
Our main goal is to provide staffing policies for the ED that ensures high resource utilization, while at the same time maintains a good quality-of-care. 
This goal relates to the philosophy of the Quality-and-Efficiency-Driven (QED) regime that is the recurring theme of this thesis. 
In this chapter, we obtain asymptotic results for the Erlang-R model with blocking in the QED regime (Section \ref{sec:QED_limit_block}). 
Following \cite{Jennings2008}, we employ a two-fold QED staffing policy: $s=R_1 +\beta \sqrt{R_1}$  for the number of nurses and $n=R_1/r+\gamma \sqrt{R_1/r}$ for the number of patients in the system (beds), where $\beta$ and $\gamma$ are constants, $R_1$ is the offered load of the servers (nurses) and $r$ is the fraction of time a patient spends in the needy state. 
We establish limiting expressions for performance measures, such as the probability of delay and blocking, in the form of explicit functions that depend solely on $\beta$ and $\gamma$. 
In deriving these limit results, we use the available product-form solution for the stationary distribution.

Likewise, we pursue QED performance for the Erlang-R model with holding.
However, a direct analytic approach is obstructed by the absence of product-form solutions.
We provide two solutions for establishing QED behavior. 
First, we provide stochastic performance bounds that stay meaningful in the QED regime, which demonstrate the non-degenerate behavior of the two-fold scaling in the large-system limit. 
Second, we develop a heuristic method that quantifies the difference between the holding model and the blocking model. 
This method is to a large extend related to the asymptotic approximation method for retrial queues discussed in Chapter 4, in the sense that we approximate the model with holding through the model with blocking, yet with an increased arrival rate. 
The increase in arrival rate turns out to be the solution of a fixed-point equation.
Using our results on the asymptotic behavior of the model with blocking in the QED regime, we then obtain approximative QED performance measures for the model with holding. 
These theoretical findings ultimately yield algorithms for dimensioning and time-varying staffing. \\
\\*
\textbf{Structure of the chapter.}
We first review related literature on the subject of staffing in health care environments in Section \ref{sec:ed_literature}. 
In Section \ref{sec:modeldescription}, we introduce the mathematical models more formally, and deduce preliminary results on their stability conditions and relative performance. 
Section \ref{sec:QED_scaling} describes the scaling regime we use for our asymptotic study of the restricted Erlang-R models, and Sections \ref{sec:QED_limit_block} and Section \ref{sec:QED_limit_holding} present our main theoretical findings. 
We turn to dimensioning problems in Section \ref{sec:dimensioning}, and show how our asymptotic QED results can be used to make resource allocation decisions in realistic settings. 
Section \ref{sec:analysis_chapter5} is devoted to the numerical and comparative analysis of the restricted Erlang-R models, and also shows how our method can be applied in time-varying environments through a case study.
We summarize our findings and give directions for future research in Section \ref{sec:conclusion}.


\section{Literature review}
\label{sec:ed_literature}
%
Due to increasing demand and tightening budgets in health care, there is a growing need for efficient workforce management \citep{Green2008}. Personnel (nurse and physician) expenditure is one of the biggest factors in hospital costs \citep{Kazahaya2005}, and inadequate nursing levels have been mentioned as a significant factor in medical errors and ED overcrowding. In order to establish appropriate nursing levels, a staffing policy requires assessment of a wide range of variables, such as differing nurse expertise and patient acuity during the day. Current methods, such as the minimum nurse-to-patient ratios, are often too inflexible to capture those varying conditions. The American Hospital Association (AHA) and others call for dynamic staffing policies that can deal with the complex and evolving nature of health care \citep{AHA2007}.
Workforce management in health care systems has been studied extensively; see \cite{Denton2013,Hall2006,Hall2012} for overviews.
In recent years it has become apparent that queueing models can be helpful in developing staffing and routing recommendations, not just for large-scale service systems, but also for the small and complicated health care systems.
 
%To understand and quantify the role of staffing levels, we show how the complex process happening within the Emergency Department can be described by the relatively tractable Erlang-R model, while concentrating on the interplay between patients (i.e.\  customers), nurses/physicians (i.e.\ servers) and ED beds (i.e.\  system capacity).
%Patients arrive to the Emergency Department seeking service from nurses (being \emph{needy}), and the service time corresponds to the duration a patient requires care. 
%After service, it is decided whether the patient leaves the ED, either to be discharged or hospitalized, or needs to reside in the ED for additional care (being \emph{content}). 
%In the latter typically occurs when a patient undergoes a medical test, is examined by a specialist or physician, or waits for lab results to return. 
%During these interruptions, the nurses may attend to other patients or perform entirely different duties such as administrative tasks.
%
%However, when patients find all beds occupied upon arrival, they cannot enter the Emergency Department immediately and have to wait in a separate holding room. Patients will leave the holding room and enter the Emergency Department as soon as a bed becomes available. Once patients are assigned to a bed, they can be looked after by a nurse.
%
%The limited availability of beds, nurses the installment of the holding room together create {\it finite-size effects} that might substantially influence the mode of operation of the Emergency Department.
%Analysis of the Erlang-R model with size restrictions is able to provide insight into these effect and ultimate propose adequate staffing levels for the number of beds and nurses in order to secure the timely and efficient access to care.
%
%As the ED is an important application of our model, we will adopt the associated terminology regarding staffing levels in the remainder of this paper. Hence, we will refer to $s$ and $n$ as the number of nurses and the number of beds, respectively.


The first to try such an approach through queueing models were Green et al.~\cite{Green2006,Green2008}, who used the single station stationary Erlang-C model to set staffing levels in EDs and panel sizes for clinics. Using a similar approach, Bekker \& de Bruin~\cite{Bekker2009a} used Erlang-B model to determine bed allocation for medical wards. 
%
The first to observe the significant impact of interrupted services in a health care setting were Jennings \& de V\'ericourt \cite{Jennings2008,Jennings2011}. Motivated by the need to set nurse-to-patient ratios for internal wards, they considered a closed queueing system with $s$ nurses and $n$ beds. This is essentially the Erlang-C model with the additional restriction that a finite population of the $n$ patients requires care. In their model, all beds are always occupied, and patients alternate between two phases: the needy phase where patients require service of a nurse and the content phase where they do not; see Figure \ref{fig:Jennings}. The system dynamics of restricted Erlang-R model are equivalent to those of the closed ward model of \cite{Jennings2008} if the holding queue would never be empty.

Campello et al.~\cite{Campello2016} analyzed a similar operational decision, referred to as ED case management, which determines the maximal number of patients a physician should handle in parallel. They also used queueing networks and analyzed the stationary distribution. Note that in practice such decision is not only affected by operational measurements such as waiting times, but also by psychological constraints that limit physician capability to manage multiple tasks (patients) in parallel.
KC \cite{diwas} provided empirical evidence that physicians should not treat more than 6-7 patients at the same time. Therefore, many hospitals in the US restrict entrance to EDs even if beds are available if physicians are overloaded. 
We too consider such constraints, and analyze their impact on performance. We take a different approach than \cite{Campello2016}; instead of analyzing numerically steady-state distributions, we develop many-server approximations that can produce insight into the system dynamics, and can be incorporated into time-varying staffing procedures; see Section  \ref{sec:case_study}.  

% This model can be retrieved from the Erlang-R model by setting $p=0$ and $n = \infty$ and thus disregarding the effects of interrupted services and finite-size bed capacity. 
%For $n=\infty$, one retrieves the Erlang-C model. 


\begin{figure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=1]
\draw [dashed, thick] (-0.5,-0.1) rectangle (3.5,2.85) node[right] {\footnotesize $n$};
%\draw [thick,->] (2.7,2) -- (2.7,3) -- (0.3,3) -- (0.3,2);
\draw [thick,->] (1.1,0.5) -- (0,0.5) -- (0,2) -- (0.6,2);
\draw [thick,->] (2.4,2) -- (3,2) -- (3,0.5) -- (1.9,0.5);
\draw [thick] (0.6,1.7) -- (1.6,1.7) -- (1.6,2.3) -- (0.6,2.3);
\draw [thick] (1,1.7) -- (1,2.3);
\draw [thick] (1.2,1.7) -- (1.2,2.3);
\draw [thick] (1.4,1.7) -- (1.4,2.3);
\draw (2.4,2) -- (3,2) -- (3,0.5) -- (1.9,0.5);
\draw (1.5,0.5) circle [radius=0.4] node[above=0.3cm] {\footnotesize $p/\d$} ;
\draw (2,2) circle [radius=0.4] node[above=0.3cm] {\footnotesize exp($\mu$)};
\node at (1.5,0.5) {\footnotesize $\infty$};
\node at (2,2) {\footnotesize $s$};
\end{tikzpicture}
\caption{The closed ward model.}
\label{fig:Jennings}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.7]
\draw [thick, ->] (0,4.5) node[above=0.3cm,right] {\footnotesize Pois$(\l)$} -- (2.5,4.5);
\draw [thick] (2.25,5) -- (3.75,5) -- (3.75,4) -- (2.25,4);
\draw [thick] (3,4) -- (3,5);
\draw [thick] (3.25,4) -- (3.25,5);
\draw [thick] (3.5,4) -- (3.5,5);
\draw [thick] (4.25,4.5) circle [radius=0.5];
\draw [thick, ->] (4.75,4.5) -- node[above=0.3cm,right] {\footnotesize $1-p$} (7,4.5);
\draw [thick,->] (5.75,4.5) -- node[right] {\footnotesize $p$} (5.75,2) -- (4,2);
\draw [thick] (3.5,2) circle [radius=0.5];
\draw [thick,->] (3,2) -- (1.5,2) -- (1.5,4.5);
\node at (4.25,4.5) {\footnotesize $s$};
\node at (3.5,2) {\footnotesize $\infty$};
\node [above] at (4,5.15) {\footnotesize exp($\mu$)};
\node [above] at (3.5,2.4) {\footnotesize exp($\delta$)};
\end{tikzpicture}
\caption{The Erlang-R model.}
\label{fig:ErlangR}
\end{subfigure}
\caption{Related queueing models.}
\end{figure}



The model in~\cite{Jennings2008,Jennings2011} was developed for modeling internal dynamics within an internal ward. However, in the ED, beds are not constantly occupied and the utilization level depends on the flow of patients that arrive from outside the system.
%While~\cite{Jennings2008,Jennings2011} focus entirely on finite-size effects,
Yom-Tov \& Mandelbaum \cite{YomTov2014} highlight the interrupted services while accounting for the transient nature of patient's arrival process, and introduced the Erlang-R model as a model for an ED. The Erlang-R model is an open two-station queueing network that has the same layout as the restricted Erlang-R model, except that all patients find a bed available upon arrival, see Figure \ref{fig:ErlangR}. In both models patients experience the interrupted services, but the Erlang-R model has no further restrictions on the bed capacity, hence neglecting the finite-size effects. Yom-Tov \& Mandelbaum \cite{YomTov2014} showed, using a simulator tailored to an Israeli ED, that the complicated small ED dynamics can be captured using the relatively simple Erlang-R model, and hence, its recommendations can be implemented in ED workforce management.
Although the feature of interrupted services is present in many systems, it is particularly important for modeling EDs, because the duration of the interruption is typically much longer than the time patients require care from a nurse. This explains why the Erlang-R model is considered to be the canonical model for EDs. The restricted Erlang-R model with holding/blocking thus extends the Erlang-R model with finite-size constraints which, like interrupted services, are expected to have a decisive impact on performance.
% \\
% \\*
% \noindent
%\textbf{Quality-and-Efficiency-Driven regime.} 
%The Quality-and-Efficiency driven (QED) regime, also known as the Halfin-Whitt regime, for many-server systems adheres to a square-root staffing rule, which is best explained for the Erlang-C model. This system can be characterized completely by the staffing level $s$ and the offered load $R=\lambda/\mu$, which is the average workload pressure per time unit on the system. Moreover, let $\rho=R/s$ denote the server utilization level. Since exact analysis provides little qualitative insight in performance with respect to the system parameters, we resort to asymptotic analysis. This in turn provides approximations for the true system behavior. In the QED regime \citep{Borst2004,HalfinWhitt1981}, the nurse utilization level is driven to unity in accordance to $(1-\rho)\sqrt{s} \rightarrow \beta$ as $s \rightarrow \infty$, for some fixed parameter $\beta >0$. This gives rise to the square-root dimensioning rule $s=R+\beta \sqrt{R}$, which prescribes that the number of nurses $s$ exceeds the minimally required offered load $R$, but only by a relatively small amount $\beta \sqrt{R}$. As $s$ grows large, the probability of delay tends to a non-degenerate function that only depends on the parameter $\beta$. This function is strictly decreasing in $\beta>0$ with range $(0,1)$. Consequently, any targeted delay probability can be achieved by adjusting $\beta$. Moreover, the mean delay is of order $1/\sqrt{s}$ and hence asymptotically negligible.
%In this paper we take the same approach, but determine capacity for nurses and beds simultaneously in such a way that both the probability to wait for a nurse and the probability to wait for a bed are non-degenerate.
%Moreover, the utilization of both nurses and beds goes to 1 as the size of the system increases. In recent years, a new approach for developing approximations of performance measures of queueing systems  with finite-size constraints in the QED regime was suggested by \cite{Leeuwaarden2015,Leeuwaarden2016}. This approach characterizes the asymptotic dynamics of these analytically intractable systems with finite-size restrictions through more tractable ones. We adopt this approach for developing the approximations for the holding model in Section \ref{sec:QED_limit_holding}.  


%\subsection{Structure of the paper}
%This paper is structured as follows. First, by introducing and analyzing the Erlang-R model with finite-capacity restrictions, we quantify the finite-size effects in large-scale systems with interrupted services. We provide an analysis of the stationary distribution of the three-station queueing network in Section~2. The exact analysis relies on matrix-geometric methods and we show that the stability condition is closely related to the closed ward model in~\cite{Jennings2008}. In Section~3, we consider the two-fold QED staffing rule. We first derive the QED limits for the model with blocking. We then turn to the model with holding and establish stochastic bounds that the blocking model to the intractable holding model. By means of extensive simulations, we verify and compare the bounds that arise due to the stochastic ordering in the QED regime. Moreover, we provide explicit approximations of the performance in the QED regime in Section~4 by establishing the relation between the model with holding and the model with blocking, but with an increased arrival rate. Finally, we translate the two-fold square-root staffing policy into an algorithm for time-varying staffing. 
%This algorithm uses the MOL method combined with the explicit approximation method developed in Section~4.
%We conclude by summarizing the managerial insights obtained from this work.

\section{Models and performance measures}
\label{sec:modeldescription}

\subsection{Three-dimensional Markov process}
\label{sec:Markov_process}

Since in the restricted Erlang-R model described the arrival process is taken Poisson, and all service and content times are assumed independent and exponential, the system can be characterized in terms of a Markov process.
Let $Q(t) = (H(t),Q_1(t),Q_2(t))$ represent the number of patients in the \emph{holding}, \emph{needy} and \emph{content} state at time $t$, respectively. 
In both variants, $n$ is the maximum number of patients admitted to system, we have $Q_1(t)+ Q_2(t)\leq n$ for all $t\geq 0$. 
Due to the absence of holding patients in the Erlang-R model with blocking,  $H(t)=0$ is enforced in this case, whereas $H(t)$ has unbounded support in the model with holding. 
This distinction requires us to explore the stationary distribution of the two variants separately. 
Before doing so, we introduce some additional notation. 
We define 
\begin{equation}
 R_1 := \frac{\l}{(1-p)\mu}, \qquad R_2 := \frac{p\l}{(1-p)\d}, 
 \label{eq:R1_R2}
 \end{equation}
where $R_1$ and $R_2$ can be interpreted as the offered workload brought towards the needy queue and the content (infinite-server) queue, respectively. 
Furthermore, we define 
\begin{equation}
r:= \frac{\d}{\d+p\m},
\label{eq:delta}
\end{equation} 
which is the fraction of time a patient spends in the needy state (in case she experienced no wait during her sojourn). \\
\\*

\begin{figure}
\centering
\begin{tikzpicture}[scale = 0.9]
\draw [thick] (-1.25,5) -- (0,5) -- (0,4) -- (-1.25,4);
\draw [thick] (0.5,4.5) circle [radius = 0.5] node {\footnotesize 1} node[above=0.5cm] {\footnotesize exp$(\l)$} 
	node[below =0.5cm] {\footnotesize \color{col1} Station 0} ;
\draw [thick] (-0.25,4) -- (-0.25,5);
\draw [thick] (-0.5,4) -- (-0.5,5);
\draw [thick] (-0.75,4) -- (-0.75,5);
\draw [thick, ->] (1,4.5) -- (2.5,4.5);
\draw [thick] (2.25,5) -- (3.75,5) -- (3.75,4) -- (2.25,4);
\draw [thick] (3,4) -- (3,5);
\draw [thick] (3.25,4) -- (3.25,5);
\draw [thick] (3.5,4) -- (3.5,5);
\draw [thick] (4.25,4.5) circle [radius=0.5] node {\footnotesize $s$} node[above=0.5cm] {\footnotesize exp$(\mu)$}
node[below = 0.5cm] {\footnotesize \color{col1} Station 1} ;
\draw [thick, ->] (4.75,4.5) -- node[right=0.8cm,above] {\footnotesize $1-p$} (6.5,4.5) -- (6.5,1.6) -- (-2,1.6) -- (-2,4.5) -- (-1.2,4.5);
\draw [thick,->] (5.75,4.5) -- node[left] {\footnotesize $p$} (5.75,2.5) -- (4,2.5);
\draw [thick] (3.5,2.5) circle [radius=0.5] node {\footnotesize $\infty$} node[above=0.4cm] {\footnotesize exp$(\d)$}
node[below right = 0.35cm] {\footnotesize \color{col1} Station 2} ;;
\draw [thick,->] (3,2.5) -- (1.5,2.5) -- (1.5,4.5);

\draw [thick, dashed] (-3,1.2) rectangle (7.25,5.75) node[right] {\footnotesize $n$};
\end{tikzpicture}
\caption{The Erlang-R model with blocking viewed as a closed Jackson network.}
\label{fig:ErlangR_blocking}
\end{figure}

\noindent
\textbf{Erlang-R model with blocking.}
In case of the blocking model, $Q(t)$ reduces to a finite-state Markov process $Q(t) = (Q_1(t),Q_2(t))$, where $Q_1(t)+Q_2(t)\leq n$ for all $t\geq 0$. 
In fact, this is equivalent to the closed Jackson network depicted in Figure \ref{fig:ErlangR_blocking} with finite population $n$. 
Station 1 in Figure \ref{fig:ErlangR_blocking} is an $M/M/s$ queue with service rate $\mu$, modeling the number of needy patients $Q_1(t)$. %We will hence also refer to this node as the \emph{nurse queue}.
Station 2 models the number of content patients $Q_2(t)$, and can therefore be represented as an infinite-server queue with service rate $\d$. 
A patient can enter the unit only if $Q_1(t)+Q_2(t)<n$. 
Station 0---a single-server queue---moderates this as it only produces output at rate $\l$ in case its queue length is positive, i.e.\ if $n-Q_1(t)-Q_2(t)>0$.

Observe that because patients finding a full network are blocked, the number of patients in the system cannot grow beyond $n$. 
Hence, the system is stable for all parameter settings, and hence a steady-state distribution exists. Moreover, the simplification of the model with blocking allows us to express the steady-state distribution of the system in explicit product-form. 
Let $\pi_b(j,k)$ denote the steady-state probabilities of having $j$ needy and $k$ content patients in the system. Then, 
%
\begin{equation}\label{eq:pih(i,j)}
\pi_b(j,k) = \left\{
\begin{array}{ll}
\pi_0\,\frac{1}{\kappa(j)}\,\frac{1}{k!}\cdot R_1^j\cdot R_2^k, & ~~~\text{if }j+k \leq n,\\
0, & ~~~\text{else,}
\end{array}\right.
\end{equation}
where 
\begin{equation*}
\kappa(j) := \left\{
\begin{array}{ll}
j! , & ~~\text{if }j \leq s,\\
s!\, s^{j-s}, &~~ \text{else,}
\end{array}\right.
\end{equation*}
and $
\pi_0^{-1} = \sum_{j+k\leq n} \frac{1}{\kappa(j)}\,\frac{1}{k!}\cdot R_1^j\cdot R_2^k$.\\
\\*
\textbf{Erlang-R model with holding.}
\label{ref:modelsoft}
The Erlang-R model with holding does not lead to a Jackson network with an elegant product-form solution for the steady-state distribution, because the holding queue cannot be modeled as a station that is independent from the other queues in the system.
 %
However, we are able to describe the system as a two-dimensional Markov process without loss of information. 
To see this, define $N:= \{N(t)\}_{t\geq 0}$ with $N(t) := H(t)+Q_1(t) + Q_2(t)$, the total number of patients in the system (including the holding queue).  
Using the restriction $Q_1(t)+Q_2(t) \leq n$ together with the fact that no bed is left vacant if a patient is waiting in the holding queue, this yields
%
\begin{equation*}
H(t) = \left(N(t) - n\right)^+, \quad t\geq 0,
\end{equation*}
%
where $(\cdot)^+ := \max\{0,\cdot\}$.
For the same reason, $Q_2(t) = N(t) - Q_1(t)$ if $H(t)=0$, and $Q_2(t) = n-Q_1(t)$ otherwise. 
In other words,
%
\begin{equation*}
Q_2(t) = \min\{N(t),n\} - Q_1(t), \quad t \geq 0.
\end{equation*}
Therefore, we can express the state of all three queues in the Erlang-R model with holding using a two-dimensional Markov process $X:= \{X(t)\}_{t\geq 0}$, where 
\begin{equation*}
X(t) :=\left( N(t), Q_1(t) \right).
\end{equation*}
%
The process $X$ lives on the semi-infinite strip
 \begin{equation*}
X(t) \in \left\{\,(i,j)\, |\, j \leq \min\{i,n\}, i\in \mathbb{N}_0, j \in \{0,1,\ldots,n\}\, \right\},
\end{equation*}
and belongs to the class of Quasi-Birth-Death (QBD) processes.
The reader is referred to Appendix~\ref{app:QBDdescription} for a detailed description of this process, in terms of its transition diagram and generator matrix.

Contrary to the model with blocking, the system with holding \emph{can} become unstable in case capacity is insufficient to satisfy patient demand. 

\begin{proposition}\label{prop:StabilityCondition}
The Erlang-R model with holding is stable if and only if 
\begin{equation}
\frac{\lambda}{(1-p)\mu s} < \frac{ \sum_{i=0}^s \frac{i}{s}\binom{n}{i} \left(\frac{\d}{p\mu}\right)^i + \sum_{i=s+1}^n \binom{n}{i} \frac{i!}{s!} s^{s-i} \left(\frac{\d}{p\m}\right)^i}
{ \sum_{i=0}^s \binom{n}{i} \left(\frac{\d}{p\mu}\right)^i + \sum_{i=s+1}^n \binom{n}{i} \frac{i!}{s!} s^{s-i} \left(\frac{\d}{p\m}\right)^i}
=: \rho_{\max}(s,n).
\label{eq:StabilityCondition} 
\end{equation}
\end{proposition}
The proof is given in Appendix~\ref{app:stability} and follows from the general theory for QBD processes. 

Observe that $\rho_{\max}(s,n)$ poses an upper bound on the occupancy level of the servers in the holding model, which is clearly smaller than 1 for all $s$ and $n$. 
In addition, this implies that the maximum workload $R_{\max}(s,n) := s\cdot\rho_{\max}(s,n)$ the system is able to handle is strictly less than $s$.
If we compare this to the open Erlang-R model, in which the maximal attainable workload equals $s$, we observe the effect of finite-size constraints on operational performance. 
Figure \ref{fig:Rmax} shows the influence of both $s$ and $n$ on the maximum feasible workload in case $r=0.25$. 
From these graphs, note that if $s\ll rn$, $R_{\max}$ grows almost linearly with $s$. 
Furthermore, $R_{\rm max}(s,n)$ is increasing in $n$ for $s$ fixed.
A logical practical consequence is that a larger number of beds allows for a larger patient volume to enter the ED with the same number of nurses.
Moreover, $R_{\rm max}(s,n)$ is increasing in $s$, but as in Figure \ref{fig:Rmax_a}, adding an extra nurse does not increase the stability region in case $n$ is too tight. 
 Conversely, adding extra beds does not increase $R_{\rm max}(s,n)$ if the number of nurses does not allow for an increase in offered load, see Figure \ref{fig:Rmax_b}. 
Additionally, it is easily verified that $R_{\rm max}(s,n)$ is upper bounded by both $s$ and $R_{\rm max}(n,n) = rn$. Therefore, a careful balance is called for between servers (nurses) and beds, so that resources will be efficiently utilized. We observe that when the ratio $s/n\approx r$, the system is better balanced. 
We will propose an appropriate balance between resources by defining a synchronized QED capacity recommendation for both servers and beds in Section  \ref{sec:QED_scaling}.

\begin{figure}
\centering
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.7]
\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0,
	ymax = 20,	
	grid = none, 
	axis line style={->},
	axis lines = left,
	xlabel = $s$,
	ylabel = {$R_{\rm max}(s,n)$},
	legend cell align=left,
	legend pos = north west
]

 	
\addplot[col1,thick,mark=*] table[x=s,y=n20] {Chapter_5/tikz/stability/r025_n_fixed.txt};
\addplot[col3,thick,mark=*] table[x=s,y=n40] {Chapter_5/tikz/stability/r025_n_fixed.txt};
\addplot[col4,thick,mark=*] table[x=s,y=n60] {tikz/stability/r025_n_fixed.txt};
\addplot[col5,thick,mark=*] table[x=s,y=n80] {Chapter_5/tikz/stability/r025_n_fixed.txt};

\legend{$n=20$,$n=40$,$n=60$,$n=80$}
\end{axis}
\end{tikzpicture}
\caption{$R_{\rm max}$ as a function of $s$.}
\label{fig:Rmax_a}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.7]
\begin{axis}[
	xmin = 0,
	xmax = 100,
	ymin = 0,
	ymax = 20,	
	grid = none, 
	axis line style={->},
	axis lines = left,
	xlabel = $n$,
	ylabel = {$R_{\rm max}(s,n)$},
	legend cell align=left,
	legend pos = north west
]

 	
\addplot[col1,thick,mark=*,mark repeat = 2] table[x=n,y=s5] {Chapter_5/tikz/stability/r025_s_fixed.txt};
\addplot[col3,thick,mark=*,mark repeat = 2] table[x=n,y=s10] {Chapter_5/tikz/stability/r025_s_fixed.txt};
\addplot[col4,thick,mark=*,mark repeat = 2] table[x=n,y=s15] {Chapter_5/tikz/stability/r025_s_fixed.txt};
\addplot[col5,thick,mark=*,mark repeat = 2] table[x=n,y=s20] {Chapter_5/tikz/stability/r025_s_fixed.txt};

\legend{$s=5$,$s=10$,$s=15$,$s=20$}
\end{axis}
\end{tikzpicture}
\caption{$R_{\rm max}$ as a function of $n$.}
\label{fig:Rmax_b}
\end{subfigure}
\caption{The maximum achievable workload in the restricted Erlang-R model with holding for $r=0.25$.}
\label{fig:Rmax}
\end{figure}

Provided that the system is stable, the stationary distribution of the QBD process $X$ can be obtained numerically by the matrix geometric method \citep{Neuts1981}.
Subsequently, we can derive the stationary distribution of the original $Q(t)$, denoted by $\pi_h(\cdot,\cdot,\cdot)$.

\subsection{Performance measures}
\label{sec:performance_metrics}
In this work, we concentrate on five performance measures that are central to our analysis. 
In the definitions that follow, we present expressions for these measures in terms of a general three-dimensional measure $\pi$, which one can replace by either $\pi_b$ or $\pi_h$, depending on the scenario considered. 
In the remainder of this work, we will augment the measures related to the Erlang-R model with blocking and holding by the superscript $b$ and $h$, respectively\footnote{In line with $H(t)=0$, we use $\pi_b(i,j,k) = \pi_b(j,k)$ if $i=0$, with $\pi_b(j,k)$ as in \eqref{eq:pih(i,j)}, and $\pi_b(i,j,k) = 0$ otherwise, when considering the model with blocking.}.

As relevant performance measures, we consider the probability of holding (cq.\\ \noindent blocking) at entering the system, the probability of delay at the needy queue, expected waiting time for a nurse, utilization of nurses and utilization of beds:
\begin{equation}
\P({\rm hold}) = \sum_{i=0}^\iy \sum_{j=0}^n \pi(i,j,n-j), \qquad
\P({\rm delay}) \approx \sum_{i=0}^\infty\sum_{j=s}^{n}\sum_{k=0}^{n-j} \pi(i,j,k), 
\label{eq:delay_probability}
\end{equation}
\begin{equation}
\label{eq:EW_exact}
\E [W] \approx \sum_{i=0}^\infty\sum_{j=s}^{n}\sum_{k=0}^{n-j} \frac{\max\{0,j-s+1\}}{\mu}\,\pi(i,j,k), 
\end{equation}
\begin{equation}
\label{eq:utilization}
\rho_s = \frac{1}{s}\,\sum_{i=0}^\infty \sum_{j=0}^n \sum_{k=0}^{n-j} \min\{j,s\} \pi(i,j,k), \qquad
\rho_n = \frac{1}{n}\,\sum_{i=0}^\infty \sum_{j=0}^n \sum_{k=0}^{n-j} \min\{i,n\} \pi(i,j,k).
\end{equation}

It should be stressed that the above expression for the delay probability and the expected waiting time for a nurse is not exact. For the blocking model one can use the Arrival Theorem, see e.g.~\cite{Chen2001a}, whereby the exact expression sums up to $n-1$ instead of $n$. 
Since we consider the system as $n\to\infty$, this discrepancy becomes negligible. 
For the holding model, a similar argument holds. 
We will therefore use the expressions in \eqref{eq:delay_probability}-\eqref{eq:utilization} as definitions for the performance measures. 

\subsection{Stochastic bounds}
\label{sec:bounds}

%\textit{
%Describe open Erlang-R and Jennings model, and discuss how they relate.\\
%Stochastic ordering of number of patients in queues: Erlang-R with holding is upper bounded by Jennings, and lower bounded by Erlang-R with blocking. }

Although the two variants of the Erlang-R model differ with respect to the admission policy, and require different mathematical treatment, we would like to be able to capture their relative performance.  
We substantiate the intuition that the holding room leads to more patients in the ED, in the following result. 

\begin{proposition}\label{thm:stochasticordering}
Let $Q_1^b$, $Q_2^b$, $Q_1^h$, $Q_2^h$ denote the nurse and content queue length processes in the Erlang-R model with blocking and holding, respectively.
Let $H(0) = 0$,  $Q_1^b(0)=Q_1^h(0)$ and $Q_2^b(0)=Q_2^b(0)$. For all $t\geq 0$, 
\begin{align}
Q_1^b(t) + Q_2^b(t) &\preceq_{\rm st} Q_1^h(t) + Q_2^h(t) \preceq_{\rm st} n ,\\
Q_2^b(t) &\preceq_{\rm st} Q_2^h(t),\\
Q_1^b(t) &\preceq_{\rm st} Q_1^h(t) + H(t),
\end{align}
where $X\preceq_{\rm st} Y$ implies $\P(X\geq k) \leq \P(Y\geq k)$ for all $k\geq 0$.
\end{proposition}
\noindent
The proof of Proposition \ref{thm:stochasticordering} uses sample path coupling and can be found in Appendix \ref{app:stochastic_ordering}.
Note that as an immediate consequence, we have
%
\[ \P^b( {\rm block}) = \lim_{t\to\iy} \P\big( Q_1^b(t)+Q_2^b(t) \geq n \big) \leq \lim_{t\to\iy} \P\big( Q_1^h(t) + Q_2^h(t) \geq n \big) = \P^h( {\rm hold }) \]
and by similar reasoning $\rho^b_n \leq  \rho_n^h$.
In other words, under similar offered load and capacity constraints, utilization levels for the nurses in the Erlang-R model with blocking are lower than in the Erlang-R model with holding. 
Moreover, the total number of waiting patients in the setting with holding is stochastically larger than in the setting with blocking, and in the open Erlang-R model. 
We further discuss the differences between both models in Section \ref{sec:dimensioning} and Section \ref{sec:analysis_chapter5}. 


\section{Two-fold QED regime}
\label{sec:QED_scaling}

We do not want to waste capacity of either servers or beds without getting significant advantage in term of performance. 
We therefore take an asymptotic approach that lets the external arrival rate $\l$ grow to infinity, while scaling $s$ and $n$ accordingly.
In doing so, we intend to establish QED-type system behavior, i.e.\ high occupancy levels of both nurses and beds and good quality-of-service.

\subsection{Two-fold scaling rule}

In order to identify the scaling of $s$ and $n$ as $\l\to\infty$, we draw inspiration from the two-fold scaling rule used by Jennings \& de V\'ericourt \cite{Jennings2008} and Khudyakov et al.~\cite{Khudyakov2010}, which follows the celebrated square-root staffing principle.
This principle suggests that, in the most general setting, capacity should be equal to the expected offered load entering the system, let us say $R$, plus an additional variability hedge that is proportional to $\sqrt{R}$.
In the restricted Erlang-R model, we have two capacity sources, namely $s$ and $n$, which experience different relevant amount of works.

The offered load the servers in the needy queue experience is given by $R_1$, as in the regular Erlang-R model; 
it does not change due to the finite-size effects, since all patients are served eventually. Hence, we only need to account for the interrupted services. It follows that the appropriate staffing rule for the nurses in the QED regime remains $s=R_1+\beta \sqrt{R_1}$ for some constant $\beta >0$.

To establish the bed capacity level, we need to reflect on the load offered to the beds. Observe that beds remain occupied both in needy and content states. This suggests that $R_n:=R_1+R_2=R_1/r$, with $R_1$ and $R_2$ as in \eqref{eq:R1_R2} and $r$ is the expected fraction of time a patient spends at the nurse station defined in \eqref{eq:delta}.
%
%In the QED regime, we strive to design a system where beds are fully occupied while the needs of patients can always be addressed immediately.
%Observe that the expected fraction of time a patient spends at the nurse station is $r=\delta/(\delta + p \mu)$, in the ideal case that his needs are always addressed immediately.
%The offered load to the beds therefore amounts $R_n:=R_s/r$ and
As a result, the appropriate staffing rule is $n=R_n+\gamma \sqrt{R_n}$ for some constant $\gamma>0$. In conclusion, the two-fold QED scaling rule is given by
\begin{equation}\label{eq:twofoldscaling}
\begin{array}{ll}
s &= R_1 + \beta \sqrt{R_1} + o(\sqrt{R_1}) \\
n &= \frac{R_1}{r}+\gamma \sqrt{\frac{R_1}{r}} + o(\sqrt{R_1})
\end{array}
\end{equation}
with $\beta,\gamma>0$ constants and $R_1:=\lambda/((1-p)\mu)$.

Recall that we saw in Figure \ref{fig:Rmax} that resources seem efficiently utilized if $s/n\approx r$. 
Scaling \eqref{eq:twofoldscaling} is in line with this reasoning since 
\[
\frac{s}{n} = r\left(1+ \frac{\beta - \gamma\sqrt{r}}{\sqrt{R_1}}+ O(1/R_1) \right) . 
\]


\begin{remark}
In \cite{Jennings2008}, a similar scaling regime is considered, which only relates $s$ and $n$ through a square-root scaling, namely the regime $s = r n + \hat\g\sqrt{n}$,
which is equivalent to the second relation in \eqref{eq:twofoldscaling} if $\hat\g = \b\sqrt{r} - \g r$.
Due to the absence of external arrivals in this closed system, they let the number of beds $n$ approach infinity as opposed to $\l$ in our settings. 
Nevertheless, this results in the same asymptotic regime.
\end{remark}

Before turning to asymptotic expressions for the performance measures concerning the Erlang-R model with blocking or holding, we conduct a few numerical experiments to confirm that the scaling in \eqref{eq:twofoldscaling} indeed leads to desired QED behavior. 

In Figure \ref{fig:sample_paths}, we plotted the sample paths of the three-dimensional queue length process of the holding model in which $\b$ and $\g$ are fixed, and $R_1$ is increased. 
Observe that the needy queue length $Q_1(t)$, plotted in orange in Figure \ref{fig:sample_paths}, fluctuates around the values $s$, and stabilizes for larger values of $R_1$. 
This naturally implies that the server (nurses) utilization approaches 100\%, while the number of patients waiting is $O(\sqrt{R_1})$.
Furthermore, we see that the percentage of occupied beds also tends to 100\%, while the holding queue length remains small. 
The holding queue is of much smaller order than $R_1$, which implies that the holding time of a patient becomes negligible as $R_1\to\iy$. 
From these empirical findings we deduce that  under scaling \eqref{eq:twofoldscaling} the restricted Erlang-R model exhibits QED behavior on two levels: Outside the facility while waiting for an available bed, and inside the facility while waiting for attention of a nurse.

\begin{figure} 
\centering
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale=0.51]

\begin{axis}[
	xmin = 0,
	xmax = 200,
	ymin = 0.0,
	ymax = 28,
	ytick = {0,5,10,15,20,25},	
	grid = none, 
	axis line style={->},
	axis lines = left,
	xlabel = $t$,
	legend cell align=left,
	legend pos = north east
]

\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
 	
\addplot[very thick,col5] file {Chapter_5/tikz/sample_paths/R5_holding.txt};
\addplot[very thick,col2] file {Chapter_5/tikz/sample_paths/R5_service.txt};
\addplot[very thick,col4] file {Chapter_5/tikz/sample_paths/R5_total.txt};
\addplot[very thick,dashed] coordinates {
	(0,7)
	(200,7)
	};
\addplot[very thick,dashed] coordinates {
	(0,24)
	(200,24)
	};

%\legend{Holding,Blocking,Closed ward};
\end{axis}

\end{tikzpicture}
\caption{$R_1=5$}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale=0.51]

\begin{axis}[
	xmin = 0,
	xmax = 200,
	ymin = 0.0,
	ymax = 128.333,
	ytick = {0,20,40,60,80,100,120},	
	grid = none, 
	axis line style={->},
	axis lines = left,
	xlabel = $t$,
	legend cell align=left,
	legend pos = north east
]

 	
\addplot[very thick,col5] file {Chapter_5/tikz/sample_paths/R25_holding.txt};
\addplot[very thick,col2] file {Chapter_5/tikz/sample_paths/R25_service.txt};
\addplot[very thick,col4] file {Chapter_5/tikz/sample_paths/R25_total.txt};
\addplot[very thick,dashed] coordinates {
	(0,30)
	(200,30)
	};
\addplot[very thick,dashed] coordinates {
	(0,110)
	(200,110)
	};
%\legend{Holding,Blocking,Closed ward};
\end{axis}

\end{tikzpicture}
\caption{$R_1=25$}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale=0.51]

\begin{axis}[
	xmin = 0,
	xmax = 200,
	ymin = 0.0,
	ymax = 490,
	ytick = {0,100,200,300,400},	
	grid = none, 
	axis line style={->},
	axis lines = left,
	xlabel = $t$,
	legend cell align=left,
	legend pos = north east
]

 	
\addplot[very thick,col5] file {Chapter_5/tikz/sample_paths/R100_holding.txt};
\addplot[very thick,col2] file {Chapter_5/tikz/sample_paths/R100_service.txt};
\addplot[very thick,col4] file {Chapter_5/tikz/sample_paths/R100_total.txt};
\addplot[very thick,dashed] coordinates {
	(0,110)
	(200,110)
	};
\addplot[very thick,dashed] coordinates {
	(0,420)
	(200,420)
	};
	
%\legend{Holding,Blocking,Closed ward};
\end{axis}

\end{tikzpicture}
\caption{$R_1=100$}
\end{subfigure}
\caption{Sample paths of $H(t)$ (blue), $Q_1(t)$ (orange) and $Q_1(t)+Q_2(t)$ (green) of the Erlang-R model with holding with parameters $\mu = 1$, $\d=0.25$, $p=0.75$ and $\b=\g=1$. The staffing levels $s$ and $n$ are depicted by the dashed lines.}
\label{fig:sample_paths}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{0.32\textwidth}
\centering
\begin{tikzpicture}[scale=0.53]
\begin{axis}[
	xmin = 0,
	xmax = 145,
	ymin = 0.0,
	ymax = 0.7,
	ytick = {0,0.1,...,0.7},
	xlabel = $\l$,
	grid = both, 
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend pos = south east
]

 	
\addplot[thick,col1,mark=*] file {Chapter_5/tikz/empirical/delayProbErlangH.txt};
\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/delayProbYomTov.txt};
\addplot[thick,col5,mark=*] file {Chapter_5/tikz/empirical/delayProbJennings.txt};
%\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/delayProbErlangR.txt};
\small
\legend{Holding,Blocking,Closed ward};
\end{axis}

\end{tikzpicture}
\caption{Delay probability nurse}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\begin{tikzpicture}[scale=0.53]

\begin{axis}[
	xmin = 0,
	xmax = 145,
	ymin = 0.0,
	ymax = 0.3,
	ytick = {0,{0.05},0.1,0.15,0.2,0.25,3},	
	grid = both, 
	axis line style={->},
	tick label style={/pgf/number format/fixed},
	axis lines = left,
	xlabel = $\l$,
	legend cell align=left,
	legend pos = north east
]

 	
\addplot[thick,col1,mark=*] file {Chapter_5/tikz/empirical/EWErlangH.txt};
\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/EWYomTov.txt};
\addplot[thick,col5,mark=*] file {Chapter_5/tikz/empirical/EWJennings.txt};
%\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/EWErlangR.txt};
\small
\legend{Holding,Blocking,Closed ward};
\end{axis}

\end{tikzpicture}
\caption{Expected wait}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering
\begin{tikzpicture}[scale=0.53]

\begin{axis}[
	xmin = 0,
	xmax = 145,
	ymin = 0.7,
	ymax = 1.02,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\l$,
	legend cell align=left,
	legend pos = south east
]
 	
\addplot[thick,col1,mark=*] file {Chapter_5/tikz/empirical/rhoErlangH.txt};
\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/rhoYomTov.txt};
\addplot[thick,col5,mark=*] file {Chapter_5/tikz/empirical/rhoJennings.txt};
%\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/rhoErlangR.txt};
\small
\legend{Holding,Blocking,Closed ward};
\end{axis}

\end{tikzpicture}
\caption{Nurse utilization}
\end{subfigure}
\caption{Asymptotic behavior of the restricted Erlang-R model with holding and blocking, and the closed ward model for $\m=1$, $\d = 0.2$, $p=0.8$ and $\b=\g=0.5$.}
\label{fig:empiricalAsymptotics}
\end{figure}


We also check how the Erlang-R model with blocking or holding  and the closed ward model of \cite{Jennings2008} relate under scaling \eqref{eq:twofoldscaling}. 
In Figure~\ref{fig:empiricalAsymptotics}, we plot the performance measures, obtained through simulation, for the three models in which we fix $\b=\g=0.5$ and vary the arrival rate $\l$. 
First, we see that $\P({\rm delay})$ stabilizes as $\l\to\iy$ in all three models under scaling \eqref{eq:twofoldscaling}, and the delay probability of the model with holding lies in between the other two. 
Second, note that the expected waiting time for a nurse in all models converges to 0 as $\l$ increases. In fact, the rate of decay is similar in all three models.  
We observe that $\rho_s$ approaches unity in all models, and the rate of convergence seems again comparable. 
Finally, and most importantly, we notice an ordering between the three models.
Namely, in all performance measures considered in Figure \ref{fig:empiricalAsymptotics}, Erlang-R with holding appears to be upper bounded by the closed ward and lower bounded by the Erlang-R with blocking. 
In a multitude of parameter settings of $(\b,\g)$, we have seen the same ordering, leading to the following conjecture: 
%
\begin{conjecture}\label{conj:stochorder}
Let $Q^b_1(\iy)$, $Q_1^h(\iy)$ and $Q_1^J(\iy)$ denote the stationary number of needy patients in the Erlang-R model with blocking, holding and the closed ward, respectively. Then,
\begin{equation}
Q_1^b(\iy) \preceq_{\rm st} Q_1^h(\iy) \preceq_{\rm st} Q_1^J(\iy).
\end{equation}
\end{conjecture}
Observe that Conjecture \ref{conj:stochorder} poses a stronger statement than the third assertion in Proposition \ref{thm:stochasticordering}. 
The latter does give an upper bound to $Q_1^h(\iy)$ in terms of $Q_1^b(\iy)$, albeit supplemented with the stationary holding queue length. 

\subsection{QED limits for Erlang-R with blocking}
\label{sec:QED_limit_block}

%
We now continue our analysis by examining its limiting behavior under scaling \eqref{eq:twofoldscaling},and obtain QED limits for some performance measures of the Erlang-R model with blocking.
Using the explicit expressions for the blocking model in \eqref{eq:pih(i,j)}, we derive the limiting values of the relevant performance measures defined in Section \ref{sec:performance_metrics} in terms of $\b$ and $\g$. 

\begin{theorem}\label{thm:limits_YT}
Let $s$ and $n$ scale as in \eqref{eq:twofoldscaling} with ${-}\infty<\b<\infty,\,\g>0$ as $\l\to\infty$. Then, if $\b \neq 0$,
%
\begin{align}
g^b(\b,\g)
&:= \lim_{\l\to\iy} \P^b({\rm delay})\nonumber \\
\label{eq:yt_limit_delay}
&= 
\left(1 + 
\frac{ \b \, \int_{-\iy}^\b \Phi\left(\frac{\g-t\sqrt{r}}{\sqrt{1-r}}\right)\, \dd\Phi(t) }
{\f(\b)\Phi(\eta) -  \f(\sqrt{\b^2+\eta^2}){\rm e}^{
{1}{2} \omega^2} \Phi(\omega)}
\right)^{-1},\\
f^b(\b,\g) 
&:= \lim_{\l\to\iy} \sqrt{R_1}\cdot\P^b({\rm block}) \nonumber\\
\label{eq:yt_limit_block}
&= 
\frac{
\sqrt{r}\f(\g)\Phi(-\omega\sqrt{r}) + \f(\sqrt{\b^2+\eta^2})\,{\rm e}^{\frac{1}{2} \omega^2} \Phi(\omega)
}{
\int_{-\iy}^\b \Phi\left(\frac{\g-t\sqrt{r}}{\sqrt{1-r}}\right)\, \dd\Phi(t) +
\frac{\f(\b)\Phi(\eta)}{\b} -  \frac{\f(\sqrt{\b^2+\eta^2})}{\b}{\rm e}^{\tfrac{1}{2} \omega^2} \Phi(\omega)
 },\\
h^b(\b,\g) &:= \lim_{\l\to\iy} \sqrt{R_1}\cdot\E[W] \nonumber\\
\label{eq:yt_limit_Edelay}
&=
\frac{
\frac{\f(\b)\Phi(\eta)}{\b^2} +
 \left(\frac{\b}{r}-\frac{\g}{\sqrt{r}}-\frac{1}{\b}\right)\,\frac{\f(\sqrt{\eta^2+\b^2})}{\b}\, {\rm e}^{\tfrac{1}{2}\omega^2}\, \Phi(\omega) 
 - \sqrt{\frac{1-r}{r}}\,\frac{\f(\b)\f(\eta)}{\b}
}{
\int_{-\iy}^\b \Phi\left(\frac{\g-t\sqrt{r}}{\sqrt{1-r}}\right)\, \dd\Phi(t) +
\frac{\f(\b)\Phi(\eta)}{\b} -  \frac{\f(\sqrt{\b^2+\eta^2})}{\b}{\rm e}^{\tfrac{1}{2} \omega^2} \Phi(\omega)
 },
\end{align}
%
and if $\b=0$,
\begin{align}
g^b_0(\g) 
&:= \lim_{\l\to\iy} \P^b({\rm delay}) \nonumber\\
\label{eq:yt_limit_delay_beta0}
&=
\left(1+
\frac{
\int_{-\iy}^0 \Phi\left(\frac{\g-t\sqrt{r}}{\sqrt{1-r}}\right)\, \dd\Phi(t)
}{
\sqrt{\frac{1-r}{r}} \frac{1}{\sqrt{2\pi}}\,\left(\eta \,\Phi(\eta) + \f(\eta) \right)
}
\right)^{-1},\\
f^b_0(\g) 
&:= \lim_{\l\to\iy} \sqrt{R_1}\cdot\P^b({\rm block}) \nonumber \\
\label{eq:yt_limit_block_beta0}
&= 
\frac{
\sqrt{r}\,\f(\g)\Phi(-\omega\sqrt{r}) + \frac{1}{\sqrt{2\pi}} \Phi(\eta)
}{
\int_{-\iy}^\b \Phi\left(\frac{\g-t\sqrt{r}}{\sqrt{1-r}}\right)\, \dd\Phi(t) +
\sqrt{\frac{1-r}{r}} \frac{1}{\sqrt{2\pi}}\,\left(\eta \,\Phi(\eta) + \f(\eta) \right)
 },\\
h_0^b(\g) &:= \lim_{\l\to\iy} \sqrt{R_1}\cdot\E[W] \nonumber\\
\label{eq:yt_limit_Edelay_beta0}
&= \frac{1}{2\mu}\, \frac{ \left( \gamma^2/r+1\right) \Phi(\eta) + \eta \f(\eta) }
{ \frac{r}{1-r} \sqrt{2\pi} \int_{-\infty}^0 \Phi\left(\frac{\g-t\sqrt{r}}{\sqrt{1-r}}\right)\, \dd\Phi(t) + \sqrt{\frac{r}{1-r}} \left(\eta \Phi(\eta)+\f(\eta)\right)},
\end{align}
where $\eta = \frac{\g - \b\sqrt{r}}{\sqrt{1-r}}$ and $\omega := \frac{\g - \b/\sqrt{r}}{\sqrt{1-r}}$.
%\tr{Might it be more clear to present this theorem in terms of $\xi, \zeta_1,\zeta_2$, etc?}
\end{theorem}
The proof of Theorem \ref{thm:limits_YT} is given in Appendix C of \cite{YomTov2010} under a parameter transformation.

Theorem \ref{thm:limits_YT} proves that the scaling \eqref{eq:twofoldscaling} results in QED behavior: the probability of waiting in Equations \eqref{eq:yt_limit_delay} and \eqref{eq:yt_limit_delay_beta0} converges to a limit that is strictly between 0 and 1. 
Notice that all limits in Theorem \ref{thm:limits_YT} are functions of three parameters: $\beta$ and $\gamma$, which are decision variables, and the fraction of needy time $r$, which is dictated by the physics of the system. Furthermore, the theorem also shows that the probability of blocking (Equations \eqref{eq:yt_limit_block} and \eqref{eq:yt_limit_block_beta0}) is of order $1/\sqrt{R_1}$. 
For example, assume that the fraction of needy time $r$ is $0.5$ and the system is large (100 servers). 
Using Figure \ref{fig:pdelay_pblock}, we observe that, by choosing the pair $\gamma = 1$ and $\beta = 0.245$, we actually aim at a probability of getting served immediately to be 40\%. At the same time, the probability of getting immediately a bed is 97\%. 
Thus, waiting inside the ED occurs at a reasonable level, while wait outside the facility becomes negligible. 


\begin{figure}
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale = 0.8]
\small
\begin{axis}[
	xmin = -2,
	xmax = 2,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	tick label style={/pgf/number format/fixed},
	xlabel = $\beta$,
	ylabel = {$g(\beta,\gamma)$},
	y label style = {at = {(axis cs: -2.4,0.5)}},
	xscale = 0.9,
	yscale = 0.75,
	legend cell align=left,
	legend style = {at = {(axis cs: 1.95,0.99)},anchor = north east}
]
%\draw[thick,dashed,->,col1] (axis cs: -2,0.6) -- (axis cs: -1.0633,0.6) -- (axis cs: -1.0633,0.0);
%\draw[thick,dashed,->,col2] (axis cs: -2,0.5) -- (axis cs: -0.35460,0.5) -- (axis cs: -0.35460,0.0);
%\draw[thick,dashed,->,col3] (axis cs: -2,0.4) -- (axis cs: 0.245,0.4) -- (axis cs: 0.245,0);
%\draw[thick,dashed,->,col4] (axis cs: -2,0.3) -- (axis cs: 0.6944,0.3) -- (axis cs: 0.6944,0);


\addplot[thick,col1] table[x=beta,y=g_min1] {Chapter_5/tikz/limit_probabilities_delay.txt};
\addplot[thick,col3] table[x=beta,y=g_0] {Chapter_5/tikz/limit_probabilities_delay.txt};
\addplot[thick,col4] table[x=beta,y=g_1] {Chapter_5/tikz/limit_probabilities_delay.txt};
\addplot[thick,col5] table[x=beta,y=g_2] {Chapter_5/tikz/limit_probabilities_delay.txt};

\legend{{$\gamma = -1$},{$\gamma = 0$},{$\gamma = 1$},{$\gamma = 2$}};
\end{axis}
\end{tikzpicture}
\caption{Delay probability}
\label{fig:pdelay_pblock_a}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale = 0.8]
\small
\begin{axis}[
	xmin = -2,
	xmax = 2,
	ymin = 0,
	ymax = 2,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\beta$,
	tick label style={/pgf/number format/fixed},
	ylabel = {$f(\beta,\gamma)$},
	y label style = {at = {(axis cs: -2.4,1)}},
	xscale = 0.9,
	yscale = 0.75,
	legend cell align=left,
	legend style = {at = {(axis cs: 1.95,1.98)},anchor = north east}
]


\addplot[thick,col1] table[x=beta,y=g_min1] {Chapter_5/tikz/limit_probabilities_block.txt};
\addplot[thick,col3] table[x=beta,y=g_0] {Chapter_5/tikz/limit_probabilities_block.txt};
\addplot[thick,col4] table[x=beta,y=g_1] {Chapter_5/tikz/limit_probabilities_block.txt};
\addplot[thick,col5] table[x=beta,y=g_2] {Chapter_5/tikz/limit_probabilities_block.txt};

%\draw[thick,dashed,->,col1] (axis cs: -1.0633,0.0) -- (axis cs: -1.0633,0.131477) -- (axis cs: -2,0.131477) ;
%\draw[thick,dashed,->,col2] (axis cs: -0.3546,0) -- (axis cs: -0.35460,0.072794) -- (axis cs: -2,0.072794);
%\draw[thick,dashed,->,col3] (axis cs: 0.245,0) -- (axis cs: 0.245,0.0303026) -- (axis cs: -2,0.0303026);
%\draw[thick,dashed,->,col4] (axis cs: 0.6944,0) -- (axis cs: 0.6944,0.00832892) -- (axis cs: -2,0.00832892);


\legend{{$\gamma = -1$},{$\gamma = 0$},{$\gamma = 1$},{$\gamma = 2$}};
\end{axis}
\end{tikzpicture}
\caption{Scaled blocking probability}
\label{fig:pdelay_pblock_b}
\end{subfigure}
\caption{Asymptotic delay and scaled blocking probability for $r=0.5$ based on Theorem \ref{thm:limits_YT}. }
\label{fig:pdelay_pblock}
\end{figure}


Theorem \ref{thm:limits_YT} further shows that the expected waiting (Equations \eqref{eq:yt_limit_Edelay} and \eqref{eq:yt_limit_Edelay_beta0})
is of order $1/\sqrt{R_1}$ too and hence vanishes in the large-system limit.

We see from Theorem \ref{thm:limits_YT} that achieving target service levels is always an interplay between $\beta$ and $\gamma$.
Figure \ref{fig:pdelay_pblock_a} shows for instance that in order to keep $\P({\rm delay})\in (0.25,0.75)$,  choosing $\gamma=-1$ requires $\beta$ to stay within the range $[-1.4,-0.5]$, while $\gamma=1$ corresponds to values of $\beta$ in $[-0.4,0.5]$.

While the two-fold scaling rule in \eqref{eq:twofoldscaling} automatically captures the right dimensioning ratio as the system scales up, Theorem \ref{thm:limits_YT} shows that the parameters $\beta$ and $\gamma$ provide a means to fine-tune the performance.
Figure \ref{fig:pdelay_pblock_b} confirms how adding nurses, i.e.~increasing $\beta$, does not improve the blocking probability if the number of beds, i.e.~$\gamma$, is too tight.
This is in accordance with our previous observations in Figure \ref{fig:Rmax} for the exact steady-state distribution.

To test the accuracy of the asymptotic results in Theorem \ref{thm:limits_YT} as approximations in a realistic setting, we plot in Figure \ref{fig:accuracy_blocking} the exact probability of delay and blocking for an Erlang-R model with $R=8$ and $r=0.25$, as a function of $s$. The exact probabilities are given by Equation %\eqref{eq:holding_probability} and 
\eqref{eq:delay_probability}, and their respective asymptotic approximations are based on Theorem \ref{thm:limits_YT}. 
Despite the realistic moderate size of the system ($R=8$), we see that the QED approximations are remarkably accurate for many settings $(s,n)$. 
This fast relaxation is in line with observations made earlier in the QED literature \cite{Borst2004,Janssen2011}.
\begin{table}[htb]
\centering
\begin{tabular}{|r|rrrr|}
\hline
		&	$\mu$	&	$\d$	&	$p$	&	$r$ \\
\hline
Case 1  &   1   & 0.10 & 0.90 & 0.10 \\
Case 2 	& 	1	& 0.25 &  0.75 &  0.25\\
Case 3  &   1	& 0.50  &  0.50  &  0.50 \\
\hline
\end{tabular}
\caption{Parameter settings for numerical experiments.}
\label{tab:parameter_settings}
\end{table} 


\begin{table}[h] \centering
\begin{tabular}{|r|rrr|rrr|}
\cline{2-7}\multicolumn{1}{r|}{} & \multicolumn{3}{c|}{$\beta = 1,\ \g = 1$} & \multicolumn{3}{c|}{$\beta = 1,\ \g = 2$} \bigstrut\\
\hline
$R_1$   & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.1270 & 0.0900 & 0.2283 & 0.1553 & 0.0212 & 0.1085 \bigstrut[t]\\
10    & 0.1340 & 0.0910 & 0.1919 & 0.1628 & 0.0206 & 0.1205 \\
25    & 0.1981 & 0.0945 & 0.1614 & 0.2356 & 0.0216 & 0.2145 \\
50    & 0.1513 & 0.0963 & 0.1588 & 0.1830 & 0.0205 & 0.1496 \\
100   & 0.1880 & 0.0956 & 0.1532 & 0.2231 & 0.0224 & 0.2055 \\
250   & 0.1797 & 0.0971 & 0.1399 & 0.2143 & 0.0219 & 0.2057 \\
\hline
\multicolumn{1}{r|}{} & \textit{0.1767} & \textit{0.0981} & \textit{0.1437} & \textit{0.2108} & \textit{0.0217} & \textit{0.1947} \bigstrut[b]\\
\cline{2-7}\end{tabular}%
\vspace{5mm}
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{tabular}{|r|rrr|rrr|}
\cline{2-7}\multicolumn{1}{r|}{} & \multicolumn{3}{c|}{$\beta = 2,\ \g = 1$} & \multicolumn{3}{c|}{$\beta = 2,\ \g = 2$} \bigstrut\\
\hline
$R_1$   & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0237 & 0.0868 & 0.0282 & 0.0322 & 0.0192 & 0.0391 \bigstrut[t]\\
10    & 0.0206 & 0.0872 & 0.0188 & 0.0278 & 0.0183 & 0.0264 \\
25    & 0.0277 & 0.0876 & 0.0123 & 0.0363 & 0.0174 & 0.0174 \\
50    & 0.0185 & 0.0913 & 0.0116 & 0.0249 & 0.0175 & 0.0166 \\
100   & 0.0232 & 0.0888 & 0.0103 & 0.0303 & 0.0183 & 0.0145 \\
250   & 0.0203 & 0.0905 & 0.0079 & 0.0267 & 0.0179 & 0.0109 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{} & \textit{0.0188} & \textit{0.0914} & \textit{0.0084} & \textit{0.0247} & \textit{0.0177} & \textit{0.0118} \bigstrut\\
\cline{2-7}\end{tabular}%

\caption{Numerical results for Erlang-R model with blocking for Case 1.}
\label{tab:numerics_case1}
\end{table}
\begin{table}[h] \centering
\begin{tabular}{|r|rrr|rrr|}
\cline{2-7}\multicolumn{1}{r|}{} & \multicolumn{3}{c|}{$\beta = 1,\ \g = 1$} & \multicolumn{3}{c|}{$\beta = 1,\ \g = 2$} \bigstrut\\
\hline
$R_1$   & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0911 & 0.1538 & 0.0479 & 0.1431 & 0.0345 & 0.0909 \bigstrut[t]\\
10    & 0.1010 & 0.1498 & 0.0560 & 0.1520 & 0.0326 & 0.1025 \\
25    & 0.1594 & 0.1509 & 0.1058 & 0.2192 & 0.0405 & 0.1785 \\
50    & 0.1201 & 0.1506 & 0.0726 & 0.1697 & 0.0381 & 0.1248 \\
100   & 0.1514 & 0.1539 & 0.1001 & 0.2088 & 0.0398 & 0.1704 \\
250   & 0.1459 & 0.1524 & 0.0957 & 0.2003 & 0.0397 & 0.1618 \\
\hline
\multicolumn{1}{r|}{} & \textit{0.1429} & \textit{0.1569} & \textit{0.0940} & \textit{0.1976} & \textit{0.0391} & \textit{0.1617} \bigstrut[b]\\
\cline{2-7}\end{tabular}%

\vspace{5mm}

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{tabular}{|r|rrr|rrr|}
\cline{2-7}\multicolumn{1}{r|}{} & \multicolumn{3}{c|}{$\beta = 2,\ \g = 1$} & \multicolumn{3}{c|}{$\beta = 2,\ \g = 2$} \bigstrut\\
\hline
$R_1$   & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0130 & 0.1484 & 0.0044 & 0.0277 & 0.0294 & 0.0109 \bigstrut[t]\\
10    & 0.0121 & 0.1432 & 0.0042 & 0.0244 & 0.0267 & 0.0098 \\
25    & 0.0182 & 0.1383 & 0.0070 & 0.0319 & 0.0295 & 0.0141 \\
50    & 0.0119 & 0.1415 & 0.0043 & 0.0216 & 0.0301 & 0.0090 \\
100   & 0.0154 & 0.1413 & 0.0059 & 0.0270 & 0.0290 & 0.0119 \\
250   & 0.0136 & 0.1403 & 0.0051 & 0.0236 & 0.0291 & 0.0103 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{\textit{}} & \textit{0.0126} & \textit{0.1445} & \textit{0.0048} & \textit{0.0220} & \textit{0.0284} & \textit{0.0097} \bigstrut\\
\cline{2-7}\end{tabular}%
\caption{Numerical results for Erlang-R model with blocking for Case 2.}
\label{tab:numerics_case2}
\end{table}

\begin{table}[h] \centering
% Table generated by Excel2LaTeX from sheet 'Sheet4'
% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{tabular}{|r|rrr|rrr|}
\cline{2-7}\multicolumn{1}{r|}{} & \multicolumn{3}{c|}{$\beta = 1,\ \g = 1$} & \multicolumn{3}{c|}{$\beta = 1,\ \g = 2$} \bigstrut\\
\hline
$R_1$   & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0547 & 0.1945 & 0.0221 & 0.1181 & 0.0604 & 0.0617 \bigstrut[t]\\
10    & 0.0579 & 0.2158 & 0.0237 & 0.1325 & 0.0526 & 0.0746 \\
25    & 0.1113 & 0.2086 & 0.0544 & 0.1959 & 0.0641 & 0.1311 \\
50    & 0.0813 & 0.2050 & 0.0363 & 0.1523 & 0.0562 & 0.0933 \\
100   & 0.1060 & 0.2146 & 0.0509 & 0.1873 & 0.0632 & 0.1250 \\
250   & 0.1006 & 0.2179 & 0.0475 & 0.1820 & 0.0596 & 0.1214 \\
\hline
\multicolumn{1}{r|}{} & \textit{0.1011} & \textit{0.2185} & \textit{0.0478} & \textit{0.1792}& \textit{0.0605} & \textit{0.1199} \bigstrut[b]\\
\cline{2-7}\end{tabular}%

\vspace{5mm}

% Table generated by Excel2LaTeX from sheet 'Sheet4'
\begin{tabular}{|r|rrr|rrr|}
\cline{2-7}\multicolumn{1}{r|}{} & \multicolumn{3}{c|}{$\beta = 2,\ \g = 1$} & \multicolumn{3}{c|}{$\beta = 2,\ \g = 2$} \bigstrut\\
\hline
$R_1$   & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\P({\rm b})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0034 & 0.1888 & 0.0009 & 0.0175 & 0.0510 & 0.0057 \bigstrut[t]\\
10    & 0.0030 & 0.2093 & 0.0008 & 0.0172 & 0.0416 & 0.0058 \\
25    & 0.0070 & 0.1937 & 0.0020 & 0.0243 & 0.0440 & 0.0089 \\
50    & 0.0043 & 0.1946 & 0.0011 & 0.0163 & 0.0414 & 0.0056 \\
100   & 0.0061 & 0.1999 & 0.0017 & 0.0207 & 0.0431 & 0.0076 \\
250   & 0.0052 & 0.2037 & 0.0014 & 0.0185 & 0.0401 & 0.0067 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{} & \textit{0.0052} & \textit{0.2039} & \textit{0.0014} & \textit{0.0173} & \textit{0.0404} & \textit{0.0063} \bigstrut\\
\cline{2-7}\end{tabular}%

\caption{Numerical results for Erlang-R model with blocking for Case 3.}
\label{tab:numerics_case3}
\end{table}

We furthermore compare the asymptotic delay and blocking probability in the three scenarios given in Table \ref{tab:parameter_settings}. 
In Tables \ref{tab:numerics_case1}--\ref{tab:numerics_case3} we compute the exact probabilities of delay and blocking through the explicit forms in \eqref{eq:delay_probability} for increasing values of the offered load, $R_1$.

The numerical results show that $g^b(\b,\g)$, $f^b(\b,\g)$ and $h^b(\b,\g)$ provide accurate approximations to $\P({\rm delay})$, $\sqrt{R_1}\P({\rm block})$ and $\sqrt{R_1}\,\E[W]$ in pre-limit systems.
The quality of the approximations increases with $R_1$.  
Naturally, fluctuations occur for relatively small values of $R_1$, because $s$ and $n$ need to be rounded to an integer. 

\begin{figure}
\centering
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.87]
\small
\begin{axis}[
	xmin = 0,
	xmax = 16,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $s$,
	xscale = 0.9,
	yscale = 0.75,
	legend cell align=left,
	legend style = {at = {(axis cs: 0.1,0.01)},anchor = south west}
]
 

\addplot[thick,col1,mark = *] table[x=s,y=n24] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col2,mark = *] table[x=s,y=n28] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col3,mark = *] table[x=s,y=n32] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col4,mark = *] table[x=s,y=n36] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col5,mark = *] table[x=s,y=n40] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};

\addplot[thick,col1,dashed] table[x=s,y=approx_n24] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col2,dashed] table[x=s,y=approx_n28] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col3,dashed] table[x=s,y=approx_n32] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col4,dashed] table[x=s,y=approx_n36] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};
\addplot[thick,col5,dashed] table[x=s,y=approx_n40] {Chapter_5/tikz/accuracy/accuracy_pdelay_case2.txt};

\legend{{$n=24$},{$n=28$},{$n=32$},{$n=36$},{$n=40$}};
\end{axis}
\end{tikzpicture}
\caption{Delay probability}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.87]
\small
\begin{axis}[
	xmin = 0,
	xmax = 16,
	ymin = 0,
	ymax = 2,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $s$,
	xscale = 0.9,
	yscale = 0.75,
	legend cell align=left,
	legend style = {at = {(axis cs: 0.1,0.01)},anchor = south west}
]
 

\addplot[thick,col1,mark = *] table[x=s,y=n24] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col2,mark = *] table[x=s,y=n28] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col3,mark = *] table[x=s,y=n32] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col4,mark = *] table[x=s,y=n36] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col5,mark = *] table[x=s,y=n40] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};

\addplot[thick,col1,dashed] table[x=s,y=approx_n24] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col2,dashed] table[x=s,y=approx_n28] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col3,dashed] table[x=s,y=approx_n32] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col4,dashed] table[x=s,y=approx_n36] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};
\addplot[thick,col5,dashed] table[x=s,y=approx_n40] {Chapter_5/tikz/accuracy/accuracy_pblock_case2.txt};

\legend{{$n=24$},{$n=28$},{$n=32$},{$n=36$},{$n=40$}};
\end{axis}
\end{tikzpicture}
\caption{Scaled blocking probability}
\end{subfigure}
%\begin{subfigure}{0.32\textwidth}
%
%\caption{Scaled expected wait}
%\end{subfigure}
\caption{Comparison of exact performance measures (solid) against asymptotic approximations (dashed) with $\beta=(s-R_1)/\sqrt{R_1}$ and $\gamma=(n-R_1/r)/\sqrt{R_1/r}$ for $\lambda = 2$, $\mu=1$, $\delta=0.25$ and $p=0.75$.}
\label{fig:accuracy_blocking}
\end{figure}


\subsection{QED limits for Erlang-R with holding}
\label{sec:QED_limit_holding}

As explained in Section \ref{sec:QED_scaling}, the model with holding has no product-form steady-state distribution, which makes it hard (if not impossible) to obtain QED limits.
Instead, we derive QED approximations by exploiting a connection with the blocking model. 

We first prove that under scaling \eqref{eq:twofoldscaling}, the upper bound on the utilization level of the nurses needed to achieve stability in the model with holding, as given in Proposition \ref{prop:StabilityCondition}, converges to unity as $R\to\infty$. 
This facilitates high utilization levels of both nurses and beds, a key characteristic of the QED regime.

\begin{proposition}\label{prop:stability_convergence}
Let $s$ and $n$ scale with $R_1\to\infty$ as in \eqref{eq:twofoldscaling}. Then for $\l\to\infty$,
\[
\rho_{\max}(s,n) \to 1.
\]
\end{proposition}

The proof can be found in Appendix \ref{app:proof_stability_convergence}. 
Combining Proposition \ref{prop:stability_convergence} with Proposition \ref{prop:StabilityCondition} shows that indeed the scaling we use results in a highly utilized system.

As observed before, the nature of the two variants of the model is similar up to the fact that a fraction of the patients is deferred on arrive in the setting with blocking, whereas all the arriving patients are eventually admitted into the system in the holding model. 
This implies that, given $s$ and $n$, the nurses face an increased workload in case of a holding room. 
In fact, Theorem \ref{thm:limits_YT} shows that the blocking probability is of order $1/\sqrt{R_1}$, yielding a volume of blocked patients of order $\sqrt{R_1}$ in setting with blocking. 
Accordingly, if $R^b = R_1$ and $R^h$ denote the nominal load arriving to the nurses in the model with blocking and holding, respectively, we can argue that 
\[R^h = R^b + \a \sqrt{R^b} + o(\sqrt{R^b}),\] 
for some $\a>0$. 
Notice that this additional load is of the same order as the safety staffing in the blocking model staffing rule \eqref{eq:twofoldscaling}. 
As $s$ and $n$ remain unchanged, we rewrite \eqref{eq:twofoldscaling} in terms of $R^h$,
\begin{align}
s &= R^h + (\b-\a)\sqrt{R^h} + o(\sqrt{R^h}), \nonumber \\
n &= \frac{R^h}{r} + \left(\g-\a/\sqrt{r}\right)\sqrt{\frac{R^h}{r}} + o(\sqrt{R^h}),
\label{eq:fixed_point_scaling}
\end{align} 
where we have used $R^b = O(R^h)$.
Observe that the square-root principle prevails also after this substitution, albeit with different hedging parameters.
We therefore heuristically argue that the holding model under scaling \eqref{eq:twofoldscaling} with parameters $\b$ and $\g$ mimics the blocking model with parameters $\b-\a$ and $\g-\a/\sqrt{r}$, respectively. 

Observe, however, that we have not yet specified the value of $\a$. 
By definition, $\a\sqrt{R^b}$ is the expected volume of patients that would be rejected in the model with blocking, that is, $R^h$ times the probability of not being admitted to the ED directly. 
By the construction in \eqref{eq:fixed_point_scaling}, this volume asymptotically equals $R^h \cdot \P^b({\rm block})$, with parameters $\b-\a$ and $\g-\a/\sqrt{r}$, which by Theorem \ref{thm:limits_YT} is approximated by
\[f^b\left(\b-\a,\gamma-\a/\sqrt{r}\right) / \sqrt{R^h}\]
as $R^h$ grows large.
In conclusion, $\a$ is characterized as the solution of the fixed-point equation
\begin{equation}
 \label{eq:fixedpoint}
 \a = f^h\left(\b-\a,\gamma-\a/\sqrt{r}\right),
 \end{equation} 
 and as a result, we are able to approximate the nurse delay probability in the Erlang-R model with holding as
 \begin{equation}
 \P^h({\rm delay}) \approx g^b(\b-\a,\g-\a/\sqrt{r}) =: g^h(\b,\g).
 \label{eq:fixed_point_Pwait}
 \end{equation}
Likewise, the scaled the mean waiting time for a nurse can be approximated by
 \begin{equation}
 \sqrt{R_1} \cdot \E[W] \approx h^b(\b-\a,\g-\a/\sqrt{r}) =: h^h(\b,\g).
 \label{eq:fixed_point_Ewait}
 \end{equation}

This also implies that the holding queue is $O(\sqrt{R_1})$.
Subsequently, we argue that the expected holding time (pre-entering wait) under the QED policy is $O(1/\sqrt{R_1})$ and hence asymptotically negligible. 
We justify this claim numerically in Section \ref{sec:analysis_chapter5}. 

\begin{remark}
\label{rem:holding_limit}
Notice that in the reasoning leading to \eqref{eq:fixedpoint}, we implicitly assumed that the additional volume $\a\sqrt{R^b}$ is an independent Poisson process, which is obviously not the case. Therefore, \eqref{eq:fixed_point_Pwait}-\eqref{eq:fixed_point_Ewait} are approximations for pre-limit systems that are not asymptotically correct as $R_1\to\iy$.
Nevertheless, we heuristic approach seems to performs well as we confirm numerically next. 
\end{remark} 
 
In Figure \ref{fig:accuracy_holding}, we repeat the numerical experiments of Figure \ref{fig:accuracy_blocking} for the model with holding. 
Since the heuristic does not provide an approximation for the holding probability, Figure \ref{fig:accuracy_holding_b} only plots the simulated holding probabilities. 
Those are provided to better understand the implication of operational decisions.
Recall that the holding system is only stable (i.e. $\P({\rm hold})<1$) if both $s>R_1=8$ and $n > R_1/r  = 32$.
We nevertheless included the boundary case $n=32$ for illustrative purposes. 
The graphs in Figure \ref{fig:accuracy_holding} show that the heuristic captures the congestion levels well, even for this moderate-size system.

To see how this heuristic approach performs under different settings, and particularly if $R_1\to \infty$, we compare the approximated delay probability in the Erlang-R model with holding as solution of the fixed-point procedure to the outcomes of simulation experiments for the three scenarios in Table \ref{tab:parameter_settings} again. 
We performed 100 runs of length $10^4$ for each parameter setting and all values of $R$, yielding the results presented in Tables \ref{tab:heuristic_case1}--\ref{tab:heuristic_case3}, which are accurate up to a 95\% confidence interval of width $10^{-3}$. 


\begin{table}[h] \centering
\begin{tabular}{|r|rr|rr|}
\cline{2-5}\multicolumn{1}{r|}{} & \multicolumn{2}{c|}{$\b=1,\ \g=1$} & \multicolumn{2}{c|}{$\b=1,\ \g=2$} \bigstrut\\
\hline
$R_1$     & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.1532 & 0.1031 & 0.1628 & 0.1216 \bigstrut[t]\\
10    & 0.1622 & 0.1272 & 0.1697 & 0.1331 \\
25    & 0.2340 & 0.2116 & 0.2413 & 0.2342 \\
50    & 0.1817 & 0.1468 & 0.1890 & 0.1678 \\
100   & 0.2199 & 0.1931 & 0.2304 & 0.2269 \\
250   & 0.2110 & 0.1852 & 0.2176 & 0.2230 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{} & \textit{0.2076} & \textit{0.1777} & \textit{0.2187} & \textit{0.2050} \bigstrut\\
\cline{2-5}\end{tabular}%

\vspace{5mm}

% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{tabular}{|r|rr|rr|}
\cline{2-5}\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{$\b=2,\ \g=1$} & \multicolumn{2}{c|}{$\b=2,\ \g=1$} \bigstrut\\
\hline
$R_1$     & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0310 & 0.0121 & 0.0344 & 0.0148 \bigstrut[t]\\
10    & 0.0267 & 0.0123 & 0.0292 & 0.0128 \\
25    & 0.0348 & 0.0171 & 0.0373 & 0.0184 \\
50    & 0.0240 & 0.0108 & 0.0258 & 0.0125 \\
100   & 0.0293 & 0.0143 & 0.0317 & 0.0163 \\
250   & 0.0256 & 0.0120 & 0.0276 & 0.0145 \\
\hline
\multicolumn{1}{r|}{\textit{}} & \textit{0.0229} & \textit{0.0104} & \textit{0.0257} & \textit{0.0124} \bigstrut[b]\\
\cline{2-5}\end{tabular}%

\caption{Simulated and approximated probability of delay in Erlang-R model with holding for Case 1.}
\label{tab:heuristic_case1}
\end{table}
%
\begin{table}[h]\centering

\begin{tabular}{|r|rr|rr|}
\cline{2-5}\multicolumn{1}{r|}{} & \multicolumn{2}{c|}{$\b=1,\ \g=1$} & \multicolumn{2}{c|}{$\b=1,\ \g=2$} \bigstrut\\
\hline
$R_1$     & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.1327 & 0.0740 & 0.1620 & 0.1096 \bigstrut[t]\\
10    & 0.1446 & 0.0894 & 0.1683 & 0.1207 \\
25    & 0.2204 & 0.1631 & 0.2442 & 0.2203 \\
50    & 0.1694 & 0.1122 & 0.1888 & 0.1507 \\
100   & 0.2098 & 0.1524 & 0.2322 & 0.2111 \\
250   & 0.2033 & 0.1534 & 0.2190 & 0.1979 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{} & \textit{0.1840} & \textit{0.1277} & \textit{0.2109} & \textit{0.1759} \bigstrut\\
\cline{2-5}\end{tabular}%
\vspace{5mm}
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{tabular}{|r|rr|rr|}
\cline{2-5}\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{$\b=2,\ \g=1$} & \multicolumn{2}{c|}{$\b=2,\ \g=1$} \bigstrut\\
\hline
$R_1$     & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0219 & 0.0079 & 0.0322 & 0.0137 \bigstrut[t]\\
10    & 0.0199 & 0.0073 & 0.0284 & 0.0115 \\
25    & 0.0283 & 0.0128 & 0.0375 & 0.0163 \\
50    & 0.0190 & 0.0078 & 0.0255 & 0.0107 \\
100   & 0.0244 & 0.0097 & 0.0314 & 0.0151 \\
250   & 0.0214 & 0.0083 & 0.0272 & 0.0134 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{\textit{}} & \textit{0.0169} & \textit{0.0066} & \textit{0.0234} & \textit{0.0104} \bigstrut\\
\cline{2-5}\end{tabular}%

\caption{Simulated and approximated probability of delay in Erlang-R model with holding for Case 2.}
\label{tab:heuristic_case2}
\end{table}
% Table generated by Excel2LaTeX from sheet 'Sheet6'

\begin{table}
\centering
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{tabular}{|r|rr|rr|}
\cline{2-5}\multicolumn{1}{r|}{} & \multicolumn{2}{c|}{$\b=1,\ \g=1$} & \multicolumn{2}{c|}{$\b=1,\ \g=2$} \bigstrut\\
\hline
$R_1$     & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0977 & 0.0413 & 0.1521 & 0.0851 \bigstrut[t]\\
10    & 0.1070 & 0.0469 & 0.1648 & 0.1028 \\
25    & 0.1926 & 0.1076 & 0.2421 & 0.1874 \\
50    & 0.1431 & 0.0727 & 0.1876 & 0.1342 \\
100   & 0.1855 & 0.1012 & 0.2282 & 0.1714 \\
250   & 0.1775 & 0.0963 & 0.2217 & 0.1765 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{} & \textit{0.1442} & \textit{0.0711} & \textit{0.1981} & \textit{0.1354} \bigstrut\\
\cline{2-5}\end{tabular}%

\vspace{5mm}
% Table generated by Excel2LaTeX from sheet 'Sheet6'
\begin{tabular}{|r|rr|rr|}
\cline{2-5}\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{$\b=2,\ \g=1$} & \multicolumn{2}{c|}{$\b=2,\ \g=1$} \bigstrut\\
\hline
$R_1$     & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ & $\P({\rm d})$ & $\sqrt{R_1}\E[W]$ \bigstrut\\
\hline
5     & 0.0072 & 0.0019 & 0.0250 & 0.0081 \bigstrut[t]\\
10    & 0.0067 & 0.0018 & 0.0235 & 0.0082 \\
25    & 0.0148 & 0.0043 & 0.0325 & 0.0133 \\
50    & 0.0092 & 0.0025 & 0.0217 & 0.0081 \\
100   & 0.0132 & 0.0038 & 0.0277 & 0.0105 \\
250   & 0.0114 & 0.0033 & 0.0246 & 0.0099 \bigstrut[b]\\
\hline
\multicolumn{1}{r|}{\textit{}} & \textit{0.0078} & \textit{0.0022} & \textit{0.0188} & \textit{0.0069} \bigstrut\\
\cline{2-5}\end{tabular}%


\caption{Simulated and approximated probability of delay in Erlang-R model with holding for Case 3.}
\label{tab:heuristic_case3}
\end{table}


We conclude from these tables that the approximation is good. As $R$ increases, the simulated values move closer to the heuristic approximation. Extensive numerical experiments suggest that load is slightly underestimated in the limit. %We observe that the heuristic captures the trend of the delay probability and scaled mean waiting time over many parameter settings, despite being a slight underestimation of the congestion. \tr{(I am not sure what you mean here.)} 
%
The best results in terms of accuracy are attained for small $r$. 
This suggests that the quality of the heuristic method improves as $r$ gets smaller. 
These are exactly the parameter settings for which this model is relevant. 

\begin{remark}
The approximation technique that evolves around the fixed-point\\ \noindent method can be adapted to accommodate balking behavior of external arrivals. If we assume that an arriving patient finding all beds occupied joins leaves the system instantly with probability $1-q$, for some $q\in(0,1)$, independently of the rest of the arrivals, with the same argumentation, the volume of arrivals blocked is still $\a\sqrt{R_1}$, while the volume that will enter the ED eventually is $q\cdot\a\sqrt{R_1}$. Therefore, we may argue that in the QED regime, the system with holding and balking behaves as the system with blocking but with corrected parameters $(\b-q\a,\g-q\a/\sqrt{r})$, where $\a$ satisfies
\begin{equation}
\a = f^b(\b-q\a,\g-q\a/\sqrt{r}).
\end{equation}
Note that the choice of $q$ interpolates between the two system variants with holding ($q=0$) and blocking ($q=1$).
\end{remark}


\begin{figure}[h]
\centering
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.87]
\small
\begin{axis}[
	xmin = 0,
	xmax = 16,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $s$,
	xscale = 0.9,
	yscale = 0.75,
	legend cell align=left,
	legend style = {at = {(axis cs: 0.1,0.01)},anchor = south west}
]
 
\addplot[thick,col3,mark = *] table[x=s,y=sim32] {Chapter_5/tikz/accuracy/accuracy_pdelay_holding_case2.txt};
\addplot[thick,col4,mark = *] table[x=s,y=sim36] {Chapter_5/tikz/accuracy/accuracy_pdelay_holding_case2.txt};
\addplot[thick,col5,mark = *] table[x=s,y=sim40] {Chapter_5/tikz/accuracy/accuracy_pdelay_holding_case2.txt};

\addplot[thick,col3,dashed] table[x=s,y=approx32] {Chapter_5/tikz/accuracy/accuracy_pdelay_holding_case2.txt};
\addplot[thick,col4,dashed] table[x=s,y=approx36] {Chapter_5/tikz/accuracy/accuracy_pdelay_holding_case2.txt};
\addplot[thick,col5,dashed] table[x=s,y=approx40] {Chapter_5/tikz/accuracy/accuracy_pdelay_holding_case2.txt};

\legend{{$n=32$},{$n=36$},{$n=40$}};
\end{axis}
\end{tikzpicture}
\caption{Delay probability}
\label{fig:accuracy_holding_a}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.87]
\small
\begin{axis}[
	xmin = 0,
	xmax = 16,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $s$,
	xscale = 0.9,
	yscale = 0.75,
	legend cell align=left,
	legend style = {at = {(axis cs: 0.1,0.01)},anchor = south west}
]
 
\addplot[thick,col3,mark = *] table[x=s,y=sim32] {Chapter_5/tikz/accuracy/accuracy_holding_probability.txt};
\addplot[thick,col4,mark = *] table[x=s,y=sim36] {Chapter_5/tikz/accuracy/accuracy_holding_probability.txt};
\addplot[thick,col5,mark = *] table[x=s,y=sim40] {Chapter_5/tikz/accuracy/accuracy_holding_probability.txt};

\legend{{$n=32$},{$n=36$},{$n=40$}};
\end{axis}
\end{tikzpicture}
\caption{Holding probability}
\label{fig:accuracy_holding_b}
\end{subfigure}
\caption{Comparison of simulated delay probability (solid) against asymptotic approximations (dashed) with $\beta = (s-R_1)/\sqrt{R_1}$ and $\gamma = (n-R_1/r)/\sqrt{R_1/r}$ for $\lambda = 2$, $\mu=1$, $\delta=0.25$ and $p=0.75$.}
\label{fig:accuracy_holding}
\end{figure}

\section{Dimensioning}
\label{sec:dimensioning}

We will now use the accurate asymptotic approximations of the previous section to define a procedure that determines resource capacity in the restricted Erlang-R models. 
That is, we aim to set the number of nurses $s$ and the number of beds $n$, such that a preset performance level is achieved. 
We take the probability of delay at the Needy queue and the probability of blocking/holding at the pre-entrant queue as the target performance objectives.


\subsection{Capacity setting for Erlang-R with blocking}
\label{sec:dimensioning_block}
In the setting with blocking, we can readily use the asymptotic results of Theorem \ref{thm:limits_YT} to (numerically) find a pair of parameters $(\b^*,\g^*)$ to meet the performance requirements.
For instance, given that we want the delay probability to be at most $\varepsilon$, we first solve the equation $g^b(\b^*,\g^*)=\varepsilon$ and then assign $s = \lceil R_1 + \b^*\sqrt{R_1}\rceil$ and $n = \lceil R_1/r+\g^*\sqrt{R_1/r}\rceil$.  Note that there could be multiple solutions to that problem, i.e.\ there could be multiple combinations of number of beds and number of nurses that can result in the same value of a single performance level.
The ED manager can ultimately decide which of these feasible solutions fits the environment best, for instance taking into account space and cost constraints.

We illustrate the resource allocation decisions in an MU setting, using data originated from two articles: \cite{LS2001} and \cite{GY2011}. Green \& Yankovic describe an MU that has 42 beds, with average occupancy level 78\%, and Average Length of Stay (ALOS) 4.3 days. Lundgren \& Segesten studied nurses' service times in a medical-surgical ward. They found that the average service time in their unit was 15.3 minutes per service, and that the average demand rate for each patient is 0.38 requests per hour. Therefore, we take an average service time of 15 minutes and assume that there are 0.4 requests per hour from each patient. Fitting this data to our model results in the following parameters values: $\lambda =0.32, \mu =4, \delta =0.4$, $p=0.975$ and the fraction of needy time is then approximately $r=0.09$. 
This yields nominal offered load $R_1 = 3.2$ and $R_1/r = 34.4$.


\begin{figure}[h]
\centering
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
	xmin = -2,
	xmax = 2,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\beta$,
	ylabel = {$g(\beta,\gamma)$},
	y label style = {at = {(axis cs: -2.5,0.5)}},
	legend cell align=left,
	legend style = {at = {(axis cs: -1.9,0.05)},anchor = south west},
	xscale = 0.95,
	yscale = 0.9
]

\addplot[thick,col1] table[x=beta,y=delay_gmin1] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking1.txt};
\addplot[thick,col3] table[x=beta,y=delay_g0] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking1.txt};
\addplot[thick,col4] table[x=beta,y=delay_g1] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking1.txt};
\addplot[thick,col5] table[x=beta,y=delay_g2] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking1.txt};

\draw[->,col1,very thick,dashed] (axis cs: -2,0.5) -- (axis cs: -0.0552366,0.5) -- (axis cs: -0.0552366,0);
\draw[->,col2,very thick,dashed] (axis cs: -2,0.5) -- (axis cs: 0.179728,0.5) -- (axis cs: 0.179728,0);
\draw[->,col3,very thick,dashed] (axis cs: -2,0.5) -- (axis cs: 0.359034,0.5) -- (axis cs: 0.359034,0);
\draw[->,col4,very thick,dashed] (axis cs: -2,0.5) -- (axis cs: 0.459825,0.5) -- (axis cs: 0.459825,0);

\legend{$\gamma = -1$, $\gamma =0$,$\gamma=1$, $\gamma=2$}
\end{axis}

\end{tikzpicture}
\caption{Delay probability}
\label{fig:ratio01_delay}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\begin{tikzpicture}[scale = 0.75]
\begin{axis}[
	xmin = -2,
	xmax = 2,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\beta$,
	ylabel = {$f(\beta,\gamma)/\sqrt{R_1}$},
	y label style = {at = {(axis cs: -2.5,0.5)}},
	legend cell align=left,
	legend style = {at = {(axis cs: 1.9,0.95)},anchor = north east},
	xscale = 0.95,
	yscale = 0.9
]

\addplot[thick,col1] table[x=beta,y=delay_gmin1] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking2.txt};
\addplot[thick,col3] table[x=beta,y=delay_g0] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking2.txt};
\addplot[thick,col4] table[x=beta,y=delay_g1] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking2.txt};
\addplot[thick,col5] table[x=beta,y=delay_g2] {Chapter_5/tikz/staffing_example/staffing_example_with_blocking2.txt};


\draw[very thick, col1,dashed,->] (axis cs: -0.0552,0) -- (axis cs: -0.0552,0.292798) -- (axis cs: -2,0.292798);
\draw[very thick,col2,dashed,->] (axis cs: 0.179728,0)  -- (axis cs: 0.179728,0.164903)   -- (axis cs: -2,0.164903);
\draw[very thick,col3,dashed,->] (axis cs:  0.359034,0)  -- (axis cs:  0.359034,0.0705547)   -- (axis cs: -2,0.0705547);
\draw[very thick,col4,dashed,->] (axis cs: 0.459825,0)  -- (axis cs: 0.459825,0.0207909)   -- (axis cs: -2,0.0207909);

\legend{$\gamma = -1$, $\gamma =0$,$\gamma= 1$, $\gamma=2$}
\end{axis}

\end{tikzpicture}
\caption{Blocking probability}
\label{fig:ratio01_block}
\end{subfigure}
\caption{Approximate performance of restricted Erlang-R with blocking for $r \approx 0.09$ and $R_1 = 3.2$, as functions of $\beta$.}
\label{fig:ratio01}
\end{figure}


Figure \ref{fig:ratio01} visualizes the dimensioning procedure for this particular MU. 
The hospital management can find a pair of $n$ and $s$ to meet certain criteria, for example to achieve target delay probability $\varepsilon = 0.5$ with reasonable blocking probability.
Figure \ref{fig:ratio01}a indicates that this target can be achieved by a variety of pairs, for instance $(\beta_1,\gamma_1) = (-0.06,-1)$, $(\beta_2,\gamma_2) = (0.16,0)$, $(\beta_3,\gamma_3) = (0.36,1)$ or $(\beta_4,\gamma_4) = (0.46,2)$, among infinitely many others.
According to Figure \ref{fig:ratio01}b, the pairs named above lead to blocking probabilities 0.293, 0.165, 0.071 and 0.021, respectively. 
If the manager decides that probability of blocking of more than 10 percent is not acceptable, this leaves the choices $(\beta_3,\gamma_3) = (0.36,1)$ or $(\beta_4,\gamma_4) = (0.46,2)$ as candidate parameter pairs.
Using the two-fold square-root staffing rule $s_i = \lceil R_1 + \beta_i \sqrt{R_1}\rceil$ and $n_i = [R_1/r + \gamma\sqrt{R_1/r}]$, this yields feasible staffing levels $(s_3,n_3) = (4,40)$ and $(s_4,n_4)=(5,46)$. 
The ultimate decision to apply any of these solutions can be based on external factors, such as operational costs or space limitations of number of beds.



\subsection{Capacity setting for Erlang-R with holding}
For the holding model, we need a more sophisticated approach, exploiting the asymptotic approximation with the fixed-point equation in \eqref{eq:fixedpoint}.  We propose the following dimensioning procedure to achieve a preset target delay probability at the needy queue.

\begin{algorithm}
\hspace{1cm}\rule{10cm}{1pt}\\
\hspace{1.1cm}\KwIn{Target delay probability $\varepsilon$. Parameters $\l,\m,\d$ and $p$.}
\hspace{1.1cm}\KwOut{Staffing levels $s$ and $n$.}
\vspace{-1mm}
\hspace{1cm}\rule{10cm}{0.5pt}\\
\vspace{-1mm}
\begin{enumerate}
\item[] \hspace{0.5cm} 1. Set $R_1:= \frac{\l}{(1-p)\m}$ and $r = \frac{\d}{\d+p\m}$. 
\item[] \hspace{0.5cm} 2. Determine parameters $(\b^*,\g^*)$ such that $g^b(\b^*,\g^*) = \varepsilon$. 
\item[] \hspace{0.5cm} 3. Set $\b = \b^* + f^b(\b^*,\g^*)$ and $\g = \g^* + f^b(\b^*,\g^*)/\sqrt{r}$.
\item[] \hspace{0.5cm} 4. Return $s = \left\lceil R_1 + \b\sqrt{R_1}\right\rceil$ and $n = \left\lfloor R_1/r + \g \sqrt{R_1/r}\right\rfloor$.
\end{enumerate}
\vspace{-3 mm}
\hspace{1cm}\rule{10cm}{1pt}\\
\vspace{2 mm}
\caption{Stationary dimensioning algorithm for ED with holding.}
\label{alg:stationarydimensioning}
\end{algorithm}

\begin{remark}\label{rem:upperboundHW}
In Step 2 of Algorithm \ref{alg:stationarydimensioning} infinitely many pairs $(\b^*,\g^*)$ satisfy the delay probability equation. 
For practical purposes, it is convenient to fix either $\b^*$ or $\g^*$ beforehand, and then solve $g^b(\b^*,\g^*) = \varepsilon$ for the remaining unknown. 
The preset value should however be chosen with care, since $g^b(\b^*,\g^*)$ is upper bounded by the Halfin-Whitt delay probability formula 
\[g_{\rm HW}(\b^*) = \left( 1 + \frac{\b^* \Phi(\b^*)}{\f(\b^*)}\right)^{-1}.\]
Hence, if $\varepsilon > g_{\rm HW}(\b^*)$, then no feasible solution to $g^b(\b^*,\g^*)=\varepsilon$ exists.
This should be considered when choosing $\beta^*$. 
Furthermore, it is evident from Step 3 that the final values $(\b,\g)$ are always larger than $(\b^*,\g^*)$. 
\end{remark}

%\begin{remark}
%Notice that in Step 4 of Algorithm \ref{alg:stationarydimensioning}, we round the value of $s$ up, while rounding the value of $n$ down. This is related to the empirical findings of the previous section, in which we saw that the heuristic slightly underestimates the delay probability. Since increasing $n$ increases $\Pd$, just as reducing $s$ increases $\Pd$, we hope to diminish this discrepancy.
%\end{remark}
%\begin{remark}
%The adjustments needed for Algorithm \ref{alg:stationarydimensioning} to time-varying environments is given in Section \ref{sec:case_study}. Using that procedure will stabilize probability of waiting in a similar way to \cite{YomTov2014}.
%\end{remark}

We now use the same example as in Section \ref{sec:dimensioning_block} to demonstrate capacity allocation decisions for the model with holding. This can be viewed as the additional capacity the medical unit needs in terms of nurses and beds, in order to account for the fact that patients are waiting in the ED to be admitted instead of being blocked and transferred to a less preferred unit. 
Observe that the holding model leaves less flexibility for management in choosing system parameters due to stability constraints. For example, the policy with $n=30$ ($\gamma=-0.75$) is infeasible in the holding model.
For similar reasons, only nurse staffing levels with $\beta>0$, or $s > R_1=3.2$ are feasible. 


Targeting a delay probability of $0.5$ with $n=40$, Figure \ref{fig:ratio01_hold} shows that operating a MU with holding room requires $\beta = 0.475$ or $s=5$. 
Recall that under the blocking policy, only $s=4$ nurses were needed to achieve a delay probability of $0.5$. 
This example hence shows how the managerial decision to have a holding room, rather than deferring patients to less preferred medical units, requires additional workforce in that unit (as well as the ED). 
This example also shows that the facility with holding room is able to treat fewer patients simultaneously than under blocking constraints, in line with the bounds in Section \ref{sec:bounds} and Conjecture \ref{conj:stochorder}.


\begin{figure}[h]
\centering
\begin{tikzpicture}[scale = 0.8]
\begin{axis}[
	xmin = 0,
	xmax = 2,
	ymin = 0,
	ymax = 1,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\beta$,
	ylabel = {$g^h(\beta,\gamma)$},
	legend cell align=left,
	legend style = {at = {(axis cs: 1.9,0.95)},anchor = north east},
	xscale = 0.95,
	yscale = 0.9
]

\addplot[thick,col5] table[x=beta,y=delay_n35] {Chapter_5/tikz/staffing_example/staffing_example_with_holding1.txt};
\addplot[thick,col4] table[x=beta,y=delay_n40] {Chapter_5/tikz/staffing_example/staffing_example_with_holding1.txt};
\addplot[thick,col1] table[x=beta,y=delay_n45] {Chapter_5/tikz/staffing_example/staffing_example_with_holding1.txt};

\draw[very thick,col4,dashed,->] (axis cs: -2,0.5) -- (axis cs: 0.475,0.5) -- (axis cs: 0.475,0);
%\draw[very thick,col5,dashed,<-] (axis cs: -2,0.178665)  -- (axis cs: 1.044,0.178665)   -- (axis cs: 1.044,0);

\legend{$\gamma = -0.75$, $\gamma =0.102$,$\gamma= 0.955$, $\gamma=1.807$};

\end{axis}
\end{tikzpicture}
\caption{Approximate delay probability of restricted Erlang-R system with holding for $r\approx 0.09$ and $R_1=3.2$ }
\label{fig:ratio01_hold}
\end{figure}


\section{Model analysis and managerial implications}
\label{sec:analysis_chapter5}
In this section, we use the analysis and algorithms developed in earlier sections to gain insights into the importance of the capacity restrictions and patient returns in a restricted Erlang-R system by drawing a comparison to related models studied in the literature. 
\subsection{The influence of patient returns or the role of $r$}
Here we study how the parameter $r$ affects the service level in the restricted Erlang-R model with blocking, on the basis of the asymptotic expressions in Theorem \ref{thm:limits_YT}.

%\cite{YomTov2014} in their analysis of the Erlang-R model concluded that customer returns are influential only in time-varying environments, this was due to the fact that in steady-state the Erlang-R performance coincide with those of an Erlang-C model. Those results are no longer valid when considering customer returns within the restricted Erlang-R model. The capacity constraints cause the performance measures here to differ from their single-station counterpart---a loss model (M/M/s/n).

To better understand the connection with the single-station model and the importance of returns we examine the role of $r$. 
Recall the interpretation of $r$ as the fraction of time a patient is needy during his stay within the system in the idealized scenario with infinite capacity, i.e. for $r\in(0,1)$. 
The case $r=1$ corresponds to the setting in which patients are needy all the time, in this case patients get service in one time.
When $r=1$ the infinite-server queue, describing the number of content patients, disappears from the queueing system and we end up with a standard loss model---$M/M/s/n$ queue---in which capacity is scaled as
\[ s = R_1+\beta\sqrt{R_1}, \qquad n = R_1+\gamma\sqrt{R_1}. \]
This staffing rule only makes sense in case $\beta<\gamma$, since no delay is experienced if $n\leq s$. 
If indeed $\gamma>\beta$, then the asymptotic delay probability and scaled blocking probability are given by \cite{masseywallace},
\begin{align*}
g_B(\beta,\gamma) &= \frac{1-{\rm e}^{-\beta(\gamma-\beta)}}{1-{\rm e}^{-\beta(\gamma-\beta)}+\beta\Phi(\beta)/\f(\beta)}, \\
f_B(\beta,\gamma) &= \frac{\beta{\rm e}^{-\beta(\gamma-\beta)}}{1-{\rm e}^{-\beta(\gamma-\beta)}+\beta\Phi(\beta)/\f(\beta)}. 
\end{align*}


\begin{figure}
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
	xmin = 0,
	xmax = 1,
	ymin = 0,
	ymax = 0.8,
	grid = both,
	xlabel = $r$,
	axis line style={->},
	legend cell align=left,
	legend style={at={(0.98,1.28)},anchor= north east},
	yscale = 0.75
]


\addplot[thick,col1] file {Chapter_5/tikz/influence_r/PdelayB_g1_b025.txt};
\addplot[thick,col3] file {Chapter_5/tikz/influence_r/PdelayB_g1_b05.txt};
\addplot[thick,col4] file {Chapter_5/tikz/influence_r/PdelayB_g1_b1.txt};
\addplot[thick,col5] file {Chapter_5/tikz/influence_r/PdelayB_g1_b2.txt};

\legend{$\beta = 0.25$,$\beta=0.5$,$\beta=1.0$,$\beta=2.0$}
\end{axis}
\end{tikzpicture}
\caption{Delay probability $g^b(\beta,\gamma)$}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
	xmin = 0,
	xmax = 1,
	ymin = 0,
	ymax = 0.4,
	grid = both,
	xlabel = $r$,
	axis line style={->},
	legend cell align=left,
	legend style={at={(0.98,0.05)},anchor= south east},
	yscale = 0.75
]


\addplot[thick,col1] file {Chapter_5/tikz/influence_r/PblockB_g1_b025.txt};
\addplot[thick,col3] file {Chapter_5/tikz/influence_r/PblockB_g1_b05.txt};
\addplot[thick,col4] file {Chapter_5/tikz/influence_r/PblockB_g1_b1.txt};
\addplot[thick,col5] file {Chapter_5/tikz/influence_r/PblockB_g1_b2.txt};
\addplot[thick,dashed] file {Chapter_5/tikz/influence_r/PblockB_g1_inf.txt};
\legend{$\beta = 0.25$,$\beta=0.5$,$\beta=1.0$,$\beta=2.0$}
\end{axis}
\end{tikzpicture}
\caption{Scaled blocking probability $f^b(\beta,\gamma)$.}
\label{fig:influence_of_r_b}
\end{subfigure}
\caption{Asymptotic performance measures as a function of $r$ in the restricted Erlang-R model with blocking for $\gamma=1$.}
\label{fig:influence_of_r}
\end{figure}


We can see that $f^b(\beta,\gamma)$ for increasing $\b$ approaches a lower bound that is a function of $r$. 
To understand this, observe that as $\beta$ grows, delays at the nurse queue vanish. 
Then the sojourn time of an admitted patient only consists of a geometric number of needy and content periods with mean $(1/\mu+p/\delta)/(1-p) = 1/(r\mu(1-p))$. 
The blocking model can in this case be modeled as an $M/G/n/n$ queue, with offered load $\l/(r\mu(1-p)) =R_1/r$, in which the scaled blocking probability is known to be, see \cite{Avram2013},
\[\sqrt{R_1} \, \P({\rm block}) = \sqrt{R_1} \, \frac{(R_1/r)^n/n!}{\sum_{k=0}^n (R_1/r)^k / k!} \to \sqrt{r} \, \frac{\f(\gamma)}{\Phi(\gamma)},\]
as $R_1\to\infty$. 
This function of $r$ is plotted in Figure \ref{fig:influence_of_r_b} as the dashed line.

We observe that in general the probability of blocking increases with $r$, regardless of the capacity constraints on the needy station. 
We can explain this by observing that $r$ influences only $n$ in the QED staffing rule. When $n$ reduces, more patients are blocked. Therefore, if patients spend relatively more time in needy state, which usually indicates services that are less interrupted, blocking will increase. Delays, on the other hand, will decrease in such situations---the minimal delay possible can be achieved if service is given in one time ($r=1$). Returns or interruptions increase delays significantly under QED staffing.


\subsection{Comparing restricted and unrestricted Erlang-R models}
%2. Comparing Erlang-R to model with holding: The difference in the stability conditions and its implication.
%The difference in performance, and its implication on staffing.

Given the expressions for the asymptotic delay probability in the open Erlang-R model, and its restricted versions with blocking and holding, we compare the three policies for various values of $\beta$, $\gamma$ and $r$. 
Figure \ref{fig:comparison_delay} plots the delay probability for blocking ($g^b(\b,\g)$), holding ($g^h(\b,\g)$) and Erlang-R ($g_{\rm HW}(\beta)$) models,  as functions of $\gamma$, while keeping $\beta$ fixed, for three values of $r$. 
We make a couple of observations.
Notice that
\[ g^b(\beta,\gamma) \leq g^h(\beta,\gamma) \leq g_{\rm HW}(\beta) \]
for all $\beta,\gamma>0$ and $r$. 
In that sense, the holding model is an interpolation between the blocking and the open model. 
As expected, the delay probabilities in the restricted models converge to those of the open Erlang-R model, because increasing $\gamma$ is tantamount to lifting the stringent constraints on the system size. Note that the rate of conversion is fast---one can provide probability of waiting close to that of the open model with small values of $\gamma$. Indeed, the fact that when using QED staffing not much of excessive delay results from the beds restriction is important by itself.
Also, we observe that the difference between delay probabilities increases with $r$. 


%\tr{This comparison says that if $r$ is small the blocking, holding and E-R policies essentially have close performance, this agrees with what we saw in Figure 13b that when $r$ is small blocking decreases to 0, hence,  there is no blocking nor outer/pre-entrance wait, and hence the models preforming similarly.  It is not surprising that pen and hold has more wait (this agrees with our bounds). But why open has more wait than hold?  note that for open wait does not change with $r$ but as $r$ increases inner wait reduces. Maybe this is again due to "blocking"---as $r$ increases the ration n/s decreases, i.e. people are more in service, and the space constraints is more "coupled" with the dynamic in the service station, i.e the customers that are blocked are blocked directly from service, hence, as $r$ increases, $n$ relatively decreases, we have more blocking in which the customers are hold in the outer queue, which reduces inner wait. Do we have total wait? }
\begin{figure}
\centering
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale = 0.56]
\begin{axis}[
	xmin = 0,
	xmax = 3,
	ymin = 0,
	ymax = 1,
	axis line style={->},
	axis lines = left,
	xlabel = $\to \gamma$,
	xscale = 0.9,
	yscale = 0.8
]

 	
\addplot[thick,col5,dashed] file {Chapter_5/tikz/comparison/PdelayR_b01.txt};
\addplot[thick,col5,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r01_b01.txt};
\addplot[thick,col5] file {Chapter_5/tikz/comparison/PdelayH_r01_b01.txt};

\addplot[thick,col2,dashed] file {Chapter_5/tikz/comparison/PdelayR_b05.txt};
\addplot[thick,col2,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r01_b05.txt};
\addplot[thick,col2] file {Chapter_5/tikz/comparison/PdelayH_r01_b05.txt};

\addplot[thick,col4,dashed] file {Chapter_5/tikz/comparison/PdelayR_b1.txt};
\addplot[thick,col4,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r01_b1.txt};
\addplot[thick,col4] file {Chapter_5/tikz/comparison/PdelayH_r01_b1.txt};

\end{axis}
\end{tikzpicture}
\caption{$r=0.1$.}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale = 0.56]
\begin{axis}[
	xmin = 0,
	xmax = 3,
	ymin = 0,
	ymax = 1,
	axis line style={->},
	axis lines = left,
	xlabel = $\to \gamma$,
	xscale = 0.9,
	yscale = 0.8
]

 	
\addplot[thick,col5,dashed] file {Chapter_5/tikz/comparison/PdelayR_b01.txt};
\addplot[thick,col5,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r025_b01.txt};
\addplot[thick,col5] file {Chapter_5/tikz/comparison/PdelayH_r025_b01.txt};

\addplot[thick,col2,dashed] file {Chapter_5/tikz/comparison/PdelayR_b05.txt};
\addplot[thick,col2,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r025_b05.txt};
\addplot[thick,col2] file {Chapter_5/tikz/comparison/PdelayH_r025_b05.txt};

\addplot[thick,col4,dashed] file {Chapter_5/tikz/comparison/PdelayR_b1.txt};
\addplot[thick,col4,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r025_b1.txt};
\addplot[thick,col4] file {Chapter_5/tikz/comparison/PdelayH_r025_b1.txt};

\end{axis}
\end{tikzpicture}
\caption{$r=0.25$.}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale = 0.56]
\begin{axis}[
	xmin = 0,
	xmax = 3,
	ymin = 0,
	ymax = 1,
	axis line style={->},
	axis lines = left,
	xlabel = $\to \gamma$,
	xscale = 0.9,
	yscale = 0.8
]

 	
\addplot[thick,col5,dashed] file {Chapter_5/tikz/comparison/PdelayR_b01.txt};
\addplot[thick,col5,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r05_b01.txt};
\addplot[thick,col5] file {Chapter_5/tikz/comparison/PdelayH_r05_b01.txt};

\addplot[thick,col2,dashed] file {Chapter_5/tikz/comparison/PdelayR_b05.txt};
\addplot[thick,col2,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r05_b05.txt};
\addplot[thick,col2] file {Chapter_5/tikz/comparison/PdelayH_r05_b05.txt};

\addplot[thick,col4,dashed] file {Chapter_5/tikz/comparison/PdelayR_b1.txt};
\addplot[thick,col4,mark=*, mark repeat = 2] file {Chapter_5/tikz/comparison/PdelayB_r05_b1.txt};
\addplot[thick,col4] file {Chapter_5/tikz/comparison/PdelayH_r05_b1.txt};

\end{axis}
\end{tikzpicture}
\caption{$r=0.5$.}
\end{subfigure}
\caption{Asymptotic delay probability in open Erlang-R (dashed), restricted Erlang-R with blocking (marked) and restricted Erlang-R with holding (solid), as function of $\gamma$ with $\b=0.1$ (blue), $\b=0.5$ (orange) and $\b=1$ (green) fixed.}
\label{fig:comparison_delay}
\end{figure}


%\begin{figure} \centering
%\centering
%\begin{subfigure}{0.32\textwidth}
%
%\begin{tikzpicture}[scale=0.6]
%
%\begin{axis}[
%	xmin = 0,
%	xmax = 145,
%	ymin = 0.0,
%	ymax = 0.7,
%	ytick = {0,0.1,...,0.7},
%	xlabel = $\l$,
%	ylabel = $\P({\rm delay})$,
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	legend pos = south east
%]
%
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
% 	
%\addplot[thick,col1,mark=*] file {Chapter_5/tikz/empirical/delayProbErlangH.txt};
%\addplot[thick,col2,mark=*] file {Chapter_5/tikz/empirical/delayProbYomTov.txt};
%\addplot[thick,col3,mark=*] file {Chapter_5/tikz/empirical/delayProbJennings.txt};
%\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/delayProbErlangR.txt};
%\small
%\legend{Holding,Blocking,Closed ward,Erlang-R};
%\end{axis}
%
%\end{tikzpicture}
%\caption{Delay probability nurse}
%\end{subfigure}
%\begin{subfigure}{0.32\textwidth}
%
%\begin{tikzpicture}[scale=0.6]
%
%\begin{axis}[
%	xmin = 0,
%	xmax = 145,
%	ymin = 0.0,
%	ymax = 0.3,
%	ytick = {0,{0.05},0.1,0.15,0.2,0.25,3},	
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	xlabel = $\l$,
%	ylabel = {$\E[wait]$},
%	legend pos = north east
%]
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
% 	
%\addplot[thick,col1,mark=*] file {Chapter_5/tikz/empirical/EWErlangH.txt};
%\addplot[thick,col2,mark=*] file {Chapter_5/tikz/empirical/EWYomTov.txt};
%\addplot[thick,col3,mark=*] file {Chapter_5/tikz/empirical/EWJennings.txt};
%\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/EWErlangR.txt};
%\small
%\legend{Holding,Blocking,Closed ward,Erlang-R};
%\end{axis}
%
%\end{tikzpicture}
%\caption{Expected wait}
%\end{subfigure}
%\begin{subfigure}{0.32\textwidth}
%
%\begin{tikzpicture}[scale=0.6]
%
%\begin{axis}[
%	xmin = 0,
%	xmax = 145,
%	ymin = 0.7,
%	ymax = 1.02,
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	xlabel = $\l$,
%	ylabel = $\rho_s$,
%	legend pos = south east
%]
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
% 	
%\addplot[thick,col1,mark=*] file {Chapter_5/tikz/empirical/rhoErlangH.txt};
%\addplot[thick,col2,mark=*] file {Chapter_5/tikz/empirical/rhoYomTov.txt};
%\addplot[thick,col3,mark=*] file {Chapter_5/tikz/empirical/rhoJennings.txt};
%\addplot[thick,col4,mark=*] file {Chapter_5/tikz/empirical/rhoErlangR.txt};
%\small
%\legend{Holding,Blocking,Closed ward,Erlang-R};
%\end{axis}
%
%\end{tikzpicture}
%\caption{Nurse utilization}
%\end{subfigure}
%\caption{Asymptotic behavior of the original Erlang-R model, the restricted versions with holding and blocking, and the closed ward model for $\m=1$, $\d = 0.2$, $p=0.8$ and $\b=\g=0.5$.}
%\label{fig:empiricalAsymptotics1}
%\end{figure}


%3. Comparing all models: The impact of the finite size limitation on inner-wait, LOS, holding-time. (move here the model comparison of Figure 5; add to it Erlang-R or B or both.) Impact of unit on previous unit (holding).

\subsection{The impact of visit number}
\label{subsec:num_visit}
We next reflect on the impact of operational capacity decisions on different patient populations. We measure patient's complexity by the number of times she needs to see the nurse or the physician during her stay. In the ED context, simple-to-treat patients will need to see the physician once, while complex ones will need multiple visits. Hence, we divide the patients into complexity groups by the number of visits in the Needy station. Since the number of visits is geometrically distributed, we have a higher proportion of simple patients than complex ones; that fits well the health care environment.

Figure \ref{fig:wait_by_visit} shows the waiting time in the needy and pre-entring queues, and the total waiting time, as a function $n$ (number of beds), for each complexity group. % given the number of times a patients needs to see the physician for a particular parameter instance. 
Obviously, the expected waiting time in the pre-entring queue decreases with $n$, while the needy waiting time increases.
For patients who require a relative large number of visits of the physician, in this case more than 6, the total needy wait is the dominant part of the total waiting time. Therefore, as $n$ grows, the total waiting time first decreases and then increases.
In fact, Figure \ref{fig:wait_by_visit_b} suggests that there is an optimal number of beds $n$ that minimizes the total wait for each complexity type. 
Thus, size restrictions reduce the length-of-stay of patients with complex health conditions (given that the constraint is not too tight).
On the other hand, this figure also shows that no such $n$ exists for patients who only require little assistance.
Hence, there is no $n$ that improves the sojourn time of all patients in the ED simultaneously. 
This leaves the decision to the hospital manager to weigh the importance of patients of different complexity levels.

\begin{remark}
From a different perspective, note that in queueing systems such as communication systems, the partition of a job to sizable quantities and scheduling those jobs in a similar dynamic to the Erlang-R model became a popular way for increasing throughput. This is because this effectively schedule jobs by their size even though the total job requirements are uncertain. This in fact creates a shortest-job-first policy without prior knowledge of job size \citep{Comte2016}. Considering that perspective we note that the Erlang-R model actually prioritize simple jobs over complex ones. But without restrictions, when load is too high, such procedures may lead to very long LOS of long jobs. The capacity restriction we analyze in this chapter, in both of its versions, limits such delays. Hence, even in cases in which the returns themselves are created by a managerial decision, imposing the additional managerial restriction on entering the system has benefits. 
\end{remark}


\begin{figure}
\centering
\begin{subfigure}{0.38\textwidth}
\centering
\begin{tikzpicture}[scale=0.66]
\begin{axis}[
	xmin = 33,
	xmax = 60,
	ymin = 0,
	ymax = 10,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $n$,
	yscale = 0.8
]

	 	
\addplot[mark=*,black,opacity=0.1] table[x=n,y=in1] {Chapter_5/tikz/inner_vs_outer_wait.txt} node[right,pos=1] {$N=1$};	
\addplot[mark=*,black,opacity=0.2] table[x=n,y=in2] {Chapter_5/tikz/inner_vs_outer_wait.txt};
\addplot[mark=*,black,opacity=0.3] table[x=n,y=in3] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
\addplot[mark=*,black,opacity=0.4] table[x=n,y=in4] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
\addplot[mark=*,black,opacity=0.5] table[x=n,y=in5] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
\addplot[mark=*,black,opacity=0.6] table[x=n,y=in6] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
\addplot[mark=*,black,opacity=0.7] table[x=n,y=in7] {Chapter_5/tikz/inner_vs_outer_wait.txt};
\addplot[mark=*,black,opacity=0.8] table[x=n,y=in8] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
\addplot[mark=*,black,opacity=0.9] table[x=n,y=in9] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
\addplot[mark=*,black,opacity=1] table[x=n,y=in10] {Chapter_5/tikz/inner_vs_outer_wait.txt};	
 	
\addplot[mark=*,col1, thick] table[x=n,y=hold] {Chapter_5/tikz/inner_vs_outer_wait.txt};	

\end{axis}
\end{tikzpicture}
\caption{Expected pre-entering waiting (red) and needy waiting times (black)}
\end{subfigure}
\begin{subfigure}{0.6\textwidth}
\centering
\begin{tikzpicture}[scale=0.66]
\begin{axis}[
	xmin = 33,
	xmax = 60,
	ymin = 0,
	ymax = 10,
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $n$,
	yscale = 0.8,
	legend cell align=left,
	legend style = {at = {(1.05,0.58)}, anchor = west}
%	colorbar,
%	colormap name=mycolor,
%    colorbar style={
%        ylabel={$N$},
%        ytick={1,2,3,4,5,6,7,8,9,10},
%        yticklabel style={
%            text width=2em,
%            align=right
%        }
%    }
]

 	
	 	
\addplot[mark=*,black,opacity=0.1] table[x=n,y=in1] {Chapter_5/tikz/total_wait.txt} node[right,pos=1] {$N=1$};	
\addplot[mark=*,black,opacity=0.2] table[x=n,y=in2] {Chapter_5/tikz/total_wait.txt};
\addplot[mark=*,black,opacity=0.3] table[x=n,y=in3] {Chapter_5/tikz/total_wait.txt};	
\addplot[mark=*,black,opacity=0.4] table[x=n,y=in4] {Chapter_5/tikz/total_wait.txt};	
\addplot[mark=*,black,opacity=0.5] table[x=n,y=in5] {Chapter_5/tikz/total_wait.txt};	
\addplot[mark=*,black,opacity=0.6] table[x=n,y=in6] {Chapter_5/tikz/total_wait.txt};	
\addplot[mark=*,black,opacity=0.7] table[x=n,y=in7] {Chapter_5/tikz/total_wait.txt};
\addplot[mark=*,black,opacity=0.8] table[x=n,y=in8] {Chapter_5/tikz/total_wait.txt};	
\addplot[mark=*,black,opacity=0.9] table[x=n,y=in9] {Chapter_5/tikz/total_wait.txt};	
\addplot[mark=*,black,opacity=1] table[x=n,y=in10] {Chapter_5/tikz/total_wait.txt};	

\legend{{\small $N=1$},{\small $N=2$},{\small $N=3$},{\small $N=4$},{\small $N=5$},{\small $N=6$},{\small $N=7$},{\small $N=8$},{\small $N=9$},{\small $N=10$}};
\end{axis}
\end{tikzpicture}
\caption{Total expected waiting times\\
\quad \\
\quad }
\label{fig:wait_by_visit_b}
\end{subfigure}
\caption{Expected waiting times as a function of $n$ given the number of visits $N$ in the Erlang-R model with holding with $\lambda=2$ $\mu=1$, $\delta=0.25$, $p=0.75$ and $s=9$.}
\label{fig:wait_by_visit}
\end{figure}

\subsection{Case study: comparison of operational decisions}
\label{sec:case_study}
We now illustrate how the managerial decision to operate under a specific operational regime affects ED performance in terms of efficiency and quality-of-care, through a case study. 
The practical environment we investigate is the ED of a moderately-sized hospital, which faces the arrival pattern $\lambda(t)$ plotted in Figure \ref{fig:Case_study_arrival_pattern_a} on a typical workday. 
Other parameters of the model are estimated to be $\mu = 6.67,\ \delta = 2.18$ and $p = 0.76$, so that $r = 0.301$. These parameters were taken from \cite{YomTov2014}. In order to set time-varying staffing levels $s(t)$ and $n(t)$, we adopt the \textit{mean-offered load} (MOL) approximation of the demand process of~\cite{Jennings1996}.
This approach initially presumes infinite capacity to obtain the number of patients $R(t)$ in the queueing system as a function of time. 
This offered load function then replaces (constant) value of $R$ in the stationary dimensioning scheme under consideration, to determine the adequate number of servers at each point in time. 
Following this idea in our two-dimensional queueing system, we find the offered load function for the nurses $R_1(t)$ and the offered load function for the beds $R_1(t)+R_2(t)$ as the solution of the system of ODEs,
\begin{align} \label{eq:offeredloadODE}
\frac{d}{dt} R_1(t) &= \l(t) + \d R_2(t) - \m R_1(t),\\
\frac{d}{dt} R_2(t) &= p\m R_1(t) - \d R_2(t),
\end{align}
see \cite[Thm.~2]{YomTov2014} for details.
For this case study's parameters, these offered load functions are also plotted in Figure \ref{fig:Case_study_arrival_pattern_a}.
%
While the number of nurses can be adjusted in a relatively flexible manner, the value of $n$, which echoes a hard restriction on the ED capacity, is naturally less amenable to fluctuations. The reason is that the maximum ED capacity is to a large extent determined by its hardware, such as beds and medical equipment.
However, the ED manager might deliberately consider reducing $n$ during more quiet periods of the day, e.g.\ during the night, by imposing bed-to-physician constraints. This is done, for example, when setting a case management constraint \citep{EDexperiment,Campello2016}. 
%By doing so, costs of keeping vacant ED beds operational can be reduced, therefore increasing the system efficiency. 
Therefore, we consider the scenario in which both $s$ and $n$ are time-dependent but we do not force a constant case management quantity, rather let our new methodology to recommend an appropriate one. 

\begin{figure} 
\centering
\begin{subfigure}{0.46\textwidth}
\centering
\begin{tikzpicture}[scale=0.6]

\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 45,
	ytick = {0,10,20,30,40},	
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.25,
	yscale=1,
	legend cell align=left,
	legend style = {at = {(0.01,0.95)},anchor = north west}
]

 	
\addplot[very thick,black] file {Chapter_5/tikz/lambdaFunction.txt};
\addplot[very thick,col1] file {Chapter_5/tikz/R1.txt};
\addplot[very thick,col5] file {Chapter_5/tikz/R1R2.txt};

\legend{ $\lambda(t)$, $R_1(t)$, $R_1(t)+R_2(t)$};
\end{axis}
\end{tikzpicture}
\caption{Dynamic arrival rate function offered load functions}
\label{fig:Case_study_arrival_pattern_a}
\end{subfigure}
\begin{subfigure}{0.46\textwidth} 
\centering
\begin{tikzpicture}[scale=0.6]

\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 45,
	ytick = {0,10,20,30,40},	
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.25,
	yscale=1,
	legend cell align=left,
	legend pos = north west
]

 	
\addplot[very thick,col1] file {Chapter_5/tikz/casestudy_new/sFunction.txt};
\addplot[very thick,col5] file {Chapter_5/tikz/casestudy_new/nFunction.txt};

\legend{ $s(t)$, $n(t)$};
\end{axis}
\end{tikzpicture}
\caption{Capacity function for $\beta=\gamma=0.5$}
\label{fig:Case_study_arrival_pattern_b}
\end{subfigure}
\caption{Empirical arrival rate and offered load functions $R_1(t)$ and $R_1(t)+R_2(t)$ in Israeli ED and corresponding capacity functions.}
\label{fig:Case_study_arrival_pattern}
\end{figure}
%
Extrapolating Algorithm \ref{alg:stationarydimensioning} to the time-varying case, Step 4 is replaced by
\begin{align*}
s(t) &= R_1(t) + \b\sqrt{R_1(t)},\\
n(t) &= R_1(t)+R_2(t) + \g\sqrt{R_1(t)+R_2(t)},
\end{align*}
for some $\b,\g>0$. 
%
Since $R_1(t)$ and $R_2(t)$ are given, the QED staffing problem again reduces to finding the pair $(\beta,\gamma)$.
%

Figure \ref{fig:Case_study_arrival_pattern_b} plots the capacity functions for $\beta = 0.5$ and $\gamma=0.5$, assuming capacity can only be adjusted every 30 minutes. 
%
In this case study, we consider three pairs of parameters $(\beta,\gamma)$.
For each of these we investigate, using simulation, the differences in the time-varying performance indicators between the policy with blocking and holding.

\begin{figure}
\centering

\begin{subfigure}{0.32\textwidth}
%% P(delay)
\begin{tikzpicture}[scale=0.47]

\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 1.0,
	ytick = {0,0.2,0.4,0.6,0.8,1.0},	
	xtick = {0,3,6,9,12,15,18,21,24},
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.1,
	yscale=1
]

\addplot[very thick,col1] table[x=t,y=delay_b01g2] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col1,dashed] table[x=t,y=delay_b01g2] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};

\addplot[very thick,col4] table[x=t,y=delay_b1g15] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col4,dashed] table[x=t,y=delay_b1g15] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};

\addplot[very thick,col5] table[x=t,y=delay_b2g1] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col5,dashed] table[x=t,y=delay_b2g1] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};
\end{axis}
\end{tikzpicture}
\caption{$\P({\rm delay})$}
\label{fig:simulation_results_a}
\end{subfigure}
%
\begin{subfigure}{0.32\textwidth}
%% P(hold)
\begin{tikzpicture}[scale=0.47]

\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 0.52,
	ytick = {0,0.1,0.2,0.3,0.4,0.5},
	xtick = {0,3,6,9,12,15,18,21,24},	
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.1,
	yscale=1,
	legend cell align=left,
	legend style = {at = {(0.9,0.95)}, anchor = north east}
]


\addplot[very thick,col1] table[x=t,y=block_b01g2] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col4] table[x=t,y=block_b1g15] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col5] table[x=t,y=block_b2g1] {Chapter_5/tikz/casestudy_new/case_study_block.txt};

\addplot[very thick,col1,dashed] table[x=t,y=block_b01g2] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};
\addplot[very thick,col4,dashed] table[x=t,y=block_b1g15] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};
\addplot[very thick,col5,dashed] table[x=t,y=block_b2g1] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};

\legend{{$(\beta,\gamma)=(0.1,2)$},{$(\beta,\gamma)=(1,1.5)$},{$(\beta,\gamma)=(2,1)$}};
\end{axis}
\end{tikzpicture}
\caption{$\P({\rm block})$ or $\P({\rm hold})$}
\label{fig:simulation_results_b}
\end{subfigure}
%
\begin{subfigure}{0.32\textwidth}
\begin{tikzpicture}[scale=0.47]

\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 5.5,
	xtick = {0,3,6,9,12,15,18,21,24},	
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.1,
	yscale=1
]


\addplot[very thick,col1] table[x=t,y=ratio_b01g2] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col1,dashed] table[x=t,y=ratio_b01g2] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};

\addplot[very thick,col4] table[x=t,y=ratio_b1g15] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col4,dashed] table[x=t,y=ratio_b1g15] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};

\addplot[very thick,col5] table[x=t,y=ratio_b2g1] {Chapter_5/tikz/casestudy_new/case_study_block.txt};
\addplot[very thick,col5,dashed] table[x=t,y=ratio_b2g1] {Chapter_5/tikz/casestudy_new/case_study_hold.txt};
\end{axis}
\end{tikzpicture}
\caption{Nurse-to-patient ratio.}
\label{fig:simulation_results_c}
\end{subfigure}

\caption{Simulation results for case study. Solid and dashed lines represent time-varying performance in the blocking and holding model, respectively.}
\label{fig:simulation_results}
\end{figure}

The simulation results are presented in Figure \ref{fig:simulation_results}. 
Figure \ref{fig:simulation_results_a} shows that the MOL approach for capacity allocation roughly stabilizes the delay probability. 
Figure \ref{fig:simulation_results_b} shows that the fraction of patients not entering the ED on arrival in the blocking model is reasonable for all parameter pairs considered and are ordered according to $\gamma$.
We also see a significant difference with holding.
%There is a significant difference between the probability of not entering immediately in the holding model as opposed to the blocking model, given a certain parameter settings. 
%This implies that the decision to hold patients in a separate room outside the ED has a noteworthy effect on the admission process. 
Observe also that the holding probability drops in the period 8--13, which is exactly the period when the system is experiencing peak offered load. 
Hence, this temporary reduction is in line with our asymptotic findings that the probability of blocking/holding is $O(1/\sqrt{R_1})$.

Finally note that the three parameter settings lead to different nurse-to-patient ratios. 
Clearly, larger $\beta$ leads to small nurse-to-patient ratios (due do larger staffing). 
Figure \ref{fig:simulation_results_c} demonstrates that for $(\beta,\gamma) = (1,1.5)$ and $(\beta,\gamma) = (2,1)$ the difference between the holding policy and the blocking policy is small. However, for $(\beta,\gamma) = (0.1,2)$ we see a significant increase in the ratio during night hours. 
This may be due to the tight nurse schedule, that causes the holding queue to build up just before midnight. 
This queue then empties latter on, causing an increase in workload per nurse in the period 24--7.


To see the direct effect of the size restriction on the queue lengths, we plotted the mean holding and service queue lengths in the holding model as a function of the parameter $\gamma$ in Figure \ref{fig:simulation_queuelengths}.
%
\begin{figure}
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.6]
%%holding
\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 5.2,
	xtick = {0,3,6,9,12,15,18,21,24},	
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.25,
	yscale=1,
	legend cell align=left,
	legend pos = north west
]


\addplot[very thick,col1] file {Chapter_5/tikz/casestudy_new/holdingQueue_g01.txt};
\addplot[very thick,col3] file {Chapter_5/tikz/casestudy_new/holdingQueue_g025.txt};
\addplot[very thick,col4] file {Chapter_5/tikz/casestudy_new/holdingQueue_g05.txt};
\addplot[very thick,col5] file {Chapter_5/tikz/casestudy_new/holdingQueue_g1.txt};

\legend{$\gamma=0.1$, $\gamma=0.25$,$\gamma=0.5$,$\gamma=1$}
\end{axis}
\end{tikzpicture}
\caption{Mean holding queue length}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
%% service
\centering
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
	xmin = 0,
	xmax = 24,
	ymin = 0.0,
	ymax = 15,
	xtick = {0,3,6,9,12,15,18,21,24},	
	grid = both, 
	axis line style={->},
	axis lines = left,
	xlabel = $\to t$,
	xscale=1.25,
	yscale=1,
	legend cell align=left,
	legend style = {at = {(0.82,0.05)},anchor = south east}
]


\addplot[very thick,col1] file {Chapter_5/tikz/casestudy_new/serviceQueue_g01.txt};
\addplot[very thick,col3] file {Chapter_5/tikz/casestudy_new/serviceQueue_g025.txt};
\addplot[very thick,col4] file {Chapter_5/tikz/casestudy_new/serviceQueue_g05.txt};
\addplot[very thick,col5] file {Chapter_5/tikz/casestudy_new/serviceQueue_g1.txt};
\addplot[very thick,dashed] file {Chapter_5/tikz/casestudy_new/serviceQueue_R.txt};
\legend{$\gamma=0.1$, $\gamma=0.25$,$\gamma=0.5$,$\gamma=1$,Erlang-R}
\end{axis}
\end{tikzpicture}
\caption{Mean service queue length}
\end{subfigure}
\caption{Simulated queue length of holding model with different values of $\gamma$.}
\label{fig:simulation_queuelengths}
\end{figure}
%
Note that for all $\gamma$ considered, the holding queue length are, as expected, of a smaller order than the number of patients admitted. 
Also, the holding queue length decreases as we increase $\gamma$. 
The service queue lengths naturally approach the expected queue lengths in the Erlang-R model as $\gamma$ is increased.


%\tr{Add discussion and numerical results: 1. Figure 11b suggests that in order to balance wait one needs to adjust patient-to-physician ratio over the day. How much will we loos in such a system if we defined a fixed ratio that is easier to implement? 2. ED can have few operational settings: 1. block/hold only if beds are unavailable. 2. block/hold if patient-to-physician ratio is limiting. In comparing the two, what are the implication on performance? In what time of day is such decision most pronounced?  }


%\section{Erlang-R with blocking or holding with time-varying arrivals}
%
%\subsection{Modified-offered-load staffing}
%
%Algorithm \ref{alg:stationarydimensioning} determines the capacity needed to deal with a fixed arrival rate.
%However, service system typically face time-varying arrival volumes. 
%In emergency departments the arrival displays peaks during day hours and valleys during the night.
%Let $\l(t)$ represent the periodic arrival rate function.
%We modify now Algorithm \ref{alg:stationarydimensioning} to accommodate for time-varying workloads by use of a \emph{modified offered load} (MOL) approximation \cite{Jennings1996}. 
%The idea behind MOL is as follows. 
%The multi-server queue is approximated by an infinite-server queue, in which the queue length at time $t$ is Poisson distributed with mean \cite{Eick1993}
%\begin{equation}\label{eq:is_approx}
%R(t) = \E\left[\l(t-S_{\rm e})\right] \E[S_{\rm e}],
%\end{equation}
%where $S_{\rm e}$ is the excess service time. 
%Following the earlier QED reasoning in stationary environments, the square-root staffing rule then becomes
%\begin{equation}\label{eq:tv_srs}
%s(t) = R(t)+\b\sqrt{R(t)}
%\end{equation}
%with $\b>0$. 
%
%We exploit this idea in our setting in which we have two queues and two staffing decisions, namely $s(t)$ and $n(t)$.
% 
%First, we assume the system has infinite capacity, that is, there is an infinite number of nurses and beds. 
%Let $R_1(t)$ and $R_2(t)$ denote the expected workload of the nurse queue and the content queue, respectively, in this scenario. 
%Next, note that the arrival rate to the nurse queue consists of the external arrival rate $\l(t)$ and the volume of content patients becoming needy, whereas while arrivals to the content queue are generated by the patients at the nurse queue at rate $p\m$. Using the fact that service times in our setting are exponentially distributed, we get that $R_1(t)$ and $R_2(t)$ satisfies the ODE \cite[Thm.~2]{YomTov2014}
%\begin{align} \label{eq:offeredloadODE}
%\frac{d}{dt} R_1(t) &= \l(t) + \d R_2(t) - \m R_1(t),\\
%\frac{d}{dt} R_2(t) &= p\m R_1(t) - \d R_2(t).
%\end{align}
%For general arrival rate functions, the solution to this system can easily be obtained numerically. 
%Given the offered load functions $R_1(t)$ and $R_2(t)$, we deduce that under unlimited capacity the expected number of patients at the nurse queue is Poisson distributed with mean $R_1(t)$, and the total number of patients occupying a bed is Poisson distributed with mean $R_1(t)+R_2(t)$. 
%In line with \eqref{eq:tv_srs}, we propose the following two-fold staffing rule
%\begin{align*}
%s(t) &= R_1(t) + \b\sqrt{R_1(t)},\\
%n(t) &= R_1(t)+R_2(t) + \g\sqrt{R_1(t)+R_2(t)},
%\end{align*}
%for some $\b,\g>0$. 
%
%In this section we will devote our attention solely to the Erlang-R model with holding. 
%Adjusted procedures for the variant with blocking follow easily by omitting the use of the fixed-point equation when determining the parameters $\b^*$, and $\g^*$.
%
%Just as in Algorithm \ref{alg:stationarydimensioning}, these parameters can be calculated via the fixed-point equation to make the method applicable to the Erlang-R model with blocking/holding in order to achieve a preset performance level in terms of the delay probability. 
%The complete time-varying dimensioning algorithm for Erlang-R with holding is summarized in Algorithm \ref{alg:timevaryingdimensioning}.
%
%\begin{algorithm}\label{alg:timevaryingdimensioning}
%\textsc{Time-varying dimensioning algorithm}.\\
%\textbf{Input}: Target delay probability $\varepsilon$. Parameters $\m,\d$ and $p$ and arrival rate function $\l(t)$.\\
%\textbf{Output}: Time-dependent staffing levels $s(t)$ and $n(t)$.
%\begin{enumerate}[noitemsep]
%\item Compute $R_1(t)$ and $R_2(t)$ through \eqref{eq:offeredloadODE}. 
%\item Determine parameters $(\b^*,\g^*)$ such that $g^b(\b^*,\g^*) = \varepsilon$. 
%\item Set $\b = \b^* + f^b(\b^*,\g^*)$ and $\g = \g^* + f^b(\b^*,\g^*)/\sqrt{r}$.
%\item Return $s(t) = \left\lceil R_1(t) + \b\sqrt{R_1(t)}\right\rceil$ and $n(t) = \left\lfloor R_1(t)+R_2(t) + \g \sqrt{R_1(t)+R_2(t)}\right\rfloor$.
%\end{enumerate}
%\end{algorithm}
%
%\subsection{Case study: an Emergency Department}
%
%Next, we apply the dimensioning algorithm for the Erlang-R model with capacity restrictions to a realistic system. 
%The practical setting we will study is the emergency department of a medium-sized hospital in Israel, which experiences the weekly arrival pattern depicted in Figure \ref{fig:Israeli_ED}.
%
%\begin{figure} \centering
%\begin{tikzpicture}
%
%\begin{axis}[
%	width = 14cm,
%	height = 8 cm,
%	xmin = 0,
%	xmax = 170,
%	ymin = 0.0,
%	ymax = 34,
%	ytick = {0,5,10,15,20,25,30},	
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	xlabel = $t$,
%	ylabel = $\l(t)$,
%	legend pos = north east
%]
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
% 	
%\addplot[very thick] file {Chapter_5/tikz/casestudy_ed/arrival_rate.txt};
%\addplot[very thick,col2] file {Chapter_5/tikz/casestudy_ed/R1_function.txt};
%\addplot[very thick,col3] file {Chapter_5/tikz/casestudy_ed/R1_R2_function.txt};
%\legend{$\l(t)$, $R_1(t)$,$R_1(t)+R_2(t)$};
%\end{axis}
%
%\end{tikzpicture}
%\caption{Arrival rate function $\l(t)$ per hour to Israeli ED.}
%\label{fig:Israeli_ED}
%\end{figure}
%
%It is clear to see that the arrival pattern is roughly similar for weekkdays, albeit slightly elevated the first weekday (Sunday), with two daily peeks, one around 11 am and one around 8 pm.  
%During the weekend the number of arrivals is smaller and the daily pattern is much different. 
%From observations, we deduces the following estimates for the Erlang-R model with holding: $\mu = 10.9$, $\d=2.3$, $p = 0.69697$, which yields $r=0.232394$.
%
%In this case study, we intend to stabilize the ED performance in terms of the probability of delay for a nurse. 
%That is, we choose a service level threshold $\varepsilon \in (0,1)$ and wish to determine staffing levels $s(t)$ and $n(t)$ for each hour of the week, such that a patient arriving to the ED at any time of the week receives the same level of service. 
%
%In the first step, we compute for each threshold $\varepsilon$ a corresponding pair $(\b,\g)$ such that $g^h(\b,\g) = \varepsilon$. 
%In the second step, deduce the staffing levels $s(t)$ and $n(t)$ through two methods, the first naive choice being PSA staffing, which prescribes:
%\begin{align*}
%s(t) &= \left[ \frac{\l(t)}{(1-p)\mu} + \b\sqrt{\frac{\l(t)}{(1-p)\mu}} \right],\\
%n(t) &= \left[ \frac{\l(t)}{(1-p)\mu\, r} + \g\sqrt{\frac{\l(t)}{(1-p)\mu\, r}} \right].
%\end{align*}
%The second approach uses the MOL functions as in Algorithm \ref{alg:timevaryingdimensioning}.
%The MOL function $R_1(t)$ and $R_2(t)$ are plotted in Figure \ref{fig:Israeli_ED} as well. 
%
%Based upon these plotted figures, we see that $R_1(t)$ is mostly in sync with the arrival rate function,
%whereas a noticeable time lag is seen in the offered load for the beds $R_1(t)+R_2(t)$.
%Furthermore, we see that $R_1(t)$ drops as low as 1 during night hours, and reaches as high as 7.5 around Monday 11pm. 
%This causes large fluctuations in the nurse staffing levels. 
%Also, the low offered load during the night hours may cause deterioration of the stabilizing effect of our staffing approach, as it relies on asymptotic QED behavior.
%
%We investigate the quality of both the PSA staffing method and Algorithm \ref{alg:timevaryingdimensioning} using simulation for service targets $\varepsilon = 0.1, 0.2, 0.3$. 
%The resulting values for $\b$ and $\g$ are given in Table \ref{tab:betagamma_star}. Since Algorithm \ref{alg:timevaryingdimensioning} may produce infinitely many pairs $(\b,\g)$, we consider to outcome pairs, in which the value of $\gamma$ differs.
%In all examples, we adjusted staffing levels on the instance of the hour, and simulated 50000 consecutive weeks. 
%The results are plotted in Figures \ref{fig:simresults_01}-\ref{fig:simresults_03}.
%
%\begin{table} \centering
%\centering
%\begin{tabular}{|r||r|r||r|r|}
%\hline 
%$\varepsilon$ & $\b$ & $\g$  & $\b$ & $\g$ \\
%\hline
%0.1 & 1.388 &  2.064 &  1.294 & 0.916 \\
%0.2 & 1.035 &  2.077 &  0.960 & 0.945 \\
%0.3 & 0.804 &  2.097 &  0.742 & 0.985 \\
%\hline
%\end{tabular}
%\caption{Outcomes of step 3 of Algorithm \ref{alg:timevaryingdimensioning} for two initial values $\g^*$.}
%\label{tab:betagamma_star}
%\end{table}
%
%\begin{figure} \centering
%\begin{tikzpicture}
%
%\begin{axis}[
%	width = 12cm,
%	height = 7 cm,
%	xmin = 0,
%	xmax = 170,
%	ymin = 0.0,
%	ymax = 1.0,
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	xlabel = $t$,
%	ylabel = $\P({\rm delay})$,
%	legend pos = north east
%]
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
% 	
%\addplot[very thick,gray] file {Chapter_5/tikz/casestudy_ed/result_PSA_01.txt}; 	
%\addplot[very thick,col1] file {Chapter_5/tikz/casestudy_ed/result_MOL_01.txt};
%%\addplot[very thick,col2] file {Chapter_5/tikz/casestudy_ed/result_MOL_01_gamma1.txt};
%\addplot[very thick,col4] file {Chapter_5/tikz/casestudy_ed/result_MOL_01_gamma025.txt};
%
%\legend{PSA, {MOL $(\b,\g) = (1.388,2.064)$}, {MOL $(\b,\g) =(1.294,0.916)$} };
%\end{axis}
%\end{tikzpicture}
%\caption{Simulated time-varying probability of delay for $\varepsilon=0.1$.}
%\label{fig:simresults_01}
%\end{figure}
%\begin{figure} \centering
%\begin{tikzpicture}
%
%\begin{axis}[
%	width = 12cm,
%	height = 7 cm,
%	xmin = 0,
%	xmax = 170,
%	ymin = 0.0,
%	ymax = 1.0,
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	xlabel = $t$,
%	ylabel = $\P({\rm delay})$,
%	legend pos = north east
%]
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
%\addplot[very thick,gray] file {Chapter_5/tikz/casestudy_ed/result_PSA_02.txt}; 	
%\addplot[very thick,col1] file {Chapter_5/tikz/casestudy_ed/result_MOL_02.txt};
%%\addplot[very thick,col3] file {Chapter_5/tikz/casestudy_ed/result_MOL_02_gamma1.txt};
%\addplot[very thick,col4] file {Chapter_5/tikz/casestudy_ed/result_MOL_02_gamma025.txt};
%\legend{PSA, {MOL $(\b,\g) = (1.035,2.077)$}, {MOL $(\b,\g) =(0.960,0.945)$} };
%\end{axis}
%\end{tikzpicture}
%\caption{Simulated time-varying probability of delay for $\varepsilon=0.2$.}
%\label{fig:simresults_02}
%\end{figure}
%\begin{figure} \centering
%\begin{tikzpicture}
%
%\begin{axis}[
%	width = 12cm,
%	height = 7 cm,
%	xmin = 0,
%	xmax = 170,
%	ymin = 0.0,
%	ymax = 1.0,
%	grid = both, 
%	axis line style={->},
%	axis lines = left,
%	xlabel = $t$,
%	ylabel = $\P({\rm delay})$,
%	legend pos = north east
%]
%
%\definecolor{col1}{rgb}{0.368417, 0.506779, 0.709798}
% 	\definecolor{col2}{rgb}{0.880722, 0.611041, 0.142051}
% 	\definecolor{col3}{rgb}{0.560181, 0.691569, 0.194885}	
% 	\definecolor{col4}{rgb}{0.922526, 0.385626, 0.209179}
% 	
%\addplot[very thick,col1] file {Chapter_5/tikz/casestudy_ed/result_MOL_03.txt};
%%\addplot[very thick,col3] file {Chapter_5/tikz/casestudy_ed/result_MOL_03_gamma1.txt};
%\addplot[very thick,col4] file {Chapter_5/tikz/casestudy_ed/result_MOL_03_gamma025.txt};
%\addplot[thick,gray] file {Chapter_5/tikz/casestudy_ed/result_PSA_03.txt};
%\legend{PSA, {MOL $(\b,\g) = (0.804,2.097)$}, {MOL $(\b,\g) =(0.742,0.985)$} };
%\end{axis}
%\end{tikzpicture}
%\caption{Simulated time-varying probability of delay for $\varepsilon=0.3$.}
%\label{fig:simresults_03}
%\end{figure}
%
%From these figures we immediate note the superiority of Algorithm \ref{alg:timevaryingdimensioning} over the PSA method when focusing on the stabilization of the delay probability. 
%Not only does $\P({\rm delay})$ fluctuate severely over the course of a week under PSA staffing, its weekly average does not even come close to the target delay probability either, which equal 0.221, 0.338 and 0.416, for targets $\varepsilon = 0.1,\, 0.2$ and 0.3, respectively.   
%
%The staffing functions resulting from Algorithm \ref{alg:timevaryingdimensioning} clearly do a better job as stabilizing performance, although we do see that the effect weakens as the target probability grows. 
%We may explain this by that by allowing more congestion to occur in the system, we amount of overcapacity to accommodate the stochastic fluctuation become more tight. Hence, rounding effect become more apparent in these cases, because allocated one nurse more (or less) can have a big effect on the system performance. 
%Nonetheless, for all $\varepsilon$ considered, the performance constraints are, up to a small margin, satisfied by the staffing functions deduced through our algorithm. 
%Namely, the average delay probability achieved equals 0.105, 0.187 and 0.262, for $\varepsilon = 0.1,\, 0.2$ and 0.3, respectively.
%In Appendix \ref{app:casestudy_plus} we conducted the same simulation experiment, but with an increased arrival rate, namely $\l^*(t) = 10\cdot \l(t)$. 
%The weekly arrival pattern is hence maintained, whereas the nominal arrival volume and staffing levels are increased. 
%The figures in Appendix \ref{app:casestudy_plus} show a delay probability that is even more stable than observed in Figures \ref{fig:simresults_01}-\ref{fig:simresults_03}. 
%Hence, the moderate fluctuations can be safely attributed to rounding errors for finite-size systems. 
%Moreover, the delay probability in case of PSA staffing gets even more volatile when increasing the arrival volume.
%\subsection{Case study: second example?}

\section{Conclusion \& future research}
\label{sec:conclusion}

In this chapter we developed and analyzed a queueing network tailored to a health care environment with finite-size restrictions. 
Using the asymptotic approximations, numerical analysis and simulation, we gained insight into staffing problems that arise in EDs, and proposed an efficient, flexible, and easy to implement methodology to dimension medical facilities through a two-fold staffing rule.

The dimensioning scheme we developed provides a powerful and elegant way of finding adequate staffing levels in emergency departments. 
Nonetheless, we see some avenues for further research. 

The asymptotic approximations we developed based enabled us to take the first step towards characterizing the pre-entering queue behavior in the 
QED regime.  
We observed how the holding queue length vanishes at that $1/\sqrt{R_1}$ as $R_1\to\infty$.
Yet, our analysis did not yield explicit characteristics on the holding queue and holding times.
These performance indicators are naturally important to study if one wants to consider the trade-off between waiting time inside the ED and waiting time outside the ED (holding) time. 

Furthermore, it is worthwhile to study the robustness of our approximations against the service and content time distributions. Since the content phase of a patient is modeled after an infinite-server queue, we expect our approximations to be useful for content time distributions beyond the exponential distribution as well, due to distributional insensitivity of the service time in infinite-server queues. For the needy phase, modeled after a multi-server queue, this insensitivity result does not hold and hence this needs further research. 

Finally, the restricted Erlang-R model obviously gives a highly a simplify view of the complex reality of the ED. 
In practice, distinctive features such as a triage system (with patient priorities), patient boarding time and availability of medical equipment may play a decisive role on congestion in EDs.
However, we think the analysis and dimensioning algorithms presented in this chapter can serve as a building block for staffing procedures that do account for these case-specific factors.

\section*{Appendix}

\addcontentsline{toc}{section}{\hspace{7.1mm} Appendix}

\begin{subappendices}

\settocdepth{chapter}


\section{Description of the QBD process}
\label{app:QBDdescription}

\subsection{The QBD-process}
\label{app:theQBDprocess}
We consider the QBD-process $X(t)=(N(t),Q_1(t))$ in stationarity. Let $\nu(i)=\min\{i,s\}\mu$. To determine the (outgoing) transition rates of the process $X$ we distinguish between the following cases:
\begin{itemize}
\item \emph{Transitions from $(0,0)$:} There are no patients in the Emergency Department and thus the only possible occurrence is when a new patient arrives. This results in a transition to $(1,1)$ and occurs with rate $\lambda$.
\item \emph{Transitions from $(i,0), 1 \leq i < n$:} There are exactly $i$ patients assigned to a bed of which none are seen by a nurse. Then either one of those patients becomes needy, or a new patient arrives at the Emergency Department that can immediately be seen by a nurse. The first results in a transition to $(i,1)$ and occurs at rate $i \delta$, and the second results in a transition to $(i+1,1)$ and occurs with rate $\lambda$.
\item \emph{Transitions from $(i,0), i \geq n$:} Again, the only possible transitions arises from either a newly arrived patient or a patient assigned to a bed becoming needy. However, a newly arrived patient finds all beds occupied and needs to wait. Thus, with rate $\lambda$ we have a transition to $(i+1,0)$ and with rate $n \delta$ a transition to $(i,1)$.
\item \emph{Transitions from $(i,i), i < n$:} In this case all patients assigned to a bed are in need of service. With rate $\lambda$ a new patient arrives at the Emergency Department. She joins the (possible) queue to be seen by a nurse immediately, so this results in a transition to $(i+1,i+1)$. Moreover, since there are only $s < n$ nurses, a service completion occurs with rate $\nu(i)$. With probability $p$ the patient turns to the holding phase, so in total we still have $i$ patients with one patient less in queue for a nurse. With probability $1-p$ the patient leaves the Emergency Department, decreasing both $N$ and $Q_1$ by one. In other words, with rate $p \nu(i)$ we have a transition to $(i,i-1)$ and with rate $(1-p)\nu(i)$ we have a transition to $(i-1,i-1)$.
\item \emph{Transitions from $(n,n)$:} Similar to the previous case, we have a transition to $(n,n-1)$ with rate $p s \mu$ and with rate $(1-p)s \mu$ we have a transition to $(n-1,n-1)$. In this case however, a newly arrived patient finds all beds occupied, resulting in a transition to $(n+1,n)$ with rate $\lambda$.
\item \emph{Transitions from $(i,n), i > n$:} We have a transition to $(i+1,n)$ with rate $\lambda$ and a transition to $(i,n-1)$ with rate $p s \mu$. In case that a patient leaves the Emergency Department there are $i-n>0$ patients in the holding room waiting for an available bed. Thus, one of the $i-n$ patients in the holding room is assigned to the available bed in need of service. That is, with rate $(1-p) s \mu$ we have a transition to $(i-1,n)$.
\item \emph{Transitions from $(i,j), 1 \leq j < i  < n$:} There are four possible transitions. First, with rate $\lambda$ there is a new arrival which results in a transition to $(i+1,j+1)$. Second, with rate $(i-j) \delta$ a patient in one of the beds becomes needy, which results in a transition to $(i,j+1)$. Third, with rate $p \nu(j)$ a patient turns to the content state after service completion, which results in a transition to $(i,j-1)$. Last, with rate $(1-p) \nu(j)$ a patient leaves the Emergency Department after service completion, which results in a transition to $(i-1,j-1)$.
\item \emph{Transitions from $(n,j), 1 \leq j  < n$:} This case is similar to the previous one. The only difference arises when a new patient arrives, since all $n$ beds are already occupied. Thus, with rate $\lambda$ we have a transition to $(n+1,j)$.
\item \emph{Transitions from $(i,j), i > n, 1 \leq j  \leq n$:} This case is the previous one, except when a patient leaves the Emergency Department after service completion. Then one of the $(i-n)$ patients in the holding room will be assigned to a bed in need of service. This results in a transition to $(i-1,j)$ with rate $(1-p) \nu(j)$.
\end{itemize}

\noindent
The state space and transition rates of the Erlang-R model with holding are illustrated in Figure~\ref{fig:QBDIllustration}.

\begin{figure}
 \centering
\begin{tikzpicture}[scale=0.7]
\draw[step=1cm,gray!50!,very thin] (0,0) grid (15.5,8.5);
\draw[thick,->] (0,0) -- (15.5,0);
\draw[thick,->] (0,0) -- (0,8.5);
\draw[thick] (0,0) -- (8,8);
\draw[thick,dashed,black!50!] (8,0) -- (8,8);
\draw[thick] (8,8) -- (15.5,8);
\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15}
	\foreach \y in {0,1,2,3,4,5,6,7,8}
    \draw[fill] (\x,\y) circle [radius=0.025];

\node [below left] at (0,0) {$0$};
\node [left] at (0,2) {$j$};
\node [left] at (0,5) {$k$};
\node [left] at (0,8) {$n$};
\node [below] at (6,0) {$i$};
\node [below] at (8,0) {$n$};
\node [above left] at (0,8.5) {$Q_1$}; 
\node [below right] at (15.5,0) {$N$}; 

\path [->,thick,-latex] (0,0) edge [bend right] (1,1);

\path [->,thick,-latex] (3,0) edge (3,1);
\path [->,thick,-latex] (3,0) edge (4,1);

\path [->,thick,-latex] (4,4) edge [bend right] (5,5);
\path [->,thick,-latex] (4,4) edge (4,3);
\path [->,thick,-latex] (4,4) edge [bend right] (3,3);

\path [->,thick,-latex] (6,2) edge (6,3);
\path [->,thick,-latex] (6,2) edge (7,3);
\path [->,thick,-latex] (6,2) edge (6,1);
\path [->,thick,-latex] (6,2) edge (5,1);

\path [->,thick,-latex] (8,5) edge (8,6);
\path [->,thick,-latex] (8,5) edge (8,4);
\path [->,thick,-latex] (8,5) edge (9,5);
\path [->,thick,-latex] (8,5) edge (7,4);

\path [->,thick,-latex] (8,8) edge (8,7);
\path [->,thick,-latex] (8,8) edge [bend right] (7,7);
\path [->,thick,-latex] (8,8) edge [bend left] (9,8);

\path [->,thick,-latex] (11,8) edge (11,7);
\path [->,thick,-latex] (11,8) edge [bend left] (12,8);
\path [->,thick,-latex] (11,8) edge [bend left] (10,8);

\path [->,thick,-latex] (11,0) edge (11,1);
\path [->,thick,-latex] (11,0) edge [bend left] (12,0);

\path [->,thick,-latex] (12,5) edge (12,6);
\path [->,thick,-latex] (12,5) edge (12,4);
\path [->,thick,-latex] (12,5) edge (13,5);
\path [->,thick,-latex] (12,5) edge (11,5);

\node [above] at (12.75,5) {\scriptsize $\lambda$};
\node [above] at (11.25,5) {\scriptsize $(1-p)\nu(k)$};
\node [right] at (12,5.75) {\scriptsize $(n-k)\delta$};
\node [right] at (12,4.25) {\scriptsize $p \nu(k)$};

\node [above] at (6.75,2.25) {\scriptsize $\lambda$};
\node [below] at (5,2) {\scriptsize $(1-p)\nu(j)$};
\node [above] at (6,3) {\scriptsize $(i-j)\delta$};
\node [right] at (6,1.25) {\scriptsize $p \nu(j)$};

\end{tikzpicture}
\caption{Illustration of state space and the transitions for the Erlang-R model with holding.}
\label{fig:QBDIllustration}
\end{figure}

The state space can be partitioned according to its levels, where level $i$ corresponds to a total queue length $N=i$ patients. This results in an infinite-sized matrix consisting of blocks, where each block corresponds to the transition flow from one level to another. Since the only transitions allowed are within the same level or between two adjacent levels in a QBD-process, we obtain a tridiagonal block structure. Each block consists of elements representing the transition rate of one state to another, and therefore each block is a matrix of size at most $(n+1) \times (n+1)$.

For the Erlang-R model with holding this gives the following result. Let $P$ denote the transition matrix of the process $(N(t),Q_1(t))$. We have the boundary levels $\{1,2,...,n\}$ and $P$ is of the form

\[
P = \left( \begin{array}{cccccccccc}
B_{00} & B_{01} & & & & & & & & \\
B_{10} & B_{11} & B_{12} & & & & & & & \\
 & B_{21} & B_{22} & B_{23} & & & & & & \\
 & & \ddots & \ddots &\ddots & & & & & \\
 & & & & & B_{n \, n-1} & & & & \\
 & & & & B_{n-1 \, n} & B_{nn} & A_0 & & & \\
 & & & & & A_2 & A_1 & A_0 & &  \\
 & & & & & & A_2 & A_1 & A_0 & \\
 & & & & & & & \ddots & \ddots & \ddots \\
\end{array} \right),
\]
where $B_{ii} \in \mathbb{R_1}^{(i+1) \times (i+1)}$, $B_{i \, i-1} \in \mathbb{R_1}^{(i+1) \times i}$, $B_{i-1 \, i} \in \mathbb{R_1}^{i \times (i+1)}$, and $A_0,A_1,A_2 \in \mathbb{R_1}^{(n+1)\times(n+1)}$. The matrices of transition rates for the boundary states are given by
\[
B_{00}=(-\lambda), 
\qquad
B_{i-1 \, i} = \left( \begin{array}{ccccc}
0 & \lambda & & &  \\
& \ddots & \lambda & & \\
 & & \ddots & \ddots &\\
 & & & 0 & \lambda  \\
\end{array} \right), 
\]
\[
B_{i \, i-1} = \left( \begin{array}{cccc}
0 & & &   \\
 (1-p)\mu & 0 & &  \\
 & (1-p)\nu(2)& \ddots &  \\
 & & \ddots & 0 \\
 & & & (1-p)\nu(i)\\
\end{array} \right),
\]
and
\[
\scriptsize
B_{ii} = \left(
\begin{array}{ccccccccc}
-(\lambda+i \delta) & i \delta & & & &\\
p \mu & -(\lambda+\mu+(i-1)\delta) & (i-1)\delta & & &\\
& \ddots & \ddots & \ddots & & \\
& & p \nu(i-1) & -(\lambda+\nu(i-1)+\delta) & \delta \\
& & & & p \nu(i) & -(\lambda+\nu(i)) \\
\end{array} \right).
\]
Moreover, the transition rates are given by
\[
A_0 = \left( \begin{array}{ccccc}
\lambda & & & & \\
& \lambda & & & \\
 & & & \ddots & \\
 & & & & \lambda  \\
\end{array} \right)
\]
\[ A_2 = \left( \begin{array}{ccccccc}
0 & & & & & & \\
& (1-p)\mu & & & & & \\
& & 2(1-p)\mu & & & & \\
& & & \ddots & & & \\
& & & & s(1-p)\mu & & \\
& & & & & \ddots & \\
& & & & & & s(1-p)\mu \\
\end{array} \right),
\]
and
\[
\scriptsize
A_1 = \left( \arraycolsep=0.55pt
\begin{array}{cccccccc}
-(\lambda+n \delta) & n \delta & & & & & & \\
p \mu & -(\lambda+\mu+(n-1)\delta) & (n-1)\delta & & & & & \\
& \ddots & \ddots & \ddots & & & & \\
& & s p\mu & -(\lambda+s\mu+(n-s)\delta) & (n-s)\delta & & & \\
& & & \ddots & \ddots & \ddots & & \\
& & & & s p\mu & -(\lambda+s\mu+\delta) & \delta & \\
& & & & & s p\mu & -(\lambda+s\mu)\\
\end{array} \right).
\]

\subsection{Stability condition}
\label{app:stability}
From the general theory of QBD processes \citep{Neuts1981} follows that the Markov process $(N(t),Q_1(t))$ is ergodic (stable) if and only if
\begin{equation}
\pi A_0 e < \pi A_2 e,
\label{eq:QBDstableCondition}
\end{equation}
where $e$ is the all one column vector and $\pi=(\pi_0,...,\pi_n)$ is the equilibrium distribution of the Markov process with generator $A_0+A_1+A_2$. In other words, $\pi$ is such that
\begin{equation}
\begin{array}{ll}
\pi(A_0+A_1+A_2) =0, & \pi e =1,
\end{array}
\label{eq:QBDstableProbabilityVector}
\end{equation}
and
\[
A_0+A_1+A_2 = \qquad\qquad\qquad
\]
\begin{align*} 
{\scriptsize
\left(
\begin{array}{cccccccc}
-n \delta & n \delta & & & & & & \\
p \mu & -(p\mu+(n-1)\delta) & (n-1)\delta & & & & & \\
& \ddots & \ddots & \ddots & & & & \\
& & s p\mu & -(ps\mu+(n-s)\delta) & (n-s)\delta & & & \\
& & & \ddots & \ddots & \ddots & & \\
& & & & p s \mu & -(ps\mu+\delta) & \delta & \\
& & & & & p s \mu & -ps\mu\\
\end{array} \right).
}
\end{align*}

Then $\pi$ must satisfy the balance equations
\begin{align*}
- n \delta \pi_0 + p \mu \pi_1 &= 0, \\
(n-j+1)\delta \pi_{j-1} - (p\nu(j) +(n-j)\delta) \pi_j + p \nu(j+1) \pi_{j+1} &= 0, \\
\delta \pi_{n-1} - p s \mu \pi_n &= 0,
\end{align*}
with $\nu(j)=\min\{j,s\}\mu$, and the normalization condition
\[
\sum_{i=0}^n \pi_i=1.
\]
It is readily verified that
\begin{equation}
\pi_i =
\left\{\begin{array}{ll}
\pi_0 \binom{n}{i} \left(\frac{\delta}{p \mu}\right)^i & \textrm{\normalfont for } 0 \leq i \leq s, \\
\pi_0 \binom{n}{i} \frac{i!}{s!} s^{s-i} \left(\frac{\delta}{p \mu}\right)^i & \textrm{\normalfont for } s+1 \leq i \leq n \\
\end{array} \right.
\label{eq:eqdistr}
\end{equation}
with
\begin{align*}
\pi_0= \left(\sum_{i=0}^{s} \binom{n}{i} \left(\frac{\delta}{p \mu}\right)^i + \sum_{i=s+1}^{n} \binom{n}{i} \frac{i!}{s!} s^{s-i} \left(\frac{\delta}{p \mu}\right)^i \right)^{-1}.
\end{align*}
satisfies the balance equations and the normalization condition.
%\end{proof}

\begin{proposition}
The distribution of the closed two-node Jackson network illustrated in Figure~\ref{fig:Jennings} is given by
\begin{equation}
\hat{\pi_i} =
\left\{\begin{array}{ll}
\hat{\pi}_0 \binom{n}{i} \left(\frac{\delta}{p \mu}\right)^i & \textrm{\normalfont for } 0 \leq i \leq s, \\
\hat{\pi_0} \binom{n}{i} \frac{i!}{s!} s^{s-i} \left(\frac{\delta}{p \mu}\right)^i & \textrm{\normalfont for } s+1 \leq i \leq n \\
\end{array} \right.
\label{eq:eqdistrTwistedJennings}
\end{equation}
with
\begin{align*}
\hat{\pi}_0= \left[\sum_{i=0}^{s} \binom{n}{i} \left(\frac{\delta}{p \mu}\right)^i + \sum_{i=s+1}^{n} \binom{n}{i} \frac{i!}{s!} s^{s-i} \left(\frac{\delta}{p \mu}\right)^i \right]^{-1}.
\end{align*}
\label{prop:CriticalTilburgdistr}
\end{proposition}

\begin{proof}
We have a two-node closed Jackson network, with probability transition matrix
\[
P = \left(
\begin{array}{cc}
1-p & p \\
1 & 0
\end{array} \right).
\]
Let $r_i(m)$ denote the rate of service when there are $m$ patient at queue $i$, so $r_1(m)=\min\{m,s\}$ and $r_2(m)=m$. The throughput vector $\gamma = (\gamma_1,\gamma_2) \in \mathbb{R_1}^2$ must satisfy $\gamma = \gamma P$ and we find that $\gamma=(p,1)$ suffices. From the general theory of Jackson networks, see \cite{Jackson1963}, it follows that the stationary distribution is given by
\begin{align*}
\pi_i = G^{-1} g_1(i) g_2(n-i)
\end{align*}
with
\begin{align*}
\begin{array}{ll}
g_1(i)= \frac{(\gamma_1/\mu)^i}{\prod_{m=1}^i r_1(m)}, & g_2(n-i)= \frac{(\gamma_2/\delta)^{n-i}}{\prod_{m=1}^{n-i} r_2(m)},
\end{array}
\end{align*}
and normalization constant $G= \sum_{i=0}^n g_1(i) g_2(n-i)$. Then,
\begin{align*}
g_1(i) &=  \left\{\begin{array}{ll}
\frac{1}{i! \mu^i} & \textrm{\normalfont for } 0 \leq i \leq s, \\
\frac{1}{s! s^{i-s} \mu^i} & \textrm{\normalfont for } s+1 \leq i \leq n, \\
\end{array} \right.\\
g_2(n-i) &=\frac{1}{(n-i)!} \left(\frac{p}{\delta}\right)^n \left(\frac{\delta}{p}\right)^i,
\end{align*}
and rewriting the expressions yields~\eqref{eq:eqdistrTwistedJennings}.
\end{proof}

\subsection{Stationary distribution}
\label{app:StationaryDistributrion}
Assuming that the stability condition is satisfied, we can determine the unique stationary distribution of the Markov process $(N(t),Q_1(t))$. The vector $\pi_i$ can be written as $\pi_{n+i}= \pi_n G^{i}$ for $i=0,1,...$, where $G$ is the minimal nonnegative solution of the non-linear matrix equation
\begin{equation}
A_0+G A_1 + G^2 A_2=0.
\label{eq:MG-G}
\end{equation}
The balance equations can be written as
\[
\begin{array}{ll}
\pi_{i-1} A_0+ \pi_i A_1 + \pi_{i+1} A_2=0, & i=n+1,n+2,...
\end{array}
\]
and using $\pi_{n+i}= \pi_n G^{i-n}$ for $i=0,1,...$, this find
\[
\begin{array}{ll}
\pi_n G^{i-n-1} \left(A_0+ G A_1 + G A_2\right)=0, & i=n+1,n+2,....
\end{array}
\]

\noindent
Moreover, we have the boundary equations
\begin{align*}
\pi_0 B_{00} + \pi_1 B_{10} &= 0 \\
\pi_0 B_{01} + \pi_1 B_{11} + \pi_2 B_{21} &= 0 \\
\pi_1 B_{12} + \pi_1 B_{22} + \pi_2 B_{32} &= 0 \\
 &\vdots&  \\
\pi_{n-2} B_{n-2 \, n-1} + \pi_{n-1} B_{n-1 \, n-1} + \pi_{n} B_{n \, n-1} &= 0 \\
\pi_{n-1} B_{n-1 \, n} + \pi_{n} B_{nn} + \pi_{n+1} A_2 &= 0, 
\end{align*}
along with the normalization equation
\[
1 = \sum_{i=0}^{\infty} \pi_i e = \sum_{i=0}^{n-1} \pi_i e + \pi_n(I-G)^{-1}e,
\]
where we slightly abuse notation by using $e$ as the all ones vector of appropriate size. We note that the matrix $G$ has a spectral radius less than one and therefore $(I-G)$ is invertible.

These equations provide the tools for finding the equilibrium probabilities. Although it is hard to solve $G$ analytically from Equation~\eqref{eq:MG-G}, it is easy to solve numerically by using the following algorithm (matrix-geometric method). Rewriting~\eqref{eq:MG-G} gives
\[
G=-(A_0+G^2 A_2) A_1^{-1},
\]
where $A_1$ is invertible, since it is a transient generator matrix. Let
\[
G_{k+1}=-(A_0+G_k^2 A_2) A_1^{-1},
\]
starting with $G_k=0$. We note that $G_k \uparrow G$ as $k$ grows to infinity \citep{Neuts1981}. Once $||G_{k+1}-G_{k}||_2$ is below a certain preset threshold, we approximate $G$ by $G_{k+1}$.


\section{Proof of Proposition \ref{thm:stochasticordering}}\label{app:stochastic_ordering}

First, note that by definition of the Erlang-R model with holding, in which no more that $n$ patients can be admitted in the ED simultaneously, that $Q_1^h(t)+Q_2^h(t) \leq n = Q_1^J(t) + Q_2^J(t)$ follows directly. 
Therefore, we only consider the relation between the states in the blocking and holding variants Erlang-R model.

As noted Section \ref{sec:Markov_process}, the model with holding can be characterized as a three-dimensional Markov chain $X^h(t) = (H(t),Q^h_1(t),Q^h_2(t))$ in which the components denote the number of holding, needy and content patients respectively. The Erlang-R model with blocking similarly admits a Markov process description, but with two dimensions, namely $X^b(t) = (Q^b_1(t),Q^b_1(t))$.

We prove the result by constructing a coupling between the Markov processes $X^h$ and $X^b$. Let $Z(t) := \left(\hat{X}^h(t),\hat X^b(t)\right) = \left(\hat{H}(t),\hat{Q}_1^h(t),\hat{Q}_2^h(t),\hat{Q}^b_1(t),\hat{Q}^b_2(t)\right)$.

We first define the transition rates of this five-dimensional Markov process, which naturally only depend on the current state of the system. 
After that we show that the transition rates relevant to $\hat{X}^h(t)$ and $X^{h}(t)$ coincide with those of either $X^h(t)$ or $\hat{X}^b(t)$, respectively. The latter implies that the marginal transitions of $\hat{X}^h(t)$ and $X^b(t)$ (and $\hat{X}^b(t)$ and $X^h(t)$) are equal, and hence so are their probability distribution of the Markov processes. 

Let $Z(t) = (h,\qh,\ch,\qy,\cy)$. While defining the reachable states from this state and associated transition rates, we distinguish four transition types, and further differentiate the transition rates depending on the current state.\\
\\*
\textbf{Arrival.}
Arrivals to occur in both models simultaneously, but are handled differently according to the current queue lengths.
\begin{enumerate}
\item If $\qh+\ch < n$ and $\qy+\cy < n$,
\begin{equation}
\label{eq:arr1}
(h,\qh+1,\ch,\qy+1,\cy) \qquad \text{with rate }\l,
\end{equation}
\item if $\qh+\ch = n$ and $\qy+\cy < n$,
\begin{equation}
\label{eq:arr2}
(h+1,\qh,\ch,\qy+1,\cy) \qquad \text{with rate }\l,
\end{equation}
\item if $\qh+\ch < n$ and $\qy+\cy = n$,
\begin{equation}
\label{eq:arr3}
(h,\qh+1,\ch,\qy,\cy) \qquad \text{with rate }\l,
\end{equation}
\item if $\qh+\ch = n$ and $\qy+\cy = n$,
\begin{equation}
\label{eq:arr4}
(h+1,\qh+1,\ch,\qy,\cy) \qquad \text{with rate }\l,
\end{equation}
\end{enumerate}
 
\noindent \textbf{Departure.}
Basically, we align service completions in the two models, but allow a completion occurring solely in either of one of the two models, only if the queue length in this model is strictly larger than in the other one.
\begin{enumerate}
\item If $\qh \geq \qy$ and $h > 0$
\begin{equation}
\label{eq:dep1}
\left\{
\begin{array}{ll}
(h-1,\qh,\ch,\qy-1,\cy) & \text{with rate }(\qy \wedge s)(1-p)\mu,\\
(h-1,\qh,\ch,\qy,\cy) & \text{with rate }[(\qh \wedge s)-(\qy \wedge s)](1-p)\mu.
\end{array}
\right.
\end{equation}

\item If $\qh < \qy$ and $h > 0$
\begin{equation}
\label{eq:dep2}
\left\{
\begin{array}{ll}
(h-1,\qh,\ch,\qy-1,\cy) & \text{with rate }(\qh \wedge s)(1-p)\mu,\\
(h,\qh,\ch,\qy-1,\cy) & \text{with rate }[(\qy \wedge s)-(\qh \wedge s)](1-p)\mu.
\end{array}
\right.\end{equation}

\item If $\qh \geq \qy$ and $h = 0$
\begin{equation}
\label{eq:dep3}
\left\{
\begin{array}{ll}
(0,\qh-1,\ch,\qy-1,\cy) & \text{with rate }(\qy \wedge s)(1-p)\mu,\\
(0,\qh-1,\ch,\qy,\cy) & \text{with rate }[(\qh \wedge s)-(\qy \wedge s)](1-p)\mu.
\end{array}
\right.\end{equation}

\item If $\qh < \qy$ and $h = 0$
\begin{equation}
\label{eq:dep4}
\left\{
\begin{array}{ll}
(0,\qh-1,\ch,\qy-1,\cy) & \text{with rate }(\qh \wedge s)(1-p)\mu,\\
(0,\qh,\ch,\qy-1,\cy) & \text{with rate }[(\qy \wedge s)-(\qh \wedge s)](1-p)\mu.
\end{array}
\right.\end{equation}
\end{enumerate}

\noindent\textbf{Become content.} 
The differentiation between transitions is similar to those in the \textit{departure} transition type.
\begin{enumerate}
\item If $\qh \geq \qy$,
\begin{equation}
\label{eq:con1}
\left\{
\begin{array}{ll}
(h,\qh-1,\ch+1,\qy-1,\cy+1) & \text{with rate }(\qy \wedge s)p\mu,\\
(h,\qh-1,\ch+1,\qy,\cy) & \text{with rate }[(\qh \wedge s)-(\qy \wedge s)]p\mu.
\end{array}
\right.\end{equation}

\item If $\qh < \qy$,
\begin{equation}
\label{eq:con2}
\left\{
\begin{array}{ll}
(h,\qh-1,\ch+1,\qy-1,\cy+1) & \text{with rate }(\qh \wedge s)p\mu,\\
(h,\qh,\ch,\qy-1,\cy+1) & \text{with rate }[(\qy \wedge s)-(\qh \wedge s)]p\mu.
\end{array}
\right.\end{equation}
\end{enumerate}
\noindent
\textbf{Become needy.}
 \begin{enumerate}
\item If $\ch \geq \cy$,
\begin{equation}
\label{eq:ne1}
\left\{
\begin{array}{ll}
(h,\qh+1,\ch-1,\qy+1,\cy-1) & \text{with rate } \cy\delta,\\
(h,\qh+1,\ch-1,\qy,\cy) & \text{with rate }(\ch-\cy)\delta,\\
\end{array}
\right.\end{equation}

\item If $\ch < \cy$,
\begin{equation}
\label{eq:ne2}
\left\{
\begin{array}{ll}
(h,\qh+1,\ch-1,\qy+1,\cy-1) & \text{with rate } \ch\delta,\\
(h,\qh,\ch,\qy+1,\cy-1) & \text{with rate }(\cy-\ch)\delta,\\
\end{array}
\right.\end{equation}
\end{enumerate}

This set of transitions defines the dynamics of the Markov process $Z(t) = (\hat{X}^h(t),\hat{X}^b(t))$.
Let us now restrict our attention to the transitions in which (at least one of the) first three coordinates of $Z(t)$ changes, that is, the marginal transitions of the process $\hat{X}^h$. 
Let $\hat{X}^h(t) = (h,\qh,\ch)$, then according to the transition scheme above, $\hat{X}^h$ moves to state

\begin{enumerate}
\item If $\qh+\ch < n$ (and hence necessarily $h=0$),
\[
\left\{
\begin{array}{ll}
(0,\qh+1,\ch) & \text{with rate } \l,\\
(0,\qh-1,\ch) & \text{with rate }(\qh\wedge s)(1-p)\mu,\\
(0,\qh-1,\ch+1) & \text{with rate }(\qh\wedge s)p\mu,\\
(0,\qh+1,\ch-1) & \text{with rate }\ch \delta.
\end{array}
\right.\]

\item if $\qh+\ch = n$ and $h=0$,
\[
\left\{
\begin{array}{ll}
(1,\qh,\ch) & \text{with rate } \l,\\
(0,\qh,\ch) & \text{with rate }(\qh\wedge s)(1-p)\mu,\\
(0,\qh-1,\ch+1) & \text{with rate }(\qh\wedge s)p\mu,\\
(0,\qh+1,\ch-1) & \text{with rate }\ch \delta.
\end{array}
\right.\]

\item if $h>0$ (and hence necessarily $\qh+\ch = n$),
\[
\left\{
\begin{array}{ll}
(h+1,\qh,\ch) & \text{with rate } \l,\\
(h-1,\qh,\ch) & \text{with rate }(\qh\wedge s)(1-p)\mu,\\
(h,\qh-1,\ch+1) & \text{with rate }(\qh\wedge s)p\mu,\\
(h,\qh+1,\ch-1) & \text{with rate }\ch \delta.
\end{array}
\right.\]
\end{enumerate}
One can check that these transitions indeed coincide with the transitions in the original holding model, hence $\hat{X}^h(t) \equalD X^h(t)$.

Similarly, when the focusing on transitions of $Z(t)$ that are relevant for $\hat{X}^b(t)$, we deduce the following transition scheme. If $\hat{X}^b(t) = (\qy,\cy)$, then the next move according to the transitions of $Z(t)$ is
\[
\left\{
\begin{array}{ll}
(\qy+\mathbbm{1}_{\{\qy + \cy < n\}},\cy) & \text{with rate } \l,\\
(\qy-1,\cy) & \text{with rate }(\qy\wedge s)(1-p)\mu,\\
(\qy-1,\cy+1) & \text{with rate }(\qy\wedge s)p\mu,\\
(\qy+1,\cy-1) & \text{with rate }\cy \delta.
\end{array}
\right.\]
These transition rates clearly coincide with the original Erlang-R model with blocking, and also hence $\hat{X}^b(t) \equalD X^h(t)$.

Next, we show that under this coupling scheme we have that if $\hat{H}(0) = 0$,  $\hat{Q}_1^h(0)=\hat{Q}_1^b(0)$ and $\hat{Q}_1^h(0)=\hat{Q}^b(0)$ then for all $t\geq 0$, $Z(t)$ satisfies the hypothesis:
\begin{itemize}
\item[(i)] $\hat{Q}_1^b(t) + \hat{Q}_2^b(t) \leq \hat{Q}_1^h(t) + \hat{Q}_2^h(t)$,
\item[(ii)] $\hat{Q}_2^b(t) \leq \hat{Q}_2^h(t)$,
\item[(iii)] $\hat{Q}_1^b(t) \leq \hat{Q}_1^h(t) + H(t)$.
\end{itemize}
We do so by induction on the next state reached after a transition of the joint Markov process $Z=(\hat{X}^h,\hat{X}^b)$.
First of all, $Z(0)$ clearly satisfies (i)-(iii). 
Next, assume $Z(t^-) = (h,\qh,\ch,\qy,\cy)$ satisfies the hypothesis and a transition occurs at $t$. 
We show that under the specified coupling scheme, the state reached after the next transition, $Z(t)$ must satisfy (i)-(iii) as well. To do so, we differentiate between the four types of transitions that could occur: arrival, departure, become content and become needy.\\
\\*
\noindent\textbf{Arrival.}
Recall that under our coupling scheme an arrival always occurs in both the holding and blocking model simultaneously, see \eqref{eq:arr1}--\eqref{eq:arr4}. Furthermore, $\ch$ and $\cy$ are unchanged during this transition, rendering (ii) trivial.

By hypothesis $\qy + \cy \leq \qh+\cy$, hence the event $\qh+\ch < n$ and $\qh+\cy =n$, with resulting state $(0,\qh+1,\ch,\qy,\cy)$,  can be excluded from our analysis
We check the conditions for the remaining three cases.

\begin{enumerate}[noitemsep]
\item If $Z(t)= (0,\qh+1,\ch,\qy+1,\cy)$, then $\qy + \cy<n$ and $\qh + \ch <n$.
\begin{itemize}[noitemsep]
\item[(i)] $\QY +\CY = \qy+\cy+1 \less[i] \qh+\ch+1 =\QH+\CH$.
\item[(iii)] $\QY  = \qy+1 \less[iii] \qh+1 = \QH = \QH+\hat{H}(t)$.
\end{itemize}

\item If $Z(t)= (h+1,\qh,\ch,\qy+1,\cy)$, then $\qy + \cy<n$ and $\qh + \ch =n$.
\begin{itemize}[noitemsep]
\item[(i)] $\QY +\CY = \qy+\cy+1 \leq n = \qh+\ch =\QH+\CH$.
\item[(iii)] $\QY = \qy+1 \less[iii] \qh +1= \QH +\hat{H}(t)$.
\end{itemize}

\item If $Z(t)= (h+1,\qh,\ch,\qy,\cy)$, then $\qy + \cy = \qh+\ch=n$.
\begin{itemize}[noitemsep]
\item[(i)] $\QY +\CY = \qy+\cy \less[i] \qh+\ch =\QH+\CH$.
\item[(iii)] $\QY = \qy \less[iii] \qh+h < \qh+h+1 = \hat{H}(t)$.
\end{itemize}
\end{enumerate}

\noindent\textbf{Departure.}
By carefully examining the possible state transitions of $Z(t)$ following a departure, we list six reachable states. However, by (iii), we have that if $h=0$, then $\qy \leq \qh$, which excludes the state $(0,\qh,\ch,\qy,\cy)$ in \eqref{eq:dep4} from the reachability graph. 
We check the remaining states for conditions (i)--(iii). Again, during a departure, $\cy$ and $\ch$ are unchanged, so (ii) is automatically satisfied by the induction hypothesis.
\begin{enumerate}[noitemsep]
\item If $Z(t) = (h-1,\qh,\ch,\qy-1,\cy)$, then $h>0$. 
\begin{itemize}
\item[(i)] $\QY+\CY = \qy+\cy-1 \less[i] \qh+\ch-1 < \qh+\ch = \QH+\CH$. 
\item[(iii)] $\QY = \qy-1 \less[iii] \qh + h-1 = \QH +\hat{H}(t)$.
\end{itemize}

\item If $Z(t) = (h-1,\qh,\ch,\qy,\cy)$, then $h>0$ and $\qh \geq \qy$ (*). 
\begin{itemize}
\item[(i)] $\QY+\CY = \qy+\cy \less[i] \qh+\ch = \QH+\CH$.
\item[(iii)] $\QY = \qy \less[*] \qh-1 \leq \qh+h-1 = \QH+\hat{H}(t)$.
\end{itemize}

\item If $Z(t) = (h,\qh,\ch,\qy-1,\cy)$, then $h>0$ and $\qh < \qy$ (*). 
\begin{itemize}
\item[(i)] $\QY+\CY = \qy+\cy-1 < \qy+\cy \less[i] \qh+\ch = \QH+\CH$.
\item[(iii)] $\QY = \qy-1 < \qy \less[*] \qh + h = \QH+\hat{H}(t)$.
\end{itemize}

\item If $Z(t) = (h,\qh-1,\ch,\qy-1,\cy)$, then $h=0$. 
\begin{itemize}
\item[(i)] $\QY+\CY = (\qy-1)+\cy-1 <  \less[i] (\qh-1)+\ch = \QH+\CH$.
\item[(iii)] $\QY  = \qy-1 \less[iii] \qh-1 = \QH + \hat{H}(t)$.
\end{itemize}

\item If $Z(t) = (0,\qh-1,\ch,\qy,\cy)$, then $h=0$ and $\qh>\qy$ (*). 
\begin{itemize}
\item[(i)] $\QY+\CY = \qy+\cy  \less[i] (\qh-1)+\cy \less[ii] (\qh-1)+\ch = \QH+\CH$.
\item[(iii)] $\QY = qy \less[*] \qh-1 =\QH+ \hat{H}(t)$.
\end{itemize}

\end{enumerate}

\noindent\textbf{Content start.}
On the event of a patient becoming content, it is clear that the sums $\QH+\CH$ and $\QY+\CY$ and $H(t)$ are unaffected. This means that (i) is directly satisfied by the induction hypothesis.
According to \eqref{eq:con1}--\eqref{eq:con2}, three states can be reached.  
\begin{enumerate}[noitemsep]
\item If $Z(t) = (h,\qh-1,\ch+1,\qy-1,\cy+1)$,
\begin{itemize}[noitemsep]
\item[(ii)] $\CY = \cy+1 \less[ii] \ch+1 = \CH$. 
\item[(iii)] $\QY = \qy-1 \less[iii] \qh+h-1 = \QH+\hat{H}(t)$.
\end{itemize}
\item If $Z(t) = (h,\qh-1,\ch+1,\qy,\cy)$, then $\qh > \qy$ (*),
\begin{itemize}[noitemsep]
\item[(ii)] $\CY = \cy \less[ii] \ch < \ch+1 = \CH$. 
\item[(iii)] $\QY = \qy \less[iii] \qh+h < \qh+1+h = \QH+ \hat{H}(t)$.
\end{itemize}
\item If $Z(t) = (h,\qh,\ch,\qy-1,\cy+1)$, then $\qy > \qh$ and hence by (iii) $h > 0$. The latter is only possible if $\qh+\ch=n$ (*),
\begin{itemize}[noitemsep]
\item[(ii)] $\CY = \cy+1 \leq n-\qy+1 = (\qh+\ch)-\qy+1 \less[*] \ch = \CH$. 
\item[(iii)] $\QY = \qy-1 < \qh+h-1 \less[*] \qh+h = \QH+\hat{H}(t)$.
\end{itemize}
\end{enumerate}

\noindent \textbf{Become needy.}
Just as in the event of content start, the sums $\QH+\CH$ and $\QY+\CY$ and $H(t)$ are unaffected, whereby  (i) is directly satisfied by the induction hypothesis.
By (ii), we have $\ch \geq \cy$. This excludes the state $(h,\qh,\ch,\qy+1,\cy-1)$ from being reached, see \eqref{eq:ne2}. 
We check the remaining two possibilities.

\begin{enumerate}
\item If $Z(t) = (h,\qh+1,\ch-1,\qy+1,\cy-1)$. 
\begin{itemize}[noitemsep]
\item[(ii)] $\CY = \cy-1 \less[ii] \ch-1 = \CH$. 
\item[(iii)] $\QY = \qy+1 \less[iii] \qh+h+1 = \QH+\hat H(t)$.
\end{itemize}
\item If $Z(t) = (h,\qh+1,\ch-1,\qy,\cy)$, then $\ch > \cy$ (*). 
\begin{itemize}
\item[(ii)] $\CY = \cy \less[*] \ch-1 = \CH$.
\item[(iii)] $\QY = \qy \less[iii] \qh+h < \qh+1+h =\QH + \hat H(t)$.
\end{itemize}
\end{enumerate}

Hence, the state reached after any feasible transition under the coupling scheme satisfies the conditions (i)--(iii).
Thus we conclude that the joint process\\  $(\hat{H}(t),\QH,\CH,\QY,\CY)$ adheres to (i)--(iii) for all $t$. Consequently, we have that (i) implies
\begin{align*}
\P\left(Q_1^b(t) + Q_2^b(t) \geq k\right) &= \P\left(Q_1^b(t) + Q_2^b(t) \geq k\right)\\
&=\sum_{j=0}^n \P\left( \QY + \CY \geq k , \QH+\CH = j \right) \\
&=\sum_{j=k}^n \P\left( \QY + \CY \geq k , \QH+\CH = j \right) \\
&\leq \sum_{j=h}^n \P\left( \QH+\CH = j \right)\\
&= \P\left( Q_1^h(t) + Q_2^h(t) \geq k\right) = \P\left(Q_1^h(t) + Q_2^h(t) \geq k\right).
\end{align*}
The other two orderings follow similarly.


\begin{remark}
Note that under this coupling scheme we cannot get the ordering $\QH(t) \geq \QY(t)$ for all $t\geq 0$. A minimal counter example occurs for $s=n=1$. Let $Z(0) = ((0,0,0),(0,0))$. First, two arrivals occur, such that state $((1,1,0),(1,0))$ is reached, followed by a departure transition, yielding $((0,1,0),(0,0))$. Next, the one patient left in the model with holding system becomes content, so that we obtain $((0,0,1),(0,0))$. 
At this stage, if an arrival occurs, the arriving patient will be put in the holding queue in the model with holding, and admitted to nurse queue in the model with blocking. Hence we end up in state $((1,0,1),(1,0))$, in which $\QH < \QY$. 
\end{remark}

\section{Proof of Proposition \ref{prop:stability_convergence}}\label{app:proof_stability_convergence}
 
Define 
\[
A(s,n) = \sum_{k=0}^s \frac{k}{s} \, \binom{n}{k} b^k ,\quad 
B(s,n) = \sum_{k=s+1}^n \frac{k!}{s!} \, \binom{n}{k} s^{s-k} b^k, \quad
C(s,n) = \sum_{k=0}^s \binom{n}{k} \, b^k,
\]
\[
\]
where $b = \delta/p\mu = r/(1-r)$. Then
\[
\rho_{\rm max}(s,n) = \frac{A(s,n)+B(s,n)}{C(s,n)+B(s,n)}.
\]
Proving that $\rho_{\rm max}(s,n) \to 1$ as $R_1\to\infty$ with $s$ and $n$ as in \eqref{eq:twofoldscaling} is equivalent to showing that
\begin{equation}\label{eq:proof_stab_1}
1-\rho_{\rm max}(s,n) = \frac{C(s,n)-A(s,n)}{C(s,n)+B(s,n)} = \frac{(1+b)^{-n}[C(s,n)-A(s,n)]}{(1+b)^{-n}[C(s,n)+B(s,n)]} \to 0.
\end{equation}
First, we rewrite
\begin{align*}
(1+b)^{-n} A(s,n) 
&= (1+b)^{-n} \sum_{k=1}^s \frac{n}{s} \binom{n-1}{k-1} b^k  \\
&= \frac{n}{s}\left(\frac{b}{1+b}\right)\sum_{k=0}^{s-1} \binom{n-1}{k} \left(\frac{b}{1+b}\right)^k \left(\frac{1}{1+b}\right)^{n-1-k}\\
&= \frac{r n}{s}\sum_{k=0}^{s-1} \binom{n-1}{k} r^k (1-r)^{n-1-k}\\
&= \frac{r n}{s} \P( {\rm Bin}(n-1,r) \leq s-1 ) \\
&= \frac{rn}{s} \P\left( \frac{{\rm Bin}(n-1,r) - (n-1)r}{\sqrt{nr(1-r)}} \leq \frac{s-1 - (n-1)r}{\sqrt{nr(1-r)}} \right)\\
&\to \Phi\left(\frac{\beta-\gamma\sqrt{r}}{\sqrt{1-r}}\right),
\end{align*}
since $nr/s = 1 + O(1/\sqrt{R_1})$.
Also, 
\begin{align*}
(1+b)^{-n} C(s,n) 
&= \sum_{k=0}^s \binom{n}{k} \left(\frac{b}{1+b}\right)^k \left(\frac{1}{1+b}\right)^{n-k}\\
&= \sum_{k=0}^s \binom{n}{k} r^k (1-r)^{n-k}\\
&= \P( {\rm Bin}(n,r) \leq s) \to \Phi\left(\frac{\beta-\gamma\sqrt{r}}{\sqrt{1-r}}\right).
\end{align*}
Therefore, we have $(1+b)^{-n}[C(s,n)-A(s,n)] \to 0$ as $\l\to\infty$.
For the remaining term,
\begin{align*}
(1+b)^{-n} B(s,n) 
&= (1+b)^{-n}\sum_{k=s+1}^n \binom{n}{k}\,\frac{k!}{s!} s^{s-k} b^k  \\
&= (1+b)^{-n}\frac{n!}{s!}\, s^s\sum_{k=s+1}^n \frac{1}{(n-k)!} \left(\frac{s}{b}\right)^{-k}\\
&= (1+b)^{-n} \frac{n!}{s!}\, s^s\, \left(\frac{b}{s}\right)^n \sum_{k=s+1}^n \frac{1}{(n-k)!} \left(\frac{s}{b}\right)^{n-k}\\
&=  r^n\, \frac{n!}{s!} s^{s-n} \sum_{m=0}^{n-s-1} \frac{1}{m!} \left(\frac{s}{b}\right)^m\\
&= \left(\frac{r}{s}\right)^n \frac{n!}{s!} s^s \,{\rm e}^{s/b} \, \P({\rm Pois}(s/b)\leq n-s-1),
\end{align*}
%
in which 
\begin{align*}
\P({\rm Pois}(s/b)\leq n-s-1) 
&= \P\left(\frac{{\rm Pois}(s/b)-s/b}{\sqrt{s/b}} \leq \frac{n-s-1-s/b}{\sqrt{s/b}}\right) \\
&\to \Phi\left(\frac{\gamma-\beta/\sqrt{r}}{\sqrt{1-r}}\right),
\end{align*}
as $\l\to\infty$.
By Stirling's approximation,
\begin{align*}
\left(\frac{r}{s}\right)^n \frac{n!}{s!} s^s \,{\rm e}^{s/b} 
&\sim \left(\frac{r}{s}\right)^n \sqrt{\frac{n}{s}} \,\frac{n^n {\rm e}^{-n}}{s^s {\rm e}^{-s}}\, s^s \,{\rm e}^{s/b} \\
&= \left(\frac{rn}{s}\right)^n \sqrt{\frac{n}{s}} {\rm e}^{-n+s+s/b} = \left(\frac{rn}{s}\right)^n \sqrt{\frac{n}{s}} {\rm e}^{-n+s/r}.
\end{align*}
%
Since, 
\[
\frac{rn}{s} = 1 + \frac{\gamma\sqrt{r}-\beta}{\sqrt{R_1}} + O(1/R),
\]
we find $\sqrt{n/s} = 1/\sqrt{r} + O(1/\sqrt{R_1})$ and 
\begin{align*}
\log\left[ \left(\frac{rn}{s}\right)^n \sqrt{\frac{n}{s}} {\rm e}^{-n+\tfrac{s}{r}} \right]
&= n \log\left[ \frac{rn}{s}\right] - n+\frac{s}{r}\\
&= -n \left[ \left(1-\frac{rn}{s}\right) + \frac{1}{2}\left(1-\frac{rn}{s}\right)^2 + O(R^{-\tfrac{3}{2}}) \right] + \frac{s}{r}\left(1-\frac{rn}{s}\right)\\
&= \frac{s}{r}\left(1-\frac{rn}{s}\right)^2 - \frac{n}{2}\left(1-\frac{rn}{s}\right)^2 + O(1/\sqrt{R_1})\\
&= \frac{(\gamma\sqrt{r} - \beta)^2}{2r} + O(1/\sqrt{R_1}),
\end{align*}
as $\l\to\infty$ and hence, 
\[
(1+b)^{-n} B(s,n) \to \f\left(\frac{\gamma\sqrt{r}-\beta}{\sqrt{r}}\right)\Phi\left(\frac{\gamma-\beta/\sqrt{r}}{\sqrt{1-r}}\right).
\]
Hence, we conclude that the denominator of \eqref{eq:proof_stab_1} converges to a constant value as $R_1$ grows, and hence the $1-\rho_{\rm max}(s,n)\to 0$ as $\l\to\infty$.

\resettocdepth

\end{subappendices}


==> Chapter_6/Chapter_6i.tex <==



\chapter{Transient error approximation in a L\'evy queue}

\begin{chapterstart}
Motivated by a capacity allocation problem within a finite planning period, we conduct a transient analysis of a single-server queue with L\'evy input. From a cost minimization perspective, we investigate the error induced by using stationary congestion measures as opposed to time-dependent measures. Invoking recent results from fluctuation theory of L\'evy processes, we derive a refined cost function, that accounts for transient effects. This leads to a corrected capacity allocation rule for the transient single-server queue. Extensive numerical experiments indicate that the cost reductions achieved by this correction can by significant.
\end{chapterstart}

\begin{flushright}
Based on\\
\textbf{Transient error approximation in a L\'evy queue}\\
\textit{Britt Mathijsen and Bert Zwart}\\
To appear in \textit{Queueing Systems}
\end{flushright}
\newpage

\section{Introduction}

The issue of matching a service system's capacity to stochastic demand induced by its clients arises in many practical settings. Typically, the resources available to satisfy demand are scarce and hence expensive. This forces the manager to consider a trade-off between the system efficiency and the quality of service perceived by its clients. In this chapter, we focus on this trade-off in the context of the $M/G/1$ queue, in which the variable amenable for optimization is the server speed $\mu$.

In general, optimizing the server speed $\m$ in a single-server queue in a time-homogeneous environment, while trading off congestion levels against capacity allocation costs, does not pose any technical challenges. Typically, the objective function to be minimized, the total cost function, has the shape
%
\begin{equation}\label{eq:intro}
\Pi_\iy(\mu) = \E[Q_\mu(\infty)] + \aaa\mu = \frac{\la\E[B^2] }{2(\mu-\la\E[B])} + \aaa\mu,
\end{equation}
%
where $\E[Q_\mu(\infty)]$ denotes the expected steady-state amount of work given server speed $\m$, and $B$ describes the service requirement per arrival. The parameter $\aaa>0$ represents the relative capacity allocation costs incurred by deploying service rate $\mu$. This one-dimensional optimization problem yields the optimizer
%
\begin{equation*}
\mui = \lambda \E[B] + \sqrt{\frac{\la\E[B^2]}{2\aaa}}.
\end{equation*}
%
Despite the simplicity and tractability of the problem described above, the presence of the \emph{steady-state} measure in the cost function in \eqref{eq:intro} should be handled carefully. By employing this particular cost structure, one automatically agrees with the underlying assumption of the system being sufficiently close to its steady state. 
However, referring the practical applications of the single-server model, system parameters rarely remain constant over time. Moreover, planning periods for the optimization problem are naturally finite. Hence, the \emph{true} expected costs incurred, which we denote by $\Pi_T(\mu)$, in addition depend on the length of the planning period $T$. Consequently, the usage of steady-state models for decision making needs to be justified by a more elaborate time-dependent or \emph{transient} analysis for these type of settings.\\
\\*
\noindent
\textbf{Related literature}. 
The time-dependent behavior of the single-server queue received much attention in queueing theory. First efforts to analyze the time-dependent properties of the $M/G/1$ queue date back to the 1950s and 1960s, e.g. \cite{Benes1957,Gaver1959,Kendall1951,Takacs1955,Takacs1962}. The analyses in these papers mostly yield implicit expressions for performance characteristics through Laplace transforms, integro-differential equations and infinite convolutions.
More specifically, there is vast literature on the transient analysis of the $M/M/1$ queue, with the goal to derive explicit expressions for queue length characteristics, see e.g. \cite{Abate1987,Cohen1982,Pegden1982,Prabhu1964}. 
These works provide a variety of explicit expressions for the transient dynamics, although the complexity of the resulting expressions, typically involving Bessel functions, expose the intricate intractability of the matter. Consequently, approximation methods for insightful quantification of the dynamics based on numerical \cite{Neuts1966} or asymptotic methods, have become prevalent in more recent literature.
The asymptotic methods either exploit knowledge on the evolution of the queueing process as time $t$ grows large \cite{Abate1987,Newell1982,Odoni1983}, or as the arrival rate $\la$ is increased to infinity \cite{Abate1987a,Abate1987b,Gaver1968}. 
It is noteworthy that a substantial contribution to the transient literature is made by Abate and Whitt \cite{Abate1987a,Abate1987b,Abate1987,Abate1994}, who exploit the existence of a decomposition of the mean transient queue length and obtain expressions for the moments of the queue length and virtual waiting through probabilistic arguments in several queueing models. 
More recently, asymptotic methods have been used to justify the application of stationary performance measures in Markovian environments or to refine them, see e.g. \cite{Green1991,Whitt1991}.
Other approximative methods known as uniform acceleration expansions \cite{Massey1998} have been developed to reveal the asymptotic behavior of the single-server queue as a function of $t$, which are moreover able to capture time-varying arrival rates.
The majority of the works mentioned above do reflect on the error imposed by usage of steady-state performance metrics instead of the correct time-dependent counterpart. However, no light has been shed on the accumulation of this error over a finite period of time. To the best of our knowledge, the only work that addresses this issue is the paper by Steckley and Henderson \cite{Steckley2007}, who compute an approximation for the error accumulated between the steady-state and transient delay probability. Our analysis on the other hand is centered around the mean workload, which requires a different approach. In addition, the focus in \cite{Steckley2007} is on performance measures only, while the main goal of our work is to investigate the quality of staffing rules. \\
\\*
\noindent\textbf{L\'evy input}.
Although the $M/G/1$ queue serves as the leading example in our analysis, we choose to use a more general framework for the arrival process of the queue. Namely, we let the server face a L\'evy process.
This gives the advantage that once we have obtained the results, we can apply them to broader queue input classes, such as Brownian motion and the Gamma process.
To shed light on the influence of the transience of the queueing process on traditional staffing questions, we will study the capacity allocation problem in the context of cost minimization in which the objective function is $\Pi_T(\mu)$, i.e. a function of both $\mu$ and $T$. We investigate how the invalidity of the stationary assumption is echoed through the operational cost accounting for congestion-related penalties. 
Furthermore, we establish a result on the strict convexity of the function $\Pi_T(\mu)$, for almost all values of $T$ (with a few minor exceptions for certain deterministic initial states), which is an essential property for convergence of both cost function and corresponding minimizer to their stationary counterparts.
\\
\\*
\noindent\textbf{Corrected staffing rule}. 
As it will appear that an exact analysis of this disparity is intractable, we will present an explicit approximate correction to the conventional stationary objective function given by $\Psi(\mu)/T$ and prove that
%
\begin{equation*}
\Pi_T(\mu) = \Pi_\iy(\mu) + \frac{\Psi(\mu)}{T} + O(1/T^2),
\end{equation*}
%
with the help of recent results from the fluctuation theory of L\'evy processes. 
 Based on this refinement we ultimately examine how incorporating transient effects\\ \noindent changes the optimal capacity level and propose a refinement to the steady-state capacity allocation rule, 
%
\begin{equation*}
\muT = \mui + \frac{\mu_\bullet}{T} + o(1/T).
\end{equation*}
% 
We moreover deduce an explicit expression for $\mu_\bullet$ in terms of the initial state and the first three moments of the service requirement per arrival.
It is noteworthy that similar refined square-root staffing rules have been proposed for multi-server queues in the Halfin-Whitt regime, see e.g. \cite{Janssen2015,Janssen2008,Janssen2011,Randhawa2014,Zhang2012}. In those cases, the relevant decision value is the number of servers  and refinements are derived for $\la\to\iy$, whereas we consider the regime $T\to\infty$. 

  Building upon the insights gained through the analysis of this optimality gap, we reflect on the parameter settings of the underlying queueing process in which our refined capacity sizing rule yields significant improvement and in which cases it has little effect. Special emphasis is put on the relationship between the accuracy of the standard procedure and the length of the planning period.
\\
\\*
\noindent\textbf{Structure of the chapter}.
The remainder of this chapter is structured as follows. Section \ref{sec:model_description} is devoted to the model description and presents some preliminary results. The main result will be given in Section \ref{sec:analysis} and results regarding the optimization problem will be discussed in Section \ref{sec:optimization}, followed by the validation of our novel techniques through numerical experiments in Section \ref{sec:numerics}. We will give some concluding remarks and topics for further research in Section \ref{sec:conclusion_chapter6}. We have deferred all proofs to the appendix.

\section{Model description}
\label{sec:model_description}

\subsection{A queueing model with L\'evy input \label{sec:levymodel}}
The model that inspired our study is the standard $M/G/1$ queue starting out of equilibrium. Customers arrive to the queue according to a Poisson process with rate $\la$ and each arrival has iid service requirement $B_i$, stemming from a common random variable $B$. 
Without loss of generality we will assume $\E[B] = 1$ throughout. The server is able to remove $\mu$ amounts of work from the system per time unit; a variable we will refer to as the \emph{server speed}. 
E.g. if $\mu = 3$ and two customers are in the system with remaining service times $4$ and $2$, then  the queue will be empty 2 time units later, provided that no new arrivals occur in the meantime.
Let $N_\la(t)$ denote the number of arrivals until time $t$.
Accordingly, the total work generated by the customers is given by
%
\begin{equation*}
Z_\la(t) = \sum_{i=1}^{N_\la(t)} B_i.
 \end{equation*} 
%
Furthermore, define $X_{\la,\mu}(t) := Z_\la(t) - \mu t$. We call $X_{\la,\mu}$ the \emph{net-input process}. 
More generally, we assume throughout the chapter that $X_{\la,\mu}$ is a L\'evy process.
Specifically, we let $Z_\la$ be of the form $Z_\la(t) = U(\la t)$, where $U$ is a spectrally positive L\'evy process generated by the triplet $(a,\s,\nu)$ and $\E[U(1)] = 1$. 
This restriction to spectrally positive processes is equivalent to stating $\nu(-\infty,0)=0$ and is a vital assumption to our analysis. 
Subsequently, we assume the net-input process $X_{\la,\mu}$ to be
%
\begin{equation}
\label{eq:Xlmprocess}
X_{\la,\mu}(t) = U(\la t) - \mu t, \qquad t \geq 0.
\end{equation}
%
Note that by setting $a=\s=0$ and $\nu = \la\, F_B$, where $F_B$ is the cumulative distribution function of $B$, we retrieve the original $M/G/1$ queue. 
%
The stochastic process central to our analysis is the \emph{workload process} $Q_{\la,\mu}(t)$, $t\geq 0$, which describes the amount of work the server is facing at time $t$. 
The net-input process $X_{\la,\mu}$ completely determines the trajectory of $Q_{\la,\mu}$, namely
%
\begin{equation}\label{eq:Qlm}
Q_{\la,\mu}(t) = \max\left\{ Q(0) + X_{\la,\mu}(t), \sup_{s\in[0,t]} [X_{\la,\mu}(t)-X_{\la,\mu}(s)]\right\}, \qquad t\geq 0,
\end{equation}
%
where $Q(0)$ is the initial workload in the system. 
In fact, $Q_{\la,\mu}$ is the reflected version of $X_{\la,\mu}$ with reflection barrier at zero.
Careful inspection of the structure also reveals that $X_{\la,\m}(t) \equiv X_{\la/\mu,1}(\mu t) \equiv X_{1,\mu/\la}(\la t)$, so that
%
\begin{equation}
\label{eq:Qidentity}
Q_{\la,\m}(t) \equalD Q_{\la/\mu,1}(\mu t) \equalD Q_{1,\mu/\la}(\la t)
\end{equation}
%
for all $\la,\m,t>0$.
This identity will prove to be convenient for the numerical analysis in Section \ref{sec:numerics}. For reasons of clarity, we omit the subscript $\la$ in our expressions if no ambiguity is possible.

The process $Q_{\m}$ is a natural indicator of the level of congestion in the system and therefore a good choice for quantifying the Quality of Service (QoS) received by a client.
We remark that alternative processes characterizing congestion in the system can be deduced directly from $Q_{\m}(t)$. For example, consider the virtual waiting time process $V_{\mu}(t)$, which is the waiting time a customer would experience if he arrives at time $t$. This satisfies the relation $V_{\mu}(t) \equiv Q_{\m}(t)/\mu$ for all $t\geq 0$.
Likewise, the expected number of the customers in the system $L_{\m}(t)$ at time $t\geq 0$ is given by Little's law
%
\begin{equation*}
\E[L_{\m}(t)] = \la\, \E[V_{\m}(t)] = \frac{\la}{\mu}\, \E[Q_{\mu}(t)].
\end{equation*}
%
To facilitate our investigation of the queueing model, we end this subsection by introducing some notation regarding the net-input and workload process and by stating a useful preliminary result concerning the stationary process $\Qlm(\iy)$. 
Throughout the chapter we assume $\mu>\la$ to ensure ergodicity of the queue and convergence in distribution to the limit
%
\begin{equation*}
\Qlm(\iy) := \lim_{t\to\iy} \Qlm(t),
\end{equation*}
%
for any initial state $Q(0)<\iy$. This random variable necessarily coincides with the stationary distribution of $\Qlm(t)$. 
By $\ka_U(\cdot)$ and $\ka_{\mu}(\cdot)$ we denote the L\'evy exponents of the processes $U$ and $\Xlm$, respectively:
%
\begin{equation*}
\ka_{\m}(\thh) = \log \E[\ee^{\thh \Xlm(1)}] = \log \E[\ee^{\thh(U(\la) - \mu)}] = \la \ka_U(\thh) - \mu \thh.
\end{equation*}
%
Furthermore, define $u_k = \E[\{U(1) - \E U(1)\}^k]$ for $k=2,3,...$. 
Using this representation we obtain the following preliminary result.
%
\begin{lemma}\label{lemma:workloadmoments}
Let $\E|U(1)|<\infty$, $u_2, u_3 < \iy$ and $\mu > \la$. If $Q_{\mu}(\infty)$ represents the steady-state distribution of the workload process, then
\begin{equation*}
\E[\Qlm(\infty)] = \frac{\la u_2}{2(\mu-\la)},\qquad \E[Q_{\mu}^2(\iy)]=\frac{\la^2u_2^2}{2(\mu-\la)^2} + \frac{\la u_3}{3(\mu-\la)}.
\end{equation*}
\end{lemma}
The proof of Lemma \ref{lemma:workloadmoments} follows directly by differentiation of the Laplace transform of $Q_\mu(\iy)$ and is given in Appendix \ref{app:proof_lemma_workload_moments}.
\subsection{Finite horizon}

For the purpose of our research, we are interested in the dynamics of the workload process within a fixed time frame of length $T>0$. 
For all $0\leq t \leq T$, we assume that the parameters of the queue, $\la,\m,u_2,u_3$, remain unchanged. 
If at $t=0$ the queue is not in steady-state corresponding to the specified parameters of the starting period, the process $\{\Qlm(t)\}_{t\in[0,T]}$ differs from its stationary counterpart $\Qlm(\infty)$. 
To illustrate this, Figure \ref{fig:transientmeans} depicts the expected value $\Qlm$ in a $M/M/1$ queue as a function of time for several initial workloads $Q(0)$ for a particular setting of $\la$ and $\m$. 
Clearly, transient behavior of $\E[\Qlm(t)]$, for $Q(0) \neq \Qlm(\iy)$, differs significantly from the steady-state mean with the same system parameters. 
Note that even if $Q(0) \equiv \E[\Qlm(\iy)]$, the time-dependent mean does not coincide with the steady-state mean. Moreover, $\E[\Qlm(t)]$ is not even a strictly increasing nor decreasing function of time. This phenomenon is a consequence of the decomposition of the transient mean into one strictly increasing, and a strictly decreasing term for $Q(0)>0$, as discussed in \cite{Abate1987}.
Nonetheless, $\Qlm(t)$ converges in distribution to $\Qlm(\infty)$ as $t\to\iy$, if $\mu>\la$. 
 
\begin{figure}
\centering
\begin{tikzpicture}[xscale=0.15,yscale=0.225]
\draw (0,0) -- coordinate (x axis mid) (50,0);
    \draw (0,0) -- coordinate (y axis mid) (0,21);
	%labels      
	\node[right] at (51,0) {$t$};
	\node[rotate=90, above=0.7 cm] at (y axis mid) {$\E[\Qlm(t)]$};
	
	\draw[dashed, thick, gray] (0,10) -- coordinate (eq) (51,10);
%	\node at (55,10) {$\E[Q_\mu(\infty)]$};
	
	
	%arrows
	\draw[->] (24,6.4) --  coordinate (a1) (21.65,8.49574);
	\node[right=0.6cm,below=0.3cm] at (a1) {$Q(0)\equiv 0$};
	\draw[->] (14,6.2) --  coordinate (a2) (13.,8.49434);
	\node[right=0.2cm,below=0.3cm] at (a2) {$Q(0)\equiv10$};
	\draw[->] (9,15.5) --  coordinate (a3) (7.5,13.7648);
	\node[right=0.6cm,above=0.1cm] at (a3) {$Q(0)\equiv20$};
	\draw[->] (40,12.5) -- coordinate (a4) (38,10.9712);
	\node[right,above=0.3cm] at (a4) { $Q(0)\sim \exp\left(\tfrac{1}{15}\right)$ };

	%ticks
    	\foreach \x in {0,10,...,50}
     		\draw (\x,1pt) -- (\x,-10pt)
			node[anchor=north] {\x};
    	\foreach \y in {5,10,15,20}
     		\draw (1pt,\y) -- (-20pt,\y)
     			node[anchor=east] {\y};
	
	
	%plots
	\draw[thick,color = col1] plot
			file {Chapter_6/tikz/means0.txt};
	\draw[thick,color = col3] plot
			file {Chapter_6/tikz/means10.txt};
    \draw[thick,color = col4] plot
			file {Chapter_6/tikz/means20.txt};
	\draw[thick,color = col5] plot
			file {Chapter_6/tikz/meansExp.txt};		
\end{tikzpicture}
\caption{Time-dependent mean workload in a $M/M/1$ queue with $\la = 10$ and $\mu=11$ for different initial states $Q(0)$. The dashed line depicts $\E\Qlm(\iy)$.}
\label{fig:transientmeans}
\end{figure}
%
Since the time horizon of our analysis is limited to $t\leq T$, the process may not approach the steady-state distribution sufficiently close to appropriately use its steady-state properties for capacity allocation. 
To overcome this disparity, we propose a way to include the influence of this transient phase in the capacity allocation problem.
 
\subsection{Cost structure}

As mentioned before, we are interested in balancing the QoS and efficiency of the queue by choosing the optimal server speed $\mu$. 
The adjective \emph{optimal} indicates that we intend to choose the speed according to some objective function. 
In our case, we conduct our analysis based on a cost function, which consists of a part accounting for the penalty for congestion in the system and a part for staffing cost. The cost value of both parts is governed by the variable $\mu$. 
The instantaneous cost incurred at time $t$ equals
%
\begin{equation*}
\E[\Qlm(t)] + \aaa \mu,
\end{equation*}
%
where $\aaa$ is a positive constant defining the \emph{relative staffing cost}. 
Hence, the cost structure we apply is a combination of the transient mean of the workload process and a linear staffing cost. 
Accumulated and normalized over the period $[0,T]$, the cost function on which the rest of this chapter will be based equals
%
\begin{equation}\label{eq:PiT}
\Pi_{T}(\mu) := \frac{1}{T}\int_0^T\left(  \E[\Qlm(t)] + \aaa\mu\, \right) \dd t 
 = \frac{1}{T} \int_0^T \E[\Qlm(t)] \dd t + \aaa\mu.
\end{equation}
% 
We use shorthand notation for the normalized congestion costs:
%
\begin{equation}\label{eq:CTmu}
C_{T}(\mu) := \frac{1}{T}\int_0^T \E[Q_{\mu}(t)] \dd t,
\end{equation}
%
and $C_{\iy}(\mu) := \E[\Qlm(\iy)]$. 
In order to compare the actual costs incurred over the interval $[0,T]$ to the cost function of the queue in stationary conditions, we define
%
\begin{equation}\label{eq:PiInf}
\Pi_{\iy}(\mu) := C_{\iy}(\mu) + \aaa \mu = \E[Q_\mu(\iy)] + \aaa\mu,
\end{equation}
%
which allows an explicit expression by Lemma \ref{lemma:workloadmoments}. 
Under mild conditions on the net-input process and the distribution of the initial state, the cost functions coincide for $T\to\iy$.
%
\begin{proposition}\label{prop:cost_convergence}
Let $\mu>\la$ and assume $\E[U(1)],\, \E[Q(0)] < \iy$. Then
\begin{equation*}
\lim_{T\to\iy} \Pi_{T}(\mu) = \Pi_{\iy}(\mu).
\end{equation*} 
\end{proposition}
\noindent Rewriting \eqref{eq:PiT} gives the relation
%
\begin{align}
\Pi_{T}(\mu) &= \frac{1}{T}\int_0^{T} \left( \E[\Qlm(t)] - \E[\Qlm(\iy)] \right) \dd t + \E[\Qlm(\iy)] + \aaa\mu =  \Omega_{T}(\mu) + \Pi_{\infty}(\mu).
\label{eq:decomp}
\end{align}
%
Section \ref{sec:analysis} is concerned with the analysis of the correction factor $\Omega_{T}(\mu)$.

Ultimately, we are concerned with the additional costs incurred by choosing the server speed through minimization of $\Pi_{\iy}(\mu)$ instead of $\Pi_{T}(\mu)$. 
Therefore, we formulate the exact and approximate optimization problems as follows
%
\begin{equation}\label{eq:muStar}
\mu_T^\star := \arg\min_{\mu\geq 0} \Pi_{T}(\mu), \qquad \qquad \mu_\infty^\star := \arg\min_{\mu\geq 0} \Pi_{\iy}(\mu),
\end{equation}
\begin{equation}\label{eq:piStar}
\Pi_{T}^\star := \Pi_{T}(\mu_T^\star), \qquad \qquad \Pi_{\iy}^\star := \Pi_{T}(\mu_\iy^\star).
\end{equation}
%
In Section \ref{sec:optimization} we turn to the comparison of $\mu_T^{\star}$ and $\mu_\iy^\star$ as well as the \emph{optimality gap} $\Pi_{\iy}^\star - \Pi_{T}^\star$.
%

\section{Analysis of the objective function}
\label{sec:analysis}
From \eqref{eq:decomp} it is evident that, for finding an explicit characterization of $\Pi_{T}(\mu)$, it suffices to study the term $\Omega_T(\mu)$ in more detail. We start by stating the main result of this section, which describes the leading order behavior of $\Omega_T(\mu)$ as $T$ increases.
%
\begin{theorem}\label{thm:mainresult}
Let $X_\mu(t)$ be of the form \eqref{eq:Xlmprocess}. If $\E[\max(Q(0),Q_\mu(\infty))^3] < \iy$ and $u_2,u_3 < \iy$, then
%
\begin{align*}
\Omega_T(\mu) &= \frac{\E[Q(0)^2] - \E[Q_\mu(\iy)^2]}{2T(\mu-\la)} + O\left(\frac{1}{T^2}\right) \nonumber\\
&= \frac{1}{2T(\mu-\la)}\left( \E[Q(0)^2] - \frac{\la^2 u_2^2}{2(\mu-\la)^2} - \frac{\la u_3}{3(\mu-\la)}\right) + O\left(\frac{1}{T^2}\right),
\end{align*} 
for $\mu>\la$.
\end{theorem}
%
Note that this expression provides an \emph{approximation} of the actual cost function
$\Pi_T(\mu)$. We elaborate on the implications of this additional information on the optimization problem in Section \ref{sec:optimization}. 

In the remainder of this section we provide a detailed description of the steps taken to obtain this outcome.
We assume a fixed service rate $\mu$ throughout the analysis in this section and therefore omit the subscript $\mu$. Proofs of the intermediate results can be found in Appendix \ref{app:proofs_analysis}.
\subsection{Constructing a coupling}

Before starting our analysis of the correction term $\Omega_{T}(\mu)$ we introduce some auxiliary notation. 
By $Q^A(t)$ we denote the workload process as described in Subsection \ref{sec:levymodel} with initial state $A$ and $\E_A$ the expectation with respect to any non-negative random variable $A$, which is independent of the net-input process $X$.
To be able to compare $\E[Q(t)]$ and $\E[Q(\iy)]$ as in $\Omega_T(\mu)$, we will use a coupling technique.
Observe that by definition of the stationary distribution $Q(\iy) \equalD Q^{Q(\iy)}(t)$ for all $t \geq 0$ and therefore $\E[Q(\iy)] = \E_{Q(\iy)}[Q^{Q(\iy)}(t)]$. Furthermore, $\E[Q(t)] = \E_{Q(0)}[Q^{Q(0)}(t)]$.
Hence, quantifying the difference between the transient and stationary mean is equivalent to comparing the workload processes of two queues starting in two different (random) states at $t=0$. 

We starting our analysis for two queues starting in two \textit{deterministic} states $x,y\geq 0$, respectively. At the end of our analysis we will obtain the original form by replacing $x$ with $Q(0)$ and $y$ with $Q(\iy)$.

Equation \eqref{eq:Qlm} shows that all randomness in the workload process originates from the process $X(t)$. 
With this in mind, we couple the processes $Q^x(t)$ and $Q^{y}(t)$ on a sample path level by feeding both queues the same net-input process $X(t)$ for $t\geq 0$. 
This allows us to compare the processes in the same probability space, so that $\E[Q^x(t)] - \E[Q^y(t)] = \E[Q^x(t) - Q^y(t)]$ for all $t\geq 0$.
% 
Define
%
\begin{equation*}
Y^{x,y}(t) := Q^x(t) - Q^y(t)
\end{equation*}
%
and 
%
\begin{equation*}
\Omega_{T}^{x,y} := \frac{1}{T}\,\int_0^T \E\left[Y^{x,y}(t)\right] \, \dd t.
\end{equation*}

%
A possible sample path triple for $Q^x(t)$, $Q^0(t)$ and $Y^{x,0}(t)$ is depicted in Figure \ref{fig:samplePaths}.
 As we see from this figure, $Y^{x,0}(t)$ has nice structural properties which we will exploit in the next subsection. 

\begin{figure}
\centering
\begin{tikzpicture}[y=0.6cm, x=0.01cm]
 	%axis
	\draw (0,0) -- coordinate (x axis mid) (800,0);
    \draw (0,0) -- coordinate (y axis mid) (0,6.5);
	%labels      
	\node[below=0.2cm] at (x axis mid) {$\to t$};
	\node[rotate=90, above=0.2cm] at (y axis mid) {$Q(t)$};
	\node[above=1.3cm,left =0.08 cm] at (y axis mid) {$x$};
	
	
	%plots
	\draw plot
			file {Chapter_6/tikz/samplePathLevy.txt};
	\draw[color = gray] plot
			file {Chapter_6/tikz/samplePathLevy2.txt};
	\draw[thick,color=col1] plot
			file {Chapter_6/tikz/runningMinimumLevy.txt};
\end{tikzpicture}
\caption{Sample path visualization of the processes $Q^x(t)$ (solid), $Q^0(t)$ (gray) and $Y^{x,0}(t)$ (red).}
\label{fig:samplePaths}
\end{figure}

\subsection{Difference process and leading order behavior of the correction term}

We further examine the \emph{difference process} $Y^{x,y}(t)$ with $x>y$. Recall from \eqref{eq:Qlm},
%
\begin{equation}\label{eq:Wz}
Q^z(t) = \max\{ z + X(t),\, \sup_{0<s\leq t} [X(t)-X(s)]\} = X(t) + \max\{ z, -\inf_{0\leq s\leq t} X(s)\},
\end{equation}
%
for any initial state $z\geq 0$, where $X(t)$ is a L\'evy process with no negative jumps.
Let $\tau^z(w)$, $0\leq w<z$ denote the first passage time of level $w$ by the process starting in $z$, i.e.
%
\begin{equation*}
\tau^z(w) := \inf \left\{ t \geq 0\, |\, Q^z(t) \leq w \,\right\}.
\end{equation*}
%
Then it is easily seen that for all $z\geq 0$,
%
\begin{equation*}
Q^z(t) = \left\{
\begin{array}{ll}
z + X(t), & {\rm if }\ t <\tau^z(0), \\
\sup_{0<s\leq t} [X(t)-X(s)], & {\rm if }\ t \geq \tau^z(0).
\end{array}\right.
\end{equation*}
Consequently,
%
\begin{equation}\label{eq:Yxy}
Y^{x,y}(t) = \left\{
\begin{array}{ll}
x - y, & \text{if }t < \tau^y(0),\\
\inf_{0<s\leq t} \{ x+X(s)\}, & \text{if }\tau^y(0) \leq t < \tau^x(0),\\
0, & \text{if }t \geq \tau^x(0).
\end{array}\right.
\end{equation}
%
Using this representation we can identify
%
\begin{equation*}
\Omega^{x,y}_T = \frac{1}{T}\,\E\left[\int_0^{\tau^x(0)\wedge T} Y^{x,y}(t) \dd t\right],
\end{equation*}
%
where $\wedge$ denotes the minimum operator, due to the fact $Y^{x,y}(t) = 0$ for $t\geq \tau^x(0)$. 
Subsequently, we decompose $\Omega_T^{x,y}$ into two terms 
\begin{equation}
\Psi^{x,y}_T := \frac{1}{T} \int_0^\infty \E[Y^{x,y}(t)]\, \dd t  \qquad
\text{and}
\qquad
\Delta_T^{x,y} := \Omega_T^{x,y} - \Psi_T^{x,y}.
\label{eq:Deltaxy}
\end{equation}
Note that $\Psi_T^{x,y}$ is obtained by replacing $T$ by $\infty$ only in the integration bound.
It is customary in the literature, particularly in the area of stochastic simulation, to compare the truncated integral to its natural expansion of the integration range to a  semi-infinite interval, see e.g. \cite[Prop.~2.1]{Awad2007}.The truncated integral connects to the long-run average estimator of a certain performance metric, whereas the infinite integral reflects its exact expectation.
The decomposition in \eqref{eq:Deltaxy} is insightful, because $\Psi_T^{x,y}$ prescribes the leading order behavior of $\Omega_T^{x,y}$, while $\Delta_T^{x,y}$ captures the smaller order error term.
In this section, we only consider $\Psi_T^{x,y}$. Subsection \ref{sec:trunc} investigates the magnitude of $\Delta_T^{x,y}$.
The next preliminary result presents a useful property of $\Psi_T^{x,y}$.
\begin{lemma}\label{lemma:psixy}
Let $x>y$. If $\E[\tau^x(0)]<\iy$, then
%
\begin{equation}\label{eq:H(x,y)}
\Psi^{x,y}_T = \frac{1}{T}\,\E[\tau^{y}(0)](x-y) + \Psi^{x-y,0}_T.
\end{equation}
\end{lemma}
%
This leaves us with two unknowns $\E[\tau^y(0)]$ and $\Psi_T^{x-y,0}$.
The next lemma gives an equivalent form for the latter.
%
\begin{lemma}\label{lemma:psiz0}
If $\E[\tau^z(0)] < \iy$, then for all $z\geq 0$
\begin{equation}\label{eq:H(x,0)}
\Psi^{z,0}_T = \int_0^z \E[\tau^w(0)]\, \dd w.
\end{equation}
\end{lemma}
%
Since the term $\E[\tau^z(0)]$, for several values of $z$, appears in many of the preliminary results, we devote our attention to this in the next subsection.\\
\\*
\noindent
\textbf{First passage time}.
When studying the first passage time of level $0\leq w < z$, $\tau^z(w)$, of the workload process starting in $z$, we first observe that $\{\tau^z(z-w)\}_{w=0}^z$ is a spectrally positive L\'evy process itself, also visible through Figure \ref{fig:samplePaths}.
More precisely, it is a subordinator, i.e. a L\'evy process whose paths are almost surely non-decreasing \cite{Kyprianou2006}. 
In order to calculate $\E[\tau^z(z-w)]$ we use theory presented in \cite[Section 46]{Sato1999}, although results presented there are valid for spectrally \emph{negative} L\'evy processes, as opposed to the absence of negative jumps in our case. 
Nonetheless, our setting is easily transformed into this framework by observing that $\hat{X} \equiv -X$, that is $\hat{X}(t) = -X(t)$ for all $t\geq 0$, is spectrally negative. 
Furthermore, let
\begin{equation}
\label{eq:transformedTau}
\hat{\tau}^0(w) := \inf\{ t \geq 0\,:\, \hat{X}(t) \geq w\} =  \inf\{ t \geq 0\,:\, z+X(t) \leq z-w\} = \tau^z(z-w).
\end{equation}
%
For completeness, we cite \cite[Thm.~46.3]{Sato1999}.
%
\begin{theorem}
Let $\hat{X}(t)$ be a spectrally negative L\'evy process with generating triplet $(-a,\s,\hat{\nu})$ and $\hat{\tau}^0(y)$ its corresponding hitting time process. Define $\Upsilon(\thh)$ for $\thh\geq 0$ as
\begin{equation}\label{eq:thmCharExp}
\Upsilon(\thh) = -a\thh + \tfrac{1}{2}\s^2\thh^2 + \int_{-\infty}^0 (\ee^{\thh x}-1-\thh x{\bf 1}_{[-1,0)}(x))\, \hat{\nu}(\dd x).
\end{equation}
%
Then $\Upsilon(\thh)$ is strictly increasing and continuous, $\Upsilon(0)=0$, and $\Upsilon(\thh)\to\infty$ as $\thh\to\infty$. For $w\geq 0$ and $0\leq u < \infty$ we have
%
\begin{equation}\label{eq:invCharExp}
\E[\exp(-u\hat{\tau}^0(w))] = \exp(-w\,\Upsilon^{-1}(u)),
\end{equation}
where $\thh=\Upsilon^{-1}(u)$ is the inverse function of $u=\Upsilon(\thh)$. 
\end{theorem}
%
\noindent This immediately induces an expression for $\E[\tau^w(0)]$ and henceforth $\Psi^{z,0}$.
%
\begin{corollary}\label{cor:Psixy}
Let $X(t)$ be a spectrally positive L\'evy process defined as in \eqref{eq:Xlmprocess} with $\mu > \la$. Let $\Psi^{z,0}_T$ as in \eqref{eq:H(x,0)}. Then 
\begin{equation*}
\Psi^{z,0}_T = \frac{z^2}{2T(\mu-\la)}.
\end{equation*}
Furthermore, if $x,y\geq 0$, then
\begin{equation}\label{eq:mainResult}
\Psi^{x,y}_T = \frac{x^2-y^2}{2T(\mu-\la)}.
\end{equation}
\end{corollary}
%
\noindent\textbf{Randomization}.
As we stated before, we easily obtain the original $\Omega_T$ from $\Omega_T^{x,y}$ through substitution of $x$ and $y$ by $Q(0)$ and $Q(\iy)$, respectively, and taking the expectation. 
In the previous paragraph, we deduced an explicit expression for $\Psi_T^{x,y}$, the leading order term for $\Omega_T^{x,y}$. 
Therefore we equivalently get an approximation for $\Omega_T$, given by
\begin{equation*}
\Psi_T := \frac{1}{T} \int_0^\iy \left( \E[Q(t)]-\E[Q(\iy)] \right)\, \dd t,
\end{equation*}
%
through randomization of $x$ and $y$ in $\Psi_T^{x,y}$.
By combining the results in Corollary \ref{cor:Psixy}, Lemma \ref{lemma:workloadmoments} and Proposition \ref{prop:truncation_error}, which is given at the end of this section, we directly prove the result in Theorem \ref{thm:mainresult}.
%

\subsection{Truncation error}\label{sec:trunc}

In order to get a better comprehension of the properties of $\Psi_T$, we depict the value in terms of the (infinite) region between the curves $\E[Q(t)]$, $\E[Q(\iy)]$ and the vertical axis for the case $Q(0)\equiv 0$ in Figure \ref{fig:PsiVisualization}.
In this figure, $\Omega_T$ is given by the area enclosed by the two curves, the vertical axis and the line $t=T$. 
One can see that the main contribution to the correction term $\Omega_T$ is given for small $t$. 
As $t$ increases, the difference between transient and stationary mean decreases.
Hence for moderate values of $T$, the contribution to the integral in \eqref{eq:Deltaxy} is only minor compared to the contribution over the interval $[0,T]$. 

\begin{figure}
\centering
\begin{tikzpicture}[xscale=0.13,yscale=0.3]
	%labels      
	\node[below=0.4cm,right=0.5cm] at (x axis mid) {$\to t$};
	
	\draw[dashed, thick, fill =gray!30] (0,0) rectangle coordinate (eq) (50,10);
	\node[] at (-7,10) {$\E[Q(\infty)]$};
	\node[] at (-3,0) {$0$};

	
	%arrows
	\draw[->] (18,6.4) coordinate (a1) --   (21.65,8.49574);
	\node[below] at (a1) {$x=0$}; 

	%ticks
    	\foreach \x in {30}
     		\draw (\x,1pt) -- (\x,-10pt)
			node[anchor=north] {$T$};
    	\foreach \y in {10}
     		\draw (1pt,\y) -- (-20pt,\y);
	
	
	%plots
	\draw[thick,color = gray,fill=white] plot
			file {Chapter_6/tikz/means0_2.txt};
		
	\draw[thick] (0,0) -- coordinate (x axis mid) (50,0);
    \draw[thick] (0,0) -- coordinate (y axis mid) (0,12);		
    \draw[color=white,very thick] (50,0.05) -- (50,9.56);
    
    \draw[very thick, dotted] (30,0) -- (30,10);
    
    \draw[->] (18,6.8) coordinate (delta) -- (17,8.7);
    \node[below] at (delta) {$\Psi_{T}$};
    
    \draw[->] (38,8.1) coordinate (delta) -- (36,9.7);
    \node[below] at (delta) {$\Delta_{T}$};
\end{tikzpicture}
\caption{Visualization of $\Omega_T$ and $\Psi_T$ as the area between the curves $\E[Q(t)]$, $\E[Q(\iy)]$ for $Q(0) = 0$.}
\label{fig:PsiVisualization}
\end{figure}
%
Recall the definition of $\Delta^{x,y}_T$ as in \eqref{eq:Deltaxy}. As we eluded to in Subsection 3.2
we claim the contribution of $\Delta^{x,y}_T$ to $\Omega_T^{x,y}$ is negligible compared to $\Psi^{x,y}_T$. Also note that
%
\begin{equation}
\label{eq:Delta}
\Delta_T := \Omega_T - \Psi_T = {-}\frac{1}{T} \int_T^\iy \E[Q(t)] - \E[Q(\iy)]\,\dd t.
\end{equation}
% 
can be derived through $\Delta^{x,y}_T$ in a similar manner as we did for $\Psi^{x,y}_T$ to obtain $\Psi_T$.
%
To substantiate our claim, we compute an upper bound for $\Delta^{x,y}_T$ of order $1/T^2$. The existence of such an upper bound poses a limit on the error this tail integral contributed to the cost structure as a whole. 
%
\begin{proposition} \label{prop:truncation_error}
Let $x,y\geq 0$ and $\E[\max(Q(0),Q_\m(\iy))^3] < \iy$. Then
\begin{equation*}
|\Delta^{x,y}_T| \leq \frac{1}{T^2}\left(\frac{\max(y,x)^3}{3(\mu-\la)^2}+\frac{u_2 \max(y,x)^2}{2(\m-\la)^3}\right) 
\end{equation*}
and
\begin{equation*}
|\Delta_T| \leq \frac{1}{T^2}\left(\frac{\E[\max(Q(0),Q_\m(\iy))^3]}{3(\mu-\la)^2}+\frac{u_2 \E[\max(Q(0),Q_\m(\iy))^2]}{2(\m-\la)^3}\right).
\end{equation*}
\end{proposition}

\textit{Remark.} In case the net-input process $X$ is light-tailed, that is there exists $u>0$ such that $\E[{\rm e}^{u X(1)}] < \iy$, it can be shown that the truncation error is of order ${\rm e}^{-\beta T}/T$ for some $\beta>0$. See Appendix \ref{sec:proof_truncation} for details.

\section{Optimization}
\label{sec:optimization}
The result in Theorem \ref{thm:mainresult}, characterizing the leading order behavior of $\Omega_T(\mu)$, also reveals the behavior of $\Pi_T(\mu)$ in leading order. Namely, 
%
\begin{equation*}
\Pi_T(\mu) = \Pi_\iy(\mu) + \Psi_T(\mu) + O(1/T^2).
\end{equation*}
%
In fact, this representation naturally gives rise to an \emph{approximation} of the actual cost function:
\begin{align}\label{eq:decomposition}
\hat{\Pi}_{T}(\mu) := \Pi_{\iy}(\mu) + \Psi_T(\mu) 
\end{align}
Denote the corresponding minimizer of $\Pih$ by
%
\begin{equation}\label{eq:muhat}
\hat{\mu}_T^\star := \arg\min_{\m\geq 0} \Pih(\mu), \qquad \Pih^\star := \Pih(\hat{\mu}_T^\star)
\end{equation}
%
in addition to the definitions in \eqref{eq:muStar} and \eqref{eq:piStar}.
This section is devoted to the analysis of the minimizers $\muT$, $\muh$ and $\mui$, and the optimality gap for the two approximations. 

Throughout this section, we assume that $u_2, u_3 <\iy$ and $\E[Q(0)^2] <\iy$.

By its definition in \eqref{eq:PiInf} and Lemma \ref{lemma:workloadmoments}, we have an exact expression for the steady-state cost function:
%
\begin{equation*}
\Pi_{\iy}(\mu) = \frac{\la u_2}{2(\mu-\la)} + \aaa\mu.
\end{equation*}
%
It is easily verified that $\Pi_{\iy}$ is strictly convex in $\mu$, for instance by observing that $\Pi_{\iy}''(\mu) > 0$ for all $\mu > \la$. Therefore $\Pi_{\iy}$ has a unique global minimizer and 
%
\begin{equation}
\label{eq:muInf}
\mui = \la + \sqrt{\frac{\la u_2}{2\aaa}}, \qquad  \Pi_{\iy}^\star = \aaa\la + \sqrt{2\aaa\la u_2}.
\end{equation}
%
We are interested in the relation between $\mui$ and $\muT$, and between $\muh$ and $\muT$. 
Since $\Pi_{T}(\mu) = \Pi_{\iy}(\mu) + O(1/T)$ for all $\mu > \la$, we have pointwise convergence of the sequence $\Pi_{T}$, as well as $\hat{\Pi}_{T}$, to $\Pi_{\iy}$ for $T\to\iy$, we also expect $\muT \to \mui$ and $\muh\to\mui$ for $T\to\iy$.
Before proving that this convergence indeed holds, we present a result on the strict convexity of the function $\Pi_{T}$. 

\begin{lemma}\label{lemma:strict_convexity}
Let $\mu\geq 0$. The function $\Pi_{T}(\mu)$ is 
\begin{itemize}
\item convex in $\m$, if $Q(0)\equiv x$, $T<x/\mu$ and $\sigma=0$,
\item strictly convex in $\mu$, otherwise. 
\end{itemize}
\end{lemma}
%
Building upon strict convexity of both $\Pi_T(\mu)$ and $\Pi_\iy(\mu)$ for $\mu>\la$, we derive the following convergence result. 
%
\begin{proposition}\label{prop:min_convergence_mu}
Let $\muT$, $\muh$ and $\mui$ be as defined in \eqref{eq:muStar} and \eqref{eq:muhat}. Then 
\begin{equation*}
\muT \to \mui\, \qquad \text{\rm and } \qquad \muh \to \mui,
\end{equation*}
for $T\to\infty$.
\end{proposition}
% 
The next result describes a refinement of $\muT$ in terms of $\mui$.
%
\begin{proposition}\label{prop:muBullet}
For $T$ sufficiently large,
\begin{equation*}
\muT = \mui + \frac{\mu_\bullet}{T} + o(1/T),
\end{equation*}
where
\begin{equation}\label{eq:muBullet}
\mu_\bullet = \frac{\E[Q(0)^2]}{\sqrt{8\la u_2\aaa}} - \frac{u_3}{3 u_2} - 3\sqrt{\frac{\aaa\la u_2}{8}}.
\end{equation}
\end{proposition}
%
Based on Proposition \ref{prop:muBullet} we propose a \emph{corrected staffing rule}, accounting for the finite horizon
%
\begin{equation}
\label{eq:correctedMu}
\tilde{\mu}_T^\star = \left[\mui + \frac{\mu_\bullet}{T}\right]^+, 
\end{equation}
%
with $\mu_\bullet$ as in \eqref{eq:muBullet}.
Here $[x]^+ := \max\{x,0\}$, which ensures the value of $\tilde{\mu}_T^\star$ is non-negative and thus is a feasible solution of the optimization problem.
% 
This refined capacity allocation rule is expected to reduce the costs incurred in transient settings.
 However, the value of particular interest to us is the cost penalty for using either one of the approximations rather than the actual minimum $\muT$, that is, the \emph{optimality gap}.
 As it happens, we deduce the order of the optimality gap for $\mui$ with the help of the explicit form of $\mu_\bullet$ given in \eqref{eq:muBullet}, which is stated in the next proposition. The proof is given in Appendix \ref{sec:proofProp4}.

\begin{proposition}\label{prop:optimalitygap_mui}
Let $\mui$ be as in \eqref{eq:muInf}. Then,
\begin{equation*}
\Pi_\iy^\star- \Pi_T^\star = O(1/T^2).
\end{equation*}
\end{proposition}

\section{Numerical experiments}
\label{sec:numerics}

\subsection{Influence of $\Omega_{T}(\mu)$}
\label{sec:influence_omega}
We first assess the contribution of the correction to the cost function provided by Theorem 1. In other words, we investigate whether $\hat{\Pi}_{T}(\mu)$ as in \eqref{eq:PiT} yields a significantly better fit to $\Pi_{T}(\mu)$, than $\Pi_{\iy}(\mu)$ does. 
Note that these three functions only differ in the costs describing the congestion. 
Therefore, we limit our study in this subsection to the evaluation of $C_T(\mu)$ as in \eqref{eq:CTmu} with stationary equivalent $C_{\iy}(\mu) = \E[Q_{\m}(\iy)]$. 
Our novel approximation hence reads 
%
\begin{equation*}
\hat{C}_{T}(\mu) := C_{\infty}(\mu) + \Omega_{T}(\mu),
\end{equation*}
%
with $\Omega_{T}(\mu)$ given in Theorem \ref{thm:mainresult}.
We conduct our numerical experiments based on three models, namely: 
%
\begin{enumerate}
\item \underline{$M/M/1$ queue}: $U(t)$ is a unit rate compound Poisson process with exponentially distributed increments. We have $u_2 = 2$, $u_3=3$, so that
\begin{equation}\label{eq:MM1cor}
\hat{C}_{T}(\mu) = \frac{\la} {\mu-\la}  + \frac{1}{T(\mu-\la)} \left(\frac{x^2}{2} - \frac{\la^2}{(\mu-\la)^2} - \frac{\la} {\mu-\la} \right).
\end{equation}
\item \underline{$M/{\rm Pareto}/1$ queue}: $U(t)$ is a unit rate compound Poisson process with Pareto increments. The Pareto distribution deserves special attention due to its heavy-tailed nature, having tail probability $\bar{F}(x) = (x/k)^{-\g}$, if $x\geq k$ and 1 otherwise. 
It is well-known that heavy-tailed service times lead to long relaxation time. For our purposes, we fix shape parameter $\g = 16/5$ and scale parameter $k=11/16$, so that $\beta = 1$, $u_2 = 121/96$, $u_3 = 1331/256$ and $u_k=\iy$ for all $k>3$. Hence, 
\begin{equation}
\label{eq:MP1cor}
\hat{C}_{T}(\mu) = \frac{121\la} {192(\mu-\la)} + \frac{1}{2T(\mu-\la)}
\left( x^2 - \frac{(121\la/96)^2}{2(\mu-\la)^2} - \frac{ 1331\la/256 }{2(\mu-\la)}\right)
\end{equation}
\item \underline{Reflected Brownian motion}: $U(t)$ is Brownian motion with drift 1 and infinitesimal variance $\s^2$. We have $u_2 = \sigma^2$, $u_3=0$, so that
\begin{equation}\label{eq:RBMcor}
\hat{C}_{T}(\mu) = \frac{\la\sigma^2}{2(\mu-\la)} + \frac{1}{2T(\mu-\la)} \left( x^2 - \frac{\la^2\sigma^4}{2(\mu-\la)^2}\right).
\end{equation}
\end{enumerate} 
%
In light of the equivalence relations in \eqref{eq:Qidentity} we only consider the case $\la=1$. The cost values for general values of $\la$ follow by appropriate rescaling of $\mu$ and $T$.\\
\\*
\noindent
For the $M/M/1$ and $M/{\rm Pareto}/1$ queue, we obtained the function $C_{T}(\mu)$ through simulation and the results are accurate up until a 95\% confidence interval of width $10^{-3}$. For reflected Brownian motion, we used the explicit distribution function given in \cite{Harrison1985} for double numerical integration. The results for several values of $T$ and two different starting states are depicted in Figures 4-6. These plots also include the approximated functions $\hat{C}_{T}(\mu)$. 

%
\begin{figure}%
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
	xmin = 1,
	xmax = 5,
	ymin = 0,
	ymax = 2,
	xlabel = {$\to \mu$},
%	x label style={at={(0.6,0.04)}},
%	y label style={at={(0.075,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 5,2)},anchor = north east},
	legend columns=2,
	yscale = 0.8,
	xscale = 1
]


\addplot[col1, thick] table[x = mu,y=T2] {tikz/mm1_0.txt};
\addplot[col1, dashed, thick] table[x = mu,y=ap2] {tikz/mm1_0.txt};
\addplot[col4, thick] table[x = mu,y=T5] {tikz/mm1_0.txt};
\addplot[col4, dashed, thick] table[x = mu,y=ap5] {tikz/mm1_0.txt};
\addplot[col5, thick] table[x = mu,y=T10] {tikz/mm1_0.txt};
\addplot[col5, dashed, thick] table[x = mu,y=ap10] {tikz/mm1_0.txt};
\addplot[thick] table[x = mu,y=PSA] {tikz/mm1_0.txt};

\legend{{$C_2(\mu)$},{$\hat C_2(\mu)$},{$C_5(\mu)$},{$\hat C_5(\mu)$},{$C_{10}(\mu)$},{$\hat C_{10}(\mu)$},{$C_\infty(\mu)$}}
\end{axis}

\end{tikzpicture}
\caption{$x=0$}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
	xmin = 1,
	xmax = 5,
	ymin = 0,
	ymax = 3,
	xlabel = {$\to \mu$},
%	x label style={at={(0.6,0.04)}},
%	y label style={at={(0.075,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 5,3)},anchor = north east},
	legend columns=2,
	yscale = 0.8,
	xscale = 1
]


\addplot[col1, thick] table[x = mu,y=T2] {tikz/mm1_25.txt};
\addplot[col1, dashed, thick] table[x = mu,y=ap2] {tikz/mm1_25.txt};
\addplot[col4, thick] table[x = mu,y=T5] {tikz/mm1_25.txt};
\addplot[col4, dashed, thick] table[x = mu,y=ap5] {tikz/mm1_25.txt};
\addplot[col5, thick] table[x = mu,y=T10] {tikz/mm1_25.txt};
\addplot[col5, dashed, thick] table[x = mu,y=ap10] {tikz/mm1_25.txt};
\addplot[thick] table[x = mu,y=PSA] {tikz/mm1_25.txt};

\legend{{$C_2(\mu)$},{$\hat C_2(\mu)$},{$C_5(\mu)$},{$\hat C_5(\mu)$},{$C_{10}(\mu)$},{$\hat C_{10}(\mu)$},{$C_\infty(\mu)$}}
\end{axis}

\end{tikzpicture}
\caption{$x=2.5$}
\end{subfigure}
\caption{Comparison of exact waiting cost function $C_T(\mu)$ against corrected cost function $\hat{C}_T(\mu)$ and PSA cost function $C_\infty(\mu)$ for $T=2,5$ and 10 for the $M/M/1$ queue with $\la=1$.}
\label{fig:cont}%
\end{figure}
%
\begin{figure}[h!]
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
	xmin = 1,
	xmax = 5,
	ymin = 0,
	ymax = 2,
	xlabel = {$\to \mu$},
%	x label style={at={(0.6,0.04)}},
%	y label style={at={(0.075,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 5,2)},anchor = north east},
	legend columns=2,
	yscale = 0.8,
	xscale = 1
]


\addplot[col1, thick] table[x = mu,y=T2] {tikz/mp1_0.txt};
\addplot[col1, dashed, thick] table[x = mu,y=ap2] {tikz/mp1_0.txt};
\addplot[col4, thick] table[x = mu,y=T5] {tikz/mp1_0.txt};
\addplot[col4, dashed, thick] table[x = mu,y=ap5] {tikz/mp1_0.txt};
\addplot[col5, thick] table[x = mu,y=T10] {tikz/mp1_0.txt};
\addplot[col5, dashed, thick] table[x = mu,y=ap10] {tikz/mp1_0.txt};
\addplot[thick] table[x = mu,y=PSA] {tikz/mp1_0.txt};

\legend{{$C_2(\mu)$},{$\hat C_2(\mu)$},{$C_5(\mu)$},{$\hat C_5(\mu)$},{$C_{10}(\mu)$},{$\hat C_{10}(\mu)$},{$C_\infty(\mu)$}}
\end{axis}
\end{tikzpicture}
\caption{$x=0$}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
	xmin = 1,
	xmax = 5,
	ymin = 0,
	ymax = 3,
	xlabel = {$\to \mu$},
%	x label style={at={(0.6,0.04)}},
%	y label style={at={(0.075,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 5,3)},anchor = north east},
	legend columns=2,
	yscale = 0.8,
	xscale = 1
]


\addplot[col1, thick] table[x = mu,y=T2] {tikz/mp1_25.txt};
\addplot[col1, dashed, thick] table[x = mu,y=ap2] {tikz/mp1_25.txt};
\addplot[col4, thick] table[x = mu,y=T5] {tikz/mp1_25.txt};
\addplot[col4, dashed, thick] table[x = mu,y=ap5] {tikz/mp1_25.txt};
\addplot[col5, thick] table[x = mu,y=T10] {tikz/mp1_25.txt};
\addplot[col5, dashed, thick] table[x = mu,y=ap10] {tikz/mp1_25.txt};
\addplot[thick] table[x = mu,y=PSA] {tikz/mp1_25.txt};

\legend{{$C_2(\mu)$},{$\hat C_2(\mu)$},{$C_5(\mu)$},{$\hat C_5(\mu)$},{$C_{10}(\mu)$},{$\hat C_{10}(\mu)$},{$C_\infty(\mu)$}}
\end{axis}
\end{tikzpicture}
\caption{$x=2.5$}
\end{subfigure}
\caption{Comparison of exact waiting cost function $C_T(\mu)$ against corrected cost function $\hat{C}_T(\mu)$ and PSA cost function $C_\infty(\mu)$ for $T=2,5$ and 10 for the $M/$Pareto$/1$ queue with $\la=1$.}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
	xmin = 1,
	xmax = 5,
	ymin = 0,
	ymax = 2,
	xlabel = {$\to \mu$},
%	x label style={at={(0.6,0.04)}},
%	y label style={at={(0.075,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 5,2)},anchor = north east},
	legend columns=2,
	yscale = 0.8,
	xscale = 1
]


\addplot[col1, thick] table[x = mu,y=T2] {tikz/rbm1_0.txt};
\addplot[col1, dashed, thick] table[x = mu,y=ap2] {tikz/rbm1_0.txt};
\addplot[col4, thick] table[x = mu,y=T5] {tikz/rbm1_0.txt};
\addplot[col4, dashed, thick] table[x = mu,y=ap5] {tikz/rbm1_0.txt};
\addplot[col5, thick] table[x = mu,y=T10] {tikz/rbm1_0.txt};
\addplot[col5, dashed, thick] table[x = mu,y=ap10] {tikz/rbm1_0.txt};
\addplot[thick] table[x = mu,y=PSA] {tikz/rbm1_0.txt};

\legend{{$C_2(\mu)$},{$\hat C_2(\mu)$},{$C_5(\mu)$},{$\hat C_5(\mu)$},{$C_{10}(\mu)$},{$\hat C_{10}(\mu)$},{$C_\infty(\mu)$}}
\end{axis}
\end{tikzpicture}
\caption{$x=0$}
\end{subfigure}
\begin{subfigure}{0.48\textwidth}
\centering
\begin{tikzpicture}[scale=0.75]
\begin{axis}[
	xmin = 1,
	xmax = 5,
	ymin = 0,
	ymax = 3,
	xlabel = {$\to \mu$},
%	x label style={at={(0.6,0.04)}},
%	y label style={at={(0.075,0.6)}},
	axis line style={->},
	axis lines = left,
	legend cell align=left,
	legend style = {at = {(axis cs: 5,3)},anchor = north east},
	legend columns=2,
	yscale = 0.8,
	xscale = 1
]


\addplot[col1, thick] table[x = mu,y=T2] {tikz/rbm1_25.txt};
\addplot[col1, dashed, thick] table[x = mu,y=ap2] {tikz/rbm1_25.txt};
\addplot[col4, thick] table[x = mu,y=T5] {tikz/rbm1_25.txt};
\addplot[col4, dashed, thick] table[x = mu,y=ap5] {tikz/rbm1_25.txt};
\addplot[col5, thick] table[x = mu,y=T10] {tikz/rbm1_25.txt};
\addplot[col5, dashed, thick] table[x = mu,y=ap10] {tikz/rbm1_25.txt};
\addplot[thick] table[x = mu,y=PSA] {tikz/rbm1_25.txt};

\legend{{$C_2(\mu)$},{$\hat C_2(\mu)$},{$C_5(\mu)$},{$\hat C_5(\mu)$},{$C_{10}(\mu)$},{$\hat C_{10}(\mu)$},{$C_\infty(\mu)$}}
\end{axis}
\end{tikzpicture}
\caption{$x=2.5$}
\end{subfigure}
\caption{Comparison of exact waiting cost function $C_T(\mu)$ against corrected cost function $\hat{C}_T(\mu)$ and PSA cost function $C_\infty(\mu)$ for $T=2,5$ and 10 for reflected Brownian motion with $\sigma=1$.}
\end{figure}

We name a few observations based on these figures. 
First, we indeed note the pointwise convergence of $\hat{C}_{T}(\mu)$ to $\hat{C}_{\iy}(\mu)$ as $T$ grows, for all $\mu$ in all three cases. However, the difference between the stationary costs and those for small values of $T$ can be significant. This is most clear in the plots with $x=2.5$ and when $\mu$ is close to $\la$, i.e. it is in heavy-traffic. In these scenarios, it is evident that refinements to the stationary cost function are needed. $\hat{C}_{T}(\mu)$ does a fairly good job at providing such correction, especially for moderate values of $\mu$. 

Furthermore, we note that $C_{T}(\mu)$ approaches $C_{\iy}(\mu)$ from below for $x=0$ for any value of $\mu$, while this is not strictly the case for $x>0$. 
$\hat{C}_{T}(\mu)$ correctly captures the sign of this correction. 

Finally, observe that $\hat{C}_{T}(\mu)\to -\iy$ as $\mu$ approaches $\la$ from above. This divergence is clear from the expressions in \eqref{eq:MM1cor}-\eqref{eq:RBMcor}. 
Our correction term relies on the premise that under the coupling scheme, the sample paths of the two queues starting from different states have hit with high probability.
This is equivalent to stating that the `largest' of the two queues is has emptied at least once before time $T$. However, as $\mu$ approaches $\la$, the system enters heavy traffic, and hence the hitting time of the zero barrier is set to run off to infinity. 
Consequently, this causes our approximation to be inaccurate for small values of $\mu$. 


\subsection{Validation of corrected staffing rule}
\label{sec:num_opt}
In this section, we examine whether the corrected staffing rule $\tilde{\mu}_T^\star$ as in \eqref{eq:correctedMu} indeed yields a significant cost reduction over the choice of $\mui$ by comparing their true costs $\Pi_{T}(\tilde{\mu}_T^\star)$ and $\Pi_{T}(\mui)$.
We conduct this comparison for different values of the parameters, $\aaa$, $T$ and starting state $x$ through numerical experiments.  
The three models on which we do our calculations are the $M/M/1$ queue, the $M/$Pareto$/1$ queue and the reflected Brownian motion, as introduced in the previous subsection. 
We again focus on $\la=1$ only.

For each of the three models, we adhere to the following set-up. The quality of both staffing rules is assessed for $\aaa = 0.1, 1$ and 2, resembling three modes of valuation of the QoS in the system. 
As a benchmark, observe that the expected workload in steady-state conditions with staffing level $\mui$ equals
%
\begin{equation*}
C_\iy(\mui) = \sqrt{\frac{\aaa\la u_2}{2}}.
\end{equation*}
%
For each value of $\aaa$, we consider two scenarios: one in which the system starts empty, i.e. $x=0$, and one in which the initial state is double this benchmark value, thus $x=\sqrt{2\aaa\la u_2}$.
The numerics are presented for each model separately. We discuss general conclusions drawn from these results afterwards.\\
\\*
\noindent\textbf{$M/M/1$ queue}
As we discussed before, if $U$ is a unit rate compound Poisson process with exponentially distributed increments, then $\Qlm$ describes the workload process in an $M/M/1$ queue. 
For this setting we get
%
\begin{equation*}
\mui = \la + \sqrt{\frac{\la} {\aaa}},\qquad \tilde{\mu}_T^\star = \left[\la + \sqrt{\frac{\la} {\aaa}} + \frac{1}{T}\left( \frac{x^2}{4\sqrt{\la\aaa}} - 1 - \frac{3}{2} \sqrt{\la\aaa}\right)\right]^+.
\end{equation*} 
%
Table \ref{tab:mm1} presents the actual costs corresponding to these two staffing levels for different value of $x$ and $\aaa$. 
%
\begin{table}[h!]
\centering
\resizebox{13cm}{!} {
\begin{tabular}{|c|r|r @{}r|r@{}r|r||r@{}r|r@{}r|r|}
\cline{3-12}
\multicolumn{1}{c}{} & \multicolumn{1}{r|}{} & \multicolumn{5}{c||}{$x = 0$} & \multicolumn{5}{c|}{$x = 2\sqrt{\aaa}$} \\
\hline
$\aaa$ & $T$     & $\mui$  & \hspace{1pt} $\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt} $\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. & $\mui$  & \hspace{1pt}$\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt}$\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. \\
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{0.1}} & 1     & 4.162 & 0.620 & 2.688 & 0.536 & 0.136 & 4.162 & 0.682 & 2.688 & 0.536 & 0.214 \\
\multicolumn{1}{|c|}{} & 2     & 4.162 & 0.669 & 3.425 & 0.641 & 0.041 & 4.162 & 0.700 & 3.425 & 0.641 & 0.085 \\
\multicolumn{1}{|c|}{} & 5     & 4.162 & 0.706 & 3.867 & 0.703 & 0.005 & 4.162 & 0.719 & 3.867 & 0.703 & 0.022 \\
\multicolumn{1}{|c|}{} & 10    & 4.162 & 0.719 & 4.015 & 0.719 & 0.001 & 4.162 & 0.726 & 4.015 & 0.719 & 0.010 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{1}} & 1     & 2.000 & 2.309 & 0.000 & 0.500 & 0.783 & 2.000 & 3.500 & 0.500 & 2.750 & 0.214 \\
\multicolumn{1}{|c|}{} & 2     & 2.000 & 2.461 & 0.750 & 1.480 & 0.398 & 2.000 & 3.218 & 1.250 & 3.125 & 0.029 \\
\multicolumn{1}{|c|}{} & 5     & 2.000 & 2.675 & 1.500 & 2.400 & 0.103 & 2.000 & 3.043 & 1.700 & 2.968 & 0.025 \\
\multicolumn{1}{|c|}{} & 10    & 2.000 & 2.810 & 1.750 & 2.726 & 0.030 & 2.000 & 3.007 & 1.850 & 2.980 & 0.009 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{2}} &1     & 1.707 & 3.744 & 0.000 & 0.500 & 0.866 & 1.707 & 5.889 & 0.000 & 3.328 & 0.435 \\
\multicolumn{1}{|c|}{} &2     & 1.707 & 3.924 & 0.146 & 1.232 & 0.686 & 1.707 & 5.547 & 0.854 & 4.682 & 0.156 \\
\multicolumn{1}{|c|}{} &5     & 1.707 & 4.209 & 1.083 & 3.343 & 0.206 & 1.707 & 5.114 & 1.366 & 4.910 & 0.040 \\
\multicolumn{1}{|c|}{} &10    & 1.707 & 4.424 & 1.395 & 4.108 & 0.071 & 1.707 & 4.945 & 1.536 & 4.868 & 0.016 \\
\hline
\end{tabular}
}
\caption{Comparison of costs for the $M/M/1$ queue for steady-state and corrected staffing rules and relative cost improvement (r.c.i.).}
\label{tab:mm1}
\end{table}

\noindent
\textbf{$M$/Pareto/1 queue}
In case the service requirements follow a Pareto distribution with shape parameter $\gamma = 16/5$, the staffing rule becomes
\begin{equation*}
 \mui = \la + \frac{11}{8}\sqrt{\frac{ \la }{3 \aaa}}, \  \tilde{\mu}_T^\star = \left[\la + \frac{11}{8}\sqrt{\frac{ \la }{3 \aaa}} + \frac{1}{T}\left( \frac{2 x^2}{11\sqrt{\la\aaa/3}} - \frac{11}{8} - \frac{11\sqrt{3\la\aaa}}{16}\right)\right]^+.
 \end{equation*} 
The numerical results are given in Table \ref{tab:mp1}. 
\begin{table}[h!]
\centering
\resizebox{13cm}{!} {
\begin{tabular}{|c|r|r @{}r|r@{}r|r||r@{}r|r@{}r|r|}
\cline{3-12}
\multicolumn{1}{c}{} & \multicolumn{1}{r|}{} & \multicolumn{5}{c||}{$x = 0$} & \multicolumn{5}{c|}{$x = 11/4\cdot \sqrt{\aaa/3}$} \\
\hline
$\aaa$ & $T$     & $\mui$  & \hspace{1pt} $\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt} $\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. & $\mui$  & \hspace{1pt}$\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt}$\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. \\
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{0.1}} & 1     & 3.510 & 0.524 & 1.759 & 0.461 & 0.120 & 3.510 & 0.573 & 2.010 & 0.562 & 0.019 \\
\multicolumn{1}{|c|}{} & 2     & 3.510 & 0.555 & 2.635 & 0.539 & 0.029 & 3.510 & 0.580 & 2.760 & 0.574 & 0.010 \\
\multicolumn{1}{|c|}{} & 5     & 3.510 & 0.580 & 3.160 & 0.578 & 0.003 & 3.510 & 0.591 & 3.210 & 0.589 & 0.002 \\
\multicolumn{1}{|c|}{} & 10    & 3.510 & 0.590 & 3.335 & 0.590 & 0.000 & 3.510 & 0.596 & 3.360 & 0.595 & 0.001 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{1}} & 1     & 1.794 & 2.076 & 0.000 & 0.500 & 0.759 & 1.794 & 2.989 & 0.000 & 2.088 & 0.302 \\
\multicolumn{1}{|c|}{} & 2     & 1.794 & 2.190 & 0.511 & 1.291 & 0.411 & 1.794 & 2.790 & 0.610 &  2.588 & 0.072 \\
\multicolumn{1}{|c|}{} & 5     & 1.794 & 2.345 & 1.281 & 2.108 & 0.101 & 1.794 & 2.638 & 1.320 & 2.607 & 0.012 \\
\multicolumn{1}{|c|}{} & 10    & 1.794 & 2.441 & 1.537 & 2.371 & 0.029 & 1.794 & 2.597 & 1.557 & 2.585 & 0.005 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{2}} & 1     & 1.561 & 3.427 & 0.000 & 0.500 & 0.854 & 1.561 & 5.087 & 0.000 & 2.745 & 0.460 \\
\multicolumn{1}{|c|}{} & 2     & 1.561 & 3.567 & 0.032 & 1.050 & 0.706 & 1.561 & 4.832 & 0.172 & 3.417 & 0.293 \\
\multicolumn{1}{|c|}{} & 5     & 1.561 & 3.779 & 0.950 & 3.012 & 0.203 & 1.561 & 4.499 & 1.006 & 4.313 & 0.041 \\
\multicolumn{1}{|c|}{} & 10    & 1.561 & 3.935 & 1.255 & 3.356 & 0.147 & 1.561 & 4.351 & 1.284 & 4.304 & 0.011 \\
\hline
\end{tabular}
}
\caption{Comparison of costs for the $M/{\rm Pareto}/1$ queue for steady-state and corrected staffing rules and relative cost improvement (r.c.i.).}
\label{tab:mp1}
\end{table}
Just as in the results for the $M/M/1$ queue, we observe a higher reduction for larger value of $\aaa$ and $T$. Also, again $\tilde{\mu}_T < \mui$. Hence, the conclusions for the $M/{\rm Pareto}/1$ queue are similar to those of the $M/M/1$ queue. \\
\\*
\noindent\textbf{Reflected Brownian motion}.
In case the input process $U$ is Brownian motion with drift 1 and infinitesimal variance $\s^2$, the steady-state staffing rule and its corrected version reduce to 

\begin{equation*}
\mui = \la + \sqrt{\frac{\la\s^2}{2\aaa}}, \qquad  
\tilde{\mu}_T^\star = \left[\la + \sqrt{\frac{\la\s^2}{2\aaa}} + \frac{1}{2\sqrt{2}\,T}\left(\frac{x^2}{\sqrt{\la \aaa}\s} - 3\s\sqrt{\aaa\la}  \right)\right]^+.
\end{equation*}

In Tables \ref{tab:rbm1} and \ref{tab:rbm2}, the costs obtained through numerical evaluation are presented for several values of $x$, $T$. We also vary $\s$ to examine the influence of the volatility of arrival process on the quality of the staffing rules.

The observations on the influence of $\aaa, x$ and $T$ are similar to those of the $M/M/1$ queue and the $M/{\rm Pareto}/1$ queue. 
However, here we see little improvement by the corrected staffing rule for small values of $\aaa$ for both values of $x$. 
The results in Tables \ref{tab:rbm1}-\ref{tab:rbm2} also suggest that the reduction is smaller for larger values of $\s$. 

\begin{table}
\centering
\resizebox{13cm}{!} {
\begin{tabular}{|c|r|r @{}r|r@{}r|r||r@{}r|r@{}r|r|}
\cline{3-12}
\multicolumn{1}{c}{} & \multicolumn{1}{r|}{} & \multicolumn{5}{c||}{$x = 0$} & \multicolumn{5}{c|}{$x = \sqrt{2\aaa} $} \\
\hline
$\aaa$ & $T$     & $\mui$  & \hspace{1pt} $\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt} $\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. & $\mui$  & \hspace{1pt}$\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt}$\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. \\
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{0.1}} & 1     & 3.236 & 0.525 & 2.901 & 0.518 & 0.013 & 3.236 & 0.565 & 3.124 & 0.564 & 0.001 \\
\multicolumn{1}{|c|}{} & 2     & 3.236 & 0.536 & 3.068 & 0.534 & 0.003 & 3.236 & 0.556 & 3.180 & 0.556 & 0.000 \\
\multicolumn{1}{|c|}{} & 5     & 3.236 & 0.543 & 3.169 & 0.542 & 0.000 & 3.236 & 0.551 & 3.214 & 0.551 & 0.000 \\
\multicolumn{1}{|c|}{} & 10    & 3.236 & 0.545 & 3.203 & 0.545 & 0.000 & 3.236 & 0.549 & 3.225 & 0.549 & 0.000 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{1}} & 1     & 1.500 & 3.420 & 0.000 & 0.833 & 0.756 & 1.500 & 4.741 & 1.000 & 3.984 & 0.160 \\
\multicolumn{1}{|c|}{} & 2     & 1.500 & 3.539 & 0.750 & 2.386 & 0.326 & 1.500 & 4.579 & 1.250 & 4.293 & 0.063 \\
\multicolumn{1}{|c|}{} & 5     & 1.500 & 3.707 & 1.200 & 3.363 & 0.093 & 1.500 & 4.335 & 1.400 & 4.274 & 0.014 \\
\multicolumn{1}{|c|}{} & 10    & 1.500 & 3.820 & 1.350 & 3.705 & 0.030 & 1.500 & 4.190 & 1.450 & 4.175 & 0.004 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{2}} & 1     & 1.500 & 3.420 & 0.000 & 0.833 & 0.756 & 1.500 & 4.741 & 1.000 & 3.984 & 0.160 \\
\multicolumn{1}{|c|}{} & 2     & 1.500 & 3.539 & 0.750 & 2.386 & 0.326 & 1.500 & 4.579 & 1.250 & 4.293 & 0.063 \\
\multicolumn{1}{|c|}{} & 5     & 1.500 & 3.707 & 1.200 & 3.363 & 0.093 & 1.500 & 4.335 & 1.400 & 4.274 & 0.014 \\
\multicolumn{1}{|c|}{} & 10    & 1.500 & 3.820 & 1.350 & 3.705 & 0.030 & 1.500 & 4.190 & 1.450 & 4.175 & 0.004 \\
\hline
\end{tabular}
}
\caption{Comparison of costs for RBM with $\sigma = 1$ for steady-state and corrected staffing rules and relative cost improvement (r.c.i.).}
\label{tab:rbm1}
\end{table}

%%%%%%%% SIGMA = 2

\begin{table}
\centering
\resizebox{13cm}{!} {
\begin{tabular}{|c|r|r @{}r|r@{}r|r||r@{}r|r@{}r|r|}
\cline{3-12}
\multicolumn{1}{c}{} & \multicolumn{1}{r|}{} & \multicolumn{5}{c||}{$x = 0$} & \multicolumn{5}{c|}{$x = 2\sqrt{2\aaa} $} \\
\hline
$\aaa$ & $T$     & $\mui$  & \hspace{1pt} $\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt} $\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. & $\mui$  & \hspace{1pt}$\Pi_T(\mui)$ & $\tilde{\mu}_T^\star$  & \hspace{1pt}$\Pi_T(\tilde{\mu}_T^\star)$ & r.c.i. \\
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{0.1}} & 1     & 5.472 & 0.950 & 4.801 & 0.936 & 0.015 & 5.472 & 1.030 & 5.249 & 1.029 & 0.001 \\
\multicolumn{1}{|c|}{} & 2     & 5.472 & 0.972 & 5.137 & 0.968 & 0.003 & 5.472 & 1.012 & 5.360 & 1.012 & 0.000 \\
\multicolumn{1}{|c|}{} & 5     & 5.472 & 0.985 & 5.338 & 0.985 & 0.000 & 5.472 & 1.002 & 5.427 & 1.002 & 0.000 \\
\multicolumn{1}{|c|}{} & 10    & 5.472 & 0.990 & 5.405 & 0.990 & 0.000 & 5.472 & 0.998 & 5.450 & 0.998 & 0.000 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{1}} & 1     & 2.414 & 3.176 & 0.293 & 1.546 & 0.513 & 2.414 & 4.633 & 1.707 & 4.228 & 0.087 \\
\multicolumn{1}{|c|}{} & 2     & 2.414 & 3.356 & 1.354 & 2.690 & 0.199 & 2.414 & 4.375 & 2.061 & 4.247 & 0.029 \\
\multicolumn{1}{|c|}{} & 5     & 2.414 & 3.573 & 1.990 & 3.411 & 0.045 & 2.414 & 4.094 & 2.273 & 4.073 & 0.005 \\
\multicolumn{1}{|c|}{} & 10    & 2.414 & 3.689 & 2.202 & 3.646 & 0.012 & 2.414 & 3.966 & 2.344 & 3.962 & 0.001 \\
\hline
\hline
\multicolumn{1}{|c|}{\multirow{4}[2]{*}{2}} & 1     & 2.000 & 4.839 & 0.000 & 1.339 & 0.723 & 2.000 & 7.481 & 1.000 & 5.967 & 0.202 \\
\multicolumn{1}{|c|}{} & 2     & 2.000 & 5.078 & 0.500 & 2.773 & 0.454 & 2.000 & 7.158 & 1.500 & 6.585 & 0.080 \\
\multicolumn{1}{|c|}{} & 5     & 2.000 & 5.414 & 1.400 & 4.726 & 0.127 & 2.000 & 6.670 & 1.800 & 6.549 & 0.018 \\
\multicolumn{1}{|c|}{} & 10    & 2.000 & 5.639 & 1.700 & 5.409 & 0.041 & 2.000 & 6.380 & 1.900 & 6.349 & 0.005 \\
\hline
\end{tabular}
}
\caption{Comparison of costs for RBM with $\sigma = 2$ for steady-state and corrected staffing rules and relative cost improvement (r.c.i.).}
\label{tab:rbm2}
\end{table}

\subsection{Discussion}

Based upon these numerical results in Tables \ref{tab:mm1}-\ref{tab:rbm2}, we make a few remarks. The three models roughly exhibit similar behavior as $T$, $x$ and $\aaa$ are varied.

Non-surprisingly, we note that $\tilde{\mu}_T$ approaches $\mui$ with increasing $T$, which also implies that the cost reduction achieved by the corrected staffing rule vanishes as $T\to\iy$. 
Also, we observe that in all scenarios examined, the cost reduction increases with $\aaa$. This can be explained through investigation of the objective function $\Pi_T$ as function of $\m$. Namely, for $\aaa$ small, the curve is relatively flat around the true optimum $\muT$. Hence, in this case a moderate deviation from $\muT$ will likely not lead to a significant cost increase. However, as $\aaa$ becomes larger, i.e. server efficiency is valued more than minimization of congestion, the curve becomes more sharp around $\muT$, and hence more accurate approximations of $\muT$ are required to achieve an acceptable cost level. Hence, the corrected staffing rule \eqref{eq:correctedMu} proves particularly useful in these cases.

Another point we highlight is that the relative improvement is higher for $x=0$ than for $x=\sqrt{2\aaa\la u_2}$. Moreover, even though the initial state of the system is above the optimal equilibrium, $\tilde{\mu}_T$ is smaller than $\mui$. This is somewhat counter-intuitive. In fact, from \eqref{eq:muBullet} it follows that $\mu_\bullet$ positively contributes to the corrected staffing function if
%
\begin{equation*}
\E[Q^2(0)] >  3\aaa\la u_2 + \frac{2 u_2}{3 u_3}\,\sqrt{2\aaa\la u_2}.
\end{equation*}
%
%Even more surprisingly, obverse that if $Q(0)\equiv Q(\iy)$ with $\mu \equiv \mui = \la + \sqrt{\la u_2/(2\aaa)}$ we get with Lemma \ref{lemma:workloadmoments}
%%
%\begin{equation*}
%\E[Q^2(0)] = \aaa\la u_2 + \frac{u_3}{3} \sqrt{\frac{2\aaa\la} {u_2}},
%\end{equation*}
%%
%so that
%%
%\begin{equation*}
%\mu_\bullet = {-}\frac{u_3}{2 u_2} - \sqrt{2\aaa\la u_2} < 0.
%\end{equation*}
%%
%This suggests that even when the process is started in equilibrium with the corresponding optimal steady-state speed $\mui$, it is more cost efficient to change the server speed. This seems strange, but we provide an explanation for this phenomenon. 
%In our particular setting, we strictly focus on the period $[0,T]$, and do not care about what happens after time $T$. Hence, it might be beneficial to let the queue build up towards the end of the period, thereby employing a smaller server speed than stipulated by the steady-state optimum. 
%Naturally, this effect diminishes with increasing $T$.
\section{Conclusion \& further research}
\label{sec:conclusion_chapter6}
Motivated by the time-varying nature of queues in practical applications, we studied the impact that the transient phase has on traditional capacity allocation questions.
By defining a cost minimization problem, in which the objective function contains a correction accounting for the transient period, we identified the leading and second-order behavior of the cost function as a function of the interval length $T$. 
As a by-product, this result yields an approximation for the actual cost function, which is a refinement to its stationary counterpart.
Our numerical experiments in Section \ref{sec:influence_omega} demonstrate the improved accuracy achieved by this approximation in a number of settings. 
By perturbation analysis of the optimization problem, this furthermore gives rise to a correction to the steady-state optimal capacity allocation of order $1/T$. 
The necessity of the refined capacity allocation level is substantiated by the numerics in Section \ref{sec:num_opt}, which show the cost reduction that can be achieved in the number of settings, compared to settings in which stationary metrics are used.  
Especially for small values of $T$ and large values of $\alpha$ this reduction is significant.
Additionally, these results also indicate that it is relatively safe to use the stationary cost when $T$ is moderate, or $\alpha$ is small. 
The latter reflects the scenario in which QoS is much more valued than service efficiency. 
This observation links to the flat nature of the cost function around its optimal value for $\alpha$ small, a statement on the optimality gap that we formally proved in Proposition \ref{prop:optimalitygap_mui}.

Besides the validation of our theoretical results of Sections \ref{sec:analysis} and \ref{sec:optimization}, the numerical results also reveal some phenomena that require more investigation. 
As noted, our corrected capacity allocation level $\tilde{\mu}_T^\star$ is in most studied cases less than the steady-state optimal value $\mu_{\iy}^\star$. This implies that congestion levels tends to be higher under our staffing scheme then under stationary staffing. 
A possible explanation for this may be the fact that the planning period under consideration is finite. 
Clearly, in the setting we analyzed, anything that happens after time $T$ is neglected. 
Therefore, it might be beneficial from the cost perspective to end the period with a higher expected congestion level, as it does not need to be canceled out in the future. 
Related to this observation, it would be interesting to look at the setting in which staffing decisions need to be made in consecutive periods of equal length, in which the arrival rate changes at the start of each period. 
This case requires careful consideration of the correlation among the staffing decisions within the separate periods.

Another question that arises concerns the translation of our (qualitative) findings to more general queues, in particular the $M/G/s$ queue. 
Whereas in our analysis, the central decision variable is the server speed $\mu$, the variable of interest in multi-server queues is typically the number of servers. 
It may well be that similar explicit corrections to staffing levels can be deduced to account for transience.
Since our analysis heavily relies on the comparibility of the sample paths of two single-server queues, which is due to the equal negative drift for the two processes, another approach must be taken to tackle this extension.

The analysis and findings for the single-server queue with L\'evy input presented in this chapter may serve a stepping stone for investigation of these more elaborate problems.


\section*{Appendix}

\addcontentsline{toc}{section}{\hspace{7.1mm} Appendix}

\begin{subappendices}

\settocdepth{chapter}


\section{Proofs of Section \ref{sec:model_description}}
\label{app:proofs_model}

\subsection{Proof of Lemma \ref{lemma:workloadmoments}}
\label{app:proof_lemma_workload_moments}
\begin{proof}
The conditions of \cite[Cor.IX3.4]{Asmussen2003} are satisfied and therefore $Q_{\mu}(t)\Rightarrow \Qlm(\infty)$ in distribution for $t\rightarrow\infty$. Furthermore, its Laplace transform is for ${\rm Re}(s) < 0$
%
\[\tilde{Q}_{\mu}(s) = \E[s \Qlm(\infty)] = \frac{s \ka_{\mu}'(0)}{\ka_{\mu}(s)} = \frac{s(\la\ka_U'(0) - \mu)}{\la\ka_U(s) - \mu s} = \frac{s(\mu-\la)}{\mu s-\la \ka_U(s)}.\]
%
It can be checked that $\ka_U'(0) = \E[U(1)] = 1$, $\ka_U''(0) = u_2$ and $\ka_U'''(0) = u_3$, and $\klm'(0) = \la-\mu$, $\klm''(0) = \la u_2$ and $\klm'''(0) = \la u_3$.
Using l'H\^opital's rule we obtain the first moment of $\Qlm(\infty)$:
%
\begin{align*}
\E[\Qlm(\iy)] &= {-}\lim_{s\to 0} \frac{d}{ds} \tilde{Q}_{\mu}(s) = \lim_{s\to 0} \klm'(0)\, \frac{s\klm'(s)-\klm(s)}{\klm(s)^2}\\
&= \lim_{s\to 0} \klm'(0)\, \frac{{-}s\klm''(s)}{2\klm(s)\klm'(s)} 
= \lim_{s\to 0} \klm'(0)\,\frac{ s\klm'''(s)-\klm''(s)}{2\klm'(s)^2 + 2\klm(s)\klm'''(s)} \\
&= {-}\frac{\klm''(0)}{2\klm'(0)} = \frac{\la u_2}{2(\mu-\la)}.
\end{align*}
%
Similarly we derive the second moment:
%
\begin{align*}
\E[\Qlm^2(\iy)] &= \lim_{s\to 0} \frac{d^2}{ds^2} \tilde{Q}_{\mu}(s) 
= \lim_{s\to 0} \klm'(0)\, \frac{3 \klm''(0)^2 - 2\klm'(0)\klm'''(0)}{6 \klm'(0)^3}\\
&= (\la-\mu)\frac{3\la^2u_2^2 - 2\la u_3(\la-\mu)}{6(\la-\mu)^3}
= \frac{\la^2u_2^2}{2(\mu-\la)^2} +\frac{\la u_3}{3(\mu-\la)}.
\end{align*}
\end{proof}


\subsection{Proof of Proposition \ref{prop:cost_convergence}}
\begin{proof}
We prove the limit by showing that the difference
\[
\Pi_T(\mu) - \Pi_\iy(\mu) = \frac{1}{T} \int_0^T \E[Q_\mu(t)] - \E[Q_\mu(\iy)] \, \dd t
\]
converges to zero as $T\to\iy$ for $\mu>\la$ fixed. The assumption $\E[U(1)], \E[Q(0)] < \iy$ implies by \cite[Prop.~1]{Abate1994} that $\E[Q_\mu(t)]<\iy$ for all $t\geq 0$.
Following \cite{Abate1994}, we use the decomposition
\[
\E[Q_\mu(t)] = \E[Q^0_\mu(t)] + \left\{ \E[Q_\mu(t)] - \E[Q_\mu^0(t)]\right\},
\]
where $Q_\mu^0(t)$ represents the workload process if the system starts empty. 
From this decomposition it is revealed that $\E[Q^0_\mu(t)]$ and $\left\{ \E[Q_\mu(t)] - \E[Q_\mu^0(t)]\right\}$ are non-negative monotonically increasing and decreasing functions of $t$, respectively, see \cite[Prop.~2,Thm.~11]{Abate1994}. 
 Recall $\E[Q_\mu(t)] \to \E[Q_\mu(\iy)]$ for $t\to\iy$ by ergodicity of the workload process for any initial state $\E[Q(0)]< \iy$, if $\mu>\la$.
 Henceforth,
\begin{align*}
\E[Q_\mu(t)] &\leq \sup_t \E[Q_\mu^0(t)] + \sup_t  \left\{ \E[Q_\mu(t)] - \E[Q_\mu^0(t)]\right\} \\
&= \E[Q_\mu(\iy)] + \left\{\E[Q_\mu(0)] - \E[Q_\mu^0(0)]\right\} = \E[Q_\mu(\iy)] + \E[Q(0)],
\end{align*}
for all $t\geq 0$, which proves that the expected workload is bounded.
Fix $\varepsilon>0$. By convergence of $\E[Q_\mu(t)]$ for $t\to\iy$, there exists a value $t^* := t^*(\varepsilon)$ such that for all $t\geq t^*$
\begin{equation}
\left| \E[Q_\mu(t)] - \E[Q_\mu(\iy)] \right| < \varepsilon/2.
\end{equation}
Next, set
\[
T^* := T^*(\varepsilon) = \frac{2\,t^*(\varepsilon)}{\varepsilon}\, ( 2 \E[Q_\mu(\iy)] + \E[Q(0)]).
\]
Then for $T\geq \hat{T}:= \max\{ t^*,T^* \}$, we have
\begin{align*}
\left| \frac{1}{T} \int_0^T \E[Q_\mu(t)] - \E[Q_\mu(\iy)] \, \dd t \right| 
&\leq \frac{1}{T} \int_0^{t^*} \left| \E[Q_\mu(t)] - \E[Q_\mu(\iy)] \right|  \dd t \\
& \qquad+ \frac{1}{T} \int_{t^*}^T \left| \E[Q_\mu(t)] - \E[Q_\mu(\iy)] \right| \, \dd t \\
&\leq \frac{1}{T} \int_0^{t^*} \E[Q_\mu(t)] + \E[Q_\mu(\iy)] \, \dd t + \frac{1}{T} \int_{t^*}^T \frac{\varepsilon}{2}\, \dd t \\
&< \frac{t^*}{T}\,( 2 \E[Q_\mu(\iy)] + \E[Q(0)]) + \frac{T-t^*}{T} \,\frac{\varepsilon}{2}\\
&< \frac{t^*}{T^*} \,( 2 \E[Q_\mu(\iy)] + \E[Q(0)]) + \frac{\varepsilon}{2} = \varepsilon.
\end{align*}
Hence, for any choice of $\varepsilon>0$ we can find a value $\hat{T}$ such that $\Pi_{\hat{T}}(\mu)$ approaches $\Pi_\iy(\mu)$ within distance $\varepsilon$, which proves the limit.
\end{proof}


\section{Proofs of Section \ref{sec:analysis}}
\label{app:proofs_analysis}
\subsection{Proof of Lemma \ref{lemma:psixy}}
\begin{proof}
Using the representation in \eqref{eq:Yxy} we write
%
\begin{align*}
\Psi^{x,y}_T &= \frac{1}{T}\int_0^{\infty} \E[Y^{x,y}(t)]\dd t \\
&= \frac{1}{T}\,\E\left[\int_0^{\tau^y(0)}Y^{x,y}(t)\right] \dd t + \frac{1}{T}\,\E\left[\int_{\tau^y(0)}^{\tau^x(0)} Y^{x,y}(t) \dd t\right]
+ \frac{1}{T}\,\E\left[\int_{\tau^y(0)}^\infty Y^{x,y}(t) \dd t\right] ,\\
&= \frac{1}{T}\,\E\left[\int_0^{\tau^y(0)}(x-y) \dd t\right] + \frac{1}{T}\,\E\left[\int_{\tau^y(0)}^{\tau^x(0)} Y^{x,y}(t) \dd t\right] \\
&= \frac{1}{T}\,\E[\tau^y(0)](x-y) + \frac{1}{T}\,\E\left[\int_{\tau^y(0)}^{\tau^x(0)} Y^{x,y}(t) \dd t\right].
\end{align*}
By \eqref{eq:Yxy} and the Strong Markov property holding for L\'evy processes \cite{Asmussen2003}, observe that \\* $Y^{x-y,0}(t) \equalD Y^{x,y}(\tau^y(0)+t)$, whereby
%
\begin{equation*}
\frac{1}{T}\,\E\left[\int_{\tau^y(0)}^{\tau^x(0)} Y^{x,y}(t)\,\dd t\right] = \frac{1}{T}\,\E\left[\int_{0}^{\tau^{x-y}(0)} Y^{x-y,0}(t) \dd t\right] = \Psi^{x-y,0}_T,
\end{equation*}
% 
which completes the proof.
\end{proof}

\subsection{Proof of Lemma \ref{lemma:psiz0}}
\begin{proof}
Note that $Y^{z,0}(t)$ and $\tau^z(w)$ are intimately related. Namely, due to the fact that $X$ has no negative jumps 
\begin{equation*}
\{ \tau^z(w) \leq t\} = \{Y^{z,0}(t) \leq w \}.
\end{equation*}
In fact, $Y^{z,0}(\tau^z(w)) = w$, which implies that $\tau^z$ is a right inverse for $Y^{z,0}(t)$. Therefore, the following equality holds
%
\begin{equation*}
\int_0^{\tau^z(0)} Y^{z,0}(t)\, \dd t = \int_0^z \tau^z(w)\, \dd w,
\end{equation*}
%
which implies with the help of Fubini's theorem
%
\begin{equation*}
\Psi^{z,0}_T = \frac{1}{T}\,\int_0^z \E[\tau^z(w)]\, \dd w = \frac{1}{T}\,\int_0^z \E[\tau^{z-w}(0)]\,\dd w =\frac{1}{T}\, \int_0^z \E[\tau^{w}(0)] \,\dd w.
\end{equation*}
\end{proof}

\subsection{Proof of Corollary \ref{cor:Psixy}}
\begin{proof}
From \eqref{eq:invCharExp},
%
\begin{equation}\label{eq:corEq1}
\E[\hat{\tau}^0(w)] = -\tfrac{\dd}{\dd u} \left. \E[\exp(-u\,\hat{\tau}^0(w))]\right|_{u=0} = w\left.\frac{\dd}{\dd u} \Upsilon^{-1}(u)\right|_{u=0}.
\end{equation}
%
Since $\Upsilon(\theta)$ is strictly increasing and $\Upsilon(0)=0$, we get $\Upsilon^{-1}(0)=0$ and
%
\begin{equation*}
\left.\tfrac{\dd}{\dd u}\Upsilon^{-1}(u)\right|_{u=0} = \frac{1}{\Upsilon'(\Upsilon^{-1}(0))} = \{ \Upsilon'(0) \}^{-1}.
\end{equation*}
%
Furthermore,
%
\begin{align*}
\Upsilon'(\thh) &= -a+ \s^2\thh + \int_{-\infty}^0 (x\, \ee^{\thh x} - x{\bf 1}_{[-1,0)}(x)) \hat{\nu}(\dd x) \\
&=  -a + \s^2\thh - \int_0^\infty (y\, \ee^{-\thh y} - y{\rm 1}_{(0,1]}(y)) \nu(\dd y).
\end{align*}
%
Thus, $\Upsilon'(0) = -\E[X(1)] = \mu-\la$ and $\E[\hat{\tau}^0(w)] = w/(\mu-\la)$. By \eqref{eq:H(x,0)} and \eqref{eq:transformedTau}, we deduce that
%
\begin{equation*}
\Psi^{z,0}_T = \frac{1}{T}\, \int_0^z \E[\tau^w(0)] \,\dd w = \frac{1}{T}\, \int_0^z \E[\hat{\tau}^0(w)] \dd w = \frac{z^2}{2T(\mu-\la)}.
\end{equation*}
For $x>y$, we use Lemma \ref{lemma:psixy} to conclude
%
\begin{equation*}
\Psi^{x,y}_T =  \frac{y(x-y)}{T(\mu-\la)} + \frac{(x-y)^2}{2 T(\mu-\la)} = \frac{x^2-y^2}{2T(\mu-\la)}.
\end{equation*}
The result for $x<y$ follows directly by the observation $\Psi^{x,y}_T = -\Psi_T^{x,y}$.

\end{proof}


\subsection{Proof of Proposition \ref{prop:truncation_error}}\label{sec:proof_truncation}

\begin{proof}
To derive the upper bound for $\Delta^{x,y}_T$, we apply the same coupling argument as in described in Section 3. Let us assume without loss of generality $x>y$. 
In this case, 
%
\begin{equation*}
|\Delta^{x,y}_T| = \frac{1}{T} \int_T^\iy \E[Q^x(t)-Q^y(t)] \dd t \leq \frac{1}{T}\int_T^\iy \E[Q^x(t)-Q^0(t)]\dd t.
\end{equation*}
%
By the decomposition in \eqref{eq:Yxy},
%
\begin{align}
 \int_T^\infty \E[Q^x(t) - Q^0(t)] \dd t
	&= \int_T^\infty \E[(x+\inf_{s\leq t} X(s))\mathbbm{1}_{\{\tau^x(0)>t\}}] \dd t \nonumber\\
	&= \int_T^\infty \int_0^x P( x-u + \inf_{s\leq t}X(s) > 0) \dd u \dd t \nonumber\\
	&= \int_T^\infty \int_0^x P( \tau^{x-u}(0) > t ) \dd u\dd t \\
	&\leq \int_T^\iy \int_0^x \frac{\E[\tau^{x-u}(0)^2]}{t^2}\dd u \dd t \nonumber\\
	&=  \int_0^x \int_T^\iy \frac{\E[\tau^{x-u}(0)^2]}{t^2}\dd t\dd u
	= \int_0^x \frac{\E[\tau^{w}(0)^2]}{T}\,\dd w. \nonumber
	\label{eq:tailprobIntegral}
\end{align}
%
We obtain $\E[\tau^w(0)^2]$ with the help of its Laplace transform in \eqref{eq:invCharExp}. Namely,
%
\begin{align*}
\E[\tau^w(0)^2] &= \left.\tfrac{\dd^2}{\dd u^2}\E[\exp(-u \tau^w(0))]\right|_{u=0} \\
&= w^2\,\left(\left.\tfrac{\dd}{\dd u}\Upsilon^{-1}(u)\right|_{u=0}\right)^2 - w\left. \tfrac{\dd^2}{\dd u^2}\Upsilon^{-1}(u)\right|_{u=0}.
\end{align*}
%
As in the previous subsection we have $\left.\tfrac{\dd}{\dd u}\Upsilon^{-1}(u)\right|_{u=0} = (\mu-\la)^{-1}$, and 
%
\begin{equation*}
\left.\tfrac{\dd^2}{\dd u^2}\Upsilon^{-1}(u)\right|_{u=0} = {-}\frac{\Upsilon''(\Upsilon^{-1}(0))}{\Upsilon'(\Upsilon^{-1}(0))^3} = {-}\frac{\Upsilon''(0)}{\Upsilon'(0)^3}.
\end{equation*}
%
Since $\Upsilon'(0) = \mu-\la$ and 
%
\begin{equation*}
\Upsilon''(0) = \s^2 + \int_0^\infty x^2\,\nu(\dd x) = u_2,
\end{equation*}
%
we conclude
%
\begin{equation*}
\E[\tau^w(0)^2] = \frac{w^2}{(\m-\la)^2} + \frac{u_2w}{(\m-\la)^3},
\end{equation*}
%
so that
\begin{equation}\label{eq:delta_upper}
|\Delta^{x,y}_T| \leq \frac{1}{T^2}\int_0^x \frac{w^2}{(\m-\la)^2} + \frac{u_2w}{(\m-\la)^3} \dd w = \frac{1}{T^2}\left(\frac{x^3}{3(\mu-\la)^2}+\frac{u_2 x^2}{2(\m-\la)^3}\right).
\end{equation}
%
For general $x,y\geq 0$, 
%
\begin{equation*}
|\Delta^{x,y}_T| \leq \frac{1}{T^2}\left(\frac{\max(y,x)^3}{3(\mu-\la)^2}+\frac{u_2 \max(y,x)^2}{2(\m-\la)^3}\right).
\end{equation*}
%
As a direct consequence,
\begin{equation*}
|\Delta_T| \leq \frac{1}{T^2}\left(\frac{\E[\max(Q(0),Q_\m(\iy))^3]}{3(\mu-\la)^2}+\frac{u_2 \E[\max(Q(0),Q_\m(\iy))^2]}{2(\m-\la)^3}\right).
\end{equation*}
\end{proof}
\noindent\textit{Remark.} 
Observe that if $X$ is light-tailed, that is $\E[\exp\{ -\theta X(1) \}]$ $= \E[\exp\{\kappa(\theta)\}] < \iy$ for some $\theta<0$, then $\Upsilon(\theta)$ as in \eqref{eq:invCharExp} has an analytic continuation in the negative half-plane, and in this region $\Upsilon(\theta)<0$. Consequently, we can replace the upper bound on the tail probability of $\tau^{x-u}(0)$ by 
\begin{equation*}
\mathbb{P}\left( \tau^{x-u}(0) > t\right) = \mathbb{P}\left( \ee^{\beta \tau^{x-u}(0)} > \ee^{\beta t} \right) \leq \ee^{-\beta t} \, \ee^{ (x-u)\Upsilon^{-1}(-\beta)},
\end{equation*}
for some $\beta > 0$, so that
%
\[ \int_T^\infty \E[Q^x(t) - Q^0(t)]\, \dd t \leq \ee^{-\beta T}\, \frac{\ee^{x\Upsilon^{-1}(-\beta)}-1}{\beta\,\Upsilon^{-1}(-\beta)}. \]
Along similar lines we deduce
\[ |\Delta^{x,y}_T| \leq \frac{ \ee^{-\beta T}}{T}\, \frac{\ee^{x\Upsilon^{-1}(-\beta)} + \ee^{y\Upsilon^{-1}(-\beta)} -2}{\beta\,\Upsilon^{-1}(-\beta)}
\]
and 
\[ |\Delta_T| \leq \frac{\ee^{-\beta T}}{T}\, \frac{\E[\ee^{Q(0)\Upsilon^{-1}(-\beta)}] + \E[\ee^{Q_\mu(\iy)\Upsilon^{-1}(-\beta)}] -2}{\beta\,\Upsilon^{-1}(-\beta)},\]
assuming that $\E[{\rm e}^{-y Q(0)}] < \iy$ for all $y>0$. The condition $\E[{\rm e}^{Q_\mu(\iy)\Upsilon^{-1}(-\beta)}]<\iy$ follows from Lemma \ref{lemma:workloadmoments}. 
Hence, the error decays exponentially fast for light-tailed input processes.
\section{Proofs of Section \ref{sec:optimization}}
\label{app:proofs_optimization}

\subsection{Proof of Lemma \ref{lemma:strict_convexity}}
\begin{proof}

Since the term $\aaa\mu$ is convex, the strictness should come from  the term $C_T(\mu)$. 
Furthermore, observe that if a function $f_\mu(t)$ is convex for all $t\geq 0$, and strictly convex for all $t\geq\e$ for some $\e\in[0,T)$, i.e. for any $\mu_1,\mu_2>0$ and $a\in (0,1)$
\begin{equation*}
a\, f_{\mu_1}(t) + (1-a) f_{\mu_2}(t) > f_{a\mu_1+(1-a)\mu_2}(t),
\end{equation*}
then,
\begin{equation*}
a\int_0^T \, f_{\mu_1}(t)\, \dd t + (1-a)\int_0^T f_{\mu_2}(t) \dd t =
\int_0^T \, a f_{\mu_1}(t) + (1-a)f_{\mu_2}(t) \dd t 
\end{equation*}
\begin{align*}
&=  \int_0^\e a f_{\mu_1}(t) + (1-a)f_{\mu_2}(t) \dd t  + \int_\ee^T \, a f_{\mu_1}(t) + (1-a)f_{\mu_2}(t) \dd t \\
&> \int_0^\e  f_{a\mu_1+(1-a)\mu_2}(t) \dd t + \int_\ee^T  f_{a\mu_1+(1-a)\mu_2}(t)  \dd t. \\
&= \int_0^T  f_{a\mu_1+(1-a)\mu_2}(t)  \dd t.
\end{align*}
Hence, it suffices to prove the convexity of $\E[Q_\mu(t)]$ as a function of $\mu$ for all $t\geq 0$, and strict convexity for $t\geq \e$ for some $\e\in[0,T)$.
Let $\tau^x_{\mu}(0)$ denote the first passage time of level  0 is the process $Q_\mu$ with $Q(0)=x$. Then,
%
\begin{align}
Q_\mu(t) &= U(t)-\mu t + \max\left\{ x , -\inf_{s\leq t} [ U(s)-\mu s] \right\}\\
&=
\left\{
\begin{array}{ll}
x+U(t)-\mu t, & \text{if } t<\tau^x_{\mu}(0),\\
U(t)-\mu t  -\inf_{s\leq t} [ U(s)-\mu s], & \text{if } t\geq \tau^x_{\mu}(0) ,
\end{array}\right.\label{eq:Qrep}
\end{align}
%
where
\begin{equation*}
 \tau^x_{\mu}(0) := \inf\{ t \geq 0\,:\, x+U(t)-\mu t \leq 0\}
 \end{equation*} 
%
and $U(t)$ is a spectrally positive L\'evy process.
Fix $\mu_1, \mu_2>0$ and $a\in(0,1)$. Define $\mu_3 := a\mu_1+(1-a)\mu_2$, and
%
\begin{equation*}
D(t) := a Q_{\mu_1}(t) + (1-a) Q_{\mu_2}(t) - Q_{\mu_3}(t).
\end{equation*}
In order to prove strict convexity we have to show that $D(t) \geq 0$ for all $t\geq 0$, thereby implying $\E [D(t)] \geq 0$, i.e. convexity, for all $t\geq 0$, and $D(t)>0$ with positive probability for $t\in[\e,T]$, for some $\e \in[0,T)$. 
We distinguish two cases: $x>0$ and $x=0$. \\
\\*
\textbf{The case $x>0$.}
We start by noticing that if $Q_{\mu_1}$, $Q_{\mu_2}$ and $Q_{\mu_3}$ experience the same input process $U(t)$, then by absence of negative jumps in $U(t)$, it holds that
\begin{equation}\label{eq:stochDom}
\tau^x_{\mu_2}(0) < \tau^x_{\mu_3}(0) < \tau^x_{\mu_1}(0).
\end{equation}
%
We use shorthand notation 
\begin{equation*}
I_k(t) := \inf_{0\leq s\leq t}[U(s)-\mu_k s],
\end{equation*}
%
for $k=1,2,3$.
Using representation \eqref{eq:Qrep} of the workload process, we obtain 
%
\begin{equation*}
D(t) = \left\{
\begin{array}{ll}
0,  
& \text{if } t < \tau^x_{\mu_2}(0),\\
-(1-a)\left(x+I_2(t) \right), 
& \text{if } \tau^x_{\mu_2}(0) \leq t < \tau^x_{\mu_3}(0),\\
a x - (1-a)I_2(t) + I_3(t),
& \text{if } \tau^x_{\mu_3}(0) \leq t < \tau^x_{\mu_1}(0),\\
- a I_1(t) - (1-a) I_2(t)
+ I_3(t),
& \text{if } t \geq \tau^x_{\mu_1}(0).
\end{array}
\right.
\end{equation*}
%
This partition allows us to spot when strict convexity can occur.
Note that by definition $t \geq \tau^x_{\mu_2}(0)$, $I_2(t) = \inf_{0\leq s\leq t}[U(s)-\mu_2s]\leq -x$, so that $D(t)\geq 0$ if $\tau^x_{\mu_2}(0) \leq t < \tau^x_{\mu_3}(0)$. 
Moreover, by subadditivity of the infimum, 
\begin{align*}
I_3(t) &= \inf_{0\leq s\leq t}[U(s)-\mu_3s] = \inf_{0\leq s\leq t}[a(U(s)-\mu_1s)+(1-a)(U(s)-\mu_2s)] \\
&\geq a \inf_{0\leq s\leq t}[U(s)-\mu_1s] + (1-a) \inf_{0\leq s\leq t}[U(s)-\mu_2s] = a I_1(t) + (1-a) I_2(t),
\end{align*}
%
and hence $D(t)\geq 0$ for $t \geq \tau^x_{\mu_1}(0)$.
Using the same argument, we deduce
%
\begin{equation*}
ax - (1-a)I_2(t) + I_3(t) \geq a x - (1-a) I_2(t) + a I_1(t) + (1-a) I_2(t) = a(x + I_1(t)).
\end{equation*}
%
In particular for $t < \tau^x_{\mu_1}(0)$, this value is strictly positive. 
As a result, $D(t)\geq 0$ for all $t\geq 0$.
On top of that $D(t) > 0$ for $t\in[\tau^x_{\mu_3}(0),\tau^x_{\mu_1}(0))$.
Accordingly, the latter implies strict positivity of $\E D(t)$, and therefore strict convexity of $\E Q_\mu(t)$, if the event $\{\tau^x_{\mu_3}(0)\leq t< \tau^x_{\mu_1}(0)\}$ occurs with positive probability. 
That is, 
%
\begin{align}
P(D(t)>0) &\geq P\left( a(x+I_1(t))\mathbbm{1}_{\{\tau^x_{\mu_3}(0)\leq t < \tau^x_{\mu_1}(0)\}}  > 0 \right)\nonumber\\
&= P\left( x+ I_1(t) > 0 , \tau^x_{\mu_3}(0)\leq t < \tau^x_{\mu_1}(0)\right)\nonumber\\
&= P\left( x+ I_1(t) > 0 | \tau^x_{\mu_3}(0)\leq t < \tau^x_{\mu_1}(0)\right)P\left(\tau^x_{\mu_3}(0)\leq t < \tau^x_{\mu_1}(0)\right)\nonumber\\
&= P\left(\tau^x_{\mu_3}(0)\leq t < \tau^x_{\mu_1}(0)\right) = P(\tau^x_{\mu_3}(0)\leq t) - P(\tau^x_{\mu_1}(0) \leq t) > 0, \label{eq:strictConv}
\end{align}
by the stochastic dominance in \eqref{eq:stochDom}. To ensure the strict inequality in \eqref{eq:strictConv} we have to enforce the condition
\begin{equation}\label{eq:condition}
P(\tau^x_{\mu_1}(0)<T) > 0.
\end{equation}
%
\textit{Remark.}
An example illustrating the need for this condition is the case in which $U(t)$ is a compound Poisson process and $T < x/\mu_2 < x/\mu_1$. Then 
%
\[Q_{\mu_k}(t) = x + U(t) - \mu_k t,\]
% 
for all $t\in[0,T]$, since $U(t)\geq 0$ and therefore $\tau^x_{\mu_1}(0) > T$. Consequently, for all $a\in(0,1)$, 
\[ a\,Q_{\mu_1} + (1-a)\,Q_{\mu_2}(t) = Q_{\mu_3}(t),\]
proving only convexity of $\E Q_{\mu}(t)$ and subsequently $\int_0^T \E[Q_\mu(t)]\,\dd t$. In case $\sigma>0$, the probability in \eqref{eq:condition} is necessarily positive.
\\*

\noindent \textbf{The case $x=0$.}
By the fact that $\tau_{\mu}(0) = 0$ for all $\mu>0$, proving that $D(t)>0$ for in the case $x=0$ reduces to showing that the probability of 
%
\begin{equation*}
D(t) = a I_1(t) + (1-a) I_2(t) - I_3(t)>0
\end{equation*}
 happening is positive for all $t>0$. Define 
%
\begin{equation*}
 t_0 := \inf\{ t > 0\, :\, U(t) > 0 \},
 \end{equation*} 
%
and
\begin{equation*}
\tilde{\tau}_\mu := \inf\{ t > t_0\,: U(t) - \mu t \leq 0\}.
\end{equation*}
% 
We note that $t_0$ as defined above, also defines the epoch of the start of a new excursion of the reflection $Q_\mu$ for all $\mu>0$. Namely,
%
\[U(s) \leq 0  \quad \Rightarrow\quad  U(s) - \mu s \leq -\mu s  \qquad \text{for all }0\leq s< t_0\]
%
\[\Rightarrow \inf_{0\leq s < t_0} [U(s)-\mu s] \leq -\mu t_0 \quad 
\Rightarrow U(t_0) - \mu t_0 -  \inf_{0\leq s < t_0} [U(s)-\mu s] \geq U(t_0) > 0\].
%
Then $Q_\mu(t_0-) = 0$ for all $\mu>0$. 
By the virtue of the Strong Markov Property, not that $Q_\mu(t_0+t) \equalD Q_\mu(t)$. 
Hence we assume without loss of generality $t_0=0$. 
Again, we have a stochastic dominance relation similar to \eqref{eq:stochDom}:
\begin{equation*}
\tilde{\tau}_{\mu_2} < \tilde{\tau}_{\mu_3} < \tilde{\tau}_{\mu_1},
\end{equation*}
for all $\mu_1<\mu_3<\mu_2$. 
Then 

\begin{equation*}
D(t) \equalD \left\{
\begin{array}{ll}
0,  
& \text{if } t < \tilde{\tau}_{\mu_2},\\
-(1-a)I_2(t), 
& \text{if } \tilde{\tau}_{\mu_2} \leq t < \tilde{\tau}_{\mu_3},\\
(1-a)I_2(t) + I_3(t),
& \text{if } \tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1},\\
- a I_1(t) - (1-a) I_2(t)
+ I_3(t),
& \text{if } t \geq \tilde{\tau}_{\mu_1}.
\end{array}
\right.
\end{equation*}
%
Clearly, $D(t)\geq 0$ for all $t\geq 0$ and 
%
\begin{equation*}
-(1-a)I_2(t) + I_3(t) \geq a I_1(t) > 0,
\end{equation*}
% 
for $\tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1}$. 
Hence, in a similar manner to \eqref{eq:strictConv},
\begin{align}
P(D(t)>0) &\geq P\left( aI_1(t)\mathbbm{1}_{\{\tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1}\}}  > 0 \right)\nonumber\\
&= P\left( I_1(t) > 0 , \tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1}\right)\nonumber\\
&= P\left( I_1(t) > 0 | \tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1}\right)P\left(\tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1}\right)\nonumber\\
&= P\left(\tilde{\tau}_{\mu_3} \leq t < \tilde{\tau}_{\mu_1}\right) = P(\tilde{\tau}_{\mu_3}\leq t) - P(\tilde{\tau}_{\mu_1} \leq t) > 0, \label{eq:strictConv2}
\end{align}
The last inequality is satisfied it $P(\tilde{\tau}_{\mu_1} < T) >0$, which is  equivalent to $P( U(T) - \mu T \leq 0 ) >0$, a condition that is clearly true for all our choice of $U$. 
In conclusion, for $x=0$, $\E[D(t)] >0$ and therefore $\E[Q_\mu(t)]$ is a strictly convex function of $\mu$. 
\end{proof}


\subsection{Proof of Proposition \ref{prop:min_convergence_mu}}
The proof of the proposition relies on the following auxiliary lemma, of which we include the proof for completeness.
\begin{lemma}\label{lemma:minimizerConvergence}
Consider the sequence of functions $f_n:\, [x_0,\infty) \to \mathbb{R}$ and let $f: [x_0,\infty) \to\mathbb{R}$ be the pointwise limit for some $x_0\in \mathbb{R}$. 
Assume $f$ and $f_n$ are strictly convex for all $n$. 
Furthermore, let $f(y) \to \infty$ for both $y\to x_0^+$ and $y\to \infty$.  
If $x_n$ and $x$ are the minimizers for $f_n$ and $f$, respectively, then $x_n\to x$ for $n\to\infty$.  
\end{lemma}
\begin{proof}
We start by showing that the sequence $x_n$ is bounded. Fix $u_l, u_r$ such that $x_0<u_l < x < u_r$. We claim that there exists a $N\in\mathbb{N}$ such that $x_n\in[u_l,u_r]$ for all $n \geq N$. First, we prove the upper bound on $x_n$. For any strictly convex function $h$ with minimizer $x_h$, the following statement holds true:
%
\begin{equation}\label{eq100}
x_h < u_r \quad \Leftrightarrow \quad h \text{ is strictly increasing at } u_r.
\end{equation}
%
The first implication follows from observing that $h(x_h) < h(y)$ for all $y> x^*$ and definition of convexity:
%
\[ 0<\frac{h(u_r)-h(x_h)}{u_r-x_h} \leq \frac{h(u_r+\de)-h(u_r)}{\de}, \]
%
for all $\de>0$. So that $h(u_r)<h(u_r+\de)$, i.e. $h$ is increasing at $u_r$. The converse follows immediately by observing that $h(u_r) < h(u_r+\de)$ for all $\de>0$, so that $x_h < u_r$. 
%
Next, we show that $f_n$ must be increasing at $u_r$ for $n$ sufficiently large. By pointwise convergence of $f_n$ we have
%
\[ \lim_{n\to\infty} [f_n(u_r+\de) - f_n(u_r)] = f(u_r+\de) - f(u_r).\]
%
Let $w_r:= f(u_r+\de) - f(u_r)>0$. Then 
\[ \exists N_r \in \mathbb{N}:\, \forall n\geq N_r:\, |[f_n(u_r+\de) - f_n(u_r)] - [f(u_r+\de)-f(u_r)] | < w_r/2.\]
%
Hence for $n\geq N_r$,
\[f(u_r+\de)-f(u_r) - w_r/2 <  f_n(u_r+\de) - f_n(u_r) < f(u_r+\de)-f(u_r) + w_r/2\]
\[\Rightarrow 0 < w_r/2 < f_n(u_r+\de) - f_n(u_r).
\]
Hence by \eqref{eq100}, $x_n < u_r$ for sufficiently large $n$. Similarly, we argue
%
\begin{equation*}
x_h > u_l \quad \Leftrightarrow \quad h \text{ is strictly decreasing at } u_l,
\end{equation*}
for any strictly convex function $h$ with minimizer $x_h$. Note that $x_h > u_l$ implies $h(x_h) - h(u_l) < 0$ and for all $\de>0$ we get by strict convexity
%
\[\frac{h(u_l)-h(u_l-\de)}{\de} < \frac{h(x_h)-h(u_l)}{x_h-u_l} < 0,\]
%
by which $h(u_l-\de)>h(u_l)$, i.e. $h$ is decreasing in $u_l$. Moreover, if $h$ is decreasing at $u_l$, then it is decreasing for all $y < u_l$, by arguments similar to the above. Therefore, $h(u_l-\de)> h(u_l)$ for all $\de>0$ and it must hold that $x_h>u_l$. Define $f(u_l) - f(u_l-\de) :=w_l < 0$, then again by pointwise convergence, we have that
\[ \exists N_l \in \mathbb{N}:\, \forall n\geq N_l:\, |[f_n(u_l) - f_n(u_l-\de)] - [f(u_l)-f(u_l-\de)] | < w_l,\]
whereupon
\[ f_n(u_l) - f_n(u_l-\de) < f(u_l) - f(u_l-\de) + w_l = 2w_l < 0.\]
Hence, for sufficiently large $n$, we also have $x_n > u_l$. Fix $N = \max\{N_l,N_r\}$, then for $n\geq N$, $x_n\in( u_l,u_r)$. That is, the sequence $x_n$ is bounded. Therefore, by the theorem of Bolzano-Weierstrass, $x_n$ has to have a convergent subsequence. That is, there exists a sequence $n_k$ such that $n_k \to\infty$ and $x_{n_k}\to a$ as $k\to \infty$ for some $a \in [u_l,u_r]$. 
We prove that every subsequence must converge to $x$ by contradiction. Suppose there exists a subsequence $n_k$ such that $x_{n_k}\to a\neq x$. Since, $x_n\in [u_l,u_r]$ for $n\geq N$, we may restrict our attention on the sequence of functions $\hat{f}_n:[u_l,u_r] \to \mathbb{R^+}$, consisting of the original function $f_n$ restricted to the domain $[u_l,u_r]$. To be precise $x_n = \arg\min_y f_n(y) = \arg\min_y \hat{f}_n(y)$ for $n\geq N$. Because $\hat{f}_n$ and $\hat{f}$ are bounded, we furthermore $\hat{f}_n \to \hat{f}$ uniformly.

Fix $\e>0$. By uniform convergence, there exists an $K_0 \in\mathbb{N}$ such that
\[  | \hat{f}_{n_k}( y ) - \hat{f}( y)| < \e /2,\quad \forall k\geq K_0,\ y \in[u_l,u_r].\]
Also, because $\hat{f}$ is convex, it is continuous, so that there exists a $\de := \de(\e)$ so that
\[ |z-y| < \de \quad \Rightarrow \quad |\hat{f}(z) - \hat{f}(y)| < \e/2.\]
Let $K_1$ be such that $|x_{n_k}-a| < \de$ for all $k\geq K_1$. Then for $k \geq K= \max\{K_0,K_1\}$ this implies 
\begin{align*}
|f_{n_k}(x_{n_k}) - f(a)| &= |\hat{f}_{n_k}(x_{n_k}) - \hat{f}(a)| \\
&\leq  |\hat{f}_{n_k}(x_{n_k}) - \hat{f}(x_{n_k})| + | \hat{f}(x_{n_k}) - f(a)| < \e/2 + \e/2 = \e.
\end{align*} 
Hence we conclude $\lim_{k\to\infty} \hat{f}_{n_k}(x_{n_k}) = f(a)$. 
Therefore, 
\[ \limsup_{n\to \infty} f_n(x_n) \geq f(a) > f(x),\]
by minimality of $x$. However, $f_n(x_n) \leq f_n(x)$, which implies $\limsup_{n\to\infty} f_n(x_n) \leq \lim_{n\to\infty} f_n(x) = f(x)$, contradicting the strict inequality above. Hence we deduce $x=a$. Consequently, every subsequence of $x_n$ converges to $x$ and therefore $x_n\to x$ as $n\to \infty$.
%
Applying Lemma \ref{lemma:minimizerConvergence} to the functions $\Pi_T$ and $\Pi_\iy$ with $x_0=\la$, together with Lemma \ref{lemma:strict_convexity}, we obtain the result immediately.

\end{proof}


\subsection{Proof of Proposition \ref{prop:muBullet}}
\begin{proof}
Note that $\Pi_\infty$ is a smooth function. 
By the first optimality condition $\Pi_\infty'(\mui)$ $= 0$. 
We first prove that also $\Pi_T(\mu)$ is differentiable with respect to $\mu$ for all $\mu\geq 0$. 
Recall \eqref{eq:PiT}, which defines the cost function as a combination of the accumulated expected transient queue length, and linear staffing costs.
The latter term is clearly differentiable, hence it remains to be proved that 
\begin{equation*}
C_T(\mu) = \frac{1}{T}\int_0^\iy \E[Q_\mu(t)] \, \dd t,
\end{equation*}
admits a derivative for all $\mu\geq 0$ with $T$ fixed.
This holds if and only if $\E[Q_\mu(t)]$ is differentiable for all $t\geq 0$. 
Let $Q(0)= x\geq 0$. 
Following \eqref{eq:Qlm},
\begin{align*}
\E[Q_\mu(t)] &= \E[X_\mu(t)] + \E\Big[ \max\{ x, \sup_{s\in[0,t]}\{- X_\mu(s)\} \}\Big]\\
&= (\la-\mu)t+ \E\Big[ \max\{ x, \sup_{s\in[0,t]}\{- X_\mu(s)\} \}\Big],
\end{align*}
where the first term is differentiable. 
Furthermore, 
\begin{align*}
 \E[ \max\{ x, \sup_{s\in[0,t]} \{ - X_\mu(s) \} \} ]
  &= x + \int_x^\iy P(\sup_{s\in[0,t]} \{ - X_\mu(s) \} > u )\dd u \\
 &= x+\int_x^\infty P(\hat\tau^0(u) \leq t ) \dd u,
\end{align*}
with $\hat{\tau}^0(u)$ as defined in \eqref{eq:transformedTau}.

Since $-X_\mu$ is a process with no positive jumps, we may apply Corollary VII3 of \cite{Bertoin1996}, which states that the following equivalence between measures holds:
\begin{equation}
s\,P( \hat\tau^0(u) \in ds ) du = u\,P( -X_\mu(s) \in du ) ds,
\end{equation}
so that 
\begin{align}
 \int_{u=x}^\infty P(\hat{\tau}^0(u) \leq t )\, \dd u 
&= 
\int_{u=x}^\iy \int_{s=0}^t P( \hat\tau^0(u) \in ds ) \dd u \nonumber \\
&= \int_{u=x}^\iy \int_{s=0}^t\,s^{-1} u\,\,P( -X_\mu(s) \in \dd u ) \dd s \nonumber  \\
&= \int_{u=x}^\iy \int_{s=0}^t\,s^{-1}  u\,P( X_\mu(s) \in \dd u ) \dd s \nonumber  \\
&= \int_{s=0}^t s^{-1} \E[ \max\{x, X_\mu(s)\} ]  \dd s \nonumber \\
&= \int_{s=0}^t \int_{v=x/s}^\iy P( X_\mu(s)/s > v ) \dd v \dd s \nonumber \\
&= \int_{s=0}^t \int_{v=x/s}^\iy P( U(\la s)/s > v + \mu ) \dd v \dd s \nonumber \\
&= \int_{s=0}^t \int_{w=x/s+\mu}^\iy P( U(\la s)/s > w) \dd w \dd s,
\end{align}
where the interchange of integrals is justified by Fubini's theorem and this last form is differentiable with respect to $\mu$. 
Substituting $Q(0)$ for $x$ straightforwardly yields differentiability of the complete cost function $\Pi_T$ for all $T$. 

Consequently we invoke the first optimality condition for $\muT$ to find
\begin{align*}
0=\Pi_T'(\muT)  
&= \Pi_\infty'(\muT) + \Psi_T'(\muT) + O(1/T^2)\\
&= \Pi_\infty'(\mui) + \Psi_T'(\mui) + (\muT-\mui)\left[ \Pi_\infty''(\mui) + \Psi_T''(\mui) \right] \\
&\qquad + \frac{1}{2}(\mu_T-\mui)^2\left[\Pi_T'''(\xi)+\Psi_T'''(\xi) \right] + O(1/T^2)\\
&= \Psi_T'(\mui) + (\muT-\mui)\left[ \Pi_\infty''(\mui) + \Psi_T''(\mui) \right] \\
&\qquad + \frac{1}{2}(\mu_T-\mui)^2\left[\Pi'''(\xi)+\Psi_T'''(\xi)\right] + O(1/T^2).
\end{align*}
for some $\xi \in [\muT,\mui]$. Rearranging this gives
\begin{align*}
\muT-\mui &= \frac{-\Psi_T'(\mui)}{\Pi_\infty''(\mui)+\Psi_T''(\mui) + \frac{1}{2}(\muT-\mui)(\Pi_\infty'''(\muT)+\Psi_T'''(\xi))} + O(1/T)\\
&= {-}\frac{\Psi_T'(\mui)}{\Pi_\iy''(\mui)} \left[1 - \frac{\Psi_T''(\mu)}{\Pi_\infty''(\mui)} - \frac{\muT-\mu_\infty}{2}\frac{\Pi_\infty'''(\mui)+\Psi_T'''(\mui)}{\Pi_\infty''(\mui)}\right] + O(1/T)\\
&= {-}\frac{\Psi_T'(\mui)}{\Pi_\iy''(\mui)} [1 + o(1)]
\end{align*}
%
for $T\to\infty$, since both $\mu_T - \mu_\infty$ and $\Psi_T''(\mui)$ are $o(1)$. 
Let
%
\begin{equation*}
\mu_\bullet := \lim_{T\to\iy} \frac{T \Psi_T'(\mui)}{\Pi_\iy''(\mui)}.
\end{equation*}
%
By \eqref{eq:mainResult} we have
%
\begin{equation*}
T \Psi'_T(\mu) = {-} \frac{\E[Q(0)^2]}{2(\mu-\la)^2} + \frac{\la u_3}{3(\mu-\la)^3} + \frac{3\la^2u_2^2}{4(\mu-\la)^4}.
\end{equation*}
%
Together with 
%
\begin{equation*}
\Pi_\iy''(\mu) = \frac{\la u_2}{(\mu-\la)^3}
\end{equation*}
%
and \eqref{eq:muInf} we obtain the expression for $\mu_\bullet$ in \eqref{eq:muBullet}.
\end{proof}
\subsection{Proof of Proposition \ref{prop:optimalitygap_mui}}\label{sec:proofProp4}
\begin{proof}
We upper bound the optimality gap by using the decomposition in \eqref{eq:decomposition}.
%
\begin{align}
|\Pi_\iy^\star - \Pi_T^\star| &= \left|\hat{\Pi}_T(\mu_\infty) + \Delta_T(\mui) - \hat{\Pi}_T(\muT) - \Delta_T(\muT)\right|\nonumber\\
&\leq |\hat{\Pi}_T(\mui) - \hat{\Pi}_T(\muT)| + |\Delta_T(\mui)| + |\Delta_T(\muT)|\nonumber\\
&= |\hat{\Pi}_T(\mui) - \hat{\Pi}_T(\muT)| + O(1/T^2),
\end{align}
%
since $\Delta_T(\mu) = O(1/T^2)$ by Proposition \ref{prop:truncation_error}. Next, we find an upper bound for $|\hat{\Pi}_T(\gamma) - \hat{\Pi}_T(\beta)|$, with $\hat{\Pi}_T(\cdot)$ as in \eqref{eq:decomposition}, in terms of the difference between $\gamma$ and $\beta$. 
For simplicity, denote $\hat{\gamma} = \gamma - \la$ and $\hat{\beta} = \beta-\la$, implying $\hat{\gamma}-\hat{\beta}=\gamma-\beta$. Then, using \eqref{eq:mainResult}, we get
%
\begin{align*}
|\hat{\Pi}_T(\mui) - \hat{\Pi}_T(\muT)| &= 
\left| \aaa(\hat{\gamma}-\hat{\beta})
+\left(\frac{\la u_2}{2} + \frac{\E[Q(0)^2]}{2T}\right)\left(\frac{1}{\hx}-\frac{1}{\hy}\right) \right. \\
& \qquad \left. -\frac{\la^2 u_2^2}{4T}\left(\frac{1}{\hx^3}-\frac{1}{\hy^3}\right) 
-\frac{\la u_3}{6T}\left(\frac{1}{\hx^2} - \frac{1}{\hy^2}\right)
\right|.
\end{align*}
%
Furthermore, we have 
%
\begin{align*}
\frac 1 \hx - \frac 1 \hy &= -\frac{\hx-\hy}{\hy^2} + \frac{(\hx-\hy)^2}{\hy^3} + O\left((\gamma-\beta)^3\right),\\
\frac 1 {\hx^2} - \frac 1 {\hy^2} &= -\frac{2(\hx-\hy)}{\hy^3} + \frac{3(\hx-\hy)^2}{\hy^4} + O\left((\gamma-\beta)^3\right),\\
\frac 1 {\hx^3} - \frac  1 {\hy^3} &= -\frac{3(\hx-\hy)}{\hy^4} + \frac{6(\hx-\hy)^2}{\hy^5} + O\left((\gamma-\beta)^3\right).\\
\end{align*}
%
Substituting these yields 
%
\begin{align*}
|\hat{\Pi}_T(\gamma) - \hat{\Pi}_T(\beta)| &= \left|(\gamma-\beta)\left[ \aaa - \frac{\la u_2}{2 \hy^2} + \frac{1}{2T\hy^2}\left(\E[Q(0)^2] + \frac{3\la^2 u_2^2}{2\hy^2} + \frac{2\la u_3}{3 \hy}\right)\right]\right. \\
&\qquad \left. - (\gamma-\beta)^2\left[ \frac{\la u_2}{2 \hy^3} + \frac{1}{2T\hy^3}\left(\E[Q(0)^2] - \frac{3\la^2 u_2^2}{\hy^2} - \frac{\la u_3}{\hy}\right)\right]\right| \\
& \qquad \qquad + O\left((\gamma-\beta)^3\right).
\end{align*}
%
Given that $\muT = \mui + \mu_\bullet/T + o(1/T)$, we find
%
\begin{align*}
|\hat{\Pi}_T(\mui) - \hat{\Pi}_T(\muT)| &= \frac{|\mu_\bullet|}{T}\left(\aaa - \frac{\la u_2}{2(\mui-\la )^2}\right) + O(1/T^2)\\
&= \frac{|\mu_\bullet|}{T}\left(\aaa - \frac{\la u_2}{2(\sqrt{\la u_2/2\aaa})^2}\right) + O(1/T^2) = O(1/T^2),
\end{align*}
%
which concludes the proof. 
\end{proof}

\resettocdepth 

\end{subappendices}

